Amplituhedra and origami, I: tree level

We establish a precise correspondence between points of the $m=4$ tree momentum amplituhedron and origami crease patterns. As an application, we prove that the BCFW (Britto-Cachazo-Feng-Witten) cells triangulate the $m=4$ tree amplituhedron both in momentum space and in momentum-twistor space. As another application, we show that every nondegenerate weighted planar bipartite graph $\Gamma$ admits a t-embedding, i.e., an embedding of the planar dual of $\Gamma$ such that the sum of angles of white (equivalently, black) faces around each vertex is equal to $\pi$.

==> loop_ampl_aux.tex <==
\relax 
\providecommand \babel@aux [2]{\global \let \babel@toc \@gobbletwo }
\@nameuse{bbl@beforestart}
\providecommand\hyper@newdestlabel[2]{}
\providecommand\HyField@AuxAddToFields[1]{}
\providecommand\HyField@AuxAddToCoFields[2]{}
\babel@aux{english}{}
\citation{AHT}
\citation{BCFW}
\citation{AHBC_all_loop}
\citation{origami1}
\citation{KLRR}
\citation{CLR1}
\citation{origami1}
\citation{DFLP}
\citation{AHT}
\citation{Zono}
\citation{LPW}
\citation{PSBW}
\citation{ELT}
\citation{ELPTSBW}
\citation{origami1}
\citation{ELT}
\citation{Tessler_notes}
\citation{ELPTSBW}
\citation{origami1}
\citation{ELT}
\citation{ELPTSBW}
\citation{Tessler_notes}
\citation{origami1}
\citation{AHT}
\citation{AHTT}
\citation{FL}
\citation{FGLS}
\citation{FGLS}
\citation{FGLS}
\citation{AHBC_all_loop}
\citation{abcgpt}
\citation{Pos}
\@writefile{toc}{\contentsline {section}{\tocsection {}{}{Introduction}}{2}{section*.2}\protected@file@percent }
\newlabel{sec:intro}{{}{2}{Introduction}{section*.2}{}}
\@writefile{lla}{\contentsline {section}{\numberline {\crtrefnumber{sec:intro}}sec:intro}{2}{section*.2}\protected@file@percent }
\newlabel{sec:intro@cref}{{}{[1][2][]2}{}{}{}}
\@writefile{loe}{\contentsline {theoremintro}{\ifthmt@listswap Theorem~A\else \numberline {A}Theorem\fi }{2}{theoremintro.1}\protected@file@percent }
\newlabel{thm:main_triangulation}{{A}{2}{}{theoremintro.1}{}}
\@writefile{lla}{\contentsline {section}{\numberline {\crtrefnumber{thm:main_triangulation}}thm:main_triangulation}{2}{theoremintro.1}\protected@file@percent }
\newlabel{thm:main_triangulation@cref}{{[theoremintro][1][]A}{[1][2][]2}{}{}{}}
\@writefile{toc}{\contentsline {subsection}{\tocsubsection {}{}{Defining amplituhedra and BCFW tiles}}{2}{section*.3}\protected@file@percent }
\citation{Pos}
\citation{AHT}
\citation{BaiHe}
\citation{BHL}
\citation{DFLP}
\@writefile{lof}{\contentsline {figure}{\numberline {1}{\ignorespaces  T-duality for $L$-punctured\xspace  planar bipartite graphs; see \crefrange  {sec:shift}{sec:LPUNC}.}}{3}{figure.caption.4}\protected@file@percent }
\newlabel{fig:intro-G-ddG}{{1}{3}{T-duality for \Lpunc planar bipartite graphs; see \crefrange {sec:shift}{sec:LPUNC}}{figure.caption.4}{}}
\@writefile{lla}{\contentsline {section}{\numberline {\crtrefnumber{fig:intro-G-ddG}}fig:intro-G-ddG}{3}{figure.caption.4}\protected@file@percent }
\newlabel{fig:intro-G-ddG@cref}{{[figure][1][]1}{[1][2][]3}{}{}{}}
\citation{Zono}
\citation{BaWe}
\citation{HSP}
\citation{crit}
\citation{LPW}
\citation{PSBW}
\citation{CLSBW}
\citation{AHCC}
\citation{abcgpt}
\citation{LPW}
\citation{PSBW}
\citation{origami1}
\citation{origami1}
\citation{origami1}
\citation{KLRR}
\citation{CLR1}
\citation{Kawasaki}
\citation{origami1}
\citation{Pos}
\@writefile{lof}{\contentsline {figure}{\numberline {2}{\ignorespaces  Possible generic origami reconstruction steps\xspace  are precisely the planar duals of the loop BCFW recursion steps. An example of a non-generic origami reconstruction step\xspace  is shown in \cref  {fig:fout-cliques}. }}{4}{figure.caption.6}\protected@file@percent }
\newlabel{fig:BCFW-vertices}{{2}{4}{Possible generic \ORsts are precisely the planar duals of the loop BCFW recursion steps. An example of a non-generic \ORst is shown in \cref {fig:fout-cliques}}{figure.caption.6}{}}
\@writefile{lla}{\contentsline {section}{\numberline {\crtrefnumber{fig:BCFW-vertices}}fig:BCFW-vertices}{4}{figure.caption.6}\protected@file@percent }
\newlabel{fig:BCFW-vertices@cref}{{[figure][2][]2}{[1][4][]4}{}{}{}}
\@writefile{toc}{\contentsline {subsection}{\tocsubsection {}{}{T-duality}}{4}{section*.5}\protected@file@percent }
\@writefile{toc}{\contentsline {subsection}{\tocsubsection {}{}{Origami-amplituhedron correspondence\xspace  }}{4}{section*.7}\protected@file@percent }
\citation{origami1}
\citation{origami1}
\citation{origami1}
\@writefile{lof}{\contentsline {figure}{\numberline {3}{\ignorespaces  Applying the origami reconstruction algorithm\xspace  \ /\ loop BCFW recursion.}}{5}{figure.caption.8}\protected@file@percent }
\newlabel{fig:BCFW-full}{{3}{5}{Applying the \ORA \ /\ loop BCFW recursion}{figure.caption.8}{}}
\@writefile{lla}{\contentsline {section}{\numberline {\crtrefnumber{fig:BCFW-full}}fig:BCFW-full}{5}{figure.caption.8}\protected@file@percent }
\newlabel{fig:BCFW-full@cref}{{[figure][3][]3}{[1][5][]5}{}{}{}}
\@writefile{toc}{\contentsline {subsection}{\tocsubsection {}{}{Origami reconstruction algorithm\xspace  }}{5}{section*.9}\protected@file@percent }
\citation{Kenyon_Sheffield}
\citation{Kenyon_height}
\citation{Streinu}
\citation{Streinu_ptr}
\citation{RSS_expansive}
\citation{RSS}
\citation{origami1}
\citation{origami1}
\citation{origami1}
\@writefile{toc}{\contentsline {subsection}{\tocsubsection {}{}{Outline}}{6}{section*.10}\protected@file@percent }
\@writefile{toc}{\contentsline {subsection}{\tocsubsection {}{}{Acknowledgments}}{6}{section*.11}\protected@file@percent }
\citation{applets}
\@writefile{toc}{\contentsline {section}{\tocsection {}{1}{Preliminaries}}{7}{section.1}\protected@file@percent }
\@writefile{toc}{\contentsline {subsection}{\tocsubsection {}{1.1}{Minkowski space, decorated null polygons, and positive kinematic space}}{7}{subsection.1.1}\protected@file@percent }
\newlabel{eq:x_vs_ap_vs_am}{{1.1}{7}{Minkowski space, decorated null polygons, and positive kinematic space}{equation.1.1}{}}
\@writefile{lla}{\contentsline {section}{\numberline {\crtrefnumber{eq:x_vs_ap_vs_am}}eq:x_vs_ap_vs_am}{7}{equation.1.1}\protected@file@percent }
\newlabel{eq:x_vs_ap_vs_am@cref}{{[equation][1][1]1.1}{[1][7][]7}{}{}{}}
\newlabel{eq:det_xM_vs_Pmom^2}{{1.2}{7}{Minkowski space, decorated null polygons, and positive kinematic space}{equation.1.2}{}}
\@writefile{lla}{\contentsline {section}{\numberline {\crtrefnumber{eq:det_xM_vs_Pmom^2}}eq:det_xM_vs_Pmom^2}{7}{equation.1.2}\protected@file@percent }
\newlabel{eq:det_xM_vs_Pmom^2@cref}{{[equation][2][1]1.2}{[1][7][]7}{}{}{}}
\@writefile{loe}{\contentsline {definition}{\ifthmt@listswap Definition~1.1\else \numberline {1.1}Definition\fi }{7}{definition.1.1}\protected@file@percent }
\newlabel{dfn:BACKGR:bispinor}{{1.1}{7}{}{definition.1.1}{}}
\@writefile{lla}{\contentsline {section}{\numberline {\crtrefnumber{dfn:BACKGR:bispinor}}dfn:BACKGR:bispinor}{7}{definition.1.1}\protected@file@percent }
\newlabel{dfn:BACKGR:bispinor@cref}{{[definition][1][1]1.1}{[1][7][]7}{}{}{}}
\newlabel{eq:TE:bisy_bisyt_to_M}{{1.3}{7}{Minkowski space, decorated null polygons, and positive kinematic space}{equation.1.3}{}}
\@writefile{lla}{\contentsline {section}{\numberline {\crtrefnumber{eq:TE:bisy_bisyt_to_M}}eq:TE:bisy_bisyt_to_M}{7}{equation.1.3}\protected@file@percent }
\newlabel{eq:TE:bisy_bisyt_to_M@cref}{{[equation][3][1]1.3}{[1][7][]7}{}{}{}}
\newlabel{eq:BACKGR:brla_brlat}{{1.4}{7}{Minkowski space, decorated null polygons, and positive kinematic space}{equation.1.4}{}}
\@writefile{lla}{\contentsline {section}{\numberline {\crtrefnumber{eq:BACKGR:brla_brlat}}eq:BACKGR:brla_brlat}{7}{equation.1.4}\protected@file@percent }
\newlabel{eq:BACKGR:brla_brlat@cref}{{[equation][4][1]1.4}{[1][7][]7}{}{}{}}
\newlabel{eq:intro:wind}{{1.5}{7}{Minkowski space, decorated null polygons, and positive kinematic space}{equation.1.5}{}}
\@writefile{lla}{\contentsline {section}{\numberline {\crtrefnumber{eq:intro:wind}}eq:intro:wind}{7}{equation.1.5}\protected@file@percent }
\newlabel{eq:intro:wind@cref}{{[equation][5][1]1.5}{[1][7][]7}{}{}{}}
\newlabel{eq:TE:LALAK}{{1.7}{7}{Minkowski space, decorated null polygons, and positive kinematic space}{equation.1.7}{}}
\@writefile{lla}{\contentsline {section}{\numberline {\crtrefnumber{eq:TE:LALAK}}eq:TE:LALAK}{7}{equation.1.7}\protected@file@percent }
\newlabel{eq:TE:LALAK@cref}{{[equation][7][1]1.7}{[1][7][]7}{}{}{}}
\newlabel{eq:lak_latk}{{1.8}{7}{Minkowski space, decorated null polygons, and positive kinematic space}{equation.1.8}{}}
\@writefile{lla}{\contentsline {section}{\numberline {\crtrefnumber{eq:lak_latk}}eq:lak_latk}{7}{equation.1.8}\protected@file@percent }
\newlabel{eq:lak_latk@cref}{{[equation][8][1]1.8}{[1][7][]7}{}{}{}}
\newlabel{eq:lak_latk2}{{1.9}{7}{Minkowski space, decorated null polygons, and positive kinematic space}{equation.1.9}{}}
\@writefile{lla}{\contentsline {section}{\numberline {\crtrefnumber{eq:lak_latk2}}eq:lak_latk2}{7}{equation.1.9}\protected@file@percent }
\newlabel{eq:lak_latk2@cref}{{[equation][9][1]1.9}{[1][7][]7}{}{}{}}
\citation{origami1}
\citation{HZ_notes}
\citation{DFLP}
\citation{origami1}
\@writefile{loe}{\contentsline {definition}{\ifthmt@listswap Definition~1.2\else \numberline {1.2}Definition\fi }{8}{definition.1.2}\protected@file@percent }
\newlabel{dfn:TODO:null_polygons}{{1.2}{8}{}{definition.1.2}{}}
\@writefile{lla}{\contentsline {section}{\numberline {\crtrefnumber{dfn:TODO:null_polygons}}dfn:TODO:null_polygons}{8}{definition.1.2}\protected@file@percent }
\newlabel{dfn:TODO:null_polygons@cref}{{[definition][2][1]1.2}{[1][8][]8}{}{}{}}
\@writefile{loe}{\contentsline {lemma}{\ifthmt@listswap Lemma~1.3\else \numberline {1.3}Lemma\fi \thmtformatoptarg {\cite  [\cref  *{M-lemma:Mbd=>simple}]{origami1}\xspace  }}{8}{lemma.1.3}\protected@file@percent }
\newlabel{lemma:TOP:Mpos=>simple}{{1.3}{8}{\Mref {lemma:Mbd=>simple}}{lemma.1.3}{}}
\@writefile{lla}{\contentsline {section}{\numberline {\crtrefnumber{lemma:TOP:Mpos=>simple}}lemma:TOP:Mpos=>simple}{8}{lemma.1.3}\protected@file@percent }
\newlabel{lemma:TOP:Mpos=>simple@cref}{{[lemma][3][1]1.3}{[1][8][]8}{}{}{}}
\@writefile{loe}{\contentsline {definition}{\ifthmt@listswap Definition~1.4\else \numberline {1.4}Definition\fi }{8}{definition.1.4}\protected@file@percent }
\newlabel{dfn:TREE:lalat_vs_xbd}{{1.4}{8}{}{definition.1.4}{}}
\@writefile{lla}{\contentsline {section}{\numberline {\crtrefnumber{dfn:TREE:lalat_vs_xbd}}dfn:TREE:lalat_vs_xbd}{8}{definition.1.4}\protected@file@percent }
\newlabel{dfn:TREE:lalat_vs_xbd@cref}{{[definition][4][1]1.4}{[1][8][]8}{}{}{}}
\newlabel{eq:TE:decor_dfn}{{1.10}{8}{}{equation.1.10}{}}
\@writefile{lla}{\contentsline {section}{\numberline {\crtrefnumber{eq:TE:decor_dfn}}eq:TE:decor_dfn}{8}{equation.1.10}\protected@file@percent }
\newlabel{eq:TE:decor_dfn@cref}{{[equation][10][1]1.10}{[1][8][]8}{}{}{}}
\@writefile{loe}{\contentsline {definition}{\ifthmt@listswap Definition~1.5\else \numberline {1.5}Definition\fi }{8}{definition.1.5}\protected@file@percent }
\newlabel{dfn:TREE:M_pos}{{1.5}{8}{}{definition.1.5}{}}
\@writefile{lla}{\contentsline {section}{\numberline {\crtrefnumber{dfn:TREE:M_pos}}dfn:TREE:M_pos}{8}{definition.1.5}\protected@file@percent }
\newlabel{dfn:TREE:M_pos@cref}{{[definition][5][1]1.5}{[1][8][]8}{}{}{}}
\newlabel{eq:TE:Mand_dfn}{{1.11}{8}{}{equation.1.11}{}}
\@writefile{lla}{\contentsline {section}{\numberline {\crtrefnumber{eq:TE:Mand_dfn}}eq:TE:Mand_dfn}{8}{equation.1.11}\protected@file@percent }
\newlabel{eq:TE:Mand_dfn@cref}{{[equation][11][1]1.11}{[1][8][]8}{}{}{}}
\@writefile{loe}{\contentsline {definition}{\ifthmt@listswap Definition~1.6\else \numberline {1.6}Definition\fi \thmtformatoptarg {Ambient tree momentum amplituhedron~{\cite  {HZ_notes,DFLP}}}}{8}{definition.1.6}\protected@file@percent }
\newlabel{dfn:TREE:MPkn}{{1.6}{8}{Ambient tree momentum amplituhedron~{\cite {HZ_notes,DFLP}}}{definition.1.6}{}}
\@writefile{lla}{\contentsline {section}{\numberline {\crtrefnumber{dfn:TREE:MPkn}}dfn:TREE:MPkn}{8}{definition.1.6}\protected@file@percent }
\newlabel{dfn:TREE:MPkn@cref}{{[definition][6][1]1.6}{[1][8][]8}{}{}{}}
\@writefile{loe}{\contentsline {definition}{\ifthmt@listswap Definition~1.7\else \numberline {1.7}Definition\fi }{8}{definition.1.7}\protected@file@percent }
\newlabel{dfn:BACKGR:decoration}{{1.7}{8}{}{definition.1.7}{}}
\@writefile{lla}{\contentsline {section}{\numberline {\crtrefnumber{dfn:BACKGR:decoration}}dfn:BACKGR:decoration}{8}{definition.1.7}\protected@file@percent }
\newlabel{dfn:BACKGR:decoration@cref}{{[definition][7][1]1.7}{[1][8][]8}{}{}{}}
\@writefile{loe}{\contentsline {definition}{\ifthmt@listswap Definition~1.8\else \numberline {1.8}Definition\fi }{8}{definition.1.8}\protected@file@percent }
\newlabel{dfn:little_group}{{1.8}{8}{}{definition.1.8}{}}
\@writefile{lla}{\contentsline {section}{\numberline {\crtrefnumber{dfn:little_group}}dfn:little_group}{8}{definition.1.8}\protected@file@percent }
\newlabel{dfn:little_group@cref}{{[definition][8][1]1.8}{[1][8][]8}{}{}{}}
\@writefile{loe}{\contentsline {lemma}{\ifthmt@listswap Lemma~1.9\else \numberline {1.9}Lemma\fi \thmtformatoptarg {\cite  [\cref  *{M-lemma:BCFW:null}]{origami1}\xspace  }}{8}{lemma.1.9}\protected@file@percent }
\newlabel{lemma:BCFW:null}{{1.9}{8}{\Mref {lemma:BCFW:null}}{lemma.1.9}{}}
\@writefile{lla}{\contentsline {section}{\numberline {\crtrefnumber{lemma:BCFW:null}}lemma:BCFW:null}{8}{lemma.1.9}\protected@file@percent }
\newlabel{lemma:BCFW:null@cref}{{[lemma][9][1]1.9}{[1][8][]8}{}{}{}}
\newlabel{eq:sum_arg_pmom_-2pi}{{1.12}{8}{\Mref {lemma:BCFW:null}}{equation.1.12}{}}
\@writefile{lla}{\contentsline {section}{\numberline {\crtrefnumber{eq:sum_arg_pmom_-2pi}}eq:sum_arg_pmom_-2pi}{8}{equation.1.12}\protected@file@percent }
\newlabel{eq:sum_arg_pmom_-2pi@cref}{{[equation][12][1]1.12}{[1][8][]8}{}{}{}}
\@writefile{loe}{\contentsline {definition}{\ifthmt@listswap Definition~1.10\else \numberline {1.10}Definition\fi }{8}{definition.1.10}\protected@file@percent }
\newlabel{dfn:BACKGR:GGsh}{{1.10}{8}{}{definition.1.10}{}}
\@writefile{lla}{\contentsline {section}{\numberline {\crtrefnumber{dfn:BACKGR:GGsh}}dfn:BACKGR:GGsh}{8}{definition.1.10}\protected@file@percent }
\newlabel{dfn:BACKGR:GGsh@cref}{{[definition][10][1]1.10}{[1][8][]8}{}{}{}}
\citation{KLRR}
\@writefile{lof}{\contentsline {figure}{\numberline {4}{\ignorespaces Notation for corners of $\Gamma $.}}{9}{figure.caption.12}\protected@file@percent }
\newlabel{fig:corners}{{4}{9}{Notation for corners of $\G $}{figure.caption.12}{}}
\@writefile{lla}{\contentsline {section}{\numberline {\crtrefnumber{fig:corners}}fig:corners}{9}{figure.caption.12}\protected@file@percent }
\newlabel{fig:corners@cref}{{[figure][4][]4}{[1][9][]9}{}{}{}}
\@writefile{toc}{\contentsline {subsection}{\tocsubsection {}{1.2}{Planar bipartite graphs: notation and basic properties}}{9}{subsection.1.2}\protected@file@percent }
\newlabel{eq:DIM:Euler}{{1.13}{9}{Planar bipartite graphs: notation and basic properties}{equation.1.13}{}}
\@writefile{lla}{\contentsline {section}{\numberline {\crtrefnumber{eq:DIM:Euler}}eq:DIM:Euler}{9}{equation.1.13}\protected@file@percent }
\newlabel{eq:DIM:Euler@cref}{{[equation][13][1]1.13}{[1][9][]9}{}{}{}}
\newlabel{eq:DIM:Euler_no_float}{{1.14}{9}{Planar bipartite graphs: notation and basic properties}{equation.1.14}{}}
\@writefile{lla}{\contentsline {section}{\numberline {\crtrefnumber{eq:DIM:Euler_no_float}}eq:DIM:Euler_no_float}{9}{equation.1.14}\protected@file@percent }
\newlabel{eq:DIM:Euler_no_float@cref}{{[equation][14][1]1.14}{[1][9][]9}{}{}{}}
\@writefile{loe}{\contentsline {definition}{\ifthmt@listswap Definition~1.11\else \numberline {1.11}Definition\fi \thmtformatoptarg {Corners}}{9}{definition.1.11}\protected@file@percent }
\newlabel{dfn:corners}{{1.11}{9}{Corners}{definition.1.11}{}}
\@writefile{lla}{\contentsline {section}{\numberline {\crtrefnumber{dfn:corners}}dfn:corners}{9}{definition.1.11}\protected@file@percent }
\newlabel{dfn:corners@cref}{{[definition][11][1]1.11}{[1][9][]9}{}{}{}}
\@writefile{loe}{\contentsline {definition}{\ifthmt@listswap Definition~1.12\else \numberline {1.12}Definition\fi \thmtformatoptarg {Boundary edge insertion/contraction}}{9}{definition.1.12}\protected@file@percent }
\newlabel{dfn:DIM:MVbd}{{1.12}{9}{Boundary edge insertion/contraction}{definition.1.12}{}}
\@writefile{lla}{\contentsline {section}{\numberline {\crtrefnumber{dfn:DIM:MVbd}}dfn:DIM:MVbd}{9}{definition.1.12}\protected@file@percent }
\newlabel{dfn:DIM:MVbd@cref}{{[definition][12][1]1.12}{[1][9][]9}{}{}{}}
\citation{Pos}
\citation{LamCDM}
\citation{Pos}
\citation{Lus2}
\@writefile{lof}{\contentsline {figure}{\numberline {5}{\ignorespaces  Local moves on planar bipartite graphs.}}{10}{figure.caption.13}\protected@file@percent }
\newlabel{fig:moves}{{5}{10}{Local moves on planar bipartite graphs}{figure.caption.13}{}}
\@writefile{lla}{\contentsline {section}{\numberline {\crtrefnumber{fig:moves}}fig:moves}{10}{figure.caption.13}\protected@file@percent }
\newlabel{fig:moves@cref}{{[figure][5][]5}{[1][10][]10}{}{}{}}
\@writefile{loe}{\contentsline {definition}{\ifthmt@listswap Definition~1.13\else \numberline {1.13}Definition\fi \thmtformatoptarg {Degree-$2$ vertex insertion/removal}}{10}{definition.1.13}\protected@file@percent }
\newlabel{dfn:DIM:MV1}{{1.13}{10}{Degree-$2$ vertex insertion/removal}{definition.1.13}{}}
\@writefile{lla}{\contentsline {section}{\numberline {\crtrefnumber{dfn:DIM:MV1}}dfn:DIM:MV1}{10}{definition.1.13}\protected@file@percent }
\newlabel{dfn:DIM:MV1@cref}{{[definition][13][1]1.13}{[1][10][]10}{}{}{}}
\@writefile{loe}{\contentsline {definition}{\ifthmt@listswap Definition~1.14\else \numberline {1.14}Definition\fi \thmtformatoptarg {Square/spider move}}{10}{definition.1.14}\protected@file@percent }
\newlabel{dfn:DIM:MV2}{{1.14}{10}{Square/spider move}{definition.1.14}{}}
\@writefile{lla}{\contentsline {section}{\numberline {\crtrefnumber{dfn:DIM:MV2}}dfn:DIM:MV2}{10}{definition.1.14}\protected@file@percent }
\newlabel{dfn:DIM:MV2@cref}{{[definition][14][1]1.14}{[1][10][]10}{}{}{}}
\@writefile{loe}{\contentsline {definition}{\ifthmt@listswap Definition~1.15\else \numberline {1.15}Definition\fi \thmtformatoptarg {Parallel edge reduction}}{10}{definition.1.15}\protected@file@percent }
\newlabel{dfn:DIM:R1}{{1.15}{10}{Parallel edge reduction}{definition.1.15}{}}
\@writefile{lla}{\contentsline {section}{\numberline {\crtrefnumber{dfn:DIM:R1}}dfn:DIM:R1}{10}{definition.1.15}\protected@file@percent }
\newlabel{dfn:DIM:R1@cref}{{[definition][15][1]1.15}{[1][10][]10}{}{}{}}
\newlabel{ssec:dimer_backgr}{{1.3}{10}{Totally nonnegative Grassmannian}{subsection.1.3}{}}
\@writefile{lla}{\contentsline {section}{\numberline {\crtrefnumber{ssec:dimer_backgr}}ssec:dimer_backgr}{10}{subsection.1.3}\protected@file@percent }
\newlabel{ssec:dimer_backgr@cref}{{[subsection][3][1]1.3}{[1][10][]10}{}{}{}}
\@writefile{toc}{\contentsline {subsection}{\tocsubsection {}{1.3}{Totally nonnegative Grassmannian}}{10}{subsection.1.3}\protected@file@percent }
\newlabel{eq:altp_dfn}{{1.15}{10}{Totally nonnegative Grassmannian}{equation.1.15}{}}
\@writefile{lla}{\contentsline {section}{\numberline {\crtrefnumber{eq:altp_dfn}}eq:altp_dfn}{10}{equation.1.15}\protected@file@percent }
\newlabel{eq:altp_dfn@cref}{{[equation][15][1]1.15}{[1][10][]10}{}{}{}}
\@writefile{loe}{\contentsline {definition}{\ifthmt@listswap Definition~1.16\else \numberline {1.16}Definition\fi }{10}{definition.1.16}\protected@file@percent }
\newlabel{eq:DIM:k_dfn}{{1.16}{10}{}{equation.1.16}{}}
\@writefile{lla}{\contentsline {section}{\numberline {\crtrefnumber{eq:DIM:k_dfn}}eq:DIM:k_dfn}{10}{equation.1.16}\protected@file@percent }
\newlabel{eq:DIM:k_dfn@cref}{{[equation][16][1]1.16}{[1][10][]10}{}{}{}}
\@writefile{loe}{\contentsline {definition}{\ifthmt@listswap Definition~1.17\else \numberline {1.17}Definition\fi }{10}{definition.1.17}\protected@file@percent }
\newlabel{dfn:DIM:apm}{{1.17}{10}{}{definition.1.17}{}}
\@writefile{lla}{\contentsline {section}{\numberline {\crtrefnumber{dfn:DIM:apm}}dfn:DIM:apm}{10}{definition.1.17}\protected@file@percent }
\newlabel{dfn:DIM:apm@cref}{{[definition][17][1]1.17}{[1][10][]10}{}{}{}}
\citation{KLS}
\citation{KLS}
\citation{Kasteleyn}
\citation{AGPR}
\citation{Kenyon_conf}
\citation{Smirnov_cluster}
\citation{origami1}
\citation{AGPR}
\citation{SpeyerVariations}
\citation{Kenyon_lectures}
\citation{origami1}
\newlabel{eq:intro:Delta_G_wt}{{1.17}{11}{Totally nonnegative Grassmannian}{equation.1.17}{}}
\@writefile{lla}{\contentsline {section}{\numberline {\crtrefnumber{eq:intro:Delta_G_wt}}eq:intro:Delta_G_wt}{11}{equation.1.17}\protected@file@percent }
\newlabel{eq:intro:Delta_G_wt@cref}{{[equation][17][1]1.17}{[1][10][]11}{}{}{}}
\@writefile{loe}{\contentsline {notation}{\ifthmt@listswap Notation~1.18\else \numberline {1.18}Notation\fi \thmtformatoptarg {Twisted cyclic symmetry}}{11}{notation.1.18}\protected@file@percent }
\newlabel{notn:BACKGR:cs}{{1.18}{11}{Twisted cyclic symmetry}{notation.1.18}{}}
\@writefile{lla}{\contentsline {section}{\numberline {\crtrefnumber{notn:BACKGR:cs}}notn:BACKGR:cs}{11}{notation.1.18}\protected@file@percent }
\newlabel{notn:BACKGR:cs@cref}{{[notation][18][1]1.18}{[1][11][]11}{}{}{}}
\newlabel{eq:BACKGR:Ptp_G}{{1.18}{11}{Totally nonnegative Grassmannian}{equation.1.18}{}}
\@writefile{lla}{\contentsline {section}{\numberline {\crtrefnumber{eq:BACKGR:Ptp_G}}eq:BACKGR:Ptp_G}{11}{equation.1.18}\protected@file@percent }
\newlabel{eq:BACKGR:Ptp_G@cref}{{[equation][18][1]1.18}{[1][11][]11}{}{}{}}
\@writefile{loe}{\contentsline {definition}{\ifthmt@listswap Definition~1.19\else \numberline {1.19}Definition\fi }{11}{definition.1.19}\protected@file@percent }
\newlabel{dfn:reduced}{{1.19}{11}{}{definition.1.19}{}}
\@writefile{lla}{\contentsline {section}{\numberline {\crtrefnumber{dfn:reduced}}dfn:reduced}{11}{definition.1.19}\protected@file@percent }
\newlabel{dfn:reduced@cref}{{[definition][19][1]1.19}{[1][11][]11}{}{}{}}
\@writefile{loe}{\contentsline {remark}{\ifthmt@listswap Remark~1.20\else \numberline {1.20}Remark\fi }{11}{remark.1.20}\protected@file@percent }
\newlabel{rmk:altp_vs_color_swap}{{1.20}{11}{}{remark.1.20}{}}
\@writefile{lla}{\contentsline {section}{\numberline {\crtrefnumber{rmk:altp_vs_color_swap}}rmk:altp_vs_color_swap}{11}{remark.1.20}\protected@file@percent }
\newlabel{rmk:altp_vs_color_swap@cref}{{[remark][20][1]1.20}{[1][11][]11}{}{}{}}
\newlabel{sec:DIM:KSprim}{{1.4}{11}{Kasteleyn theory and \KSprims }{subsection.1.4}{}}
\@writefile{lla}{\contentsline {section}{\numberline {\crtrefnumber{sec:DIM:KSprim}}sec:DIM:KSprim}{11}{subsection.1.4}\protected@file@percent }
\newlabel{sec:DIM:KSprim@cref}{{[subsection][4][1]1.4}{[1][11][]11}{}{}{}}
\@writefile{toc}{\contentsline {subsection}{\tocsubsection {}{1.4}{Kasteleyn theory and Kenyon--Smirnov primitives\xspace  }}{11}{subsection.1.4}\protected@file@percent }
\@writefile{loe}{\contentsline {definition}{\ifthmt@listswap Definition~1.21\else \numberline {1.21}Definition\fi \thmtformatoptarg {\cite  {AGPR,SpeyerVariations}}}{11}{definition.1.21}\protected@file@percent }
\newlabel{dfn:DIM:Kast}{{1.21}{11}{\cite {AGPR,SpeyerVariations}}{definition.1.21}{}}
\@writefile{lla}{\contentsline {section}{\numberline {\crtrefnumber{dfn:DIM:Kast}}dfn:DIM:Kast}{11}{definition.1.21}\protected@file@percent }
\newlabel{dfn:DIM:Kast@cref}{{[definition][21][1]1.21}{[1][11][]11}{}{}{}}
\newlabel{eq:Kast_sign}{{1.19}{11}{\cite {AGPR,SpeyerVariations}}{equation.1.19}{}}
\@writefile{lla}{\contentsline {section}{\numberline {\crtrefnumber{eq:Kast_sign}}eq:Kast_sign}{11}{equation.1.19}\protected@file@percent }
\newlabel{eq:Kast_sign@cref}{{[equation][19][1]1.19}{[1][11][]11}{}{}{}}
\@writefile{loe}{\contentsline {remark}{\ifthmt@listswap Remark~1.22\else \numberline {1.22}Remark\fi }{11}{remark.1.22}\protected@file@percent }
\newlabel{rmk:Kast_sign_float}{{1.22}{11}{}{remark.1.22}{}}
\@writefile{lla}{\contentsline {section}{\numberline {\crtrefnumber{rmk:Kast_sign_float}}rmk:Kast_sign_float}{11}{remark.1.22}\protected@file@percent }
\newlabel{rmk:Kast_sign_float@cref}{{[remark][22][1]1.22}{[1][11][]11}{}{}{}}
\citation{Kenyon_lectures}
\citation{AGPR}
\citation{origami1}
\@writefile{loe}{\contentsline {lemma}{\ifthmt@listswap Lemma~1.23\else \numberline {1.23}Lemma\fi \thmtformatoptarg {\cite  [Lemma~1]{Kenyon_lectures} and~\cite  [\cref  *{M-lemma:OCP:Kast_even}]{origami1}\xspace  }}{12}{lemma.1.23}\protected@file@percent }
\newlabel{lemma:OCP:Kast_even}{{1.23}{12}{\cite [Lemma~1]{Kenyon_lectures} and~\Mref {lemma:OCP:Kast_even}}{lemma.1.23}{}}
\@writefile{lla}{\contentsline {section}{\numberline {\crtrefnumber{lemma:OCP:Kast_even}}lemma:OCP:Kast_even}{12}{lemma.1.23}\protected@file@percent }
\newlabel{lemma:OCP:Kast_even@cref}{{[lemma][23][1]1.23}{[1][11][]12}{}{}{}}
\newlabel{eq:OCP:holom}{{1.20}{12}{Kasteleyn theory and \KSprims }{equation.1.20}{}}
\@writefile{lla}{\contentsline {section}{\numberline {\crtrefnumber{eq:OCP:holom}}eq:OCP:holom}{12}{equation.1.20}\protected@file@percent }
\newlabel{eq:OCP:holom@cref}{{[equation][20][1]1.20}{[1][12][]12}{}{}{}}
\newlabel{eq:partial_F_dfn}{{1.21}{12}{Kasteleyn theory and \KSprims }{equation.1.21}{}}
\@writefile{lla}{\contentsline {section}{\numberline {\crtrefnumber{eq:partial_F_dfn}}eq:partial_F_dfn}{12}{equation.1.21}\protected@file@percent }
\newlabel{eq:partial_F_dfn@cref}{{[equation][21][1]1.21}{[1][12][]12}{}{}{}}
\newlabel{eq:OCP:primitive}{{1.22}{12}{Kasteleyn theory and \KSprims }{equation.1.22}{}}
\@writefile{lla}{\contentsline {section}{\numberline {\crtrefnumber{eq:OCP:primitive}}eq:OCP:primitive}{12}{equation.1.22}\protected@file@percent }
\newlabel{eq:OCP:primitive@cref}{{[equation][22][1]1.22}{[1][12][]12}{}{}{}}
\newlabel{eq:TE:t_imm_bdry_vs_pFw_pFb}{{1.23}{12}{Kasteleyn theory and \KSprims }{equation.1.23}{}}
\@writefile{lla}{\contentsline {section}{\numberline {\crtrefnumber{eq:TE:t_imm_bdry_vs_pFw_pFb}}eq:TE:t_imm_bdry_vs_pFw_pFb}{12}{equation.1.23}\protected@file@percent }
\newlabel{eq:TE:t_imm_bdry_vs_pFw_pFb@cref}{{[equation][23][1]1.23}{[1][12][]12}{}{}{}}
\@writefile{loe}{\contentsline {remark}{\ifthmt@listswap Remark~1.24\else \numberline {1.24}Remark\fi }{12}{remark.1.24}\protected@file@percent }
\newlabel{rmk:DIM:Kast_gauge_eq}{{1.24}{12}{}{remark.1.24}{}}
\@writefile{lla}{\contentsline {section}{\numberline {\crtrefnumber{rmk:DIM:Kast_gauge_eq}}rmk:DIM:Kast_gauge_eq}{12}{remark.1.24}\protected@file@percent }
\newlabel{rmk:DIM:Kast_gauge_eq@cref}{{[remark][24][1]1.24}{[1][12][]12}{}{}{}}
\@writefile{loe}{\contentsline {remark}{\ifthmt@listswap Remark~1.25\else \numberline {1.25}Remark\fi }{12}{remark.1.25}\protected@file@percent }
\newlabel{rmk:DIM:otimes}{{1.25}{12}{}{remark.1.25}{}}
\@writefile{lla}{\contentsline {section}{\numberline {\crtrefnumber{rmk:DIM:otimes}}rmk:DIM:otimes}{12}{remark.1.25}\protected@file@percent }
\newlabel{rmk:DIM:otimes@cref}{{[remark][25][1]1.25}{[1][12][]12}{}{}{}}
\@writefile{loe}{\contentsline {definition}{\ifthmt@listswap Definition~1.26\else \numberline {1.26}Definition\fi }{12}{definition.1.26}\protected@file@percent }
\newlabel{dfn:MCE:WKmat}{{1.26}{12}{}{definition.1.26}{}}
\@writefile{lla}{\contentsline {section}{\numberline {\crtrefnumber{dfn:MCE:WKmat}}dfn:MCE:WKmat}{12}{definition.1.26}\protected@file@percent }
\newlabel{dfn:MCE:WKmat@cref}{{[definition][26][1]1.26}{[1][12][]12}{}{}{}}
\@writefile{loe}{\contentsline {proposition}{\ifthmt@listswap Proposition~1.27\else \numberline {1.27}Proposition\fi \thmtformatoptarg {\cite  [Corollary~6.8 and Proposition~6.9]{AGPR}}}{12}{proposition.1.27}\protected@file@percent }
\newlabel{lemma:MCE:Delta_vs_Kast}{{1.27}{12}{\cite [Corollary~6.8 and Proposition~6.9]{AGPR}}{proposition.1.27}{}}
\@writefile{lla}{\contentsline {section}{\numberline {\crtrefnumber{lemma:MCE:Delta_vs_Kast}}lemma:MCE:Delta_vs_Kast}{12}{proposition.1.27}\protected@file@percent }
\newlabel{lemma:MCE:Delta_vs_Kast@cref}{{[proposition][27][1]1.27}{[1][12][]12}{}{}{}}
\@writefile{loe}{\contentsline {corollary}{\ifthmt@listswap Corollary~1.28\else \numberline {1.28}Corollary\fi \thmtformatoptarg {\cite  [\cref  *{M-lemma:MCE:apm_vs_Kast}]{origami1}\xspace  }}{12}{corollary.1.28}\protected@file@percent }
\newlabel{lemma:MCE:apm_vs_Kast}{{1.28}{12}{\Mref {lemma:MCE:apm_vs_Kast}}{corollary.1.28}{}}
\@writefile{lla}{\contentsline {section}{\numberline {\crtrefnumber{lemma:MCE:apm_vs_Kast}}lemma:MCE:apm_vs_Kast}{12}{corollary.1.28}\protected@file@percent }
\newlabel{lemma:MCE:apm_vs_Kast@cref}{{[corollary][28][1]1.28}{[1][12][]12}{}{}{}}
\newlabel{apm_vs_Kast1}{{{{(1)}}}{12}{\Mref {lemma:MCE:apm_vs_Kast}}{Item.1}{}}
\@writefile{lla}{\contentsline {section}{\numberline {\crtrefnumber{apm_vs_Kast1}}apm_vs_Kast1}{12}{Item.1}\protected@file@percent }
\newlabel{apm_vs_Kast1@cref}{{[enumi][1][]{{(1)}}}{[1][12][]12}{}{}{}}
\newlabel{apm_vs_Kast2}{{{{(2)}}}{12}{\Mref {lemma:MCE:apm_vs_Kast}}{Item.2}{}}
\@writefile{lla}{\contentsline {section}{\numberline {\crtrefnumber{apm_vs_Kast2}}apm_vs_Kast2}{12}{Item.2}\protected@file@percent }
\newlabel{apm_vs_Kast2@cref}{{[enumi][2][]{{(2)}}}{[1][12][]12}{}{}{}}
\citation{origami1}
\citation{DFLP}
\citation{origami1}
\citation{DFLP}
\newlabel{apm_vs_Kast3}{{{{(3)}}}{13}{\Mref {lemma:MCE:apm_vs_Kast}}{Item.3}{}}
\@writefile{lla}{\contentsline {section}{\numberline {\crtrefnumber{apm_vs_Kast3}}apm_vs_Kast3}{13}{Item.3}\protected@file@percent }
\newlabel{apm_vs_Kast3@cref}{{[enumi][3][]{{(3)}}}{[1][12][]13}{}{}{}}
\newlabel{eq:MCE:alt(C)_vs_pFw}{{1.24}{13}{\Mref {lemma:MCE:apm_vs_Kast}}{equation.1.24}{}}
\@writefile{lla}{\contentsline {section}{\numberline {\crtrefnumber{eq:MCE:alt(C)_vs_pFw}}eq:MCE:alt(C)_vs_pFw}{13}{equation.1.24}\protected@file@percent }
\newlabel{eq:MCE:alt(C)_vs_pFw@cref}{{[equation][24][1]1.24}{[1][12][]13}{}{}{}}
\@writefile{loe}{\contentsline {remark}{\ifthmt@listswap Remark~1.29\else \numberline {1.29}Remark\fi }{13}{remark.1.29}\protected@file@percent }
\newlabel{rmk:MCE:BKmat}{{1.29}{13}{}{remark.1.29}{}}
\@writefile{lla}{\contentsline {section}{\numberline {\crtrefnumber{rmk:MCE:BKmat}}rmk:MCE:BKmat}{13}{remark.1.29}\protected@file@percent }
\newlabel{rmk:MCE:BKmat@cref}{{[remark][29][1]1.29}{[1][13][]13}{}{}{}}
\newlabel{eq:MCE:alt(Cp)_vs_pFb}{{1.25}{13}{}{equation.1.25}{}}
\@writefile{lla}{\contentsline {section}{\numberline {\crtrefnumber{eq:MCE:alt(Cp)_vs_pFb}}eq:MCE:alt(Cp)_vs_pFb}{13}{equation.1.25}\protected@file@percent }
\newlabel{eq:MCE:alt(Cp)_vs_pFb@cref}{{[equation][25][1]1.25}{[1][13][]13}{}{}{}}
\@writefile{loe}{\contentsline {definition}{\ifthmt@listswap Definition~1.30\else \numberline {1.30}Definition\fi \thmtformatoptarg {Boundary restriction and extension}}{13}{definition.1.30}\protected@file@percent }
\newlabel{dfn:OCP:restr_ext}{{1.30}{13}{Boundary restriction and extension}{definition.1.30}{}}
\@writefile{lla}{\contentsline {section}{\numberline {\crtrefnumber{dfn:OCP:restr_ext}}dfn:OCP:restr_ext}{13}{definition.1.30}\protected@file@percent }
\newlabel{dfn:OCP:restr_ext@cref}{{[definition][30][1]1.30}{[1][13][]13}{}{}{}}
\@writefile{loe}{\contentsline {proposition}{\ifthmt@listswap Proposition~1.31\else \numberline {1.31}Proposition\fi \thmtformatoptarg {\cite  [\cref  *{M-lemma:DIM:remove_bivertex}]{origami1}\xspace  }}{13}{proposition.1.31}\protected@file@percent }
\newlabel{lemma:DIM:remove_bivertex}{{1.31}{13}{\Mref {lemma:DIM:remove_bivertex}}{proposition.1.31}{}}
\@writefile{lla}{\contentsline {section}{\numberline {\crtrefnumber{lemma:DIM:remove_bivertex}}lemma:DIM:remove_bivertex}{13}{proposition.1.31}\protected@file@percent }
\newlabel{lemma:DIM:remove_bivertex@cref}{{[proposition][31][1]1.31}{[1][13][]13}{}{}{}}
\newlabel{eq:DIM:remove_bivertex_w}{{1.26}{13}{\Mref {lemma:DIM:remove_bivertex}}{equation.1.26}{}}
\@writefile{lla}{\contentsline {section}{\numberline {\crtrefnumber{eq:DIM:remove_bivertex_w}}eq:DIM:remove_bivertex_w}{13}{equation.1.26}\protected@file@percent }
\newlabel{eq:DIM:remove_bivertex_w@cref}{{[equation][26][1]1.26}{[1][13][]13}{}{}{}}
\newlabel{eq:DIM:remove_bivertex_b}{{1.27}{13}{\Mref {lemma:DIM:remove_bivertex}}{equation.1.27}{}}
\@writefile{lla}{\contentsline {section}{\numberline {\crtrefnumber{eq:DIM:remove_bivertex_b}}eq:DIM:remove_bivertex_b}{13}{equation.1.27}\protected@file@percent }
\newlabel{eq:DIM:remove_bivertex_b@cref}{{[equation][27][1]1.27}{[1][13][]13}{}{}{}}
\@writefile{loe}{\contentsline {proposition}{\ifthmt@listswap Proposition~1.32\else \numberline {1.32}Proposition\fi \thmtformatoptarg {Popping a black vertex}}{13}{proposition.1.32}\protected@file@percent }
\newlabel{lemma:DIM:remove_add}{{1.32}{13}{Popping a black vertex}{proposition.1.32}{}}
\@writefile{lla}{\contentsline {section}{\numberline {\crtrefnumber{lemma:DIM:remove_add}}lemma:DIM:remove_add}{13}{proposition.1.32}\protected@file@percent }
\newlabel{lemma:DIM:remove_add@cref}{{[proposition][32][1]1.32}{[1][13][]13}{}{}{}}
\newlabel{eq:DIM:remove_add}{{1.28}{13}{Popping a black vertex}{equation.1.28}{}}
\@writefile{lla}{\contentsline {section}{\numberline {\crtrefnumber{eq:DIM:remove_add}}eq:DIM:remove_add}{13}{equation.1.28}\protected@file@percent }
\newlabel{eq:DIM:remove_add@cref}{{[equation][28][1]1.28}{[1][13][]13}{}{}{}}
\@writefile{loe}{\contentsline {remark}{\ifthmt@listswap Remark~1.33\else \numberline {1.33}Remark\fi }{13}{remark.1.33}\protected@file@percent }
\newlabel{rmk:add_remove_vs_remove_two}{{1.33}{13}{}{remark.1.33}{}}
\@writefile{lla}{\contentsline {section}{\numberline {\crtrefnumber{rmk:add_remove_vs_remove_two}}rmk:add_remove_vs_remove_two}{13}{remark.1.33}\protected@file@percent }
\newlabel{rmk:add_remove_vs_remove_two@cref}{{[remark][33][1]1.33}{[1][13][]13}{}{}{}}
\newlabel{ssec:BACKGR:mom_ampl}{{1.5}{13}{Momentum amplituhedron map and immanant-nonnegativity}{subsection.1.5}{}}
\@writefile{lla}{\contentsline {section}{\numberline {\crtrefnumber{ssec:BACKGR:mom_ampl}}ssec:BACKGR:mom_ampl}{13}{subsection.1.5}\protected@file@percent }
\newlabel{ssec:BACKGR:mom_ampl@cref}{{[subsection][5][1]1.5}{[1][13][]13}{}{}{}}
\@writefile{toc}{\contentsline {subsection}{\tocsubsection {}{1.5}{Momentum amplituhedron map and immanant-nonnegativity}}{13}{subsection.1.5}\protected@file@percent }
\@writefile{loe}{\contentsline {definition}{\ifthmt@listswap Definition~1.34\else \numberline {1.34}Definition\fi }{13}{definition.1.34}\protected@file@percent }
\newlabel{dfn:BACKGR:nondeg}{{1.34}{13}{}{definition.1.34}{}}
\@writefile{lla}{\contentsline {section}{\numberline {\crtrefnumber{dfn:BACKGR:nondeg}}dfn:BACKGR:nondeg}{13}{definition.1.34}\protected@file@percent }
\newlabel{dfn:BACKGR:nondeg@cref}{{[definition][34][1]1.34}{[1][13][]13}{}{}{}}
\citation{DFLP}
\citation{origami1}
\citation{origami1}
\citation{origami1}
\citation{origami1}
\citation{AHCC}
\citation{abcgpt}
\citation{origami1}
\citation{origami1}
\citation{origami1}
\citation{KLRR}
\citation{CLR1}
\citation{origami1}
\@writefile{loe}{\contentsline {definition}{\ifthmt@listswap Definition~1.35\else \numberline {1.35}Definition\fi }{14}{definition.1.35}\protected@file@percent }
\newlabel{eq:intro:LaLat}{{1.29}{14}{}{equation.1.29}{}}
\@writefile{lla}{\contentsline {section}{\numberline {\crtrefnumber{eq:intro:LaLat}}eq:intro:LaLat}{14}{equation.1.29}\protected@file@percent }
\newlabel{eq:intro:LaLat@cref}{{[equation][29][1]1.29}{[1][13][]14}{}{}{}}
\newlabel{eq:intro:PhiLL_dfn}{{1.30}{14}{}{equation.1.30}{}}
\@writefile{lla}{\contentsline {section}{\numberline {\crtrefnumber{eq:intro:PhiLL_dfn}}eq:intro:PhiLL_dfn}{14}{equation.1.30}\protected@file@percent }
\newlabel{eq:intro:PhiLL_dfn@cref}{{[equation][30][1]1.30}{[1][13][]14}{}{}{}}
\@writefile{loe}{\contentsline {lemma}{\ifthmt@listswap Lemma~1.36\else \numberline {1.36}Lemma\fi \thmtformatoptarg {\cite  {DFLP} and~\cite  [\cref  *{M-prop:momLL_basic}]{origami1}\xspace  }}{14}{lemma.1.36}\protected@file@percent }
\newlabel{lemma:OAC:PhiLL_in_lalak}{{1.36}{14}{\cite {DFLP} and~\Mref {prop:momLL_basic}}{lemma.1.36}{}}
\@writefile{lla}{\contentsline {section}{\numberline {\crtrefnumber{lemma:OAC:PhiLL_in_lalak}}lemma:OAC:PhiLL_in_lalak}{14}{lemma.1.36}\protected@file@percent }
\newlabel{lemma:OAC:PhiLL_in_lalak@cref}{{[lemma][36][1]1.36}{[1][14][]14}{}{}{}}
\@writefile{loe}{\contentsline {remark}{\ifthmt@listswap Remark~1.37\else \numberline {1.37}Remark\fi }{14}{remark.1.37}\protected@file@percent }
\newlabel{rmk:orientation_inherits}{{1.37}{14}{}{remark.1.37}{}}
\@writefile{lla}{\contentsline {section}{\numberline {\crtrefnumber{rmk:orientation_inherits}}rmk:orientation_inherits}{14}{remark.1.37}\protected@file@percent }
\newlabel{rmk:orientation_inherits@cref}{{[remark][37][1]1.37}{[1][14][]14}{}{}{}}
\@writefile{loe}{\contentsline {definition}{\ifthmt@listswap Definition~1.38\else \numberline {1.38}Definition\fi \thmtformatoptarg {\cite  [\cref  *{M-dfn:Ttauknij}]{origami1}\xspace  }}{14}{definition.1.38}\protected@file@percent }
\newlabel{dfn:BACKGR:immp}{{1.38}{14}{\Mref {dfn:Ttauknij}}{definition.1.38}{}}
\@writefile{lla}{\contentsline {section}{\numberline {\crtrefnumber{dfn:BACKGR:immp}}dfn:BACKGR:immp}{14}{definition.1.38}\protected@file@percent }
\newlabel{dfn:BACKGR:immp@cref}{{[definition][38][1]1.38}{[1][14][]14}{}{}{}}
\@writefile{loe}{\contentsline {proposition}{\ifthmt@listswap Proposition~1.39\else \numberline {1.39}Proposition\fi \thmtformatoptarg {\cite  [\cref  *{M-lemma:LaLaimmp_nonempty_Z_dense}]{origami1}\xspace  }}{14}{proposition.1.39}\protected@file@percent }
\newlabel{lemma:LaLaimmp_nonempty_Z_dense}{{1.39}{14}{\Mref {lemma:LaLaimmp_nonempty_Z_dense}}{proposition.1.39}{}}
\@writefile{lla}{\contentsline {section}{\numberline {\crtrefnumber{lemma:LaLaimmp_nonempty_Z_dense}}lemma:LaLaimmp_nonempty_Z_dense}{14}{proposition.1.39}\protected@file@percent }
\newlabel{lemma:LaLaimmp_nonempty_Z_dense@cref}{{[proposition][39][1]1.39}{[1][14][]14}{}{}{}}
\@writefile{toc}{\contentsline {subsection}{\tocsubsection {}{1.6}{The magic projector $Q_{\lambda }$}}{14}{subsection.1.6}\protected@file@percent }
\newlabel{eq:intro:Qla}{{1.31}{14}{The magic projector \texorpdfstring {$\Qla $}{Q\_lambda}}{equation.1.31}{}}
\@writefile{lla}{\contentsline {section}{\numberline {\crtrefnumber{eq:intro:Qla}}eq:intro:Qla}{14}{equation.1.31}\protected@file@percent }
\newlabel{eq:intro:Qla@cref}{{[equation][31][1]1.31}{[1][14][]14}{}{}{}}
\newlabel{eq:Qla_Qlapp_preserve_TNN}{{1.32}{14}{The magic projector \texorpdfstring {$\Qla $}{Q\_lambda}}{equation.1.32}{}}
\@writefile{lla}{\contentsline {section}{\numberline {\crtrefnumber{eq:Qla_Qlapp_preserve_TNN}}eq:Qla_Qlapp_preserve_TNN}{14}{equation.1.32}\protected@file@percent }
\newlabel{eq:Qla_Qlapp_preserve_TNN@cref}{{[equation][32][1]1.32}{[1][14][]14}{}{}{}}
\@writefile{toc}{\contentsline {part}{\tocpart {Part}{1}{Origami-amplituhedron correspondence\xspace  and T-duality}}{14}{part.1}\protected@file@percent }
\newlabel{part1}{{1}{14}{\OACTITLE and T-duality}{part.1}{}}
\@writefile{lla}{\contentsline {section}{\numberline {\crtrefnumber{part1}}part1}{14}{part.1}\protected@file@percent }
\newlabel{part1@cref}{{[part][1][]1}{[1][14][]14}{}{}{}}
\@writefile{toc}{\contentsline {section}{\tocsection {}{2}{Origami-amplituhedron correspondence\xspace  for weak t-embeddings\xspace  }}{14}{section.2}\protected@file@percent }
\newlabel{sec:TE}{{2}{14}{\OACTITLE for \wtembsTITLE }{section.2}{}}
\@writefile{lla}{\contentsline {section}{\numberline {\crtrefnumber{sec:TE}}sec:TE}{14}{section.2}\protected@file@percent }
\newlabel{sec:TE@cref}{{[section][2][]2}{[1][14][]14}{}{}{}}
\citation{KLRR}
\citation{origami1}
\citation{KLRR}
\citation{KLRR}
\citation{KLRR}
\newlabel{ssec:TE:dfn}{{2.1}{15}{Defining \wtembsTITLE }{subsection.2.1}{}}
\@writefile{lla}{\contentsline {section}{\numberline {\crtrefnumber{ssec:TE:dfn}}ssec:TE:dfn}{15}{subsection.2.1}\protected@file@percent }
\newlabel{ssec:TE:dfn@cref}{{[subsection][1][2]2.1}{[1][14][]15}{}{}{}}
\@writefile{toc}{\contentsline {subsection}{\tocsubsection {}{2.1}{Defining weak t-embeddings\xspace  }}{15}{subsection.2.1}\protected@file@percent }
\@writefile{loe}{\contentsline {definition}{\ifthmt@listswap Definition~2.1\else \numberline {2.1}Definition\fi }{15}{definition.2.1}\protected@file@percent }
\newlabel{dfn:TE:datr}{{2.1}{15}{}{definition.2.1}{}}
\@writefile{lla}{\contentsline {section}{\numberline {\crtrefnumber{dfn:TE:datr}}dfn:TE:datr}{15}{definition.2.1}\protected@file@percent }
\newlabel{dfn:TE:datr@cref}{{[definition][1][2]2.1}{[1][14][]15}{}{}{}}
\@writefile{loe}{\contentsline {definition}{\ifthmt@listswap Definition~2.2\else \numberline {2.2}Definition\fi \thmtformatoptarg {Weak t-embedding\xspace  }}{15}{definition.2.2}\protected@file@percent }
\newlabel{dfn:TE:tembending}{{2.2}{15}{\Wtemb }{definition.2.2}{}}
\@writefile{lla}{\contentsline {section}{\numberline {\crtrefnumber{dfn:TE:tembending}}dfn:TE:tembending}{15}{definition.2.2}\protected@file@percent }
\newlabel{dfn:TE:tembending@cref}{{[definition][2][2]2.2}{[1][15][]15}{}{}{}}
\newlabel{TE:bdry_angle}{{{{(WTE1)}}}{15}{\Wtemb }{Item.4}{}}
\@writefile{lla}{\contentsline {section}{\numberline {\crtrefnumber{TE:bdry_angle}}TE:bdry_angle}{15}{Item.4}\protected@file@percent }
\newlabel{TE:bdry_angle@cref}{{[enumi][1][]{{(WTE1)}}}{[1][15][]15}{}{}{}}
\newlabel{eq:TE:weak_t_imm_bdry}{{2.1}{15}{\Wtemb }{equation.2.1}{}}
\@writefile{lla}{\contentsline {section}{\numberline {\crtrefnumber{eq:TE:weak_t_imm_bdry}}eq:TE:weak_t_imm_bdry}{15}{equation.2.1}\protected@file@percent }
\newlabel{eq:TE:weak_t_imm_bdry@cref}{{[equation][1][2]2.1}{[1][15][]15}{}{}{}}
\newlabel{eq:TE:dfn}{{2.2}{15}{\Wtemb }{equation.2.2}{}}
\@writefile{lla}{\contentsline {section}{\numberline {\crtrefnumber{eq:TE:dfn}}eq:TE:dfn}{15}{equation.2.2}\protected@file@percent }
\newlabel{eq:TE:dfn@cref}{{[equation][2][2]2.2}{[1][15][]15}{}{}{}}
\newlabel{TE:bdry_winding}{{{{(WTE2)}}}{15}{\Wtemb }{Item.5}{}}
\@writefile{lla}{\contentsline {section}{\numberline {\crtrefnumber{TE:bdry_winding}}TE:bdry_winding}{15}{Item.5}\protected@file@percent }
\newlabel{TE:bdry_winding@cref}{{[enumi][2][]{{(WTE2)}}}{[1][15][]15}{}{}{}}
\newlabel{eq:TE:bdry_winding}{{2.3}{15}{\Wtemb }{equation.2.3}{}}
\@writefile{lla}{\contentsline {section}{\numberline {\crtrefnumber{eq:TE:bdry_winding}}eq:TE:bdry_winding}{15}{equation.2.3}\protected@file@percent }
\newlabel{eq:TE:bdry_winding@cref}{{[equation][3][2]2.3}{[1][15][]15}{}{}{}}
\newlabel{TE:t_imm}{{{{(WTE3)}}}{15}{\Wtemb }{Item.6}{}}
\@writefile{lla}{\contentsline {section}{\numberline {\crtrefnumber{TE:t_imm}}TE:t_imm}{15}{Item.6}\protected@file@percent }
\newlabel{TE:t_imm@cref}{{[enumi][3][]{{(WTE3)}}}{[1][15][]15}{}{}{}}
\newlabel{eq:TE:weak_t_imm_dfn}{{2.4}{15}{\Wtemb }{equation.2.4}{}}
\@writefile{lla}{\contentsline {section}{\numberline {\crtrefnumber{eq:TE:weak_t_imm_dfn}}eq:TE:weak_t_imm_dfn}{15}{equation.2.4}\protected@file@percent }
\newlabel{eq:TE:weak_t_imm_dfn@cref}{{[equation][4][2]2.4}{[1][15][]15}{}{}{}}
\@writefile{loe}{\contentsline {definition}{\ifthmt@listswap Definition~2.3\else \numberline {2.3}Definition\fi }{15}{definition.2.3}\protected@file@percent }
\newlabel{dfn:TE:generic}{{2.3}{15}{}{definition.2.3}{}}
\@writefile{lla}{\contentsline {section}{\numberline {\crtrefnumber{dfn:TE:generic}}dfn:TE:generic}{15}{definition.2.3}\protected@file@percent }
\newlabel{dfn:TE:generic@cref}{{[definition][3][2]2.3}{[1][15][]15}{}{}{}}
\@writefile{loe}{\contentsline {remark}{\ifthmt@listswap Remark~2.4\else \numberline {2.4}Remark\fi }{15}{remark.2.4}\protected@file@percent }
\newlabel{rmk:TE:einj_nonvanishing}{{2.4}{15}{}{remark.2.4}{}}
\@writefile{lla}{\contentsline {section}{\numberline {\crtrefnumber{rmk:TE:einj_nonvanishing}}rmk:TE:einj_nonvanishing}{15}{remark.2.4}\protected@file@percent }
\newlabel{rmk:TE:einj_nonvanishing@cref}{{[remark][4][2]2.4}{[1][15][]15}{}{}{}}
\@writefile{loe}{\contentsline {example}{\ifthmt@listswap Example~2.5\else \numberline {2.5}Example\fi }{15}{example.2.5}\protected@file@percent }
\newlabel{ex:non-einj}{{2.5}{15}{}{example.2.5}{}}
\@writefile{lla}{\contentsline {section}{\numberline {\crtrefnumber{ex:non-einj}}ex:non-einj}{15}{example.2.5}\protected@file@percent }
\newlabel{ex:non-einj@cref}{{[example][5][2]2.5}{[1][15][]15}{}{}{}}
\citation{Lovasz_Plummer}
\citation{Kenyon_Sheffield}
\citation{Lovasz_Plummer}
\citation{origami1}
\citation{origami1}
\citation{origami1}
\@writefile{lof}{\contentsline {figure}{\numberline {6}{\ignorespaces  Examples of weighted graphs $(\Gamma ,\operatorname  {wt})$ (with Kasteleyn edge weights shown) satisfying $k_{\min }(\Gamma )=1$ but admitting no edge-injective\xspace  weak t-immersions\xspace  .}}{16}{figure.caption.14}\protected@file@percent }
\newlabel{fig:non-einj}{{6}{16}{Examples of weighted graphs $(\G ,\wt )$ (with Kasteleyn edge weights shown) satisfying $\helmin (\G )=1$ but admitting no \einj \wtimms }{figure.caption.14}{}}
\@writefile{lla}{\contentsline {section}{\numberline {\crtrefnumber{fig:non-einj}}fig:non-einj}{16}{figure.caption.14}\protected@file@percent }
\newlabel{fig:non-einj@cref}{{[figure][6][]6}{[1][15][]16}{}{}{}}
\newlabel{ssec:BACKGR:surplus}{{2.2}{16}{Surplus}{subsection.2.2}{}}
\@writefile{lla}{\contentsline {section}{\numberline {\crtrefnumber{ssec:BACKGR:surplus}}ssec:BACKGR:surplus}{16}{subsection.2.2}\protected@file@percent }
\newlabel{ssec:BACKGR:surplus@cref}{{[subsection][2][2]2.2}{[1][16][]16}{}{}{}}
\@writefile{toc}{\contentsline {subsection}{\tocsubsection {}{2.2}{Surplus}}{16}{subsection.2.2}\protected@file@percent }
\newlabel{eq:DIM:helWmin_dfn}{{2.5}{16}{Surplus}{equation.2.5}{}}
\@writefile{lla}{\contentsline {section}{\numberline {\crtrefnumber{eq:DIM:helWmin_dfn}}eq:DIM:helWmin_dfn}{16}{equation.2.5}\protected@file@percent }
\newlabel{eq:DIM:helWmin_dfn@cref}{{[equation][5][2]2.5}{[1][16][]16}{}{}{}}
\newlabel{eq:DIM:helWming_dfn}{{2.6}{16}{Surplus}{equation.2.6}{}}
\@writefile{lla}{\contentsline {section}{\numberline {\crtrefnumber{eq:DIM:helWming_dfn}}eq:DIM:helWming_dfn}{16}{equation.2.6}\protected@file@percent }
\newlabel{eq:DIM:helWming_dfn@cref}{{[equation][6][2]2.6}{[1][16][]16}{}{}{}}
\@writefile{loe}{\contentsline {proposition}{\ifthmt@listswap Proposition~2.6\else \numberline {2.6}Proposition\fi \thmtformatoptarg {\cite  [Theorem~1.3.1]{Lovasz_Plummer}}}{16}{proposition.2.6}\protected@file@percent }
\newlabel{prop:DIM:helWBmin_geq_0=>apm_exists}{{2.6}{16}{\cite [Theorem~1.3.1]{Lovasz_Plummer}}{proposition.2.6}{}}
\@writefile{lla}{\contentsline {section}{\numberline {\crtrefnumber{prop:DIM:helWBmin_geq_0=>apm_exists}}prop:DIM:helWBmin_geq_0=>apm_exists}{16}{proposition.2.6}\protected@file@percent }
\newlabel{prop:DIM:helWBmin_geq_0=>apm_exists@cref}{{[proposition][6][2]2.6}{[1][16][]16}{}{}{}}
\@writefile{loe}{\contentsline {lemma}{\ifthmt@listswap Lemma~2.7\else \numberline {2.7}Lemma\fi \thmtformatoptarg {\cite  [\cref  *{M-lemma:DIM:deleting_hel_verts}]{origami1}\xspace  }}{16}{lemma.2.7}\protected@file@percent }
\newlabel{lemma:DIM:deleting_hel_verts}{{2.7}{16}{\Mref {lemma:DIM:deleting_hel_verts}}{lemma.2.7}{}}
\@writefile{lla}{\contentsline {section}{\numberline {\crtrefnumber{lemma:DIM:deleting_hel_verts}}lemma:DIM:deleting_hel_verts}{16}{lemma.2.7}\protected@file@percent }
\newlabel{lemma:DIM:deleting_hel_verts@cref}{{[lemma][7][2]2.7}{[1][16][]16}{}{}{}}
\newlabel{DIM:del1}{{{{(1)}}}{16}{\Mref {lemma:DIM:deleting_hel_verts}}{Item.7}{}}
\@writefile{lla}{\contentsline {section}{\numberline {\crtrefnumber{DIM:del1}}DIM:del1}{16}{Item.7}\protected@file@percent }
\newlabel{DIM:del1@cref}{{[enumi][1][]{{(1)}}}{[1][16][]16}{}{}{}}
\newlabel{DIM:del2}{{{{(2)}}}{16}{\Mref {lemma:DIM:deleting_hel_verts}}{Item.8}{}}
\@writefile{lla}{\contentsline {section}{\numberline {\crtrefnumber{DIM:del2}}DIM:del2}{16}{Item.8}\protected@file@percent }
\newlabel{DIM:del2@cref}{{[enumi][2][]{{(2)}}}{[1][16][]16}{}{}{}}
\@writefile{loe}{\contentsline {corollary}{\ifthmt@listswap Corollary~2.8\else \numberline {2.8}Corollary\fi \thmtformatoptarg {\cite  [\cref  *{M-lemma:hel_geq_1}]{origami1}\xspace  }}{16}{corollary.2.8}\protected@file@percent }
\newlabel{lemma:hel_geq_1}{{2.8}{16}{\Mref {lemma:hel_geq_1}}{corollary.2.8}{}}
\@writefile{lla}{\contentsline {section}{\numberline {\crtrefnumber{lemma:hel_geq_1}}lemma:hel_geq_1}{16}{corollary.2.8}\protected@file@percent }
\newlabel{lemma:hel_geq_1@cref}{{[corollary][8][2]2.8}{[1][16][]16}{}{}{}}
\@writefile{loe}{\contentsline {lemma}{\ifthmt@listswap Lemma~2.9\else \numberline {2.9}Lemma\fi }{16}{lemma.2.9}\protected@file@percent }
\newlabel{lemma:DIM:from_WNEI_to_WNEIg}{{2.9}{16}{}{lemma.2.9}{}}
\@writefile{lla}{\contentsline {section}{\numberline {\crtrefnumber{lemma:DIM:from_WNEI_to_WNEIg}}lemma:DIM:from_WNEI_to_WNEIg}{16}{lemma.2.9}\protected@file@percent }
\newlabel{lemma:DIM:from_WNEI_to_WNEIg@cref}{{[lemma][9][2]2.9}{[1][16][]16}{}{}{}}
\newlabel{eq:BACKGR:helWming_vs_helWmin}{{2.7}{16}{}{equation.2.7}{}}
\@writefile{lla}{\contentsline {section}{\numberline {\crtrefnumber{eq:BACKGR:helWming_vs_helWmin}}eq:BACKGR:helWming_vs_helWmin}{16}{equation.2.7}\protected@file@percent }
\newlabel{eq:BACKGR:helWming_vs_helWmin@cref}{{[equation][7][2]2.7}{[1][16][]16}{}{}{}}
\@writefile{loe}{\contentsline {lemma}{\ifthmt@listswap Lemma~2.10\else \numberline {2.10}Lemma\fi }{16}{lemma.2.10}\protected@file@percent }
\newlabel{lemma:DIM:no_floating}{{2.10}{16}{}{lemma.2.10}{}}
\@writefile{lla}{\contentsline {section}{\numberline {\crtrefnumber{lemma:DIM:no_floating}}lemma:DIM:no_floating}{16}{lemma.2.10}\protected@file@percent }
\newlabel{lemma:DIM:no_floating@cref}{{[lemma][10][2]2.10}{[1][16][]16}{}{}{}}
\@writefile{loe}{\contentsline {lemma}{\ifthmt@listswap Lemma~2.11\else \numberline {2.11}Lemma\fi \thmtformatoptarg {\cite  [\cref  *{M-lemma:DIM:moves_vs_helWmin}]{origami1}\xspace  }}{16}{lemma.2.11}\protected@file@percent }
\newlabel{lemma:DIM:moves_vs_helWmin}{{2.11}{16}{\Mref {lemma:DIM:moves_vs_helWmin}}{lemma.2.11}{}}
\@writefile{lla}{\contentsline {section}{\numberline {\crtrefnumber{lemma:DIM:moves_vs_helWmin}}lemma:DIM:moves_vs_helWmin}{16}{lemma.2.11}\protected@file@percent }
\newlabel{lemma:DIM:moves_vs_helWmin@cref}{{[lemma][11][2]2.11}{[1][16][]16}{}{}{}}
\@writefile{loe}{\contentsline {notation}{\ifthmt@listswap Notation~2.12\else \numberline {2.12}Notation\fi }{17}{notation.2.12}\protected@file@percent }
\newlabel{not:BACKGR:RgEbd_RgEint}{{2.12}{17}{}{notation.2.12}{}}
\@writefile{lla}{\contentsline {section}{\numberline {\crtrefnumber{not:BACKGR:RgEbd_RgEint}}not:BACKGR:RgEbd_RgEint}{17}{notation.2.12}\protected@file@percent }
\newlabel{not:BACKGR:RgEbd_RgEint@cref}{{[notation][12][2]2.12}{[1][16][]17}{}{}{}}
\@writefile{loe}{\contentsline {definition}{\ifthmt@listswap Definition~2.13\else \numberline {2.13}Definition\fi }{17}{definition.2.13}\protected@file@percent }
\newlabel{dfn:gelWB_for_bip}{{2.13}{17}{}{definition.2.13}{}}
\@writefile{lla}{\contentsline {section}{\numberline {\crtrefnumber{dfn:gelWB_for_bip}}dfn:gelWB_for_bip}{17}{definition.2.13}\protected@file@percent }
\newlabel{dfn:gelWB_for_bip@cref}{{[definition][13][2]2.13}{[1][17][]17}{}{}{}}
\newlabel{eq:BACKGR:hel=sum_hel_minus_E}{{2.8}{17}{}{equation.2.8}{}}
\@writefile{lla}{\contentsline {section}{\numberline {\crtrefnumber{eq:BACKGR:hel=sum_hel_minus_E}}eq:BACKGR:hel=sum_hel_minus_E}{17}{equation.2.8}\protected@file@percent }
\newlabel{eq:BACKGR:hel=sum_hel_minus_E@cref}{{[equation][8][2]2.8}{[1][17][]17}{}{}{}}
\newlabel{eq:BACKGR:gelWmin_gelBmin_dfn}{{2.9}{17}{}{equation.2.9}{}}
\@writefile{lla}{\contentsline {section}{\numberline {\crtrefnumber{eq:BACKGR:gelWmin_gelBmin_dfn}}eq:BACKGR:gelWmin_gelBmin_dfn}{17}{equation.2.9}\protected@file@percent }
\newlabel{eq:BACKGR:gelWmin_gelBmin_dfn@cref}{{[equation][9][2]2.9}{[1][17][]17}{}{}{}}
\@writefile{loe}{\contentsline {lemma}{\ifthmt@listswap Lemma~2.14\else \numberline {2.14}Lemma\fi }{17}{lemma.2.14}\protected@file@percent }
\newlabel{lemma:BCFW:gelWmin_vs_helWmin}{{2.14}{17}{}{lemma.2.14}{}}
\@writefile{lla}{\contentsline {section}{\numberline {\crtrefnumber{lemma:BCFW:gelWmin_vs_helWmin}}lemma:BCFW:gelWmin_vs_helWmin}{17}{lemma.2.14}\protected@file@percent }
\newlabel{lemma:BCFW:gelWmin_vs_helWmin@cref}{{[lemma][14][2]2.14}{[1][17][]17}{}{}{}}
\newlabel{eq:BCFW:helWmin=min_over_gelB}{{2.10}{17}{}{equation.2.10}{}}
\@writefile{lla}{\contentsline {section}{\numberline {\crtrefnumber{eq:BCFW:helWmin=min_over_gelB}}eq:BCFW:helWmin=min_over_gelB}{17}{equation.2.10}\protected@file@percent }
\newlabel{eq:BCFW:helWmin=min_over_gelB@cref}{{[equation][10][2]2.10}{[1][17][]17}{}{}{}}
\newlabel{eq:BCFW:gelWmin_vs_helWmin}{{2.11}{17}{}{equation.2.11}{}}
\@writefile{lla}{\contentsline {section}{\numberline {\crtrefnumber{eq:BCFW:gelWmin_vs_helWmin}}eq:BCFW:gelWmin_vs_helWmin}{17}{equation.2.11}\protected@file@percent }
\newlabel{eq:BCFW:gelWmin_vs_helWmin@cref}{{[equation][11][2]2.11}{[1][17][]17}{}{}{}}
\newlabel{eq:BCFW_gelWmin_vs_helWmin_two_sided}{{2.12}{17}{Surplus}{equation.2.12}{}}
\@writefile{lla}{\contentsline {section}{\numberline {\crtrefnumber{eq:BCFW_gelWmin_vs_helWmin_two_sided}}eq:BCFW_gelWmin_vs_helWmin_two_sided}{17}{equation.2.12}\protected@file@percent }
\newlabel{eq:BCFW_gelWmin_vs_helWmin_two_sided@cref}{{[equation][12][2]2.12}{[1][17][]17}{}{}{}}
\@writefile{loe}{\contentsline {definition}{\ifthmt@listswap Definition~2.15\else \numberline {2.15}Definition\fi }{17}{definition.2.15}\protected@file@percent }
\newlabel{dfn:BACKGR:holess}{{2.15}{17}{}{definition.2.15}{}}
\@writefile{lla}{\contentsline {section}{\numberline {\crtrefnumber{dfn:BACKGR:holess}}dfn:BACKGR:holess}{17}{definition.2.15}\protected@file@percent }
\newlabel{dfn:BACKGR:holess@cref}{{[definition][15][2]2.15}{[1][17][]17}{}{}{}}
\@writefile{loe}{\contentsline {remark}{\ifthmt@listswap Remark~2.16\else \numberline {2.16}Remark\fi }{17}{remark.2.16}\protected@file@percent }
\@writefile{loe}{\contentsline {lemma}{\ifthmt@listswap Lemma~2.17\else \numberline {2.17}Lemma\fi }{17}{lemma.2.17}\protected@file@percent }
\newlabel{eq:DIM:Rg_Rgcl_Rghol}{{2.13}{17}{}{equation.2.13}{}}
\@writefile{lla}{\contentsline {section}{\numberline {\crtrefnumber{eq:DIM:Rg_Rgcl_Rghol}}eq:DIM:Rg_Rgcl_Rghol}{17}{equation.2.13}\protected@file@percent }
\newlabel{eq:DIM:Rg_Rgcl_Rghol@cref}{{[equation][13][2]2.13}{[1][17][]17}{}{}{}}
\@writefile{loe}{\contentsline {definition}{\ifthmt@listswap Definition~2.18\else \numberline {2.18}Definition\fi }{17}{definition.2.18}\protected@file@percent }
\newlabel{dfn:BACKGR:sconn}{{2.18}{17}{}{definition.2.18}{}}
\@writefile{lla}{\contentsline {section}{\numberline {\crtrefnumber{dfn:BACKGR:sconn}}dfn:BACKGR:sconn}{17}{definition.2.18}\protected@file@percent }
\newlabel{dfn:BACKGR:sconn@cref}{{[definition][18][2]2.18}{[1][17][]17}{}{}{}}
\@writefile{loe}{\contentsline {lemma}{\ifthmt@listswap Lemma~2.19\else \numberline {2.19}Lemma\fi }{17}{lemma.2.19}\protected@file@percent }
\newlabel{lemma:BCFW:dualizable_holess_sconn}{{2.19}{17}{}{lemma.2.19}{}}
\@writefile{lla}{\contentsline {section}{\numberline {\crtrefnumber{lemma:BCFW:dualizable_holess_sconn}}lemma:BCFW:dualizable_holess_sconn}{17}{lemma.2.19}\protected@file@percent }
\newlabel{lemma:BCFW:dualizable_holess_sconn@cref}{{[lemma][19][2]2.19}{[1][17][]17}{}{}{}}
\@writefile{loe}{\contentsline {lemma}{\ifthmt@listswap Lemma~2.20\else \numberline {2.20}Lemma\fi }{17}{lemma.2.20}\protected@file@percent }
\newlabel{lemma:BCFW:Rg_simply_conn_lower_bound}{{2.20}{17}{}{lemma.2.20}{}}
\@writefile{lla}{\contentsline {section}{\numberline {\crtrefnumber{lemma:BCFW:Rg_simply_conn_lower_bound}}lemma:BCFW:Rg_simply_conn_lower_bound}{17}{lemma.2.20}\protected@file@percent }
\newlabel{lemma:BCFW:Rg_simply_conn_lower_bound@cref}{{[lemma][20][2]2.20}{[1][17][]17}{}{}{}}
\citation{KLRR}
\citation{CLR1}
\citation{origami1}
\citation{origami1}
\newlabel{sconn_lower1}{{{{(1)}}}{18}{}{Item.9}{}}
\@writefile{lla}{\contentsline {section}{\numberline {\crtrefnumber{sconn_lower1}}sconn_lower1}{18}{Item.9}\protected@file@percent }
\newlabel{sconn_lower1@cref}{{[enumi][1][]{{(1)}}}{[1][17][]18}{}{}{}}
\newlabel{sconn_lower2}{{{{(2)}}}{18}{}{Item.10}{}}
\@writefile{lla}{\contentsline {section}{\numberline {\crtrefnumber{sconn_lower2}}sconn_lower2}{18}{Item.10}\protected@file@percent }
\newlabel{sconn_lower2@cref}{{[enumi][2][]{{(2)}}}{[1][17][]18}{}{}{}}
\@writefile{loe}{\contentsline {lemma}{\ifthmt@listswap Lemma~2.21\else \numberline {2.21}Lemma\fi }{18}{lemma.2.21}\protected@file@percent }
\newlabel{lemma:TE:excision_datr}{{2.21}{18}{}{lemma.2.21}{}}
\@writefile{lla}{\contentsline {section}{\numberline {\crtrefnumber{lemma:TE:excision_datr}}lemma:TE:excision_datr}{18}{lemma.2.21}\protected@file@percent }
\newlabel{lemma:TE:excision_datr@cref}{{[lemma][21][2]2.21}{[1][18][]18}{}{}{}}
\newlabel{ssec:Kawangle}{{2.3}{18}{\KawAngle condition}{subsection.2.3}{}}
\@writefile{lla}{\contentsline {section}{\numberline {\crtrefnumber{ssec:Kawangle}}ssec:Kawangle}{18}{subsection.2.3}\protected@file@percent }
\newlabel{ssec:Kawangle@cref}{{[subsection][3][2]2.3}{[1][18][]18}{}{}{}}
\@writefile{toc}{\contentsline {subsection}{\tocsubsection {}{2.3}{Kawasaki angle\xspace  condition}}{18}{subsection.2.3}\protected@file@percent }
\newlabel{eq:TE:sumT_corner_dfn}{{2.14}{18}{\KawAngle condition}{equation.2.14}{}}
\@writefile{lla}{\contentsline {section}{\numberline {\crtrefnumber{eq:TE:sumT_corner_dfn}}eq:TE:sumT_corner_dfn}{18}{equation.2.14}\protected@file@percent }
\newlabel{eq:TE:sumT_corner_dfn@cref}{{[equation][14][2]2.14}{[1][18][]18}{}{}{}}
\newlabel{eq:TE:sumT_corner_0_pi}{{2.15}{18}{\KawAngle condition}{equation.2.15}{}}
\@writefile{lla}{\contentsline {section}{\numberline {\crtrefnumber{eq:TE:sumT_corner_0_pi}}eq:TE:sumT_corner_0_pi}{18}{equation.2.15}\protected@file@percent }
\newlabel{eq:TE:sumT_corner_0_pi@cref}{{[equation][15][2]2.15}{[1][18][]18}{}{}{}}
\newlabel{eq:TE:sumbT_sumwT_sumT_dfn}{{2.16}{18}{\KawAngle condition}{equation.2.16}{}}
\@writefile{lla}{\contentsline {section}{\numberline {\crtrefnumber{eq:TE:sumbT_sumwT_sumT_dfn}}eq:TE:sumbT_sumwT_sumT_dfn}{18}{equation.2.16}\protected@file@percent }
\newlabel{eq:TE:sumbT_sumwT_sumT_dfn@cref}{{[equation][16][2]2.16}{[1][18][]18}{}{}{}}
\@writefile{loe}{\contentsline {lemma}{\ifthmt@listswap Lemma~2.22\else \numberline {2.22}Lemma\fi \thmtformatoptarg {Algebraic Kawasaki angle\xspace  condition}}{18}{lemma.2.22}\protected@file@percent }
\newlabel{lemma:TE:Kawangle_alg}{{2.22}{18}{Algebraic \Kawangle condition}{lemma.2.22}{}}
\@writefile{lla}{\contentsline {section}{\numberline {\crtrefnumber{lemma:TE:Kawangle_alg}}lemma:TE:Kawangle_alg}{18}{lemma.2.22}\protected@file@percent }
\newlabel{lemma:TE:Kawangle_alg@cref}{{[lemma][22][2]2.22}{[1][18][]18}{}{}{}}
\newlabel{eq:Kawangle_alg_int}{{2.17}{18}{Algebraic \Kawangle condition}{equation.2.17}{}}
\@writefile{lla}{\contentsline {section}{\numberline {\crtrefnumber{eq:Kawangle_alg_int}}eq:Kawangle_alg_int}{18}{equation.2.17}\protected@file@percent }
\newlabel{eq:Kawangle_alg_int@cref}{{[equation][17][2]2.17}{[1][18][]18}{}{}{}}
\newlabel{eq:Kawangle_alg_bd}{{2.18}{18}{Algebraic \Kawangle condition}{equation.2.18}{}}
\@writefile{lla}{\contentsline {section}{\numberline {\crtrefnumber{eq:Kawangle_alg_bd}}eq:Kawangle_alg_bd}{18}{equation.2.18}\protected@file@percent }
\newlabel{eq:Kawangle_alg_bd@cref}{{[equation][18][2]2.18}{[1][18][]18}{}{}{}}
\newlabel{eq:Kawangle_alg_bd_gen}{{2.19}{18}{\KawAngle condition}{equation.2.19}{}}
\@writefile{lla}{\contentsline {section}{\numberline {\crtrefnumber{eq:Kawangle_alg_bd_gen}}eq:Kawangle_alg_bd_gen}{18}{equation.2.19}\protected@file@percent }
\newlabel{eq:Kawangle_alg_bd_gen@cref}{{[equation][19][2]2.19}{[1][18][]18}{}{}{}}
\@writefile{loe}{\contentsline {proposition}{\ifthmt@listswap Proposition~2.23\else \numberline {2.23}Proposition\fi \thmtformatoptarg {Kawasaki angle\xspace  condition}}{19}{proposition.2.23}\protected@file@percent }
\newlabel{lemma:TE:angle_cond}{{2.23}{19}{\KawAngle condition}{proposition.2.23}{}}
\@writefile{lla}{\contentsline {section}{\numberline {\crtrefnumber{lemma:TE:angle_cond}}lemma:TE:angle_cond}{19}{proposition.2.23}\protected@file@percent }
\newlabel{lemma:TE:angle_cond@cref}{{[proposition][23][2]2.23}{[1][18][]19}{}{}{}}
\newlabel{eq:TE:angle_cond}{{2.20}{19}{\KawAngle condition}{equation.2.20}{}}
\@writefile{lla}{\contentsline {section}{\numberline {\crtrefnumber{eq:TE:angle_cond}}eq:TE:angle_cond}{19}{equation.2.20}\protected@file@percent }
\newlabel{eq:TE:angle_cond@cref}{{[equation][20][2]2.20}{[1][18][]19}{}{}{}}
\newlabel{eq:TE:angle_cond_bdry}{{2.21}{19}{\KawAngle condition}{equation.2.21}{}}
\@writefile{lla}{\contentsline {section}{\numberline {\crtrefnumber{eq:TE:angle_cond_bdry}}eq:TE:angle_cond_bdry}{19}{equation.2.21}\protected@file@percent }
\newlabel{eq:TE:angle_cond_bdry@cref}{{[equation][21][2]2.21}{[1][19][]19}{}{}{}}
\newlabel{eq:TE:turning_of_vertex}{{2.22}{19}{\KawAngle condition}{equation.2.22}{}}
\@writefile{lla}{\contentsline {section}{\numberline {\crtrefnumber{eq:TE:turning_of_vertex}}eq:TE:turning_of_vertex}{19}{equation.2.22}\protected@file@percent }
\newlabel{eq:TE:turning_of_vertex@cref}{{[equation][22][2]2.22}{[1][19][]19}{}{}{}}
\newlabel{eq:TE:turning_sumT}{{2.23}{19}{\KawAngle condition}{equation.2.23}{}}
\@writefile{lla}{\contentsline {section}{\numberline {\crtrefnumber{eq:TE:turning_sumT}}eq:TE:turning_sumT}{19}{equation.2.23}\protected@file@percent }
\newlabel{eq:TE:turning_sumT@cref}{{[equation][23][2]2.23}{[1][19][]19}{}{}{}}
\newlabel{eq:TE:turning_sumT_bdry}{{2.24}{19}{\KawAngle condition}{equation.2.24}{}}
\@writefile{lla}{\contentsline {section}{\numberline {\crtrefnumber{eq:TE:turning_sumT_bdry}}eq:TE:turning_sumT_bdry}{19}{equation.2.24}\protected@file@percent }
\newlabel{eq:TE:turning_sumT_bdry@cref}{{[equation][24][2]2.24}{[1][19][]19}{}{}{}}
\newlabel{eq:TE:turning_sum1}{{2.25}{19}{\KawAngle condition}{equation.2.25}{}}
\@writefile{lla}{\contentsline {section}{\numberline {\crtrefnumber{eq:TE:turning_sum1}}eq:TE:turning_sum1}{19}{equation.2.25}\protected@file@percent }
\newlabel{eq:TE:turning_sum1@cref}{{[equation][25][2]2.25}{[1][19][]19}{}{}{}}
\newlabel{eq:TE:turning_sum2}{{2.26}{19}{\KawAngle condition}{equation.2.26}{}}
\@writefile{lla}{\contentsline {section}{\numberline {\crtrefnumber{eq:TE:turning_sum2}}eq:TE:turning_sum2}{19}{equation.2.26}\protected@file@percent }
\newlabel{eq:TE:turning_sum2@cref}{{[equation][26][2]2.26}{[1][19][]19}{}{}{}}
\newlabel{eq:TE:dtsums=0}{{2.27}{19}{\KawAngle condition}{equation.2.27}{}}
\@writefile{lla}{\contentsline {section}{\numberline {\crtrefnumber{eq:TE:dtsums=0}}eq:TE:dtsums=0}{19}{equation.2.27}\protected@file@percent }
\newlabel{eq:TE:dtsums=0@cref}{{[equation][27][2]2.27}{[1][19][]19}{}{}{}}
\@writefile{loe}{\contentsline {definition}{\ifthmt@listswap Definition~2.24\else \numberline {2.24}Definition\fi }{19}{definition.2.24}\protected@file@percent }
\newlabel{dfn:DIM:degenerate_convex_polygon}{{2.24}{19}{}{definition.2.24}{}}
\@writefile{lla}{\contentsline {section}{\numberline {\crtrefnumber{dfn:DIM:degenerate_convex_polygon}}dfn:DIM:degenerate_convex_polygon}{19}{definition.2.24}\protected@file@percent }
\newlabel{dfn:DIM:degenerate_convex_polygon@cref}{{[definition][24][2]2.24}{[1][19][]19}{}{}{}}
\newlabel{eq:DIM:turnangle_cond}{{2.28}{19}{}{equation.2.28}{}}
\@writefile{lla}{\contentsline {section}{\numberline {\crtrefnumber{eq:DIM:turnangle_cond}}eq:DIM:turnangle_cond}{19}{equation.2.28}\protected@file@percent }
\newlabel{eq:DIM:turnangle_cond@cref}{{[equation][28][2]2.28}{[1][19][]19}{}{}{}}
\citation{origami1}
\@writefile{loe}{\contentsline {notation}{\ifthmt@listswap Notation~2.25\else \numberline {2.25}Notation\fi }{20}{notation.2.25}\protected@file@percent }
\newlabel{notn:TE:Rg_corners_E_WV_BV_sumTcond}{{2.25}{20}{}{notation.2.25}{}}
\@writefile{lla}{\contentsline {section}{\numberline {\crtrefnumber{notn:TE:Rg_corners_E_WV_BV_sumTcond}}notn:TE:Rg_corners_E_WV_BV_sumTcond}{20}{notation.2.25}\protected@file@percent }
\newlabel{notn:TE:Rg_corners_E_WV_BV_sumTcond@cref}{{[notation][25][2]2.25}{[1][20][]20}{}{}{}}
\@writefile{loe}{\contentsline {lemma}{\ifthmt@listswap Lemma~2.26\else \numberline {2.26}Lemma\fi }{20}{lemma.2.26}\protected@file@percent }
\newlabel{lemma:TE:weakly_convex_helWBmin=1}{{2.26}{20}{}{lemma.2.26}{}}
\@writefile{lla}{\contentsline {section}{\numberline {\crtrefnumber{lemma:TE:weakly_convex_helWBmin=1}}lemma:TE:weakly_convex_helWBmin=1}{20}{lemma.2.26}\protected@file@percent }
\newlabel{lemma:TE:weakly_convex_helWBmin=1@cref}{{[lemma][26][2]2.26}{[1][20][]20}{}{}{}}
\newlabel{eq:DIM:reg_sum_cond}{{2.29}{20}{\KawAngle condition}{equation.2.29}{}}
\@writefile{lla}{\contentsline {section}{\numberline {\crtrefnumber{eq:DIM:reg_sum_cond}}eq:DIM:reg_sum_cond}{20}{equation.2.29}\protected@file@percent }
\newlabel{eq:DIM:reg_sum_cond@cref}{{[equation][29][2]2.29}{[1][20][]20}{}{}{}}
\@writefile{toc}{\contentsline {subsection}{\tocsubsection {}{2.4}{Origami-amplituhedron correspondence\xspace  }}{20}{subsection.2.4}\protected@file@percent }
\@writefile{loe}{\contentsline {theorem}{\ifthmt@listswap Theorem~2.27\else \numberline {2.27}Theorem\fi \thmtformatoptarg {Origami-amplituhedron correspondence\xspace  }}{20}{theorem.2.27}\protected@file@percent }
\newlabel{thm:TE:OAC}{{2.27}{20}{\OACTITLE }{theorem.2.27}{}}
\@writefile{lla}{\contentsline {section}{\numberline {\crtrefnumber{thm:TE:OAC}}thm:TE:OAC}{20}{theorem.2.27}\protected@file@percent }
\newlabel{thm:TE:OAC@cref}{{[theorem][27][2]2.27}{[1][20][]20}{}{}{}}
\newlabel{eq:TE:y_to_lalat}{{2.32}{20}{\OACTITLE }{equation.2.32}{}}
\@writefile{lla}{\contentsline {section}{\numberline {\crtrefnumber{eq:TE:y_to_lalat}}eq:TE:y_to_lalat}{20}{equation.2.32}\protected@file@percent }
\newlabel{eq:TE:y_to_lalat@cref}{{[equation][32][2]2.32}{[1][20][]20}{}{}{}}
\newlabel{eq:brlaw_dfn}{{2.33}{20}{\OACTITLE }{equation.2.33}{}}
\@writefile{lla}{\contentsline {section}{\numberline {\crtrefnumber{eq:brlaw_dfn}}eq:brlaw_dfn}{20}{equation.2.33}\protected@file@percent }
\newlabel{eq:brlaw_dfn@cref}{{[equation][33][2]2.33}{[1][20][]20}{}{}{}}
\newlabel{eq:TE:lalat_vs_pFw_pFb}{{2.34}{20}{\OACTITLE }{equation.2.34}{}}
\@writefile{lla}{\contentsline {section}{\numberline {\crtrefnumber{eq:TE:lalat_vs_pFw_pFb}}eq:TE:lalat_vs_pFw_pFb}{20}{equation.2.34}\protected@file@percent }
\newlabel{eq:TE:lalat_vs_pFw_pFb@cref}{{[equation][34][2]2.34}{[1][20][]20}{}{}{}}
\citation{origami1}
\citation{origami1}
\citation{origami1}
\citation{origami1}
\citation{origami1}
\@writefile{loe}{\contentsline {proposition}{\ifthmt@listswap Proposition~2.28\else \numberline {2.28}Proposition\fi \thmtformatoptarg {\cite  [\cref  *{M-prop:from_la_to_La}]{origami1}\xspace  }}{21}{proposition.2.28}\protected@file@percent }
\newlabel{prop:from_la_to_La}{{2.28}{21}{\Mref {prop:from_la_to_La}}{proposition.2.28}{}}
\@writefile{lla}{\contentsline {section}{\numberline {\crtrefnumber{prop:from_la_to_La}}prop:from_la_to_La}{21}{proposition.2.28}\protected@file@percent }
\newlabel{prop:from_la_to_La@cref}{{[proposition][28][2]2.28}{[1][21][]21}{}{}{}}
\@writefile{loe}{\contentsline {definition}{\ifthmt@listswap Definition~2.29\else \numberline {2.29}Definition\fi \thmtformatoptarg {Tripod insertion}}{21}{definition.2.29}\protected@file@percent }
\newlabel{dfn:eksbb}{{2.29}{21}{Tripod insertion}{definition.2.29}{}}
\@writefile{lla}{\contentsline {section}{\numberline {\crtrefnumber{dfn:eksbb}}dfn:eksbb}{21}{definition.2.29}\protected@file@percent }
\newlabel{dfn:eksbb@cref}{{[definition][29][2]2.29}{[1][21][]21}{}{}{}}
\@writefile{loe}{\contentsline {corollary}{\ifthmt@listswap Corollary~2.30\else \numberline {2.30}Corollary\fi \thmtformatoptarg {\cite  [\cref  *{M-cor:lak_implies_black_imm}]{origami1}\xspace  }}{21}{corollary.2.30}\protected@file@percent }
\newlabel{lemma:TE:brla_nonzero_if_apm}{{2.30}{21}{\Mref {cor:lak_implies_black_imm}}{corollary.2.30}{}}
\@writefile{lla}{\contentsline {section}{\numberline {\crtrefnumber{lemma:TE:brla_nonzero_if_apm}}lemma:TE:brla_nonzero_if_apm}{21}{corollary.2.30}\protected@file@percent }
\newlabel{lemma:TE:brla_nonzero_if_apm@cref}{{[corollary][30][2]2.30}{[1][21][]21}{}{}{}}
\newlabel{lak_implies1}{{{{(1)}}}{21}{\Mref {cor:lak_implies_black_imm}}{Item.11}{}}
\@writefile{lla}{\contentsline {section}{\numberline {\crtrefnumber{lak_implies1}}lak_implies1}{21}{Item.11}\protected@file@percent }
\newlabel{lak_implies1@cref}{{[enumi][1][]{{(1)}}}{[1][21][]21}{}{}{}}
\newlabel{lak_implies2}{{{{(2)}}}{21}{\Mref {cor:lak_implies_black_imm}}{Item.12}{}}
\@writefile{lla}{\contentsline {section}{\numberline {\crtrefnumber{lak_implies2}}lak_implies2}{21}{Item.12}\protected@file@percent }
\newlabel{lak_implies2@cref}{{[enumi][2][]{{(2)}}}{[1][21][]21}{}{}{}}
\newlabel{lak_implies3}{{{{(3)}}}{21}{\Mref {cor:lak_implies_black_imm}}{Item.13}{}}
\@writefile{lla}{\contentsline {section}{\numberline {\crtrefnumber{lak_implies3}}lak_implies3}{21}{Item.13}\protected@file@percent }
\newlabel{lak_implies3@cref}{{[enumi][3][]{{(3)}}}{[1][21][]21}{}{}{}}
\newlabel{eq:TE:same_face_and_same_vertex}{{2.35}{21}{\Mref {cor:lak_implies_black_imm}}{equation.2.35}{}}
\@writefile{lla}{\contentsline {section}{\numberline {\crtrefnumber{eq:TE:same_face_and_same_vertex}}eq:TE:same_face_and_same_vertex}{21}{equation.2.35}\protected@file@percent }
\newlabel{eq:TE:same_face_and_same_vertex@cref}{{[equation][35][2]2.35}{[1][21][]21}{}{}{}}
\newlabel{lak_implies4}{{{{(4)}}}{21}{\Mref {cor:lak_implies_black_imm}}{Item.14}{}}
\@writefile{lla}{\contentsline {section}{\numberline {\crtrefnumber{lak_implies4}}lak_implies4}{21}{Item.14}\protected@file@percent }
\newlabel{lak_implies4@cref}{{[enumi][4][]{{(4)}}}{[1][21][]21}{}{}{}}
\@writefile{loe}{\contentsline {lemma}{\ifthmt@listswap Lemma~2.31\else \numberline {2.31}Lemma\fi \thmtformatoptarg {\cite  [\cref  *{M-lemma:OAC:nondeg}]{origami1}\xspace  }}{21}{lemma.2.31}\protected@file@percent }
\newlabel{lemma:OAC:nondeg}{{2.31}{21}{\Mref {lemma:OAC:nondeg}}{lemma.2.31}{}}
\@writefile{lla}{\contentsline {section}{\numberline {\crtrefnumber{lemma:OAC:nondeg}}lemma:OAC:nondeg}{21}{lemma.2.31}\protected@file@percent }
\newlabel{lemma:OAC:nondeg@cref}{{[lemma][31][2]2.31}{[1][21][]21}{}{}{}}
\@writefile{loe}{\contentsline {corollary}{\ifthmt@listswap Corollary~2.32\else \numberline {2.32}Corollary\fi \thmtformatoptarg {Existence of weak t-immersions\xspace  }}{21}{corollary.2.32}\protected@file@percent }
\newlabel{thm:TE:existence}{{2.32}{21}{Existence of \wtimms }{corollary.2.32}{}}
\@writefile{lla}{\contentsline {section}{\numberline {\crtrefnumber{thm:TE:existence}}thm:TE:existence}{21}{corollary.2.32}\protected@file@percent }
\newlabel{thm:TE:existence@cref}{{[corollary][32][2]2.32}{[1][21][]21}{}{}{}}
\@writefile{loe}{\contentsline {remark}{\ifthmt@listswap Remark~2.33\else \numberline {2.33}Remark\fi }{21}{remark.2.33}\protected@file@percent }
\newlabel{rmk:TE:hel>=1_necessary}{{2.33}{21}{}{remark.2.33}{}}
\@writefile{lla}{\contentsline {section}{\numberline {\crtrefnumber{rmk:TE:hel>=1_necessary}}rmk:TE:hel>=1_necessary}{21}{remark.2.33}\protected@file@percent }
\newlabel{rmk:TE:hel>=1_necessary@cref}{{[remark][33][2]2.33}{[1][21][]21}{}{}{}}
\citation{Lovasz_1987}
\citation{Kenyon_Sheffield}
\citation{Lovasz_Plummer}
\@writefile{toc}{\contentsline {section}{\tocsection {}{3}{Weak t-embeddings are weak embeddings}}{22}{section.3}\protected@file@percent }
\@writefile{loe}{\contentsline {definition}{\ifthmt@listswap Definition~3.1\else \numberline {3.1}Definition\fi }{22}{definition.3.1}\protected@file@percent }
\@writefile{loe}{\contentsline {definition}{\ifthmt@listswap Definition~3.2\else \numberline {3.2}Definition\fi }{22}{definition.3.2}\protected@file@percent }
\newlabel{dfn:TOP:wtimm}{{3.2}{22}{}{definition.3.2}{}}
\@writefile{lla}{\contentsline {section}{\numberline {\crtrefnumber{dfn:TOP:wtimm}}dfn:TOP:wtimm}{22}{definition.3.2}\protected@file@percent }
\newlabel{dfn:TOP:wtimm@cref}{{[definition][2][3]3.2}{[1][22][]22}{}{}{}}
\@writefile{loe}{\contentsline {theorem}{\ifthmt@listswap Theorem~3.3\else \numberline {3.3}Theorem\fi }{22}{theorem.3.3}\protected@file@percent }
\newlabel{thm:TOP:weak_imm=>imm}{{3.3}{22}{}{theorem.3.3}{}}
\@writefile{lla}{\contentsline {section}{\numberline {\crtrefnumber{thm:TOP:weak_imm=>imm}}thm:TOP:weak_imm=>imm}{22}{theorem.3.3}\protected@file@percent }
\newlabel{thm:TOP:weak_imm=>imm@cref}{{[theorem][3][3]3.3}{[1][22][]22}{}{}{}}
\newlabel{TOP:weak_imm1}{{{{(1)}}}{22}{}{Item.15}{}}
\@writefile{lla}{\contentsline {section}{\numberline {\crtrefnumber{TOP:weak_imm1}}TOP:weak_imm1}{22}{Item.15}\protected@file@percent }
\newlabel{TOP:weak_imm1@cref}{{[enumi][1][]{{(1)}}}{[1][22][]22}{}{}{}}
\newlabel{TOP:weak_imm2}{{{{(2)}}}{22}{}{Item.16}{}}
\@writefile{lla}{\contentsline {section}{\numberline {\crtrefnumber{TOP:weak_imm2}}TOP:weak_imm2}{22}{Item.16}\protected@file@percent }
\newlabel{TOP:weak_imm2@cref}{{[enumi][2][]{{(2)}}}{[1][22][]22}{}{}{}}
\newlabel{ssec:DIM:coll}{{3.1}{22}{Collapsible subsets}{subsection.3.1}{}}
\@writefile{lla}{\contentsline {section}{\numberline {\crtrefnumber{ssec:DIM:coll}}ssec:DIM:coll}{22}{subsection.3.1}\protected@file@percent }
\newlabel{ssec:DIM:coll@cref}{{[subsection][1][3]3.1}{[1][22][]22}{}{}{}}
\@writefile{toc}{\contentsline {subsection}{\tocsubsection {}{3.1}{Collapsible subsets}}{22}{subsection.3.1}\protected@file@percent }
\@writefile{loe}{\contentsline {lemma}{\ifthmt@listswap Lemma~3.4\else \numberline {3.4}Lemma\fi }{22}{lemma.3.4}\protected@file@percent }
\newlabel{eq:DIM:submodular}{{3.1}{22}{}{equation.3.1}{}}
\@writefile{lla}{\contentsline {section}{\numberline {\crtrefnumber{eq:DIM:submodular}}eq:DIM:submodular}{22}{equation.3.1}\protected@file@percent }
\newlabel{eq:DIM:submodular@cref}{{[equation][1][3]3.1}{[1][22][]22}{}{}{}}
\@writefile{loe}{\contentsline {definition}{\ifthmt@listswap Definition~3.5\else \numberline {3.5}Definition\fi }{22}{definition.3.5}\protected@file@percent }
\@writefile{loe}{\contentsline {lemma}{\ifthmt@listswap Lemma~3.6\else \numberline {3.6}Lemma\fi }{22}{lemma.3.6}\protected@file@percent }
\newlabel{lemma:DIM:collapsible_union}{{3.6}{22}{}{lemma.3.6}{}}
\@writefile{lla}{\contentsline {section}{\numberline {\crtrefnumber{lemma:DIM:collapsible_union}}lemma:DIM:collapsible_union}{22}{lemma.3.6}\protected@file@percent }
\newlabel{lemma:DIM:collapsible_union@cref}{{[lemma][6][3]3.6}{[1][22][]22}{}{}{}}
\@writefile{loe}{\contentsline {lemma}{\ifthmt@listswap Lemma~3.7\else \numberline {3.7}Lemma\fi }{22}{lemma.3.7}\protected@file@percent }
\newlabel{lemma:DIM:coll_sconn}{{3.7}{22}{}{lemma.3.7}{}}
\@writefile{lla}{\contentsline {section}{\numberline {\crtrefnumber{lemma:DIM:coll_sconn}}lemma:DIM:coll_sconn}{22}{lemma.3.7}\protected@file@percent }
\newlabel{lemma:DIM:coll_sconn@cref}{{[lemma][7][3]3.7}{[1][22][]22}{}{}{}}
\@writefile{loe}{\contentsline {definition}{\ifthmt@listswap Definition~3.8\else \numberline {3.8}Definition\fi }{22}{definition.3.8}\protected@file@percent }
\newlabel{dfn:DIM:collapsed_graph}{{3.8}{22}{}{definition.3.8}{}}
\@writefile{lla}{\contentsline {section}{\numberline {\crtrefnumber{dfn:DIM:collapsed_graph}}dfn:DIM:collapsed_graph}{22}{definition.3.8}\protected@file@percent }
\newlabel{dfn:DIM:collapsed_graph@cref}{{[definition][8][3]3.8}{[1][22][]22}{}{}{}}
\@writefile{lof}{\contentsline {figure}{\numberline {7}{\ignorespaces  Collapsing a graph $\Gamma $; see \cref  {dfn:DIM:collapsed_graph,dfn:DIM:CollGBW}. Here, the maximal $\circ $-collapsible (resp., $\bullet $-collapsible) subsets of $\Gamma $ are circled in green (resp., red).}}{23}{figure.caption.15}\protected@file@percent }
\newlabel{fig:collapse}{{7}{23}{Collapsing a graph $\G $; see \cref {dfn:DIM:collapsed_graph,dfn:DIM:CollGBW}. Here, the maximal \wdash collapsible (resp., \bdash collapsible) subsets of $\G $ are circled in green (resp., red)}{figure.caption.15}{}}
\@writefile{lla}{\contentsline {section}{\numberline {\crtrefnumber{fig:collapse}}fig:collapse}{23}{figure.caption.15}\protected@file@percent }
\newlabel{fig:collapse@cref}{{[figure][7][]7}{[1][22][]23}{}{}{}}
\@writefile{loe}{\contentsline {remark}{\ifthmt@listswap Remark~3.9\else \numberline {3.9}Remark\fi }{23}{remark.3.9}\protected@file@percent }
\newlabel{rmk:DIM:coll_w}{{3.9}{23}{}{remark.3.9}{}}
\@writefile{lla}{\contentsline {section}{\numberline {\crtrefnumber{rmk:DIM:coll_w}}rmk:DIM:coll_w}{23}{remark.3.9}\protected@file@percent }
\newlabel{rmk:DIM:coll_w@cref}{{[remark][9][3]3.9}{[1][22][]23}{}{}{}}
\@writefile{loe}{\contentsline {lemma}{\ifthmt@listswap Lemma~3.10\else \numberline {3.10}Lemma\fi }{23}{lemma.3.10}\protected@file@percent }
\newlabel{lemma:DIM:CollGW_geq_2}{{3.10}{23}{}{lemma.3.10}{}}
\@writefile{lla}{\contentsline {section}{\numberline {\crtrefnumber{lemma:DIM:CollGW_geq_2}}lemma:DIM:CollGW_geq_2}{23}{lemma.3.10}\protected@file@percent }
\newlabel{lemma:DIM:CollGW_geq_2@cref}{{[lemma][10][3]3.10}{[1][22][]23}{}{}{}}
\@writefile{loe}{\contentsline {definition}{\ifthmt@listswap Definition~3.11\else \numberline {3.11}Definition\fi \thmtformatoptarg {Fully collapsed graph}}{23}{definition.3.11}\protected@file@percent }
\newlabel{dfn:DIM:CollGBW}{{3.11}{23}{Fully collapsed graph}{definition.3.11}{}}
\@writefile{lla}{\contentsline {section}{\numberline {\crtrefnumber{dfn:DIM:CollGBW}}dfn:DIM:CollGBW}{23}{definition.3.11}\protected@file@percent }
\newlabel{dfn:DIM:CollGBW@cref}{{[definition][11][3]3.11}{[1][23][]23}{}{}{}}
\@writefile{loe}{\contentsline {lemma}{\ifthmt@listswap Lemma~3.12\else \numberline {3.12}Lemma\fi }{23}{lemma.3.12}\protected@file@percent }
\newlabel{lemma:DIM:CollGBW_geq_2}{{3.12}{23}{}{lemma.3.12}{}}
\@writefile{lla}{\contentsline {section}{\numberline {\crtrefnumber{lemma:DIM:CollGBW_geq_2}}lemma:DIM:CollGBW_geq_2}{23}{lemma.3.12}\protected@file@percent }
\newlabel{lemma:DIM:CollGBW_geq_2@cref}{{[lemma][12][3]3.12}{[1][23][]23}{}{}{}}
\citation{origami1}
\@writefile{loe}{\contentsline {remark}{\ifthmt@listswap Remark~3.13\else \numberline {3.13}Remark\fi }{24}{remark.3.13}\protected@file@percent }
\@writefile{toc}{\contentsline {subsection}{\tocsubsection {}{3.2}{Collapsing weak t-immersions\xspace  }}{24}{subsection.3.2}\protected@file@percent }
\@writefile{loe}{\contentsline {definition}{\ifthmt@listswap Definition~3.14\else \numberline {3.14}Definition\fi }{24}{definition.3.14}\protected@file@percent }
\newlabel{dfn:TOP:STRimm}{{3.14}{24}{}{definition.3.14}{}}
\@writefile{lla}{\contentsline {section}{\numberline {\crtrefnumber{dfn:TOP:STRimm}}dfn:TOP:STRimm}{24}{definition.3.14}\protected@file@percent }
\newlabel{dfn:TOP:STRimm@cref}{{[definition][14][3]3.14}{[1][24][]24}{}{}{}}
\newlabel{TOP:STRimm1}{{{{(1)}}}{24}{}{Item.17}{}}
\@writefile{lla}{\contentsline {section}{\numberline {\crtrefnumber{TOP:STRimm1}}TOP:STRimm1}{24}{Item.17}\protected@file@percent }
\newlabel{TOP:STRimm1@cref}{{[enumi][1][]{{(1)}}}{[1][24][]24}{}{}{}}
\newlabel{TOP:STRimm2}{{{{(2)}}}{24}{}{Item.18}{}}
\@writefile{lla}{\contentsline {section}{\numberline {\crtrefnumber{TOP:STRimm2}}TOP:STRimm2}{24}{Item.18}\protected@file@percent }
\newlabel{TOP:STRimm2@cref}{{[enumi][2][]{{(2)}}}{[1][24][]24}{}{}{}}
\newlabel{TOP:STRimm3}{{{{(3)}}}{24}{}{Item.19}{}}
\@writefile{lla}{\contentsline {section}{\numberline {\crtrefnumber{TOP:STRimm3}}TOP:STRimm3}{24}{Item.19}\protected@file@percent }
\newlabel{TOP:STRimm3@cref}{{[enumi][3][]{{(3)}}}{[1][24][]24}{}{}{}}
\@writefile{loe}{\contentsline {proposition}{\ifthmt@listswap Proposition~3.15\else \numberline {3.15}Proposition\fi }{24}{proposition.3.15}\protected@file@percent }
\newlabel{lemma:TOP:weak_imm_collapsed}{{3.15}{24}{}{proposition.3.15}{}}
\@writefile{lla}{\contentsline {section}{\numberline {\crtrefnumber{lemma:TOP:weak_imm_collapsed}}lemma:TOP:weak_imm_collapsed}{24}{proposition.3.15}\protected@file@percent }
\newlabel{lemma:TOP:weak_imm_collapsed@cref}{{[proposition][15][3]3.15}{[1][24][]24}{}{}{}}
\newlabel{TOP:coll1}{{{{(1)}}}{24}{}{Item.20}{}}
\@writefile{lla}{\contentsline {section}{\numberline {\crtrefnumber{TOP:coll1}}TOP:coll1}{24}{Item.20}\protected@file@percent }
\newlabel{TOP:coll1@cref}{{[enumi][1][]{{(1)}}}{[1][24][]24}{}{}{}}
\newlabel{TOP:coll2}{{{{(2)}}}{24}{}{Item.21}{}}
\@writefile{lla}{\contentsline {section}{\numberline {\crtrefnumber{TOP:coll2}}TOP:coll2}{24}{Item.21}\protected@file@percent }
\newlabel{TOP:coll2@cref}{{[enumi][2][]{{(2)}}}{[1][24][]24}{}{}{}}
\newlabel{TOP:coll3}{{{{(3)}}}{24}{}{Item.22}{}}
\@writefile{lla}{\contentsline {section}{\numberline {\crtrefnumber{TOP:coll3}}TOP:coll3}{24}{Item.22}\protected@file@percent }
\newlabel{TOP:coll3@cref}{{[enumi][3][]{{(3)}}}{[1][24][]24}{}{}{}}
\citation{origami1}
\@writefile{loe}{\contentsline {lemma}{\ifthmt@listswap Lemma~3.16\else \numberline {3.16}Lemma\fi }{25}{lemma.3.16}\protected@file@percent }
\newlabel{lemma:TOP:restr}{{3.16}{25}{}{lemma.3.16}{}}
\@writefile{lla}{\contentsline {section}{\numberline {\crtrefnumber{lemma:TOP:restr}}lemma:TOP:restr}{25}{lemma.3.16}\protected@file@percent }
\newlabel{lemma:TOP:restr@cref}{{[lemma][16][3]3.16}{[1][25][]25}{}{}{}}
\@writefile{loe}{\contentsline {proposition}{\ifthmt@listswap Proposition~3.17\else \numberline {3.17}Proposition\fi \thmtformatoptarg {\cite  [\cref  *{M-lemma:Mbd=>face_Mnn}]{origami1}\xspace  }}{25}{proposition.3.17}\protected@file@percent }
\newlabel{lemma:Mbd=>face_Mnn}{{3.17}{25}{\Mref {lemma:Mbd=>face_Mnn}}{proposition.3.17}{}}
\@writefile{lla}{\contentsline {section}{\numberline {\crtrefnumber{lemma:Mbd=>face_Mnn}}lemma:Mbd=>face_Mnn}{25}{proposition.3.17}\protected@file@percent }
\newlabel{lemma:Mbd=>face_Mnn@cref}{{[proposition][17][3]3.17}{[1][25][]25}{}{}{}}
\citation{Floater}
\citation{Floater}
\citation{Floater}
\@writefile{loe}{\contentsline {corollary}{\ifthmt@listswap Corollary~3.18\else \numberline {3.18}Corollary\fi }{26}{corollary.3.18}\protected@file@percent }
\newlabel{lemma:TE:hasMbd=>simple_and_MCE3}{{3.18}{26}{}{corollary.3.18}{}}
\@writefile{lla}{\contentsline {section}{\numberline {\crtrefnumber{lemma:TE:hasMbd=>simple_and_MCE3}}lemma:TE:hasMbd=>simple_and_MCE3}{26}{corollary.3.18}\protected@file@percent }
\newlabel{lemma:TE:hasMbd=>simple_and_MCE3@cref}{{[corollary][18][3]3.18}{[1][26][]26}{}{}{}}
\newlabel{ssec:TOP:proof_of_weak_imm=>imm}{{3.3}{26}{Proof of Theorem~\ref {thm:TOP:weak_imm=>imm}}{subsection.3.3}{}}
\@writefile{lla}{\contentsline {section}{\numberline {\crtrefnumber{ssec:TOP:proof_of_weak_imm=>imm}}ssec:TOP:proof_of_weak_imm=>imm}{26}{subsection.3.3}\protected@file@percent }
\newlabel{ssec:TOP:proof_of_weak_imm=>imm@cref}{{[subsection][3][3]3.3}{[1][26][]26}{}{}{}}
\@writefile{toc}{\contentsline {subsection}{\tocsubsection {}{3.3}{Proof of Theorem~\ref {thm:TOP:weak_imm=>imm}}}{26}{subsection.3.3}\protected@file@percent }
\citation{Floater}
\citation{Floater}
\citation{Floater}
\@writefile{lof}{\contentsline {figure}{\numberline {8}{\ignorespaces  Embeddings of the barycentric subdivision $\Gamma ^{\vartriangle }$ of $|\Gamma ^\ast |$ constructed via convex combination mappings of~\cite  {Floater} in the proof of \cref  {thm:TOP:weak_imm=>imm}. }}{27}{figure.caption.16}\protected@file@percent }
\newlabel{fig:bary}{{8}{27}{Embeddings of the barycentric subdivision $\Gbary $ of $\SuppGD $ constructed via convex combination mappings of~\cite {Floater} in the proof of \cref {thm:TOP:weak_imm=>imm}}{figure.caption.16}{}}
\@writefile{lla}{\contentsline {section}{\numberline {\crtrefnumber{fig:bary}}fig:bary}{27}{figure.caption.16}\protected@file@percent }
\newlabel{fig:bary@cref}{{[figure][8][]8}{[1][26][]27}{}{}{}}
\newlabel{eq:TE:Floater}{{3.2}{27}{Proof of Theorem~\ref {thm:TOP:weak_imm=>imm}}{equation.3.2}{}}
\@writefile{lla}{\contentsline {section}{\numberline {\crtrefnumber{eq:TE:Floater}}eq:TE:Floater}{27}{equation.3.2}\protected@file@percent }
\newlabel{eq:TE:Floater@cref}{{[equation][2][3]3.2}{[1][27][]27}{}{}{}}
\newlabel{eq:TE:Floater'}{{3.3}{27}{Proof of Theorem~\ref {thm:TOP:weak_imm=>imm}}{equation.3.3}{}}
\@writefile{lla}{\contentsline {section}{\numberline {\crtrefnumber{eq:TE:Floater'}}eq:TE:Floater'}{27}{equation.3.3}\protected@file@percent }
\newlabel{eq:TE:Floater'@cref}{{[equation][3][3]3.3}{[1][27][]27}{}{}{}}
\citation{Zono}
\citation{BaWe}
\citation{HSP}
\citation{PSBW}
\citation{CLSBW}
\citation{CLSBW}
\citation{HSP}
\@writefile{lof}{\contentsline {figure}{\numberline {9}{\ignorespaces  A graph $\Gamma $ (left) and its shift by $1$ (right); see \cref  {dfn:shift1}.}}{28}{figure.caption.17}\protected@file@percent }
\newlabel{fig:shift-1}{{9}{28}{A graph $\G $ (left) and its shift by $1$ (right); see \cref {dfn:shift1}}{figure.caption.17}{}}
\@writefile{lla}{\contentsline {section}{\numberline {\crtrefnumber{fig:shift-1}}fig:shift-1}{28}{figure.caption.17}\protected@file@percent }
\newlabel{fig:shift-1@cref}{{[figure][9][]9}{[1][28][]28}{}{}{}}
\@writefile{toc}{\contentsline {section}{\tocsection {}{4}{T-duality for planar bipartite graphs}}{28}{section.4}\protected@file@percent }
\newlabel{sec:shift}{{4}{28}{T-duality for planar bipartite graphs}{section.4}{}}
\@writefile{lla}{\contentsline {section}{\numberline {\crtrefnumber{sec:shift}}sec:shift}{28}{section.4}\protected@file@percent }
\newlabel{sec:shift@cref}{{[section][4][]4}{[1][28][]28}{}{}{}}
\newlabel{ssec:SHIFT:by1}{{4.1}{28}{Combinatorial shift by $1$}{subsection.4.1}{}}
\@writefile{lla}{\contentsline {section}{\numberline {\crtrefnumber{ssec:SHIFT:by1}}ssec:SHIFT:by1}{28}{subsection.4.1}\protected@file@percent }
\newlabel{ssec:SHIFT:by1@cref}{{[subsection][1][4]4.1}{[1][28][]28}{}{}{}}
\@writefile{toc}{\contentsline {subsection}{\tocsubsection {}{4.1}{Combinatorial shift by $1$}}{28}{subsection.4.1}\protected@file@percent }
\@writefile{loe}{\contentsline {definition}{\ifthmt@listswap Definition~4.1\else \numberline {4.1}Definition\fi \thmtformatoptarg {\cite  [Definition~7.14]{HSP}}}{28}{definition.4.1}\protected@file@percent }
\@writefile{loe}{\contentsline {definition}{\ifthmt@listswap Definition~4.2\else \numberline {4.2}Definition\fi \thmtformatoptarg {Combinatorial shift by $1$}}{28}{definition.4.2}\protected@file@percent }
\newlabel{dfn:shift1}{{4.2}{28}{Combinatorial shift by $1$}{definition.4.2}{}}
\@writefile{lla}{\contentsline {section}{\numberline {\crtrefnumber{dfn:shift1}}dfn:shift1}{28}{definition.4.2}\protected@file@percent }
\newlabel{dfn:shift1@cref}{{[definition][2][4]4.2}{[1][28][]28}{}{}{}}
\@writefile{loe}{\contentsline {lemma}{\ifthmt@listswap Lemma~4.3\else \numberline {4.3}Lemma\fi }{28}{lemma.4.3}\protected@file@percent }
\newlabel{lemma:shift1-top}{{4.3}{28}{}{lemma.4.3}{}}
\@writefile{lla}{\contentsline {section}{\numberline {\crtrefnumber{lemma:shift1-top}}lemma:shift1-top}{28}{lemma.4.3}\protected@file@percent }
\newlabel{lemma:shift1-top@cref}{{[lemma][3][4]4.3}{[1][28][]28}{}{}{}}
\newlabel{shift1-top1}{{{{(1)}}}{29}{}{Item.23}{}}
\@writefile{lla}{\contentsline {section}{\numberline {\crtrefnumber{shift1-top1}}shift1-top1}{29}{Item.23}\protected@file@percent }
\newlabel{shift1-top1@cref}{{[enumi][1][]{{(1)}}}{[1][28][]29}{}{}{}}
\newlabel{shift1-top2}{{{{(2)}}}{29}{}{Item.24}{}}
\@writefile{lla}{\contentsline {section}{\numberline {\crtrefnumber{shift1-top2}}shift1-top2}{29}{Item.24}\protected@file@percent }
\newlabel{shift1-top2@cref}{{[enumi][2][]{{(2)}}}{[1][28][]29}{}{}{}}
\newlabel{shift1-top3}{{{{(3)}}}{29}{}{Item.25}{}}
\@writefile{lla}{\contentsline {section}{\numberline {\crtrefnumber{shift1-top3}}shift1-top3}{29}{Item.25}\protected@file@percent }
\newlabel{shift1-top3@cref}{{[enumi][3][]{{(3)}}}{[1][29][]29}{}{}{}}
\newlabel{shift1-top4}{{{{(4)}}}{29}{}{Item.26}{}}
\@writefile{lla}{\contentsline {section}{\numberline {\crtrefnumber{shift1-top4}}shift1-top4}{29}{Item.26}\protected@file@percent }
\newlabel{shift1-top4@cref}{{[enumi][4][]{{(4)}}}{[1][29][]29}{}{}{}}
\@writefile{loe}{\contentsline {lemma}{\ifthmt@listswap Lemma~4.4\else \numberline {4.4}Lemma\fi }{29}{lemma.4.4}\protected@file@percent }
\newlabel{lemma:SHIFT:by1}{{4.4}{29}{}{lemma.4.4}{}}
\@writefile{lla}{\contentsline {section}{\numberline {\crtrefnumber{lemma:SHIFT:by1}}lemma:SHIFT:by1}{29}{lemma.4.4}\protected@file@percent }
\newlabel{lemma:SHIFT:by1@cref}{{[lemma][4][4]4.4}{[1][29][]29}{}{}{}}
\newlabel{eq:SHIFT:by1_helW_helB_ineqs}{{4.1}{29}{}{equation.4.1}{}}
\@writefile{lla}{\contentsline {section}{\numberline {\crtrefnumber{eq:SHIFT:by1_helW_helB_ineqs}}eq:SHIFT:by1_helW_helB_ineqs}{29}{equation.4.1}\protected@file@percent }
\newlabel{eq:SHIFT:by1_helW_helB_ineqs@cref}{{[equation][1][4]4.1}{[1][29][]29}{}{}{}}
\newlabel{eq:SHIFT:by1_helW_helB_ineqs2}{{4.2}{29}{}{equation.4.2}{}}
\@writefile{lla}{\contentsline {section}{\numberline {\crtrefnumber{eq:SHIFT:by1_helW_helB_ineqs2}}eq:SHIFT:by1_helW_helB_ineqs2}{29}{equation.4.2}\protected@file@percent }
\newlabel{eq:SHIFT:by1_helW_helB_ineqs2@cref}{{[equation][2][4]4.2}{[1][29][]29}{}{}{}}
\@writefile{lof}{\contentsline {figure}{\numberline {10}{\ignorespaces  Notation around trivalent vertices before and after applying T-duality. }}{30}{figure.caption.18}\protected@file@percent }
\newlabel{fig:black3}{{10}{30}{Notation around trivalent vertices before and after applying T-duality}{figure.caption.18}{}}
\@writefile{lla}{\contentsline {section}{\numberline {\crtrefnumber{fig:black3}}fig:black3}{30}{figure.caption.18}\protected@file@percent }
\newlabel{fig:black3@cref}{{[figure][10][]10}{[1][30][]30}{}{}{}}
\@writefile{loe}{\contentsline {corollary}{\ifthmt@listswap Corollary~4.5\else \numberline {4.5}Corollary\fi }{30}{corollary.4.5}\protected@file@percent }
\newlabel{sec:shift:combin}{{4.2}{30}{Combinatorial shift by $2$ (T-duality)}{subsection.4.2}{}}
\@writefile{lla}{\contentsline {section}{\numberline {\crtrefnumber{sec:shift:combin}}sec:shift:combin}{30}{subsection.4.2}\protected@file@percent }
\newlabel{sec:shift:combin@cref}{{[subsection][2][4]4.2}{[1][30][]30}{}{}{}}
\@writefile{toc}{\contentsline {subsection}{\tocsubsection {}{4.2}{Combinatorial shift by $2$ (T-duality)}}{30}{subsection.4.2}\protected@file@percent }
\@writefile{loe}{\contentsline {definition}{\ifthmt@listswap Definition~4.6\else \numberline {4.6}Definition\fi }{30}{definition.4.6}\protected@file@percent }
\newlabel{dfn:G:T_dualizable}{{4.6}{30}{}{definition.4.6}{}}
\@writefile{lla}{\contentsline {section}{\numberline {\crtrefnumber{dfn:G:T_dualizable}}dfn:G:T_dualizable}{30}{definition.4.6}\protected@file@percent }
\newlabel{dfn:G:T_dualizable@cref}{{[definition][6][4]4.6}{[1][30][]30}{}{}{}}
\@writefile{loe}{\contentsline {definition}{\ifthmt@listswap Definition~4.7\else \numberline {4.7}Definition\fi }{30}{definition.4.7}\protected@file@percent }
\newlabel{rmk:SFIFT:uncontract_black_trivalent}{{4.7}{30}{}{definition.4.7}{}}
\@writefile{lla}{\contentsline {section}{\numberline {\crtrefnumber{rmk:SFIFT:uncontract_black_trivalent}}rmk:SFIFT:uncontract_black_trivalent}{30}{definition.4.7}\protected@file@percent }
\newlabel{rmk:SFIFT:uncontract_black_trivalent@cref}{{[definition][7][4]4.7}{[1][30][]30}{}{}{}}
\@writefile{loe}{\contentsline {remark}{\ifthmt@listswap Remark~4.8\else \numberline {4.8}Remark\fi }{30}{remark.4.8}\protected@file@percent }
\newlabel{rmk:SHIFT:dG_ddG_helW_helB_connected}{{4.8}{30}{}{remark.4.8}{}}
\@writefile{lla}{\contentsline {section}{\numberline {\crtrefnumber{rmk:SHIFT:dG_ddG_helW_helB_connected}}rmk:SHIFT:dG_ddG_helW_helB_connected}{30}{remark.4.8}\protected@file@percent }
\newlabel{rmk:SHIFT:dG_ddG_helW_helB_connected@cref}{{[remark][8][4]4.8}{[1][30][]30}{}{}{}}
\newlabel{eq:dG_ddG_helW_helB}{{4.3}{30}{}{equation.4.3}{}}
\@writefile{lla}{\contentsline {section}{\numberline {\crtrefnumber{eq:dG_ddG_helW_helB}}eq:dG_ddG_helW_helB}{30}{equation.4.3}\protected@file@percent }
\newlabel{eq:dG_ddG_helW_helB@cref}{{[equation][3][4]4.3}{[1][30][]30}{}{}{}}
\@writefile{loe}{\contentsline {definition}{\ifthmt@listswap Definition~4.9\else \numberline {4.9}Definition\fi }{30}{definition.4.9}\protected@file@percent }
\newlabel{dfn:SHIFT:Sig}{{4.9}{30}{}{definition.4.9}{}}
\@writefile{lla}{\contentsline {section}{\numberline {\crtrefnumber{dfn:SHIFT:Sig}}dfn:SHIFT:Sig}{30}{definition.4.9}\protected@file@percent }
\newlabel{dfn:SHIFT:Sig@cref}{{[definition][9][4]4.9}{[1][30][]30}{}{}{}}
\@writefile{loe}{\contentsline {definition}{\ifthmt@listswap Definition~4.10\else \numberline {4.10}Definition\fi \thmtformatoptarg {T-dual graphs}}{31}{definition.4.10}\protected@file@percent }
\newlabel{dfn:SHIFT:ddG}{{4.10}{31}{T-dual graphs}{definition.4.10}{}}
\@writefile{lla}{\contentsline {section}{\numberline {\crtrefnumber{dfn:SHIFT:ddG}}dfn:SHIFT:ddG}{31}{definition.4.10}\protected@file@percent }
\newlabel{dfn:SHIFT:ddG@cref}{{[definition][10][4]4.10}{[1][30][]31}{}{}{}}
\@writefile{loe}{\contentsline {definition}{\ifthmt@listswap Definition~4.11\else \numberline {4.11}Definition\fi }{31}{definition.4.11}\protected@file@percent }
\newlabel{dfn:SHIFT:light_dark_regions}{{4.11}{31}{}{definition.4.11}{}}
\@writefile{lla}{\contentsline {section}{\numberline {\crtrefnumber{dfn:SHIFT:light_dark_regions}}dfn:SHIFT:light_dark_regions}{31}{definition.4.11}\protected@file@percent }
\newlabel{dfn:SHIFT:light_dark_regions@cref}{{[definition][11][4]4.11}{[1][31][]31}{}{}{}}
\@writefile{loe}{\contentsline {remark}{\ifthmt@listswap Remark~4.12\else \numberline {4.12}Remark\fi }{31}{remark.4.12}\protected@file@percent }
\newlabel{rmk:SHIFT:choices}{{4.12}{31}{}{remark.4.12}{}}
\@writefile{lla}{\contentsline {section}{\numberline {\crtrefnumber{rmk:SHIFT:choices}}rmk:SHIFT:choices}{31}{remark.4.12}\protected@file@percent }
\newlabel{rmk:SHIFT:choices@cref}{{[remark][12][4]4.12}{[1][31][]31}{}{}{}}
\@writefile{loe}{\contentsline {lemma}{\ifthmt@listswap Lemma~4.13\else \numberline {4.13}Lemma\fi }{31}{lemma.4.13}\protected@file@percent }
\newlabel{lemma:SHIFT:ddG=ddG'}{{4.13}{31}{}{lemma.4.13}{}}
\@writefile{lla}{\contentsline {section}{\numberline {\crtrefnumber{lemma:SHIFT:ddG=ddG'}}lemma:SHIFT:ddG=ddG'}{31}{lemma.4.13}\protected@file@percent }
\newlabel{lemma:SHIFT:ddG=ddG'@cref}{{[lemma][13][4]4.13}{[1][31][]31}{}{}{}}
\@writefile{loe}{\contentsline {corollary}{\ifthmt@listswap Corollary~4.14\else \numberline {4.14}Corollary\fi }{31}{corollary.4.14}\protected@file@percent }
\newlabel{lemma:SHIFT:ddG_admits_apms}{{4.14}{31}{}{corollary.4.14}{}}
\@writefile{lla}{\contentsline {section}{\numberline {\crtrefnumber{lemma:SHIFT:ddG_admits_apms}}lemma:SHIFT:ddG_admits_apms}{31}{corollary.4.14}\protected@file@percent }
\newlabel{lemma:SHIFT:ddG_admits_apms@cref}{{[corollary][14][4]4.14}{[1][31][]31}{}{}{}}
\newlabel{sec:shift:lambda_Kast_weights}{{4.3}{31}{\texorpdfstring {$\la $}{lambda}-Kasteleyn weights}{subsection.4.3}{}}
\@writefile{lla}{\contentsline {section}{\numberline {\crtrefnumber{sec:shift:lambda_Kast_weights}}sec:shift:lambda_Kast_weights}{31}{subsection.4.3}\protected@file@percent }
\newlabel{sec:shift:lambda_Kast_weights@cref}{{[subsection][3][4]4.3}{[1][31][]31}{}{}{}}
\@writefile{toc}{\contentsline {subsection}{\tocsubsection {}{4.3}{$\lambda $-Kasteleyn weights}}{31}{subsection.4.3}\protected@file@percent }
\newlabel{eq:wtlaK_dfn}{{4.4}{31}{\texorpdfstring {$\la $}{lambda}-Kasteleyn weights}{equation.4.4}{}}
\@writefile{lla}{\contentsline {section}{\numberline {\crtrefnumber{eq:wtlaK_dfn}}eq:wtlaK_dfn}{31}{equation.4.4}\protected@file@percent }
\newlabel{eq:wtlaK_dfn@cref}{{[equation][4][4]4.4}{[1][31][]31}{}{}{}}
\newlabel{eq:la_generic}{{4.5}{32}{\texorpdfstring {$\la $}{lambda}-Kasteleyn weights}{equation.4.5}{}}
\@writefile{lla}{\contentsline {section}{\numberline {\crtrefnumber{eq:la_generic}}eq:la_generic}{32}{equation.4.5}\protected@file@percent }
\newlabel{eq:la_generic@cref}{{[equation][5][4]4.5}{[1][31][]32}{}{}{}}
\@writefile{loe}{\contentsline {lemma}{\ifthmt@listswap Lemma~4.15\else \numberline {4.15}Lemma\fi }{32}{lemma.4.15}\protected@file@percent }
\newlabel{lemma:black_gauge_eq}{{4.15}{32}{}{lemma.4.15}{}}
\@writefile{lla}{\contentsline {section}{\numberline {\crtrefnumber{lemma:black_gauge_eq}}lemma:black_gauge_eq}{32}{lemma.4.15}\protected@file@percent }
\newlabel{lemma:black_gauge_eq@cref}{{[lemma][15][4]4.15}{[1][32][]32}{}{}{}}
\newlabel{eq:black_gauge_equivalent}{{4.6}{32}{}{equation.4.6}{}}
\@writefile{lla}{\contentsline {section}{\numberline {\crtrefnumber{eq:black_gauge_equivalent}}eq:black_gauge_equivalent}{32}{equation.4.6}\protected@file@percent }
\newlabel{eq:black_gauge_equivalent@cref}{{[equation][6][4]4.6}{[1][32][]32}{}{}{}}
\newlabel{eq:la_Cramer}{{4.7}{32}{\texorpdfstring {$\la $}{lambda}-Kasteleyn weights}{equation.4.7}{}}
\@writefile{lla}{\contentsline {section}{\numberline {\crtrefnumber{eq:la_Cramer}}eq:la_Cramer}{32}{equation.4.7}\protected@file@percent }
\newlabel{eq:la_Cramer@cref}{{[equation][7][4]4.7}{[1][32][]32}{}{}{}}
\newlabel{eq:Cext_Cramer}{{4.8}{32}{\texorpdfstring {$\la $}{lambda}-Kasteleyn weights}{equation.4.8}{}}
\@writefile{lla}{\contentsline {section}{\numberline {\crtrefnumber{eq:Cext_Cramer}}eq:Cext_Cramer}{32}{equation.4.8}\protected@file@percent }
\newlabel{eq:Cext_Cramer@cref}{{[equation][8][4]4.8}{[1][32][]32}{}{}{}}
\@writefile{toc}{\contentsline {subsection}{\tocsubsection {}{4.4}{T-dual edge weights}}{32}{subsection.4.4}\protected@file@percent }
\newlabel{eq:ddwtlaK_dfn}{{4.9}{32}{T-dual edge weights}{equation.4.9}{}}
\@writefile{lla}{\contentsline {section}{\numberline {\crtrefnumber{eq:ddwtlaK_dfn}}eq:ddwtlaK_dfn}{32}{equation.4.9}\protected@file@percent }
\newlabel{eq:ddwtlaK_dfn@cref}{{[equation][9][4]4.9}{[1][32][]32}{}{}{}}
\newlabel{eq:ddwtlap_dfn}{{4.10}{32}{T-dual edge weights}{equation.4.10}{}}
\@writefile{lla}{\contentsline {section}{\numberline {\crtrefnumber{eq:ddwtlap_dfn}}eq:ddwtlap_dfn}{32}{equation.4.10}\protected@file@percent }
\newlabel{eq:ddwtlap_dfn@cref}{{[equation][10][4]4.10}{[1][32][]32}{}{}{}}
\@writefile{loe}{\contentsline {lemma}{\ifthmt@listswap Lemma~4.16\else \numberline {4.16}Lemma\fi }{32}{lemma.4.16}\protected@file@percent }
\newlabel{eq:SHIFT:sign_triangles}{{4.11}{32}{}{equation.4.11}{}}
\@writefile{lla}{\contentsline {section}{\numberline {\crtrefnumber{eq:SHIFT:sign_triangles}}eq:SHIFT:sign_triangles}{32}{equation.4.11}\protected@file@percent }
\newlabel{eq:SHIFT:sign_triangles@cref}{{[equation][11][4]4.11}{[1][32][]32}{}{}{}}
\newlabel{eq:SHIFT:sign_cycles}{{4.12}{32}{}{equation.4.12}{}}
\@writefile{lla}{\contentsline {section}{\numberline {\crtrefnumber{eq:SHIFT:sign_cycles}}eq:SHIFT:sign_cycles}{32}{equation.4.12}\protected@file@percent }
\newlabel{eq:SHIFT:sign_cycles@cref}{{[equation][12][4]4.12}{[1][32][]32}{}{}{}}
\@writefile{loe}{\contentsline {lemma}{\ifthmt@listswap Lemma~4.17\else \numberline {4.17}Lemma\fi }{32}{lemma.4.17}\protected@file@percent }
\newlabel{lemma:SHIFT:ddepsKla_is_Kast}{{4.17}{32}{}{lemma.4.17}{}}
\@writefile{lla}{\contentsline {section}{\numberline {\crtrefnumber{lemma:SHIFT:ddepsKla_is_Kast}}lemma:SHIFT:ddepsKla_is_Kast}{32}{lemma.4.17}\protected@file@percent }
\newlabel{lemma:SHIFT:ddepsKla_is_Kast@cref}{{[lemma][17][4]4.17}{[1][32][]32}{}{}{}}
\@writefile{toc}{\contentsline {subsection}{\tocsubsection {}{4.5}{T-dual boundary measurements}}{33}{subsection.4.5}\protected@file@percent }
\newlabel{eq:ddCext_dfn}{{4.13}{33}{T-dual boundary measurements}{equation.4.13}{}}
\@writefile{lla}{\contentsline {section}{\numberline {\crtrefnumber{eq:ddCext_dfn}}eq:ddCext_dfn}{33}{equation.4.13}\protected@file@percent }
\newlabel{eq:ddCext_dfn@cref}{{[equation][13][4]4.13}{[1][33][]33}{}{}{}}
\newlabel{eq:ddCext_bdry_dfn}{{4.14}{34}{T-dual boundary measurements}{equation.4.14}{}}
\@writefile{lla}{\contentsline {section}{\numberline {\crtrefnumber{eq:ddCext_bdry_dfn}}eq:ddCext_bdry_dfn}{34}{equation.4.14}\protected@file@percent }
\newlabel{eq:ddCext_bdry_dfn@cref}{{[equation][14][4]4.14}{[1][33][]34}{}{}{}}
\@writefile{loe}{\contentsline {proposition}{\ifthmt@listswap Proposition~4.18\else \numberline {4.18}Proposition\fi }{34}{proposition.4.18}\protected@file@percent }
\newlabel{lemma:SHIFT:ddCext_in_Hwspace}{{4.18}{34}{}{proposition.4.18}{}}
\@writefile{lla}{\contentsline {section}{\numberline {\crtrefnumber{lemma:SHIFT:ddCext_in_Hwspace}}lemma:SHIFT:ddCext_in_Hwspace}{34}{proposition.4.18}\protected@file@percent }
\newlabel{lemma:SHIFT:ddCext_in_Hwspace@cref}{{[proposition][18][4]4.18}{[1][34][]34}{}{}{}}
\newlabel{eq:sum_triangles_around}{{4.15}{34}{T-dual boundary measurements}{equation.4.15}{}}
\@writefile{lla}{\contentsline {section}{\numberline {\crtrefnumber{eq:sum_triangles_around}}eq:sum_triangles_around}{34}{equation.4.15}\protected@file@percent }
\newlabel{eq:sum_triangles_around@cref}{{[equation][15][4]4.15}{[1][34][]34}{}{}{}}
\newlabel{eq:sum_triangles_bdry}{{4.16}{34}{T-dual boundary measurements}{equation.4.16}{}}
\@writefile{lla}{\contentsline {section}{\numberline {\crtrefnumber{eq:sum_triangles_bdry}}eq:sum_triangles_bdry}{34}{equation.4.16}\protected@file@percent }
\newlabel{eq:sum_triangles_bdry@cref}{{[equation][16][4]4.16}{[1][34][]34}{}{}{}}
\@writefile{loe}{\contentsline {corollary}{\ifthmt@listswap Corollary~4.19\else \numberline {4.19}Corollary\fi }{34}{corollary.4.19}\protected@file@percent }
\newlabel{eq:Meas_ddG=Chat_Qla}{{4.17}{34}{}{equation.4.17}{}}
\@writefile{lla}{\contentsline {section}{\numberline {\crtrefnumber{eq:Meas_ddG=Chat_Qla}}eq:Meas_ddG=Chat_Qla}{34}{equation.4.17}\protected@file@percent }
\newlabel{eq:Meas_ddG=Chat_Qla@cref}{{[equation][17][4]4.17}{[1][34][]34}{}{}{}}
\@writefile{loe}{\contentsline {remark}{\ifthmt@listswap Remark~4.20\else \numberline {4.20}Remark\fi \thmtformatoptarg {Inverse T-duality}}{34}{remark.4.20}\protected@file@percent }
\newlabel{rmk:SHIFT:inverse}{{4.20}{34}{Inverse T-duality}{remark.4.20}{}}
\@writefile{lla}{\contentsline {section}{\numberline {\crtrefnumber{rmk:SHIFT:inverse}}rmk:SHIFT:inverse}{34}{remark.4.20}\protected@file@percent }
\newlabel{rmk:SHIFT:inverse@cref}{{[remark][20][4]4.20}{[1][34][]34}{}{}{}}
\citation{origami1}
\citation{crit}
\citation{Affolter}
\citation{Pos}
\newlabel{sec:shift:by1}{{4.6}{35}{Shifting edge weights by $1$ twice}{subsection.4.6}{}}
\@writefile{lla}{\contentsline {section}{\numberline {\crtrefnumber{sec:shift:by1}}sec:shift:by1}{35}{subsection.4.6}\protected@file@percent }
\newlabel{sec:shift:by1@cref}{{[subsection][6][4]4.6}{[1][35][]35}{}{}{}}
\@writefile{toc}{\contentsline {subsection}{\tocsubsection {}{4.6}{Shifting edge weights by $1$ twice}}{35}{subsection.4.6}\protected@file@percent }
\@writefile{toc}{\contentsline {section}{\tocsection {}{5}{$L$-punctured\xspace  positive Grassmannian}}{35}{section.5}\protected@file@percent }
\newlabel{sec:LPUNC}{{5}{35}{\LpuncTITLE positive Grassmannian}{section.5}{}}
\@writefile{lla}{\contentsline {section}{\numberline {\crtrefnumber{sec:LPUNC}}sec:LPUNC}{35}{section.5}\protected@file@percent }
\newlabel{sec:LPUNC@cref}{{[section][5][]5}{[1][35][]35}{}{}{}}
\newlabel{ssec:LPUNC:Lfunc_graphs}{{5.1}{35}{Double dimers and \KSprims }{subsection.5.1}{}}
\@writefile{lla}{\contentsline {section}{\numberline {\crtrefnumber{ssec:LPUNC:Lfunc_graphs}}ssec:LPUNC:Lfunc_graphs}{35}{subsection.5.1}\protected@file@percent }
\newlabel{ssec:LPUNC:Lfunc_graphs@cref}{{[subsection][1][5]5.1}{[1][35][]35}{}{}{}}
\@writefile{toc}{\contentsline {subsection}{\tocsubsection {}{5.1}{Double dimers and Kenyon--Smirnov primitives\xspace  }}{35}{subsection.5.1}\protected@file@percent }
\@writefile{loe}{\contentsline {definition}{\ifthmt@listswap Definition~5.1\else \numberline {5.1}Definition\fi }{35}{definition.5.1}\protected@file@percent }
\@writefile{loe}{\contentsline {definition}{\ifthmt@listswap Definition~5.2\else \numberline {5.2}Definition\fi }{35}{definition.5.2}\protected@file@percent }
\newlabel{dfn:LPUNC:Hknk}{{5.2}{35}{}{definition.5.2}{}}
\@writefile{lla}{\contentsline {section}{\numberline {\crtrefnumber{dfn:LPUNC:Hknk}}dfn:LPUNC:Hknk}{35}{definition.5.2}\protected@file@percent }
\newlabel{dfn:LPUNC:Hknk@cref}{{[definition][2][5]5.2}{[1][35][]35}{}{}{}}
\newlabel{eq:LPUNC:primitive_knk}{{5.1}{35}{}{equation.5.1}{}}
\@writefile{lla}{\contentsline {section}{\numberline {\crtrefnumber{eq:LPUNC:primitive_knk}}eq:LPUNC:primitive_knk}{35}{equation.5.1}\protected@file@percent }
\newlabel{eq:LPUNC:primitive_knk@cref}{{[equation][1][5]5.1}{[1][35][]35}{}{}{}}
\@writefile{loe}{\contentsline {remark}{\ifthmt@listswap Remark~5.3\else \numberline {5.3}Remark\fi }{35}{remark.5.3}\protected@file@percent }
\newlabel{rmk:LPUNC:GL_x_GL}{{5.3}{35}{}{remark.5.3}{}}
\@writefile{lla}{\contentsline {section}{\numberline {\crtrefnumber{rmk:LPUNC:GL_x_GL}}rmk:LPUNC:GL_x_GL}{35}{remark.5.3}\protected@file@percent }
\newlabel{rmk:LPUNC:GL_x_GL@cref}{{[remark][3][5]5.3}{[1][35][]35}{}{}{}}
\@writefile{loe}{\contentsline {remark}{\ifthmt@listswap Remark~5.4\else \numberline {5.4}Remark\fi }{36}{remark.5.4}\protected@file@percent }
\newlabel{rmk:LPUNC:tangent}{{5.4}{36}{}{remark.5.4}{}}
\@writefile{lla}{\contentsline {section}{\numberline {\crtrefnumber{rmk:LPUNC:tangent}}rmk:LPUNC:tangent}{36}{remark.5.4}\protected@file@percent }
\newlabel{rmk:LPUNC:tangent@cref}{{[remark][4][5]5.4}{[1][36][]36}{}{}{}}
\@writefile{loe}{\contentsline {proposition}{\ifthmt@listswap Proposition~5.5\else \numberline {5.5}Proposition\fi }{36}{proposition.5.5}\protected@file@percent }
\newlabel{lemma:LPUNC:H_vs_C'(1)}{{5.5}{36}{}{proposition.5.5}{}}
\@writefile{lla}{\contentsline {section}{\numberline {\crtrefnumber{lemma:LPUNC:H_vs_C'(1)}}lemma:LPUNC:H_vs_C'(1)}{36}{proposition.5.5}\protected@file@percent }
\newlabel{lemma:LPUNC:H_vs_C'(1)@cref}{{[proposition][5][5]5.5}{[1][36][]36}{}{}{}}
\newlabel{eq:H_vs_C'(1)_invariant}{{5.2}{36}{}{equation.5.2}{}}
\@writefile{lla}{\contentsline {section}{\numberline {\crtrefnumber{eq:H_vs_C'(1)_invariant}}eq:H_vs_C'(1)_invariant}{36}{equation.5.2}\protected@file@percent }
\newlabel{eq:H_vs_C'(1)_invariant@cref}{{[equation][2][5]5.2}{[1][36][]36}{}{}{}}
\newlabel{eq:Cp_C(t)_=_sum_edges}{{5.3}{36}{Double dimers and \KSprims }{equation.5.3}{}}
\@writefile{lla}{\contentsline {section}{\numberline {\crtrefnumber{eq:Cp_C(t)_=_sum_edges}}eq:Cp_C(t)_=_sum_edges}{36}{equation.5.3}\protected@file@percent }
\newlabel{eq:Cp_C(t)_=_sum_edges@cref}{{[equation][3][5]5.3}{[1][36][]36}{}{}{}}
\newlabel{eq:Cp_C'(1)_=_H_1-H_2}{{5.4}{36}{Double dimers and \KSprims }{equation.5.4}{}}
\@writefile{lla}{\contentsline {section}{\numberline {\crtrefnumber{eq:Cp_C'(1)_=_H_1-H_2}}eq:Cp_C'(1)_=_H_1-H_2}{36}{equation.5.4}\protected@file@percent }
\newlabel{eq:Cp_C'(1)_=_H_1-H_2@cref}{{[equation][4][5]5.4}{[1][36][]36}{}{}{}}
\citation{origami1}
\newlabel{eq:LPUNC:ZSTcut}{{5.5}{37}{Double dimers and \KSprims }{equation.5.5}{}}
\@writefile{lla}{\contentsline {section}{\numberline {\crtrefnumber{eq:LPUNC:ZSTcut}}eq:LPUNC:ZSTcut}{37}{equation.5.5}\protected@file@percent }
\newlabel{eq:LPUNC:ZSTcut@cref}{{[equation][5][5]5.5}{[1][36][]37}{}{}{}}
\@writefile{loe}{\contentsline {remark}{\ifthmt@listswap Remark~5.6\else \numberline {5.6}Remark\fi }{37}{remark.5.6}\protected@file@percent }
\newlabel{rmk:LPUNC:prob_ZST}{{5.6}{37}{}{remark.5.6}{}}
\@writefile{lla}{\contentsline {section}{\numberline {\crtrefnumber{rmk:LPUNC:prob_ZST}}rmk:LPUNC:prob_ZST}{37}{remark.5.6}\protected@file@percent }
\newlabel{rmk:LPUNC:prob_ZST@cref}{{[remark][6][5]5.6}{[1][37][]37}{}{}{}}
\@writefile{loe}{\contentsline {proposition}{\ifthmt@listswap Proposition~5.7\else \numberline {5.7}Proposition\fi }{37}{proposition.5.7}\protected@file@percent }
\newlabel{lemma:LPUNC:minors_dH}{{5.7}{37}{}{proposition.5.7}{}}
\@writefile{lla}{\contentsline {section}{\numberline {\crtrefnumber{lemma:LPUNC:minors_dH}}lemma:LPUNC:minors_dH}{37}{proposition.5.7}\protected@file@percent }
\newlabel{lemma:LPUNC:minors_dH@cref}{{[proposition][7][5]5.7}{[1][37][]37}{}{}{}}
\newlabel{eq:LPUNC:minors_dH}{{5.6}{37}{}{equation.5.6}{}}
\@writefile{lla}{\contentsline {section}{\numberline {\crtrefnumber{eq:LPUNC:minors_dH}}eq:LPUNC:minors_dH}{37}{equation.5.6}\protected@file@percent }
\newlabel{eq:LPUNC:minors_dH@cref}{{[equation][6][5]5.6}{[1][37][]37}{}{}{}}
\@writefile{loe}{\contentsline {corollary}{\ifthmt@listswap Corollary~5.8\else \numberline {5.8}Corollary\fi }{37}{corollary.5.8}\protected@file@percent }
\newlabel{lemma:LPUNC:dist}{{5.8}{37}{}{corollary.5.8}{}}
\@writefile{lla}{\contentsline {section}{\numberline {\crtrefnumber{lemma:LPUNC:dist}}lemma:LPUNC:dist}{37}{corollary.5.8}\protected@file@percent }
\newlabel{lemma:LPUNC:dist@cref}{{[corollary][8][5]5.8}{[1][37][]37}{}{}{}}
\newlabel{eq:LPUNC:dist}{{5.7}{37}{}{equation.5.7}{}}
\@writefile{lla}{\contentsline {section}{\numberline {\crtrefnumber{eq:LPUNC:dist}}eq:LPUNC:dist}{37}{equation.5.7}\protected@file@percent }
\newlabel{eq:LPUNC:dist@cref}{{[equation][7][5]5.7}{[1][37][]37}{}{}{}}
\newlabel{eq:distrk<distsep}{{5.8}{37}{Double dimers and \KSprims }{equation.5.8}{}}
\@writefile{lla}{\contentsline {section}{\numberline {\crtrefnumber{eq:distrk<distsep}}eq:distrk<distsep}{37}{equation.5.8}\protected@file@percent }
\newlabel{eq:distrk<distsep@cref}{{[equation][8][5]5.8}{[1][37][]37}{}{}{}}
\@writefile{lof}{\contentsline {figure}{\numberline {11}{\ignorespaces  Computing the Kenyon--Smirnov primitive\xspace  $\textcolor {red}{H}:\mathbf  {V}^\ast \to \operatorname  {Mat}_{n-k,k}({\mathbb  {R}})$.}}{38}{figure.caption.19}\protected@file@percent }
\newlabel{fig:holom2}{{11}{38}{Computing the \KSprim $\textcolor {\puncColor }{\Hknk }:\Faces \to \Rknk $}{figure.caption.19}{}}
\@writefile{lla}{\contentsline {section}{\numberline {\crtrefnumber{fig:holom2}}fig:holom2}{38}{figure.caption.19}\protected@file@percent }
\newlabel{fig:holom2@cref}{{[figure][11][]11}{[1][38][]38}{}{}{}}
\@writefile{loe}{\contentsline {conjecture}{\ifthmt@listswap Conjecture~5.9\else \numberline {5.9}Conjecture\fi }{38}{conjecture.5.9}\protected@file@percent }
\newlabel{conj:dist}{{5.9}{38}{}{conjecture.5.9}{}}
\@writefile{lla}{\contentsline {section}{\numberline {\crtrefnumber{conj:dist}}conj:dist}{38}{conjecture.5.9}\protected@file@percent }
\newlabel{conj:dist@cref}{{[conjecture][9][5]5.9}{[1][38][]38}{}{}{}}
\newlabel{eq:conj_dist}{{5.9}{38}{}{equation.5.9}{}}
\@writefile{lla}{\contentsline {section}{\numberline {\crtrefnumber{eq:conj_dist}}eq:conj_dist}{38}{equation.5.9}\protected@file@percent }
\newlabel{eq:conj_dist@cref}{{[equation][9][5]5.9}{[1][38][]38}{}{}{}}
\@writefile{loe}{\contentsline {example}{\ifthmt@listswap Example~5.10\else \numberline {5.10}Example\fi }{38}{example.5.10}\protected@file@percent }
\newlabel{sec:LPUNC:Gr}{{5.2}{38}{\LfuncTITLE positive Grassmannian}{subsection.5.2}{}}
\@writefile{lla}{\contentsline {section}{\numberline {\crtrefnumber{sec:LPUNC:Gr}}sec:LPUNC:Gr}{38}{subsection.5.2}\protected@file@percent }
\newlabel{sec:LPUNC:Gr@cref}{{[subsection][2][5]5.2}{[1][38][]38}{}{}{}}
\@writefile{toc}{\contentsline {subsection}{\tocsubsection {}{5.2}{$L^\ast $-punctured\xspace  positive Grassmannian}}{38}{thmt@dummyctr.dummy.122}\protected@file@percent }
\@writefile{loe}{\contentsline {definition}{\ifthmt@listswap Definition~5.11\else \numberline {5.11}Definition\fi \thmtformatoptarg {$2$-separated\xspace  faces}}{38}{definition.5.11}\protected@file@percent }
\newlabel{dfn:PROP:2sep}{{5.11}{38}{\Twosep faces}{definition.5.11}{}}
\@writefile{lla}{\contentsline {section}{\numberline {\crtrefnumber{dfn:PROP:2sep}}dfn:PROP:2sep}{38}{definition.5.11}\protected@file@percent }
\newlabel{dfn:PROP:2sep@cref}{{[definition][11][5]5.11}{[1][38][]38}{}{}{}}
\@writefile{loe}{\contentsline {definition}{\ifthmt@listswap Definition~5.12\else \numberline {5.12}Definition\fi }{38}{definition.5.12}\protected@file@percent }
\newlabel{dfn:LPUNC:Lfunc_graph}{{5.12}{38}{}{definition.5.12}{}}
\@writefile{lla}{\contentsline {section}{\numberline {\crtrefnumber{dfn:LPUNC:Lfunc_graph}}dfn:LPUNC:Lfunc_graph}{38}{definition.5.12}\protected@file@percent }
\newlabel{dfn:LPUNC:Lfunc_graph@cref}{{[definition][12][5]5.12}{[1][38][]38}{}{}{}}
\citation{origami1}
\citation{RhSk}
\citation{Lam_dimers}
\citation{FoGo}
\citation{Kenyon_conf_loops}
\@writefile{loe}{\contentsline {definition}{\ifthmt@listswap Definition~5.13\else \numberline {5.13}Definition\fi }{39}{definition.5.13}\protected@file@percent }
\newlabel{dfn:fullysep}{{5.13}{39}{}{definition.5.13}{}}
\@writefile{lla}{\contentsline {section}{\numberline {\crtrefnumber{dfn:fullysep}}dfn:fullysep}{39}{definition.5.13}\protected@file@percent }
\newlabel{dfn:fullysep@cref}{{[definition][13][5]5.13}{[1][38][]39}{}{}{}}
\newlabel{eq:brnLbdsep_dfn}{{5.10}{39}{}{equation.5.10}{}}
\@writefile{lla}{\contentsline {section}{\numberline {\crtrefnumber{eq:brnLbdsep_dfn}}eq:brnLbdsep_dfn}{39}{equation.5.10}\protected@file@percent }
\newlabel{eq:brnLbdsep_dfn@cref}{{[equation][10][5]5.10}{[1][38][]39}{}{}{}}
\@writefile{loe}{\contentsline {definition}{\ifthmt@listswap Definition~5.14\else \numberline {5.14}Definition\fi \thmtformatoptarg {$L^\ast $-punctured\xspace  boundary measurement map}}{39}{definition.5.14}\protected@file@percent }
\newlabel{dfn:LPUNC:Meas_func}{{5.14}{39}{\Lfunc boundary measurement map}{definition.5.14}{}}
\@writefile{lla}{\contentsline {section}{\numberline {\crtrefnumber{dfn:LPUNC:Meas_func}}dfn:LPUNC:Meas_func}{39}{definition.5.14}\protected@file@percent }
\newlabel{dfn:LPUNC:Meas_func@cref}{{[definition][14][5]5.14}{[1][39][]39}{}{}{}}
\newlabel{eq:Measknk_dfn}{{5.11}{39}{\Lfunc boundary measurement map}{equation.5.11}{}}
\@writefile{lla}{\contentsline {section}{\numberline {\crtrefnumber{eq:Measknk_dfn}}eq:Measknk_dfn}{39}{equation.5.11}\protected@file@percent }
\newlabel{eq:Measknk_dfn@cref}{{[equation][11][5]5.11}{[1][39][]39}{}{}{}}
\@writefile{loe}{\contentsline {remark}{\ifthmt@listswap Remark~5.15\else \numberline {5.15}Remark\fi }{39}{remark.5.15}\protected@file@percent }
\newlabel{rmk:H_bdry}{{5.15}{39}{}{remark.5.15}{}}
\@writefile{lla}{\contentsline {section}{\numberline {\crtrefnumber{rmk:H_bdry}}rmk:H_bdry}{39}{remark.5.15}\protected@file@percent }
\newlabel{rmk:H_bdry@cref}{{[remark][15][5]5.15}{[1][39][]39}{}{}{}}
\@writefile{loe}{\contentsline {definition}{\ifthmt@listswap Definition~5.16\else \numberline {5.16}Definition\fi \thmtformatoptarg {$L^\ast $-punctured\xspace  totally nonnegative Grassmannian}}{39}{definition.5.16}\protected@file@percent }
\newlabel{dfn:Lfunc_tnn_Gr}{{5.16}{39}{\Lfunc totally nonnegative Grassmannian}{definition.5.16}{}}
\@writefile{lla}{\contentsline {section}{\numberline {\crtrefnumber{dfn:Lfunc_tnn_Gr}}dfn:Lfunc_tnn_Gr}{39}{definition.5.16}\protected@file@percent }
\newlabel{dfn:Lfunc_tnn_Gr@cref}{{[definition][16][5]5.16}{[1][39][]39}{}{}{}}
\@writefile{loe}{\contentsline {problem}{\ifthmt@listswap Problem~5.17\else \numberline {5.17}Problem\fi }{39}{problem.5.17}\protected@file@percent }
\newlabel{problem:GrtnnLfunc_by_ineq}{{5.17}{39}{}{problem.5.17}{}}
\@writefile{lla}{\contentsline {section}{\numberline {\crtrefnumber{problem:GrtnnLfunc_by_ineq}}problem:GrtnnLfunc_by_ineq}{39}{problem.5.17}\protected@file@percent }
\newlabel{problem:GrtnnLfunc_by_ineq@cref}{{[problem][17][5]5.17}{[1][39][]39}{}{}{}}
\@writefile{loe}{\contentsline {remark}{\ifthmt@listswap Remark~5.18\else \numberline {5.18}Remark\fi }{39}{remark.5.18}\protected@file@percent }
\@writefile{loe}{\contentsline {definition}{\ifthmt@listswap Definition~5.19\else \numberline {5.19}Definition\fi }{39}{definition.5.19}\protected@file@percent }
\newlabel{dfn:Lfunc_positroid_cell_and_reduced}{{5.19}{39}{}{definition.5.19}{}}
\@writefile{lla}{\contentsline {section}{\numberline {\crtrefnumber{dfn:Lfunc_positroid_cell_and_reduced}}dfn:Lfunc_positroid_cell_and_reduced}{39}{definition.5.19}\protected@file@percent }
\newlabel{dfn:Lfunc_positroid_cell_and_reduced@cref}{{[definition][19][5]5.19}{[1][39][]39}{}{}{}}
\@writefile{loe}{\contentsline {problem}{\ifthmt@listswap Problem~5.20\else \numberline {5.20}Problem\fi }{39}{problem.5.20}\protected@file@percent }
\@writefile{loe}{\contentsline {remark}{\ifthmt@listswap Remark~5.21\else \numberline {5.21}Remark\fi }{39}{remark.5.21}\protected@file@percent }
\citation{MuSp}
\@writefile{loe}{\contentsline {remark}{\ifthmt@listswap Remark~5.22\else \numberline {5.22}Remark\fi }{40}{remark.5.22}\protected@file@percent }
\@writefile{loe}{\contentsline {definition}{\ifthmt@listswap Definition~5.23\else \numberline {5.23}Definition\fi }{40}{definition.5.23}\protected@file@percent }
\newlabel{eq:LPUNC:Measdnk_def}{{5.13}{40}{}{equation.5.13}{}}
\@writefile{lla}{\contentsline {section}{\numberline {\crtrefnumber{eq:LPUNC:Measdnk_def}}eq:LPUNC:Measdnk_def}{40}{equation.5.13}\protected@file@percent }
\newlabel{eq:LPUNC:Measdnk_def@cref}{{[equation][13][5]5.13}{[1][40][]40}{}{}{}}
\@writefile{toc}{\contentsline {subsection}{\tocsubsection {}{5.3}{$L^\ast $-punctured\xspace  graphs of type $(1,n)$}}{40}{subsection.5.3}\protected@file@percent }
\@writefile{loe}{\contentsline {proposition}{\ifthmt@listswap Proposition~5.24\else \numberline {5.24}Proposition\fi }{40}{proposition.5.24}\protected@file@percent }
\newlabel{prop:ccc}{{5.24}{40}{}{proposition.5.24}{}}
\@writefile{lla}{\contentsline {section}{\numberline {\crtrefnumber{prop:ccc}}prop:ccc}{40}{proposition.5.24}\protected@file@percent }
\newlabel{prop:ccc@cref}{{[proposition][24][5]5.24}{[1][40][]40}{}{}{}}
\newlabel{eq:bcccloc_dfn_type_1n}{{5.14}{40}{}{equation.5.14}{}}
\@writefile{lla}{\contentsline {section}{\numberline {\crtrefnumber{eq:bcccloc_dfn_type_1n}}eq:bcccloc_dfn_type_1n}{40}{equation.5.14}\protected@file@percent }
\newlabel{eq:bcccloc_dfn_type_1n@cref}{{[equation][14][5]5.14}{[1][40][]40}{}{}{}}
\newlabel{eq:rpp_sum=1}{{5.15}{40}{\LfuncTITLE graphs of type $(1,n)$}{equation.5.15}{}}
\@writefile{lla}{\contentsline {section}{\numberline {\crtrefnumber{eq:rpp_sum=1}}eq:rpp_sum=1}{40}{equation.5.15}\protected@file@percent }
\newlabel{eq:rpp_sum=1@cref}{{[equation][15][5]5.15}{[1][40][]40}{}{}{}}
\newlabel{eq:Hbd_for_k=1}{{5.16}{40}{\LfuncTITLE graphs of type $(1,n)$}{equation.5.16}{}}
\@writefile{lla}{\contentsline {section}{\numberline {\crtrefnumber{eq:Hbd_for_k=1}}eq:Hbd_for_k=1}{40}{equation.5.16}\protected@file@percent }
\newlabel{eq:Hbd_for_k=1@cref}{{[equation][16][5]5.16}{[1][40][]40}{}{}{}}
\newlabel{eq:Simplexr_dfn}{{5.17}{40}{\LfuncTITLE graphs of type $(1,n)$}{equation.5.17}{}}
\@writefile{lla}{\contentsline {section}{\numberline {\crtrefnumber{eq:Simplexr_dfn}}eq:Simplexr_dfn}{40}{equation.5.17}\protected@file@percent }
\newlabel{eq:Simplexr_dfn@cref}{{[equation][17][5]5.17}{[1][40][]40}{}{}{}}
\citation{Pos}
\@writefile{loe}{\contentsline {definition}{\ifthmt@listswap Definition~5.25\else \numberline {5.25}Definition\fi }{41}{definition.5.25}\protected@file@percent }
\@writefile{loe}{\contentsline {lemma}{\ifthmt@listswap Lemma~5.26\else \numberline {5.26}Lemma\fi }{41}{lemma.5.26}\protected@file@percent }
\newlabel{lemma:counting_stars_type_1_n}{{5.26}{41}{}{lemma.5.26}{}}
\@writefile{lla}{\contentsline {section}{\numberline {\crtrefnumber{lemma:counting_stars_type_1_n}}lemma:counting_stars_type_1_n}{41}{lemma.5.26}\protected@file@percent }
\newlabel{lemma:counting_stars_type_1_n@cref}{{[lemma][26][5]5.26}{[1][41][]41}{}{}{}}
\newlabel{eq:counting_stars_type_1_n}{{5.18}{41}{}{equation.5.18}{}}
\@writefile{lla}{\contentsline {section}{\numberline {\crtrefnumber{eq:counting_stars_type_1_n}}eq:counting_stars_type_1_n}{41}{equation.5.18}\protected@file@percent }
\newlabel{eq:counting_stars_type_1_n@cref}{{[equation][18][5]5.18}{[1][41][]41}{}{}{}}
\newlabel{ssec:Lvunc}{{5.4}{41}{\LvuncTITLE graphs}{subsection.5.4}{}}
\@writefile{lla}{\contentsline {section}{\numberline {\crtrefnumber{ssec:Lvunc}}ssec:Lvunc}{41}{subsection.5.4}\protected@file@percent }
\newlabel{ssec:Lvunc@cref}{{[subsection][4][5]5.4}{[1][41][]41}{}{}{}}
\@writefile{toc}{\contentsline {subsection}{\tocsubsection {}{5.4}{$L^{\bullet }$-punctured\xspace  graphs}}{41}{subsection.5.4}\protected@file@percent }
\@writefile{lof}{\contentsline {figure}{\numberline {12}{\ignorespaces  Popping black vertices of a generalized $L^{\bullet }$-punctured\xspace  graph $\ddot  {\Gamma }_{\!L^{\bullet }}$.}}{42}{figure.caption.20}\protected@file@percent }
\newlabel{fig:popping}{{12}{42}{Popping black vertices of a generalized \Lvunc graph $\ddGvunc $}{figure.caption.20}{}}
\@writefile{lla}{\contentsline {section}{\numberline {\crtrefnumber{fig:popping}}fig:popping}{42}{figure.caption.20}\protected@file@percent }
\newlabel{fig:popping@cref}{{[figure][12][]12}{[1][42][]42}{}{}{}}
\@writefile{loe}{\contentsline {definition}{\ifthmt@listswap Definition~5.27\else \numberline {5.27}Definition\fi }{42}{definition.5.27}\protected@file@percent }
\newlabel{dfn:Lvunc_ordinary}{{5.27}{42}{}{definition.5.27}{}}
\@writefile{lla}{\contentsline {section}{\numberline {\crtrefnumber{dfn:Lvunc_ordinary}}dfn:Lvunc_ordinary}{42}{definition.5.27}\protected@file@percent }
\newlabel{dfn:Lvunc_ordinary@cref}{{[definition][27][5]5.27}{[1][41][]42}{}{}{}}
\@writefile{loe}{\contentsline {definition}{\ifthmt@listswap Definition~5.28\else \numberline {5.28}Definition\fi }{42}{definition.5.28}\protected@file@percent }
\newlabel{dfn:fullyind}{{5.28}{42}{}{definition.5.28}{}}
\@writefile{lla}{\contentsline {section}{\numberline {\crtrefnumber{dfn:fullyind}}dfn:fullyind}{42}{definition.5.28}\protected@file@percent }
\newlabel{dfn:fullyind@cref}{{[definition][28][5]5.28}{[1][42][]42}{}{}{}}
\@writefile{loe}{\contentsline {definition}{\ifthmt@listswap Definition~5.29\else \numberline {5.29}Definition\fi }{42}{definition.5.29}\protected@file@percent }
\newlabel{dfn:gen_Lvunc}{{5.29}{42}{}{definition.5.29}{}}
\@writefile{lla}{\contentsline {section}{\numberline {\crtrefnumber{dfn:gen_Lvunc}}dfn:gen_Lvunc}{42}{definition.5.29}\protected@file@percent }
\newlabel{dfn:gen_Lvunc@cref}{{[definition][29][5]5.29}{[1][42][]42}{}{}{}}
\@writefile{loe}{\contentsline {definition}{\ifthmt@listswap Definition~5.30\else \numberline {5.30}Definition\fi }{42}{definition.5.30}\protected@file@percent }
\newlabel{dfn:ddGlocs}{{5.30}{42}{}{definition.5.30}{}}
\@writefile{lla}{\contentsline {section}{\numberline {\crtrefnumber{dfn:ddGlocs}}dfn:ddGlocs}{42}{definition.5.30}\protected@file@percent }
\newlabel{dfn:ddGlocs@cref}{{[definition][30][5]5.30}{[1][42][]42}{}{}{}}
\newlabel{eq:ddGlocs_dfn}{{5.19}{42}{}{equation.5.19}{}}
\@writefile{lla}{\contentsline {section}{\numberline {\crtrefnumber{eq:ddGlocs_dfn}}eq:ddGlocs_dfn}{42}{equation.5.19}\protected@file@percent }
\newlabel{eq:ddGlocs_dfn@cref}{{[equation][19][5]5.19}{[1][42][]42}{}{}{}}
\@writefile{loe}{\contentsline {definition}{\ifthmt@listswap Definition~5.31\else \numberline {5.31}Definition\fi }{42}{definition.5.31}\protected@file@percent }
\newlabel{dfn:fullyind_gen}{{5.31}{42}{}{definition.5.31}{}}
\@writefile{lla}{\contentsline {section}{\numberline {\crtrefnumber{dfn:fullyind_gen}}dfn:fullyind_gen}{42}{definition.5.31}\protected@file@percent }
\newlabel{dfn:fullyind_gen@cref}{{[definition][31][5]5.31}{[1][42][]42}{}{}{}}
\citation{origami1}
\@writefile{loe}{\contentsline {definition}{\ifthmt@listswap Definition~5.32\else \numberline {5.32}Definition\fi }{43}{definition.5.32}\protected@file@percent }
\newlabel{dfn:ddwtaux}{{5.32}{43}{}{definition.5.32}{}}
\@writefile{lla}{\contentsline {section}{\numberline {\crtrefnumber{dfn:ddwtaux}}dfn:ddwtaux}{43}{definition.5.32}\protected@file@percent }
\newlabel{dfn:ddwtaux@cref}{{[definition][32][5]5.32}{[1][43][]43}{}{}{}}
\@writefile{loe}{\contentsline {definition}{\ifthmt@listswap Definition~5.33\else \numberline {5.33}Definition\fi \thmtformatoptarg {$L^{\bullet }$-punctured\xspace  boundary measurement map}}{43}{definition.5.33}\protected@file@percent }
\newlabel{dfn:LPUNC:Meas_vunc}{{5.33}{43}{\Lvunc boundary measurement map}{definition.5.33}{}}
\@writefile{lla}{\contentsline {section}{\numberline {\crtrefnumber{dfn:LPUNC:Meas_vunc}}dfn:LPUNC:Meas_vunc}{43}{definition.5.33}\protected@file@percent }
\newlabel{dfn:LPUNC:Meas_vunc@cref}{{[definition][33][5]5.33}{[1][43][]43}{}{}{}}
\newlabel{eq:LPUNC:Measbiv_dfn}{{5.20}{43}{\Lvunc boundary measurement map}{equation.5.20}{}}
\@writefile{lla}{\contentsline {section}{\numberline {\crtrefnumber{eq:LPUNC:Measbiv_dfn}}eq:LPUNC:Measbiv_dfn}{43}{equation.5.20}\protected@file@percent }
\newlabel{eq:LPUNC:Measbiv_dfn@cref}{{[equation][20][5]5.20}{[1][43][]43}{}{}{}}
\newlabel{eq:LPUNC:stack}{{5.21}{43}{\Lvunc boundary measurement map}{equation.5.21}{}}
\@writefile{lla}{\contentsline {section}{\numberline {\crtrefnumber{eq:LPUNC:stack}}eq:LPUNC:stack}{43}{equation.5.21}\protected@file@percent }
\newlabel{eq:LPUNC:stack@cref}{{[equation][21][5]5.21}{[1][43][]43}{}{}{}}
\@writefile{loe}{\contentsline {remark}{\ifthmt@listswap Remark~5.34\else \numberline {5.34}Remark\fi }{43}{remark.5.34}\protected@file@percent }
\newlabel{rmk:Drestloc_ibd}{{5.34}{43}{}{remark.5.34}{}}
\@writefile{lla}{\contentsline {section}{\numberline {\crtrefnumber{rmk:Drestloc_ibd}}rmk:Drestloc_ibd}{43}{remark.5.34}\protected@file@percent }
\newlabel{rmk:Drestloc_ibd@cref}{{[remark][34][5]5.34}{[1][43][]43}{}{}{}}
\@writefile{loe}{\contentsline {example}{\ifthmt@listswap Example~5.35\else \numberline {5.35}Example\fi }{43}{example.5.35}\protected@file@percent }
\newlabel{ex:non_ordinary_Meas_Lvunc}{{5.35}{43}{}{example.5.35}{}}
\@writefile{lla}{\contentsline {section}{\numberline {\crtrefnumber{ex:non_ordinary_Meas_Lvunc}}ex:non_ordinary_Meas_Lvunc}{43}{example.5.35}\protected@file@percent }
\newlabel{ex:non_ordinary_Meas_Lvunc@cref}{{[example][35][5]5.35}{[1][43][]43}{}{}{}}
\@writefile{loe}{\contentsline {lemma}{\ifthmt@listswap Lemma~5.36\else \numberline {5.36}Lemma\fi }{43}{lemma.5.36}\protected@file@percent }
\newlabel{lemma:LPUNC:indep<=>full_rank_Dbivloc}{{5.36}{43}{}{lemma.5.36}{}}
\@writefile{lla}{\contentsline {section}{\numberline {\crtrefnumber{lemma:LPUNC:indep<=>full_rank_Dbivloc}}lemma:LPUNC:indep<=>full_rank_Dbivloc}{43}{lemma.5.36}\protected@file@percent }
\newlabel{lemma:LPUNC:indep<=>full_rank_Dbivloc@cref}{{[lemma][36][5]5.36}{[1][43][]43}{}{}{}}
\newlabel{eq:Dbiv=Meas}{{5.22}{43}{}{equation.5.22}{}}
\@writefile{lla}{\contentsline {section}{\numberline {\crtrefnumber{eq:Dbiv=Meas}}eq:Dbiv=Meas}{43}{equation.5.22}\protected@file@percent }
\newlabel{eq:Dbiv=Meas@cref}{{[equation][22][5]5.22}{[1][43][]43}{}{}{}}
\@writefile{loe}{\contentsline {corollary}{\ifthmt@listswap Corollary~5.37\else \numberline {5.37}Corollary\fi }{44}{corollary.5.37}\protected@file@percent }
\newlabel{lemma:LPUNC:D_perp_cap_la=0}{{5.37}{44}{}{corollary.5.37}{}}
\@writefile{lla}{\contentsline {section}{\numberline {\crtrefnumber{lemma:LPUNC:D_perp_cap_la=0}}lemma:LPUNC:D_perp_cap_la=0}{44}{corollary.5.37}\protected@file@percent }
\newlabel{lemma:LPUNC:D_perp_cap_la=0@cref}{{[corollary][37][5]5.37}{[1][44][]44}{}{}{}}
\newlabel{eq:Dbivloc_cap_la=0}{{5.23}{44}{}{equation.5.23}{}}
\@writefile{lla}{\contentsline {section}{\numberline {\crtrefnumber{eq:Dbivloc_cap_la=0}}eq:Dbivloc_cap_la=0}{44}{equation.5.23}\protected@file@percent }
\newlabel{eq:Dbivloc_cap_la=0@cref}{{[equation][23][5]5.23}{[1][44][]44}{}{}{}}
\newlabel{eq:GENPUNC:dual_vector}{{5.24}{44}{\LvuncTITLE graphs}{equation.5.24}{}}
\@writefile{lla}{\contentsline {section}{\numberline {\crtrefnumber{eq:GENPUNC:dual_vector}}eq:GENPUNC:dual_vector}{44}{equation.5.24}\protected@file@percent }
\newlabel{eq:GENPUNC:dual_vector@cref}{{[equation][24][5]5.24}{[1][44][]44}{}{}{}}
\@writefile{loe}{\contentsline {definition}{\ifthmt@listswap Definition~5.38\else \numberline {5.38}Definition\fi }{45}{definition.5.38}\protected@file@percent }
\newlabel{dfn:Grtnnflamb_CDind}{{5.38}{45}{}{definition.5.38}{}}
\@writefile{lla}{\contentsline {section}{\numberline {\crtrefnumber{dfn:Grtnnflamb_CDind}}dfn:Grtnnflamb_CDind}{45}{definition.5.38}\protected@file@percent }
\newlabel{dfn:Grtnnflamb_CDind@cref}{{[definition][38][5]5.38}{[1][45][]45}{}{}{}}
\@writefile{loe}{\contentsline {definition}{\ifthmt@listswap Definition~5.39\else \numberline {5.39}Definition\fi \thmtformatoptarg {$L^{\bullet }$-punctured\xspace  totally nonnegative Grassmannian}}{45}{definition.5.39}\protected@file@percent }
\newlabel{dfn:LPUNC:Lvunc_Grtnn}{{5.39}{45}{\Lvunc totally nonnegative Grassmannian}{definition.5.39}{}}
\@writefile{lla}{\contentsline {section}{\numberline {\crtrefnumber{dfn:LPUNC:Lvunc_Grtnn}}dfn:LPUNC:Lvunc_Grtnn}{45}{definition.5.39}\protected@file@percent }
\newlabel{dfn:LPUNC:Lvunc_Grtnn@cref}{{[definition][39][5]5.39}{[1][45][]45}{}{}{}}
\@writefile{loe}{\contentsline {question}{\ifthmt@listswap Question~5.40\else \numberline {5.40}Question\fi }{45}{question.5.40}\protected@file@percent }
\newlabel{que:LPUNC:GrtnnLvuncproj=GrtnnLvuncamb}{{5.40}{45}{}{question.5.40}{}}
\@writefile{lla}{\contentsline {section}{\numberline {\crtrefnumber{que:LPUNC:GrtnnLvuncproj=GrtnnLvuncamb}}que:LPUNC:GrtnnLvuncproj=GrtnnLvuncamb}{45}{question.5.40}\protected@file@percent }
\newlabel{que:LPUNC:GrtnnLvuncproj=GrtnnLvuncamb@cref}{{[question][40][5]5.40}{[1][45][]45}{}{}{}}
\newlabel{ssec:LPUNC:T_duality_graphs}{{5.5}{45}{T-duality for \Lpunc graphs}{subsection.5.5}{}}
\@writefile{lla}{\contentsline {section}{\numberline {\crtrefnumber{ssec:LPUNC:T_duality_graphs}}ssec:LPUNC:T_duality_graphs}{45}{subsection.5.5}\protected@file@percent }
\newlabel{ssec:LPUNC:T_duality_graphs@cref}{{[subsection][5][5]5.5}{[1][45][]45}{}{}{}}
\@writefile{toc}{\contentsline {subsection}{\tocsubsection {}{5.5}{T-duality for $L$-punctured\xspace  graphs}}{45}{subsection.5.5}\protected@file@percent }
\@writefile{loe}{\contentsline {corollary}{\ifthmt@listswap Corollary~5.41\else \numberline {5.41}Corollary\fi }{45}{corollary.5.41}\protected@file@percent }
\newlabel{lemma:ddGvunc_is_oneind}{{5.41}{45}{}{corollary.5.41}{}}
\@writefile{lla}{\contentsline {section}{\numberline {\crtrefnumber{lemma:ddGvunc_is_oneind}}lemma:ddGvunc_is_oneind}{45}{corollary.5.41}\protected@file@percent }
\newlabel{lemma:ddGvunc_is_oneind@cref}{{[corollary][41][5]5.41}{[1][45][]45}{}{}{}}
\@writefile{loe}{\contentsline {definition}{\ifthmt@listswap Definition~5.42\else \numberline {5.42}Definition\fi \thmtformatoptarg {T-dual $L$-punctured\xspace  graphs}}{45}{definition.5.42}\protected@file@percent }
\newlabel{dfn:LPUNC:T_dual_Lpunc_graphs}{{5.42}{45}{T-dual \Lpunc graphs}{definition.5.42}{}}
\@writefile{lla}{\contentsline {section}{\numberline {\crtrefnumber{dfn:LPUNC:T_dual_Lpunc_graphs}}dfn:LPUNC:T_dual_Lpunc_graphs}{45}{definition.5.42}\protected@file@percent }
\newlabel{dfn:LPUNC:T_dual_Lpunc_graphs@cref}{{[definition][42][5]5.42}{[1][45][]45}{}{}{}}
\@writefile{loe}{\contentsline {remark}{\ifthmt@listswap Remark~5.43\else \numberline {5.43}Remark\fi }{45}{remark.5.43}\protected@file@percent }
\newlabel{rmk:LPUNC:choices}{{5.43}{45}{}{remark.5.43}{}}
\@writefile{lla}{\contentsline {section}{\numberline {\crtrefnumber{rmk:LPUNC:choices}}rmk:LPUNC:choices}{45}{remark.5.43}\protected@file@percent }
\newlabel{rmk:LPUNC:choices@cref}{{[remark][43][5]5.43}{[1][45][]45}{}{}{}}
\newlabel{eq:LPUNC:ddCprest_dfn}{{5.25}{46}{T-duality for \Lpunc graphs}{equation.5.25}{}}
\@writefile{lla}{\contentsline {section}{\numberline {\crtrefnumber{eq:LPUNC:ddCprest_dfn}}eq:LPUNC:ddCprest_dfn}{46}{equation.5.25}\protected@file@percent }
\newlabel{eq:LPUNC:ddCprest_dfn@cref}{{[equation][25][5]5.25}{[1][46][]46}{}{}{}}
\newlabel{eq:dual_spinor}{{5.26}{46}{T-duality for \Lpunc graphs}{equation.5.26}{}}
\@writefile{lla}{\contentsline {section}{\numberline {\crtrefnumber{eq:dual_spinor}}eq:dual_spinor}{46}{equation.5.26}\protected@file@percent }
\newlabel{eq:dual_spinor@cref}{{[equation][26][5]5.26}{[1][46][]46}{}{}{}}
\@writefile{loe}{\contentsline {proposition}{\ifthmt@listswap Proposition~5.44\else \numberline {5.44}Proposition\fi \thmtformatoptarg {T-duality for $L$-punctured\xspace  boundary measurements}}{46}{proposition.5.44}\protected@file@percent }
\newlabel{lemma:LPUNC:T_duality_D_vs_H}{{5.44}{46}{T-duality for \Lpunc boundary measurements}{proposition.5.44}{}}
\@writefile{lla}{\contentsline {section}{\numberline {\crtrefnumber{lemma:LPUNC:T_duality_D_vs_H}}lemma:LPUNC:T_duality_D_vs_H}{46}{proposition.5.44}\protected@file@percent }
\newlabel{lemma:LPUNC:T_duality_D_vs_H@cref}{{[proposition][44][5]5.44}{[1][46][]46}{}{}{}}
\newlabel{eq:LPUNC:T_duality_D_vs_H}{{5.27}{46}{T-duality for \Lpunc boundary measurements}{equation.5.27}{}}
\@writefile{lla}{\contentsline {section}{\numberline {\crtrefnumber{eq:LPUNC:T_duality_D_vs_H}}eq:LPUNC:T_duality_D_vs_H}{46}{equation.5.27}\protected@file@percent }
\newlabel{eq:LPUNC:T_duality_D_vs_H@cref}{{[equation][27][5]5.27}{[1][46][]46}{}{}{}}
\@writefile{loe}{\contentsline {remark}{\ifthmt@listswap Remark~5.45\else \numberline {5.45}Remark\fi }{46}{remark.5.45}\protected@file@percent }
\newlabel{eq:LPUNC:munk_vs_H}{{5.28}{46}{T-duality for \Lpunc graphs}{equation.5.28}{}}
\@writefile{lla}{\contentsline {section}{\numberline {\crtrefnumber{eq:LPUNC:munk_vs_H}}eq:LPUNC:munk_vs_H}{46}{equation.5.28}\protected@file@percent }
\newlabel{eq:LPUNC:munk_vs_H@cref}{{[equation][28][5]5.28}{[1][46][]46}{}{}{}}
\newlabel{eq:ddCext_vs_munk}{{5.29}{46}{T-duality for \Lpunc graphs}{equation.5.29}{}}
\@writefile{lla}{\contentsline {section}{\numberline {\crtrefnumber{eq:ddCext_vs_munk}}eq:ddCext_vs_munk}{46}{equation.5.29}\protected@file@percent }
\newlabel{eq:ddCext_vs_munk@cref}{{[equation][29][5]5.29}{[1][46][]46}{}{}{}}
\newlabel{eq:Hdnk_Cramer}{{5.30}{46}{T-duality for \Lpunc graphs}{equation.5.30}{}}
\@writefile{lla}{\contentsline {section}{\numberline {\crtrefnumber{eq:Hdnk_Cramer}}eq:Hdnk_Cramer}{46}{equation.5.30}\protected@file@percent }
\newlabel{eq:Hdnk_Cramer@cref}{{[equation][30][5]5.30}{[1][46][]46}{}{}{}}
\newlabel{ssec:T_gen}{{5.6}{47}{T-duality for generalized \Lpunc graphs}{subsection.5.6}{}}
\@writefile{lla}{\contentsline {section}{\numberline {\crtrefnumber{ssec:T_gen}}ssec:T_gen}{47}{subsection.5.6}\protected@file@percent }
\newlabel{ssec:T_gen@cref}{{[subsection][6][5]5.6}{[1][47][]47}{}{}{}}
\@writefile{toc}{\contentsline {subsection}{\tocsubsection {}{5.6}{T-duality for generalized $L$-punctured\xspace  graphs}}{47}{thmt@dummyctr.dummy.157}\protected@file@percent }
\@writefile{loe}{\contentsline {definition}{\ifthmt@listswap Definition~5.46\else \numberline {5.46}Definition\fi }{47}{definition.5.46}\protected@file@percent }
\newlabel{dfn:gen_Lfunc_graph}{{5.46}{47}{}{definition.5.46}{}}
\@writefile{lla}{\contentsline {section}{\numberline {\crtrefnumber{dfn:gen_Lfunc_graph}}dfn:gen_Lfunc_graph}{47}{definition.5.46}\protected@file@percent }
\newlabel{dfn:gen_Lfunc_graph@cref}{{[definition][46][5]5.46}{[1][47][]47}{}{}{}}
\@writefile{loe}{\contentsline {definition}{\ifthmt@listswap Definition~5.47\else \numberline {5.47}Definition\fi }{47}{definition.5.47}\protected@file@percent }
\newlabel{dfn:fullysep_gen}{{5.47}{47}{}{definition.5.47}{}}
\@writefile{lla}{\contentsline {section}{\numberline {\crtrefnumber{dfn:fullysep_gen}}dfn:fullysep_gen}{47}{definition.5.47}\protected@file@percent }
\newlabel{dfn:fullysep_gen@cref}{{[definition][47][5]5.47}{[1][47][]47}{}{}{}}
\@writefile{loe}{\contentsline {definition}{\ifthmt@listswap Definition~5.48\else \numberline {5.48}Definition\fi }{47}{definition.5.48}\protected@file@percent }
\newlabel{dfn:weighted_gen_Lfunc}{{5.48}{47}{}{definition.5.48}{}}
\@writefile{lla}{\contentsline {section}{\numberline {\crtrefnumber{dfn:weighted_gen_Lfunc}}dfn:weighted_gen_Lfunc}{47}{definition.5.48}\protected@file@percent }
\newlabel{dfn:weighted_gen_Lfunc@cref}{{[definition][48][5]5.48}{[1][47][]47}{}{}{}}
\newlabel{eq:GENPUNC:H_convex}{{5.31}{47}{}{equation.5.31}{}}
\@writefile{lla}{\contentsline {section}{\numberline {\crtrefnumber{eq:GENPUNC:H_convex}}eq:GENPUNC:H_convex}{47}{equation.5.31}\protected@file@percent }
\newlabel{eq:GENPUNC:H_convex@cref}{{[equation][31][5]5.31}{[1][47][]47}{}{}{}}
\@writefile{loe}{\contentsline {remark}{\ifthmt@listswap Remark~5.49\else \numberline {5.49}Remark\fi }{48}{remark.5.49}\protected@file@percent }
\@writefile{loe}{\contentsline {definition}{\ifthmt@listswap Definition~5.50\else \numberline {5.50}Definition\fi \thmtformatoptarg {Generalized T-duality}}{48}{definition.5.50}\protected@file@percent }
\newlabel{dfn:generalized_T-duality}{{5.50}{48}{Generalized T-duality}{definition.5.50}{}}
\@writefile{lla}{\contentsline {section}{\numberline {\crtrefnumber{dfn:generalized_T-duality}}dfn:generalized_T-duality}{48}{definition.5.50}\protected@file@percent }
\newlabel{dfn:generalized_T-duality@cref}{{[definition][50][5]5.50}{[1][48][]48}{}{}{}}
\newlabel{eq:GENPUNC:Simplex_vs_Dimplex}{{5.32}{48}{Generalized T-duality}{equation.5.32}{}}
\@writefile{lla}{\contentsline {section}{\numberline {\crtrefnumber{eq:GENPUNC:Simplex_vs_Dimplex}}eq:GENPUNC:Simplex_vs_Dimplex}{48}{equation.5.32}\protected@file@percent }
\newlabel{eq:GENPUNC:Simplex_vs_Dimplex@cref}{{[equation][32][5]5.32}{[1][48][]48}{}{}{}}
\@writefile{loe}{\contentsline {remark}{\ifthmt@listswap Remark~5.51\else \numberline {5.51}Remark\fi }{48}{remark.5.51}\protected@file@percent }
\newlabel{rmk:oneind_gen}{{5.51}{48}{}{remark.5.51}{}}
\@writefile{lla}{\contentsline {section}{\numberline {\crtrefnumber{rmk:oneind_gen}}rmk:oneind_gen}{48}{remark.5.51}\protected@file@percent }
\newlabel{rmk:oneind_gen@cref}{{[remark][51][5]5.51}{[1][48][]48}{}{}{}}
\@writefile{loe}{\contentsline {example}{\ifthmt@listswap Example~5.52\else \numberline {5.52}Example\fi }{48}{example.5.52}\protected@file@percent }
\newlabel{ex:BCFW-T-dual}{{5.52}{48}{}{example.5.52}{}}
\@writefile{lla}{\contentsline {section}{\numberline {\crtrefnumber{ex:BCFW-T-dual}}ex:BCFW-T-dual}{48}{example.5.52}\protected@file@percent }
\newlabel{ex:BCFW-T-dual@cref}{{[example][52][5]5.52}{[1][48][]48}{}{}{}}
\@writefile{lof}{\contentsline {figure}{\numberline {13}{\ignorespaces  Applying generalized T-duality to the graph $\Gamma _{\!L^\ast }$ in \figref {fig:BCFW-full}(e).}}{49}{figure.caption.21}\protected@file@percent }
\newlabel{fig:BCFW-T-dual}{{13}{49}{Applying generalized T-duality to the graph $\Gfunc $ in \protect \figref {fig:BCFW-full}(e)}{figure.caption.21}{}}
\@writefile{lla}{\contentsline {section}{\numberline {\crtrefnumber{fig:BCFW-T-dual}}fig:BCFW-T-dual}{49}{figure.caption.21}\protected@file@percent }
\newlabel{fig:BCFW-T-dual@cref}{{[figure][13][]13}{[1][48][]49}{}{}{}}
\@writefile{loe}{\contentsline {remark}{\ifthmt@listswap Remark~5.53\else \numberline {5.53}Remark\fi \thmtformatoptarg {Inverse generalized T-duality}}{49}{remark.5.53}\protected@file@percent }
\newlabel{rmk:SHIFT:inverse_gen}{{5.53}{49}{Inverse generalized T-duality}{remark.5.53}{}}
\@writefile{lla}{\contentsline {section}{\numberline {\crtrefnumber{rmk:SHIFT:inverse_gen}}rmk:SHIFT:inverse_gen}{49}{remark.5.53}\protected@file@percent }
\newlabel{rmk:SHIFT:inverse_gen@cref}{{[remark][53][5]5.53}{[1][49][]49}{}{}{}}
\@writefile{loe}{\contentsline {proposition}{\ifthmt@listswap Proposition~5.54\else \numberline {5.54}Proposition\fi }{49}{proposition.5.54}\protected@file@percent }
\newlabel{lemma:GENPUNC:T_duality_D_vs_H}{{5.54}{49}{}{proposition.5.54}{}}
\@writefile{lla}{\contentsline {section}{\numberline {\crtrefnumber{lemma:GENPUNC:T_duality_D_vs_H}}lemma:GENPUNC:T_duality_D_vs_H}{49}{proposition.5.54}\protected@file@percent }
\newlabel{lemma:GENPUNC:T_duality_D_vs_H@cref}{{[proposition][54][5]5.54}{[1][49][]49}{}{}{}}
\newlabel{eq:laextloc_munkloc_dfn}{{5.33}{49}{T-duality for generalized \Lpunc graphs}{equation.5.33}{}}
\@writefile{lla}{\contentsline {section}{\numberline {\crtrefnumber{eq:laextloc_munkloc_dfn}}eq:laextloc_munkloc_dfn}{49}{equation.5.33}\protected@file@percent }
\newlabel{eq:laextloc_munkloc_dfn@cref}{{[equation][33][5]5.33}{[1][49][]49}{}{}{}}
\newlabel{eq:Hx_CMI_laext}{{5.34}{49}{T-duality for generalized \Lpunc graphs}{equation.5.34}{}}
\@writefile{lla}{\contentsline {section}{\numberline {\crtrefnumber{eq:Hx_CMI_laext}}eq:Hx_CMI_laext}{49}{equation.5.34}\protected@file@percent }
\newlabel{eq:Hx_CMI_laext@cref}{{[equation][34][5]5.34}{[1][49][]49}{}{}{}}
\newlabel{eq:GENPUNC:Hx_rho_i}{{5.35}{49}{T-duality for generalized \Lpunc graphs}{equation.5.35}{}}
\@writefile{lla}{\contentsline {section}{\numberline {\crtrefnumber{eq:GENPUNC:Hx_rho_i}}eq:GENPUNC:Hx_rho_i}{49}{equation.5.35}\protected@file@percent }
\newlabel{eq:GENPUNC:Hx_rho_i@cref}{{[equation][35][5]5.35}{[1][49][]49}{}{}{}}
\citation{origami1}
\citation{origami1}
\@writefile{toc}{\contentsline {section}{\tocsection {}{6}{T-duality for loop amplituhedra}}{50}{section.6}\protected@file@percent }
\newlabel{sec:LOOP}{{6}{50}{T-duality for loop amplituhedra}{section.6}{}}
\@writefile{lla}{\contentsline {section}{\numberline {\crtrefnumber{sec:LOOP}}sec:LOOP}{50}{section.6}\protected@file@percent }
\newlabel{sec:LOOP@cref}{{[section][6][]6}{[1][50][]50}{}{}{}}
\newlabel{ssec:LOOP:ambient_ampl_dfn}{{6.1}{50}{Ambient loop amplituhedra}{subsection.6.1}{}}
\@writefile{lla}{\contentsline {section}{\numberline {\crtrefnumber{ssec:LOOP:ambient_ampl_dfn}}ssec:LOOP:ambient_ampl_dfn}{50}{subsection.6.1}\protected@file@percent }
\newlabel{ssec:LOOP:ambient_ampl_dfn@cref}{{[subsection][1][6]6.1}{[1][50][]50}{}{}{}}
\@writefile{toc}{\contentsline {subsection}{\tocsubsection {}{6.1}{Ambient loop amplituhedra}}{50}{subsection.6.1}\protected@file@percent }
\@writefile{loe}{\contentsline {definition}{\ifthmt@listswap Definition~6.1\else \numberline {6.1}Definition\fi \thmtformatoptarg {Ambient loop momentum amplituhedron}}{50}{definition.6.1}\protected@file@percent }
\newlabel{dfn:LPUNC:amb_loop_ampl}{{6.1}{50}{Ambient loop momentum amplituhedron}{definition.6.1}{}}
\@writefile{lla}{\contentsline {section}{\numberline {\crtrefnumber{dfn:LPUNC:amb_loop_ampl}}dfn:LPUNC:amb_loop_ampl}{50}{definition.6.1}\protected@file@percent }
\newlabel{dfn:LPUNC:amb_loop_ampl@cref}{{[definition][1][6]6.1}{[1][50][]50}{}{}{}}
\newlabel{MPknL1}{{{{(a)}}}{50}{Ambient loop momentum amplituhedron}{Item.27}{}}
\@writefile{lla}{\contentsline {section}{\numberline {\crtrefnumber{MPknL1}}MPknL1}{50}{Item.27}\protected@file@percent }
\newlabel{MPknL1@cref}{{[enumi][1][]{{(a)}}}{[1][50][]50}{}{}{}}
\newlabel{MPknL2}{{{{(b)}}}{50}{Ambient loop momentum amplituhedron}{Item.28}{}}
\@writefile{lla}{\contentsline {section}{\numberline {\crtrefnumber{MPknL2}}MPknL2}{50}{Item.28}\protected@file@percent }
\newlabel{MPknL2@cref}{{[enumi][2][]{{(b)}}}{[1][50][]50}{}{}{}}
\newlabel{MPknL4}{{{{(c)}}}{50}{Ambient loop momentum amplituhedron}{Item.29}{}}
\@writefile{lla}{\contentsline {section}{\numberline {\crtrefnumber{MPknL4}}MPknL4}{50}{Item.29}\protected@file@percent }
\newlabel{MPknL4@cref}{{[enumi][3][]{{(c)}}}{[1][50][]50}{}{}{}}
\@writefile{loe}{\contentsline {remark}{\ifthmt@listswap Remark~6.2\else \numberline {6.2}Remark\fi }{50}{remark.6.2}\protected@file@percent }
\newlabel{rmk:GGsh_action_preserves_MPknL}{{6.2}{50}{}{remark.6.2}{}}
\@writefile{lla}{\contentsline {section}{\numberline {\crtrefnumber{rmk:GGsh_action_preserves_MPknL}}rmk:GGsh_action_preserves_MPknL}{50}{remark.6.2}\protected@file@percent }
\newlabel{rmk:GGsh_action_preserves_MPknL@cref}{{[remark][2][6]6.2}{[1][50][]50}{}{}{}}
\@writefile{loe}{\contentsline {definition}{\ifthmt@listswap Definition~6.3\else \numberline {6.3}Definition\fi }{50}{definition.6.3}\protected@file@percent }
\newlabel{eq:LPUNC:MPG_dfn}{{6.1}{50}{}{equation.6.1}{}}
\@writefile{lla}{\contentsline {section}{\numberline {\crtrefnumber{eq:LPUNC:MPG_dfn}}eq:LPUNC:MPG_dfn}{50}{equation.6.1}\protected@file@percent }
\newlabel{eq:LPUNC:MPG_dfn@cref}{{[equation][1][6]6.1}{[1][50][]50}{}{}{}}
\@writefile{loe}{\contentsline {definition}{\ifthmt@listswap Definition~6.4\else \numberline {6.4}Definition\fi }{50}{definition.6.4}\protected@file@percent }
\newlabel{eq:TREE:wind_vs_varx}{{6.2}{50}{Ambient loop amplituhedra}{equation.6.2}{}}
\@writefile{lla}{\contentsline {section}{\numberline {\crtrefnumber{eq:TREE:wind_vs_varx}}eq:TREE:wind_vs_varx}{50}{equation.6.2}\protected@file@percent }
\newlabel{eq:TREE:wind_vs_varx@cref}{{[equation][2][6]6.2}{[1][50][]50}{}{}{}}
\citation{origami1}
\@writefile{loe}{\contentsline {definition}{\ifthmt@listswap Definition~6.5\else \numberline {6.5}Definition\fi }{51}{definition.6.5}\protected@file@percent }
\newlabel{dfn:TREE:AAkn}{{6.5}{51}{}{definition.6.5}{}}
\@writefile{lla}{\contentsline {section}{\numberline {\crtrefnumber{dfn:TREE:AAkn}}dfn:TREE:AAkn}{51}{definition.6.5}\protected@file@percent }
\newlabel{dfn:TREE:AAkn@cref}{{[definition][5][6]6.5}{[1][51][]51}{}{}{}}
\newlabel{eq:TREE:AAkn_dfn}{{6.3}{51}{}{equation.6.3}{}}
\@writefile{lla}{\contentsline {section}{\numberline {\crtrefnumber{eq:TREE:AAkn_dfn}}eq:TREE:AAkn_dfn}{51}{equation.6.3}\protected@file@percent }
\newlabel{eq:TREE:AAkn_dfn@cref}{{[equation][3][6]6.3}{[1][51][]51}{}{}{}}
\@writefile{loe}{\contentsline {definition}{\ifthmt@listswap Definition~6.6\else \numberline {6.6}Definition\fi }{51}{definition.6.6}\protected@file@percent }
\newlabel{eq:varVL_dfn}{{6.4}{51}{Ambient loop amplituhedra}{equation.6.4}{}}
\@writefile{lla}{\contentsline {section}{\numberline {\crtrefnumber{eq:varVL_dfn}}eq:varVL_dfn}{51}{equation.6.4}\protected@file@percent }
\newlabel{eq:varVL_dfn@cref}{{[equation][4][6]6.4}{[1][51][]51}{}{}{}}
\@writefile{loe}{\contentsline {definition}{\ifthmt@listswap Definition~6.7\else \numberline {6.7}Definition\fi \thmtformatoptarg {Ambient loop momentum-twistor\xspace  amplituhedron\xspace  }}{51}{definition.6.7}\protected@file@percent }
\newlabel{dfn:LSH:AAknL}{{6.7}{51}{Ambient loop \mta }{definition.6.7}{}}
\@writefile{lla}{\contentsline {section}{\numberline {\crtrefnumber{dfn:LSH:AAknL}}dfn:LSH:AAknL}{51}{definition.6.7}\protected@file@percent }
\newlabel{dfn:LSH:AAknL@cref}{{[definition][7][6]6.7}{[1][51][]51}{}{}{}}
\newlabel{AAknL1}{{{{(\"{a})}}}{51}{Ambient loop \mta }{Item.30}{}}
\@writefile{lla}{\contentsline {section}{\numberline {\crtrefnumber{AAknL1}}AAknL1}{51}{Item.30}\protected@file@percent }
\newlabel{AAknL1@cref}{{[enumi][1][]{{(\"{a})}}}{[1][51][]51}{}{}{}}
\newlabel{AAknL2}{{{{(\"{b})}}}{51}{Ambient loop \mta }{Item.31}{}}
\@writefile{lla}{\contentsline {section}{\numberline {\crtrefnumber{AAknL2}}AAknL2}{51}{Item.31}\protected@file@percent }
\newlabel{AAknL2@cref}{{[enumi][2][]{{(\"{b})}}}{[1][51][]51}{}{}{}}
\newlabel{AAknL4}{{{{(\"{c})}}}{51}{Ambient loop \mta }{Item.32}{}}
\@writefile{lla}{\contentsline {section}{\numberline {\crtrefnumber{AAknL4}}AAknL4}{51}{Item.32}\protected@file@percent }
\newlabel{AAknL4@cref}{{[enumi][3][]{{(\"{c})}}}{[1][51][]51}{}{}{}}
\@writefile{loe}{\contentsline {definition}{\ifthmt@listswap Definition~6.8\else \numberline {6.8}Definition\fi }{51}{definition.6.8}\protected@file@percent }
\newlabel{dfn:LSHIFT:AAddG}{{6.8}{51}{}{definition.6.8}{}}
\@writefile{lla}{\contentsline {section}{\numberline {\crtrefnumber{dfn:LSHIFT:AAddG}}dfn:LSHIFT:AAddG}{51}{definition.6.8}\protected@file@percent }
\newlabel{dfn:LSHIFT:AAddG@cref}{{[definition][8][6]6.8}{[1][51][]51}{}{}{}}
\newlabel{eq:LPUNC:AAddG_dfn}{{6.5}{51}{}{equation.6.5}{}}
\@writefile{lla}{\contentsline {section}{\numberline {\crtrefnumber{eq:LPUNC:AAddG_dfn}}eq:LPUNC:AAddG_dfn}{51}{equation.6.5}\protected@file@percent }
\newlabel{eq:LPUNC:AAddG_dfn@cref}{{[equation][5][6]6.5}{[1][51][]51}{}{}{}}
\@writefile{loe}{\contentsline {remark}{\ifthmt@listswap Remark~6.9\else \numberline {6.9}Remark\fi }{51}{remark.6.9}\protected@file@percent }
\newlabel{rmk:LSHIFT:D_perp_cap_V}{{6.9}{51}{}{remark.6.9}{}}
\@writefile{lla}{\contentsline {section}{\numberline {\crtrefnumber{rmk:LSHIFT:D_perp_cap_V}}rmk:LSHIFT:D_perp_cap_V}{51}{remark.6.9}\protected@file@percent }
\newlabel{rmk:LSHIFT:D_perp_cap_V@cref}{{[remark][9][6]6.9}{[1][51][]51}{}{}{}}
\newlabel{eq:LSHIFT:MAknL_dfn}{{6.6}{51}{Ambient loop amplituhedra}{equation.6.6}{}}
\@writefile{lla}{\contentsline {section}{\numberline {\crtrefnumber{eq:LSHIFT:MAknL_dfn}}eq:LSHIFT:MAknL_dfn}{51}{equation.6.6}\protected@file@percent }
\newlabel{eq:LSHIFT:MAknL_dfn@cref}{{[equation][6][6]6.6}{[1][51][]51}{}{}{}}
\newlabel{eq:LSHIFT:MAddG_dfn}{{6.7}{51}{Ambient loop amplituhedra}{equation.6.7}{}}
\@writefile{lla}{\contentsline {section}{\numberline {\crtrefnumber{eq:LSHIFT:MAddG_dfn}}eq:LSHIFT:MAddG_dfn}{51}{equation.6.7}\protected@file@percent }
\newlabel{eq:LSHIFT:MAddG_dfn@cref}{{[equation][7][6]6.7}{[1][51][]51}{}{}{}}
\newlabel{ssec:LOOP:ambient_ampl_T_dual}{{6.2}{51}{T-duality for ambient loop amplituhedra}{subsection.6.2}{}}
\@writefile{lla}{\contentsline {section}{\numberline {\crtrefnumber{ssec:LOOP:ambient_ampl_T_dual}}ssec:LOOP:ambient_ampl_T_dual}{51}{subsection.6.2}\protected@file@percent }
\newlabel{ssec:LOOP:ambient_ampl_T_dual@cref}{{[subsection][2][6]6.2}{[1][51][]51}{}{}{}}
\@writefile{toc}{\contentsline {subsection}{\tocsubsection {}{6.2}{T-duality for ambient loop amplituhedra}}{51}{subsection.6.2}\protected@file@percent }
\@writefile{loe}{\contentsline {lemma}{\ifthmt@listswap Lemma~6.10\else \numberline {6.10}Lemma\fi }{51}{lemma.6.10}\protected@file@percent }
\newlabel{eq:mu_vs_bdxM_vs_Qlapp}{{6.8}{51}{}{equation.6.8}{}}
\@writefile{lla}{\contentsline {section}{\numberline {\crtrefnumber{eq:mu_vs_bdxM_vs_Qlapp}}eq:mu_vs_bdxM_vs_Qlapp}{51}{equation.6.8}\protected@file@percent }
\newlabel{eq:mu_vs_bdxM_vs_Qlapp@cref}{{[equation][8][6]6.8}{[1][51][]51}{}{}{}}
\citation{origami1}
\newlabel{eq:AAshift_dfn}{{6.9}{52}{T-duality for ambient loop amplituhedra}{equation.6.9}{}}
\@writefile{lla}{\contentsline {section}{\numberline {\crtrefnumber{eq:AAshift_dfn}}eq:AAshift_dfn}{52}{equation.6.9}\protected@file@percent }
\newlabel{eq:AAshift_dfn@cref}{{[equation][9][6]6.9}{[1][52][]52}{}{}{}}
\newlabel{eq:AAiso_dfn}{{6.10}{52}{T-duality for ambient loop amplituhedra}{equation.6.10}{}}
\@writefile{lla}{\contentsline {section}{\numberline {\crtrefnumber{eq:AAiso_dfn}}eq:AAiso_dfn}{52}{equation.6.10}\protected@file@percent }
\newlabel{eq:AAiso_dfn@cref}{{[equation][10][6]6.10}{[1][52][]52}{}{}{}}
\@writefile{loe}{\contentsline {theorem}{\ifthmt@listswap Theorem~6.11\else \numberline {6.11}Theorem\fi \thmtformatoptarg {T-duality for ambient loop amplituhedra}}{52}{theorem.6.11}\protected@file@percent }
\newlabel{thm:AAshift}{{6.11}{52}{T-duality for ambient loop amplituhedra}{theorem.6.11}{}}
\@writefile{lla}{\contentsline {section}{\numberline {\crtrefnumber{thm:AAshift}}thm:AAshift}{52}{theorem.6.11}\protected@file@percent }
\newlabel{thm:AAshift@cref}{{[theorem][11][6]6.11}{[1][52][]52}{}{}{}}
\newlabel{AAshift_iso}{{{{(1)}}}{52}{T-duality for ambient loop amplituhedra}{Item.33}{}}
\@writefile{lla}{\contentsline {section}{\numberline {\crtrefnumber{AAshift_iso}}AAshift_iso}{52}{Item.33}\protected@file@percent }
\newlabel{AAshift_iso@cref}{{[enumi][1][]{{(1)}}}{[1][52][]52}{}{}{}}
\newlabel{AAshift_forg}{{{{(2)}}}{52}{T-duality for ambient loop amplituhedra}{Item.34}{}}
\@writefile{lla}{\contentsline {section}{\numberline {\crtrefnumber{AAshift_forg}}AAshift_forg}{52}{Item.34}\protected@file@percent }
\newlabel{AAshift_forg@cref}{{[enumi][2][]{{(2)}}}{[1][52][]52}{}{}{}}
\@writefile{loe}{\contentsline {theorem}{\ifthmt@listswap Theorem~6.12\else \numberline {6.12}Theorem\fi \thmtformatoptarg {\cite  [\cref  *{M-thm:AAshift}]{origami1}\xspace  }}{52}{theorem.6.12}\protected@file@percent }
\newlabel{thm:AAshift_tree}{{6.12}{52}{\Mref {thm:AAshift}}{theorem.6.12}{}}
\@writefile{lla}{\contentsline {section}{\numberline {\crtrefnumber{thm:AAshift_tree}}thm:AAshift_tree}{52}{theorem.6.12}\protected@file@percent }
\newlabel{thm:AAshift_tree@cref}{{[theorem][12][6]6.12}{[1][52][]52}{}{}{}}
\@writefile{loe}{\contentsline {definition}{\ifthmt@listswap Definition~6.13\else \numberline {6.13}Definition\fi \thmtformatoptarg {Normal form}}{52}{definition.6.13}\protected@file@percent }
\newlabel{dfn:LSHIFT:normal_form}{{6.13}{52}{Normal form}{definition.6.13}{}}
\@writefile{lla}{\contentsline {section}{\numberline {\crtrefnumber{dfn:LSHIFT:normal_form}}dfn:LSHIFT:normal_form}{52}{definition.6.13}\protected@file@percent }
\newlabel{dfn:LSHIFT:normal_form@cref}{{[definition][13][6]6.13}{[1][52][]52}{}{}{}}
\@writefile{loe}{\contentsline {lemma}{\ifthmt@listswap Lemma~6.14\else \numberline {6.14}Lemma\fi }{52}{lemma.6.14}\protected@file@percent }
\newlabel{lemma:LSHIFT:VLpunc_normal_form}{{6.14}{52}{}{lemma.6.14}{}}
\@writefile{lla}{\contentsline {section}{\numberline {\crtrefnumber{lemma:LSHIFT:VLpunc_normal_form}}lemma:LSHIFT:VLpunc_normal_form}{52}{lemma.6.14}\protected@file@percent }
\newlabel{lemma:LSHIFT:VLpunc_normal_form@cref}{{[lemma][14][6]6.14}{[1][52][]52}{}{}{}}
\citation{origami1}
\citation{origami1}
\citation{origami1}
\citation{origami1}
\newlabel{eq:LOOP:br=xdiff_combined}{{6.11}{53}{T-duality for ambient loop amplituhedra}{equation.6.11}{}}
\@writefile{lla}{\contentsline {section}{\numberline {\crtrefnumber{eq:LOOP:br=xdiff_combined}}eq:LOOP:br=xdiff_combined}{53}{equation.6.11}\protected@file@percent }
\newlabel{eq:LOOP:br=xdiff_combined@cref}{{[equation][11][6]6.11}{[1][53][]53}{}{}{}}
\citation{origami1}
\citation{origami1}
\newlabel{eq:LPUNC:V_cap_Drho=pLr*V}{{6.12}{54}{T-duality for ambient loop amplituhedra}{equation.6.12}{}}
\@writefile{lla}{\contentsline {section}{\numberline {\crtrefnumber{eq:LPUNC:V_cap_Drho=pLr*V}}eq:LPUNC:V_cap_Drho=pLr*V}{54}{equation.6.12}\protected@file@percent }
\newlabel{eq:LPUNC:V_cap_Drho=pLr*V@cref}{{[equation][12][6]6.12}{[1][54][]54}{}{}{}}
\@writefile{toc}{\contentsline {subsection}{\tocsubsection {}{6.3}{Fully $2$-separated\xspace  and fully $2$-independent\xspace  graphs}}{54}{subsection.6.3}\protected@file@percent }
\@writefile{loe}{\contentsline {proposition}{\ifthmt@listswap Proposition~6.15\else \numberline {6.15}Proposition\fi }{54}{proposition.6.15}\protected@file@percent }
\newlabel{lemma:LPUNC:twosep_vs_twoind}{{6.15}{54}{}{proposition.6.15}{}}
\@writefile{lla}{\contentsline {section}{\numberline {\crtrefnumber{lemma:LPUNC:twosep_vs_twoind}}lemma:LPUNC:twosep_vs_twoind}{54}{proposition.6.15}\protected@file@percent }
\newlabel{lemma:LPUNC:twosep_vs_twoind@cref}{{[proposition][15][6]6.15}{[1][54][]54}{}{}{}}
\@writefile{loe}{\contentsline {proposition}{\ifthmt@listswap Proposition~6.16\else \numberline {6.16}Proposition\fi \thmtformatoptarg {\cite  [\cref  *{M-lemma:PROP:Mpos}]{origami1}\xspace  }}{54}{proposition.6.16}\protected@file@percent }
\newlabel{lemma:PROP:Mpos}{{6.16}{54}{\Mref {lemma:PROP:Mpos}}{proposition.6.16}{}}
\@writefile{lla}{\contentsline {section}{\numberline {\crtrefnumber{lemma:PROP:Mpos}}lemma:PROP:Mpos}{54}{proposition.6.16}\protected@file@percent }
\newlabel{lemma:PROP:Mpos@cref}{{[proposition][16][6]6.16}{[1][54][]54}{}{}{}}
\@writefile{loe}{\contentsline {remark}{\ifthmt@listswap Remark~6.17\else \numberline {6.17}Remark\fi }{54}{remark.6.17}\protected@file@percent }
\newlabel{rmk:TE:Mpos_existence}{{6.17}{54}{}{remark.6.17}{}}
\@writefile{lla}{\contentsline {section}{\numberline {\crtrefnumber{rmk:TE:Mpos_existence}}rmk:TE:Mpos_existence}{54}{remark.6.17}\protected@file@percent }
\newlabel{rmk:TE:Mpos_existence@cref}{{[remark][17][6]6.17}{[1][54][]54}{}{}{}}
\citation{origami1}
\newlabel{eq:TE:twosep_vs_rk_Hdnk}{{6.13}{55}{\Fullysep and \twoind graphs}{equation.6.13}{}}
\@writefile{lla}{\contentsline {section}{\numberline {\crtrefnumber{eq:TE:twosep_vs_rk_Hdnk}}eq:TE:twosep_vs_rk_Hdnk}{55}{equation.6.13}\protected@file@percent }
\newlabel{eq:TE:twosep_vs_rk_Hdnk@cref}{{[equation][13][6]6.13}{[1][55][]55}{}{}{}}
\@writefile{loe}{\contentsline {corollary}{\ifthmt@listswap Corollary~6.18\else \numberline {6.18}Corollary\fi }{55}{corollary.6.18}\protected@file@percent }
\newlabel{lemma:PROP:if_not_twosep_then_M=0}{{6.18}{55}{}{corollary.6.18}{}}
\@writefile{lla}{\contentsline {section}{\numberline {\crtrefnumber{lemma:PROP:if_not_twosep_then_M=0}}lemma:PROP:if_not_twosep_then_M=0}{55}{corollary.6.18}\protected@file@percent }
\newlabel{lemma:PROP:if_not_twosep_then_M=0@cref}{{[corollary][18][6]6.18}{[1][55][]55}{}{}{}}
\newlabel{ssec:T_duality_loop_tilings}{{6.4}{55}{T-duality for loop amplituhedron tilings}{subsection.6.4}{}}
\@writefile{lla}{\contentsline {section}{\numberline {\crtrefnumber{ssec:T_duality_loop_tilings}}ssec:T_duality_loop_tilings}{55}{subsection.6.4}\protected@file@percent }
\newlabel{ssec:T_duality_loop_tilings@cref}{{[subsection][4][6]6.4}{[1][55][]55}{}{}{}}
\@writefile{toc}{\contentsline {subsection}{\tocsubsection {}{6.4}{T-duality for loop amplituhedron tilings}}{55}{subsection.6.4}\protected@file@percent }
\@writefile{loe}{\contentsline {definition}{\ifthmt@listswap Definition~6.19\else \numberline {6.19}Definition\fi \thmtformatoptarg {$\mathcal  {R}$-tiling\xspace  }}{55}{definition.6.19}\protected@file@percent }
\newlabel{dfn:BCFW:tiling_amb}{{6.19}{55}{\Mtiling }{definition.6.19}{}}
\@writefile{lla}{\contentsline {section}{\numberline {\crtrefnumber{dfn:BCFW:tiling_amb}}dfn:BCFW:tiling_amb}{55}{definition.6.19}\protected@file@percent }
\newlabel{dfn:BCFW:tiling_amb@cref}{{[definition][19][6]6.19}{[1][55][]55}{}{}{}}
\newlabel{eq:BCFW:tile_amb_dfn}{{6.14}{55}{\Mtiling }{equation.6.14}{}}
\@writefile{lla}{\contentsline {section}{\numberline {\crtrefnumber{eq:BCFW:tile_amb_dfn}}eq:BCFW:tile_amb_dfn}{55}{equation.6.14}\protected@file@percent }
\newlabel{eq:BCFW:tile_amb_dfn@cref}{{[equation][14][6]6.14}{[1][55][]55}{}{}{}}
\citation{origami1}
\citation{origami1}
\newlabel{Rtiling1}{{{{(a)}}}{56}{\Mtiling }{Item.35}{}}
\@writefile{lla}{\contentsline {section}{\numberline {\crtrefnumber{Rtiling1}}Rtiling1}{56}{Item.35}\protected@file@percent }
\newlabel{Rtiling1@cref}{{[enumi][1][]{{(a)}}}{[1][56][]56}{}{}{}}
\newlabel{Rtiling2}{{{{(b)}}}{56}{\Mtiling }{Item.36}{}}
\@writefile{lla}{\contentsline {section}{\numberline {\crtrefnumber{Rtiling2}}Rtiling2}{56}{Item.36}\protected@file@percent }
\newlabel{Rtiling2@cref}{{[enumi][2][]{{(b)}}}{[1][56][]56}{}{}{}}
\newlabel{Rtiling3}{{{{(c)}}}{56}{\Mtiling }{Item.37}{}}
\@writefile{lla}{\contentsline {section}{\numberline {\crtrefnumber{Rtiling3}}Rtiling3}{56}{Item.37}\protected@file@percent }
\newlabel{Rtiling3@cref}{{[enumi][3][]{{(c)}}}{[1][56][]56}{}{}{}}
\@writefile{loe}{\contentsline {proposition}{\ifthmt@listswap Proposition~6.20\else \numberline {6.20}Proposition\fi \thmtformatoptarg {$\setbox \z@ \hbox {\mathsurround \z@ $\textstyle \mathcal  {R}$}\mathaccent "0362{\mathcal  {R}}$-tiling\xspace  }}{56}{proposition.6.20}\protected@file@percent }
\newlabel{lemma:tMtiling}{{6.20}{56}{\tMtiling }{proposition.6.20}{}}
\@writefile{lla}{\contentsline {section}{\numberline {\crtrefnumber{lemma:tMtiling}}lemma:tMtiling}{56}{proposition.6.20}\protected@file@percent }
\newlabel{lemma:tMtiling@cref}{{[proposition][20][6]6.20}{[1][56][]56}{}{}{}}
\newlabel{eq:tRel_dfn}{{6.15}{56}{\tMtiling }{equation.6.15}{}}
\@writefile{lla}{\contentsline {section}{\numberline {\crtrefnumber{eq:tRel_dfn}}eq:tRel_dfn}{56}{equation.6.15}\protected@file@percent }
\newlabel{eq:tRel_dfn@cref}{{[equation][15][6]6.15}{[1][56][]56}{}{}{}}
\@writefile{loe}{\contentsline {proposition}{\ifthmt@listswap Proposition~6.21\else \numberline {6.21}Proposition\fi \thmtformatoptarg {\cite  [\cref  *{M-lemma:RX_triple}]{origami1}\xspace  }}{56}{proposition.6.21}\protected@file@percent }
\newlabel{lemma:RX_triple}{{6.21}{56}{\Mref {lemma:RX_triple}}{proposition.6.21}{}}
\@writefile{lla}{\contentsline {section}{\numberline {\crtrefnumber{lemma:RX_triple}}lemma:RX_triple}{56}{proposition.6.21}\protected@file@percent }
\newlabel{lemma:RX_triple@cref}{{[proposition][21][6]6.21}{[1][56][]56}{}{}{}}
\newlabel{eq:TREE:comm_diag}{{6.16}{56}{\Mref {lemma:RX_triple}}{equation.6.16}{}}
\@writefile{lla}{\contentsline {section}{\numberline {\crtrefnumber{eq:TREE:comm_diag}}eq:TREE:comm_diag}{56}{equation.6.16}\protected@file@percent }
\newlabel{eq:TREE:comm_diag@cref}{{[equation][16][6]6.16}{[1][56][]56}{}{}{}}
\newlabel{eq:RtilingS}{{6.17}{56}{\Mref {lemma:RX_triple}}{equation.6.17}{}}
\@writefile{lla}{\contentsline {section}{\numberline {\crtrefnumber{eq:RtilingS}}eq:RtilingS}{56}{equation.6.17}\protected@file@percent }
\newlabel{eq:RtilingS@cref}{{[equation][17][6]6.17}{[1][56][]56}{}{}{}}
\@writefile{loe}{\contentsline {definition}{\ifthmt@listswap Definition~6.22\else \numberline {6.22}Definition\fi }{56}{definition.6.22}\protected@file@percent }
\newlabel{dfn:RX_triple}{{6.22}{56}{}{definition.6.22}{}}
\@writefile{lla}{\contentsline {section}{\numberline {\crtrefnumber{dfn:RX_triple}}dfn:RX_triple}{56}{definition.6.22}\protected@file@percent }
\newlabel{dfn:RX_triple@cref}{{[definition][22][6]6.22}{[1][56][]56}{}{}{}}
\newlabel{eq:LOOP:Rel_dfn}{{6.18}{56}{}{equation.6.18}{}}
\@writefile{lla}{\contentsline {section}{\numberline {\crtrefnumber{eq:LOOP:Rel_dfn}}eq:LOOP:Rel_dfn}{56}{equation.6.18}\protected@file@percent }
\newlabel{eq:LOOP:Rel_dfn@cref}{{[equation][18][6]6.18}{[1][56][]56}{}{}{}}
\newlabel{eq:TREE:ddRel_dfn}{{6.19}{56}{}{equation.6.19}{}}
\@writefile{lla}{\contentsline {section}{\numberline {\crtrefnumber{eq:TREE:ddRel_dfn}}eq:TREE:ddRel_dfn}{56}{equation.6.19}\protected@file@percent }
\newlabel{eq:TREE:ddRel_dfn@cref}{{[equation][19][6]6.19}{[1][56][]56}{}{}{}}
\citation{origami1}
\@writefile{loe}{\contentsline {corollary}{\ifthmt@listswap Corollary~6.23\else \numberline {6.23}Corollary\fi \thmtformatoptarg {T-duality for $\setbox \z@ \hbox {\mathsurround \z@ $\textstyle \mathcal  {R}$}\mathaccent "0362{\mathcal  {R}}$-tilings\xspace  of ambient loop amplituhedra}}{57}{corollary.6.23}\protected@file@percent }
\newlabel{lemma:TREE:amb_tiling_equivalence}{{6.23}{57}{T-duality for \tmtilings of ambient loop amplituhedra}{corollary.6.23}{}}
\@writefile{lla}{\contentsline {section}{\numberline {\crtrefnumber{lemma:TREE:amb_tiling_equivalence}}lemma:TREE:amb_tiling_equivalence}{57}{corollary.6.23}\protected@file@percent }
\newlabel{lemma:TREE:amb_tiling_equivalence@cref}{{[corollary][23][6]6.23}{[1][57][]57}{}{}{}}
\@writefile{loe}{\contentsline {definition}{\ifthmt@listswap Definition~6.24\else \numberline {6.24}Definition\fi \thmtformatoptarg {Tiling}}{57}{definition.6.24}\protected@file@percent }
\newlabel{dfn:BCFW:tiling}{{6.24}{57}{Tiling}{definition.6.24}{}}
\@writefile{lla}{\contentsline {section}{\numberline {\crtrefnumber{dfn:BCFW:tiling}}dfn:BCFW:tiling}{57}{definition.6.24}\protected@file@percent }
\newlabel{dfn:BCFW:tiling@cref}{{[definition][24][6]6.24}{[1][57][]57}{}{}{}}
\newlabel{tiling1}{{{{(a)}}}{57}{Tiling}{Item.38}{}}
\@writefile{lla}{\contentsline {section}{\numberline {\crtrefnumber{tiling1}}tiling1}{57}{Item.38}\protected@file@percent }
\newlabel{tiling1@cref}{{[enumi][1][]{{(a)}}}{[1][57][]57}{}{}{}}
\newlabel{tiling2}{{{{(b)}}}{57}{Tiling}{Item.39}{}}
\@writefile{lla}{\contentsline {section}{\numberline {\crtrefnumber{tiling2}}tiling2}{57}{Item.39}\protected@file@percent }
\newlabel{tiling2@cref}{{[enumi][2][]{{(b)}}}{[1][57][]57}{}{}{}}
\newlabel{tiling3}{{{{(c)}}}{57}{Tiling}{Item.40}{}}
\@writefile{lla}{\contentsline {section}{\numberline {\crtrefnumber{tiling3}}tiling3}{57}{Item.40}\protected@file@percent }
\newlabel{tiling3@cref}{{[enumi][3][]{{(c)}}}{[1][57][]57}{}{}{}}
\@writefile{loe}{\contentsline {proposition}{\ifthmt@listswap Proposition~6.25\else \numberline {6.25}Proposition\fi \thmtformatoptarg {\cite  [\cref  *{M-lemma:Rtiling_to_tiling}]{origami1}\xspace  }}{57}{proposition.6.25}\protected@file@percent }
\newlabel{lemma:Rtiling_to_tiling}{{6.25}{57}{\Mref {lemma:Rtiling_to_tiling}}{proposition.6.25}{}}
\@writefile{lla}{\contentsline {section}{\numberline {\crtrefnumber{lemma:Rtiling_to_tiling}}lemma:Rtiling_to_tiling}{57}{proposition.6.25}\protected@file@percent }
\newlabel{lemma:Rtiling_to_tiling@cref}{{[proposition][25][6]6.25}{[1][57][]57}{}{}{}}
\newlabel{eq:RGraph}{{6.20}{57}{\Mref {lemma:Rtiling_to_tiling}}{equation.6.20}{}}
\@writefile{lla}{\contentsline {section}{\numberline {\crtrefnumber{eq:RGraph}}eq:RGraph}{57}{equation.6.20}\protected@file@percent }
\newlabel{eq:RGraph@cref}{{[equation][20][6]6.20}{[1][57][]57}{}{}{}}
\@writefile{toc}{\contentsline {part}{\tocpart {Part}{2}{Origami reconstruction algorithm\xspace  }}{57}{part.2}\protected@file@percent }
\newlabel{part2}{{2}{57}{\ORATITLE }{part.2}{}}
\@writefile{lla}{\contentsline {section}{\numberline {\crtrefnumber{part2}}part2}{57}{part.2}\protected@file@percent }
\newlabel{part2@cref}{{[part][2][]2}{[1][57][]57}{}{}{}}
\@writefile{toc}{\contentsline {section}{\tocsection {}{7}{Mandelstam-nonnegative embeddings\xspace  }}{57}{section.7}\protected@file@percent }
\newlabel{sec:MNE}{{7}{57}{\MNEsTITLE }{section.7}{}}
\@writefile{lla}{\contentsline {section}{\numberline {\crtrefnumber{sec:MNE}}sec:MNE}{57}{section.7}\protected@file@percent }
\newlabel{sec:MNE@cref}{{[section][7][]7}{[1][57][]57}{}{}{}}
\newlabel{ssec:MCE:cliques}{{7.1}{58}{Cliques in \Mdash nonnegative point configurations}{subsection.7.1}{}}
\@writefile{lla}{\contentsline {section}{\numberline {\crtrefnumber{ssec:MCE:cliques}}ssec:MCE:cliques}{58}{subsection.7.1}\protected@file@percent }
\newlabel{ssec:MCE:cliques@cref}{{[subsection][1][7]7.1}{[1][57][]58}{}{}{}}
\@writefile{toc}{\contentsline {subsection}{\tocsubsection {}{7.1}{Cliques in M-nonnegative point configurations}}{58}{subsection.7.1}\protected@file@percent }
\@writefile{loe}{\contentsline {definition}{\ifthmt@listswap Definition~7.1\else \numberline {7.1}Definition\fi }{58}{definition.7.1}\protected@file@percent }
\newlabel{eq:MCE:NullG_dfn}{{7.1}{58}{Cliques in \Mdash nonnegative point configurations}{equation.7.1}{}}
\@writefile{lla}{\contentsline {section}{\numberline {\crtrefnumber{eq:MCE:NullG_dfn}}eq:MCE:NullG_dfn}{58}{equation.7.1}\protected@file@percent }
\newlabel{eq:MCE:NullG_dfn@cref}{{[equation][1][7]7.1}{[1][58][]58}{}{}{}}
\@writefile{loe}{\contentsline {definition}{\ifthmt@listswap Definition~7.2\else \numberline {7.2}Definition\fi }{58}{definition.7.2}\protected@file@percent }
\newlabel{dfn:MCE:white_black_deg}{{7.2}{58}{}{definition.7.2}{}}
\@writefile{lla}{\contentsline {section}{\numberline {\crtrefnumber{dfn:MCE:white_black_deg}}dfn:MCE:white_black_deg}{58}{definition.7.2}\protected@file@percent }
\newlabel{dfn:MCE:white_black_deg@cref}{{[definition][2][7]7.2}{[1][58][]58}{}{}{}}
\@writefile{loe}{\contentsline {definition}{\ifthmt@listswap Definition~7.3\else \numberline {7.3}Definition\fi }{58}{definition.7.3}\protected@file@percent }
\newlabel{dfn:MCE:col}{{7.3}{58}{}{definition.7.3}{}}
\@writefile{lla}{\contentsline {section}{\numberline {\crtrefnumber{dfn:MCE:col}}dfn:MCE:col}{58}{definition.7.3}\protected@file@percent }
\newlabel{dfn:MCE:col@cref}{{[definition][3][7]7.3}{[1][58][]58}{}{}{}}
\@writefile{loe}{\contentsline {lemma}{\ifthmt@listswap Lemma~7.4\else \numberline {7.4}Lemma\fi }{58}{lemma.7.4}\protected@file@percent }
\newlabel{lemma:MCE:clique_convex}{{7.4}{58}{}{lemma.7.4}{}}
\@writefile{lla}{\contentsline {section}{\numberline {\crtrefnumber{lemma:MCE:clique_convex}}lemma:MCE:clique_convex}{58}{lemma.7.4}\protected@file@percent }
\newlabel{lemma:MCE:clique_convex@cref}{{[lemma][4][7]7.4}{[1][58][]58}{}{}{}}
\@writefile{loe}{\contentsline {lemma}{\ifthmt@listswap Lemma~7.5\else \numberline {7.5}Lemma\fi }{58}{lemma.7.5}\protected@file@percent }
\newlabel{lemma:MCE:clique_affine_linear}{{7.5}{58}{}{lemma.7.5}{}}
\@writefile{lla}{\contentsline {section}{\numberline {\crtrefnumber{lemma:MCE:clique_affine_linear}}lemma:MCE:clique_affine_linear}{58}{lemma.7.5}\protected@file@percent }
\newlabel{lemma:MCE:clique_affine_linear@cref}{{[lemma][5][7]7.5}{[1][58][]58}{}{}{}}
\newlabel{eq:*}{{7.2}{58}{Cliques in \Mdash nonnegative point configurations}{equation.7.2}{}}
\@writefile{lla}{\contentsline {section}{\numberline {\crtrefnumber{eq:*}}eq:*}{58}{equation.7.2}\protected@file@percent }
\newlabel{eq:*@cref}{{[equation][2][7]7.2}{[1][58][]58}{}{}{}}
\@writefile{loe}{\contentsline {notation}{\ifthmt@listswap Notation~7.6\else \numberline {7.6}Notation\fi }{58}{notation.7.6}\protected@file@percent }
\newlabel{dfn:MCE:interior_edge_face}{{7.6}{58}{}{notation.7.6}{}}
\@writefile{lla}{\contentsline {section}{\numberline {\crtrefnumber{dfn:MCE:interior_edge_face}}dfn:MCE:interior_edge_face}{58}{notation.7.6}\protected@file@percent }
\newlabel{dfn:MCE:interior_edge_face@cref}{{[notation][6][7]7.6}{[1][58][]58}{}{}{}}
\@writefile{loe}{\contentsline {corollary}{\ifthmt@listswap Corollary~7.7\else \numberline {7.7}Corollary\fi }{58}{corollary.7.7}\protected@file@percent }
\newlabel{lemma:MCE:clique_union}{{7.7}{58}{}{corollary.7.7}{}}
\@writefile{lla}{\contentsline {section}{\numberline {\crtrefnumber{lemma:MCE:clique_union}}lemma:MCE:clique_union}{58}{corollary.7.7}\protected@file@percent }
\newlabel{lemma:MCE:clique_union@cref}{{[corollary][7][7]7.7}{[1][58][]58}{}{}{}}
\@writefile{loe}{\contentsline {corollary}{\ifthmt@listswap Corollary~7.8\else \numberline {7.8}Corollary\fi }{58}{corollary.7.8}\protected@file@percent }
\newlabel{lemma:MCE:clique_edge}{{7.8}{58}{}{corollary.7.8}{}}
\@writefile{lla}{\contentsline {section}{\numberline {\crtrefnumber{lemma:MCE:clique_edge}}lemma:MCE:clique_edge}{58}{corollary.7.8}\protected@file@percent }
\newlabel{lemma:MCE:clique_edge@cref}{{[corollary][8][7]7.8}{[1][58][]58}{}{}{}}
\newlabel{ssec:MCE:near-embedd-curvy}{{7.2}{58}{\Wembs of planar graphs}{subsection.7.2}{}}
\@writefile{lla}{\contentsline {section}{\numberline {\crtrefnumber{ssec:MCE:near-embedd-curvy}}ssec:MCE:near-embedd-curvy}{58}{subsection.7.2}\protected@file@percent }
\newlabel{ssec:MCE:near-embedd-curvy@cref}{{[subsection][2][7]7.2}{[1][58][]58}{}{}{}}
\@writefile{toc}{\contentsline {subsection}{\tocsubsection {}{7.2}{Weak embeddings\xspace  of planar graphs}}{58}{subsection.7.2}\protected@file@percent }
\@writefile{loe}{\contentsline {assumption}{\ifthmt@listswap Assumption~A\else \numberline {A}Assumption\fi }{58}{assumption.1}\protected@file@percent }
\newlabel{ass:lgg_dual}{{A}{58}{}{assumption.1}{}}
\@writefile{lla}{\contentsline {section}{\numberline {\crtrefnumber{ass:lgg_dual}}ass:lgg_dual}{58}{assumption.1}\protected@file@percent }
\newlabel{ass:lgg_dual@cref}{{[assumption][1][]A}{[1][58][]58}{}{}{}}
\@writefile{lof}{\contentsline {figure}{\numberline {14}{\ignorespaces  Examples of bent\xspace  line segments.}}{59}{figure.caption.22}\protected@file@percent }
\newlabel{fig:bend}{{14}{59}{Examples of \bent line segments}{figure.caption.22}{}}
\@writefile{lla}{\contentsline {section}{\numberline {\crtrefnumber{fig:bend}}fig:bend}{59}{figure.caption.22}\protected@file@percent }
\newlabel{fig:bend@cref}{{[figure][14][]14}{[1][59][]59}{}{}{}}
\@writefile{loe}{\contentsline {definition}{\ifthmt@listswap Definition~7.9\else \numberline {7.9}Definition\fi }{59}{definition.7.9}\protected@file@percent }
\newlabel{dfn:partF}{{7.9}{59}{}{definition.7.9}{}}
\@writefile{lla}{\contentsline {section}{\numberline {\crtrefnumber{dfn:partF}}dfn:partF}{59}{definition.7.9}\protected@file@percent }
\newlabel{dfn:partF@cref}{{[definition][9][7]7.9}{[1][59][]59}{}{}{}}
\@writefile{loe}{\contentsline {definition}{\ifthmt@listswap Definition~7.10\else \numberline {7.10}Definition\fi }{59}{definition.7.10}\protected@file@percent }
\newlabel{dfn:MCE:bent_line_seg}{{7.10}{59}{}{definition.7.10}{}}
\@writefile{lla}{\contentsline {section}{\numberline {\crtrefnumber{dfn:MCE:bent_line_seg}}dfn:MCE:bent_line_seg}{59}{definition.7.10}\protected@file@percent }
\newlabel{dfn:MCE:bent_line_seg@cref}{{[definition][10][7]7.10}{[1][59][]59}{}{}{}}
\@writefile{loe}{\contentsline {definition}{\ifthmt@listswap Definition~7.11\else \numberline {7.11}Definition\fi }{59}{definition.7.11}\protected@file@percent }
\newlabel{dfn:MCE:face_inj}{{7.11}{59}{}{definition.7.11}{}}
\@writefile{lla}{\contentsline {section}{\numberline {\crtrefnumber{dfn:MCE:face_inj}}dfn:MCE:face_inj}{59}{definition.7.11}\protected@file@percent }
\newlabel{dfn:MCE:face_inj@cref}{{[definition][11][7]7.11}{[1][59][]59}{}{}{}}
\@writefile{loe}{\contentsline {definition}{\ifthmt@listswap Definition~7.12\else \numberline {7.12}Definition\fi }{59}{definition.7.12}\protected@file@percent }
\@writefile{loe}{\contentsline {lemma}{\ifthmt@listswap Lemma~7.13\else \numberline {7.13}Lemma\fi }{59}{lemma.7.13}\protected@file@percent }
\newlabel{lemma:MCE:non_inj}{{7.13}{59}{}{lemma.7.13}{}}
\@writefile{lla}{\contentsline {section}{\numberline {\crtrefnumber{lemma:MCE:non_inj}}lemma:MCE:non_inj}{59}{lemma.7.13}\protected@file@percent }
\newlabel{lemma:MCE:non_inj@cref}{{[lemma][13][7]7.13}{[1][59][]59}{}{}{}}
\newlabel{non_inj1}{{{{(1)}}}{59}{}{Item.41}{}}
\@writefile{lla}{\contentsline {section}{\numberline {\crtrefnumber{non_inj1}}non_inj1}{59}{Item.41}\protected@file@percent }
\newlabel{non_inj1@cref}{{[enumi][1][]{{(1)}}}{[1][59][]59}{}{}{}}
\newlabel{non_inj2}{{{{(2)}}}{59}{}{Item.42}{}}
\@writefile{lla}{\contentsline {section}{\numberline {\crtrefnumber{non_inj2}}non_inj2}{59}{Item.42}\protected@file@percent }
\newlabel{non_inj2@cref}{{[enumi][2][]{{(2)}}}{[1][59][]59}{}{}{}}
\@writefile{loe}{\contentsline {corollary}{\ifthmt@listswap Corollary~7.14\else \numberline {7.14}Corollary\fi }{60}{corollary.7.14}\protected@file@percent }
\newlabel{lemma:MCE:non_inj_edge}{{7.14}{60}{}{corollary.7.14}{}}
\@writefile{lla}{\contentsline {section}{\numberline {\crtrefnumber{lemma:MCE:non_inj_edge}}lemma:MCE:non_inj_edge}{60}{corollary.7.14}\protected@file@percent }
\newlabel{lemma:MCE:non_inj_edge@cref}{{[corollary][14][7]7.14}{[1][60][]60}{}{}{}}
\@writefile{loe}{\contentsline {remark}{\ifthmt@listswap Remark~7.15\else \numberline {7.15}Remark\fi }{60}{remark.7.15}\protected@file@percent }
\newlabel{rmk:MCE:near_emb_combin}{{7.15}{60}{}{remark.7.15}{}}
\@writefile{lla}{\contentsline {section}{\numberline {\crtrefnumber{rmk:MCE:near_emb_combin}}rmk:MCE:near_emb_combin}{60}{remark.7.15}\protected@file@percent }
\newlabel{rmk:MCE:near_emb_combin@cref}{{[remark][15][7]7.15}{[1][60][]60}{}{}{}}
\@writefile{toc}{\contentsline {subsection}{\tocsubsection {}{7.3}{M-nonnegative weak embeddings\xspace  }}{60}{subsection.7.3}\protected@file@percent }
\@writefile{loe}{\contentsline {definition}{\ifthmt@listswap Definition~7.16\else \numberline {7.16}Definition\fi }{60}{definition.7.16}\protected@file@percent }
\newlabel{dfn:MCE:MNE}{{7.16}{60}{}{definition.7.16}{}}
\@writefile{lla}{\contentsline {section}{\numberline {\crtrefnumber{dfn:MCE:MNE}}dfn:MCE:MNE}{60}{definition.7.16}\protected@file@percent }
\newlabel{dfn:MCE:MNE@cref}{{[definition][16][7]7.16}{[1][60][]60}{}{}{}}
\newlabel{MCE1:emb}{{{{(MCE1)}}}{60}{}{Item.43}{}}
\@writefile{lla}{\contentsline {section}{\numberline {\crtrefnumber{MCE1:emb}}MCE1:emb}{60}{Item.43}\protected@file@percent }
\newlabel{MCE1:emb@cref}{{[enumi][1][]{{(MCE1)}}}{[1][60][]60}{}{}{}}
\newlabel{MCE2:null_edges}{{{{(MCE2)}}}{60}{}{Item.44}{}}
\@writefile{lla}{\contentsline {section}{\numberline {\crtrefnumber{MCE2:null_edges}}MCE2:null_edges}{60}{Item.44}\protected@file@percent }
\newlabel{MCE2:null_edges@cref}{{[enumi][2][]{{(MCE2)}}}{[1][60][]60}{}{}{}}
\newlabel{MCE3:M-tnn}{{{{(MCE3)}}}{60}{}{Item.45}{}}
\@writefile{lla}{\contentsline {section}{\numberline {\crtrefnumber{MCE3:M-tnn}}MCE3:M-tnn}{60}{Item.45}\protected@file@percent }
\newlabel{MCE3:M-tnn@cref}{{[enumi][3][]{{(MCE3)}}}{[1][60][]60}{}{}{}}
\@writefile{loe}{\contentsline {remark}{\ifthmt@listswap Remark~7.17\else \numberline {7.17}Remark\fi }{60}{remark.7.17}\protected@file@percent }
\newlabel{eq:MCE3':Mbd}{{7.3}{60}{}{equation.7.3}{}}
\@writefile{lla}{\contentsline {section}{\numberline {\crtrefnumber{eq:MCE3':Mbd}}eq:MCE3':Mbd}{60}{equation.7.3}\protected@file@percent }
\newlabel{eq:MCE3':Mbd@cref}{{[equation][3][7]7.3}{[1][60][]60}{}{}{}}
\@writefile{loe}{\contentsline {definition}{\ifthmt@listswap Definition~7.18\else \numberline {7.18}Definition\fi }{60}{definition.7.18}\protected@file@percent }
\newlabel{dfn:MCE:deg_emb_triang_big_faces}{{7.18}{60}{}{definition.7.18}{}}
\@writefile{lla}{\contentsline {section}{\numberline {\crtrefnumber{dfn:MCE:deg_emb_triang_big_faces}}dfn:MCE:deg_emb_triang_big_faces}{60}{definition.7.18}\protected@file@percent }
\newlabel{dfn:MCE:deg_emb_triang_big_faces@cref}{{[definition][18][7]7.18}{[1][60][]60}{}{}{}}
\@writefile{loe}{\contentsline {lemma}{\ifthmt@listswap Lemma~7.19\else \numberline {7.19}Lemma\fi }{60}{lemma.7.19}\protected@file@percent }
\@writefile{loe}{\contentsline {definition}{\ifthmt@listswap Definition~7.20\else \numberline {7.20}Definition\fi }{61}{definition.7.20}\protected@file@percent }
\newlabel{eq:MCE:angle_dfn}{{7.4}{61}{}{equation.7.4}{}}
\@writefile{lla}{\contentsline {section}{\numberline {\crtrefnumber{eq:MCE:angle_dfn}}eq:MCE:angle_dfn}{61}{equation.7.4}\protected@file@percent }
\newlabel{eq:MCE:angle_dfn@cref}{{[equation][4][7]7.4}{[1][60][]61}{}{}{}}
\newlabel{eq:nearGr:angles_exist}{{7.5}{61}{\MNEs }{equation.7.5}{}}
\@writefile{lla}{\contentsline {section}{\numberline {\crtrefnumber{eq:nearGr:angles_exist}}eq:nearGr:angles_exist}{61}{equation.7.5}\protected@file@percent }
\newlabel{eq:nearGr:angles_exist@cref}{{[equation][5][7]7.5}{[1][61][]61}{}{}{}}
\@writefile{loe}{\contentsline {lemma}{\ifthmt@listswap Lemma~7.21\else \numberline {7.21}Lemma\fi }{61}{lemma.7.21}\protected@file@percent }
\newlabel{eq:M_tnn_vs_angles}{{7.6}{61}{}{equation.7.6}{}}
\@writefile{lla}{\contentsline {section}{\numberline {\crtrefnumber{eq:M_tnn_vs_angles}}eq:M_tnn_vs_angles}{61}{equation.7.6}\protected@file@percent }
\newlabel{eq:M_tnn_vs_angles@cref}{{[equation][6][7]7.6}{[1][61][]61}{}{}{}}
\newlabel{eq:M_tnn_vs_angles_eq}{{7.7}{61}{}{equation.7.7}{}}
\@writefile{lla}{\contentsline {section}{\numberline {\crtrefnumber{eq:M_tnn_vs_angles_eq}}eq:M_tnn_vs_angles_eq}{61}{equation.7.7}\protected@file@percent }
\newlabel{eq:M_tnn_vs_angles_eq@cref}{{[equation][7][7]7.7}{[1][61][]61}{}{}{}}
\@writefile{loe}{\contentsline {lemma}{\ifthmt@listswap Lemma~7.22\else \numberline {7.22}Lemma\fi }{61}{lemma.7.22}\protected@file@percent }
\newlabel{lemma:MCE:corner_angle}{{7.22}{61}{}{lemma.7.22}{}}
\@writefile{lla}{\contentsline {section}{\numberline {\crtrefnumber{lemma:MCE:corner_angle}}lemma:MCE:corner_angle}{61}{lemma.7.22}\protected@file@percent }
\newlabel{lemma:MCE:corner_angle@cref}{{[lemma][22][7]7.22}{[1][61][]61}{}{}{}}
\newlabel{corner_angle1}{{{{(1)}}}{61}{}{Item.46}{}}
\@writefile{lla}{\contentsline {section}{\numberline {\crtrefnumber{corner_angle1}}corner_angle1}{61}{Item.46}\protected@file@percent }
\newlabel{corner_angle1@cref}{{[enumi][1][]{{(1)}}}{[1][61][]61}{}{}{}}
\newlabel{corner_angle2}{{{{(2)}}}{61}{}{Item.47}{}}
\@writefile{lla}{\contentsline {section}{\numberline {\crtrefnumber{corner_angle2}}corner_angle2}{61}{Item.47}\protected@file@percent }
\newlabel{corner_angle2@cref}{{[enumi][2][]{{(2)}}}{[1][61][]61}{}{}{}}
\newlabel{eq:sumwT_sumbT_vs_sumT_sumO}{{7.8}{61}{}{equation.7.8}{}}
\@writefile{lla}{\contentsline {section}{\numberline {\crtrefnumber{eq:sumwT_sumbT_vs_sumT_sumO}}eq:sumwT_sumbT_vs_sumT_sumO}{61}{equation.7.8}\protected@file@percent }
\newlabel{eq:sumwT_sumbT_vs_sumT_sumO@cref}{{[equation][8][7]7.8}{[1][61][]61}{}{}{}}
\newlabel{eq:cos_M_tnn}{{7.9}{61}{\MNEs }{equation.7.9}{}}
\@writefile{lla}{\contentsline {section}{\numberline {\crtrefnumber{eq:cos_M_tnn}}eq:cos_M_tnn}{61}{equation.7.9}\protected@file@percent }
\newlabel{eq:cos_M_tnn@cref}{{[equation][9][7]7.9}{[1][61][]61}{}{}{}}
\@writefile{loe}{\contentsline {definition}{\ifthmt@listswap Definition~7.23\else \numberline {7.23}Definition\fi }{61}{definition.7.23}\protected@file@percent }
\newlabel{dfn:corner_active}{{7.23}{61}{}{definition.7.23}{}}
\@writefile{lla}{\contentsline {section}{\numberline {\crtrefnumber{dfn:corner_active}}dfn:corner_active}{61}{definition.7.23}\protected@file@percent }
\newlabel{dfn:corner_active@cref}{{[definition][23][7]7.23}{[1][61][]61}{}{}{}}
\@writefile{loe}{\contentsline {corollary}{\ifthmt@listswap Corollary~7.24\else \numberline {7.24}Corollary\fi }{61}{corollary.7.24}\protected@file@percent }
\newlabel{lemma:MCE:corner_M_pos}{{7.24}{61}{}{corollary.7.24}{}}
\@writefile{lla}{\contentsline {section}{\numberline {\crtrefnumber{lemma:MCE:corner_M_pos}}lemma:MCE:corner_M_pos}{61}{corollary.7.24}\protected@file@percent }
\newlabel{lemma:MCE:corner_M_pos@cref}{{[corollary][24][7]7.24}{[1][61][]61}{}{}{}}
\newlabel{corner_M_pos1}{{{{(1)}}}{61}{}{Item.48}{}}
\@writefile{lla}{\contentsline {section}{\numberline {\crtrefnumber{corner_M_pos1}}corner_M_pos1}{61}{Item.48}\protected@file@percent }
\newlabel{corner_M_pos1@cref}{{[enumi][1][]{{(1)}}}{[1][61][]61}{}{}{}}
\newlabel{corner_M_pos2}{{{{(2)}}}{61}{}{Item.49}{}}
\@writefile{lla}{\contentsline {section}{\numberline {\crtrefnumber{corner_M_pos2}}corner_M_pos2}{61}{Item.49}\protected@file@percent }
\newlabel{corner_M_pos2@cref}{{[enumi][2][]{{(2)}}}{[1][61][]61}{}{}{}}
\@writefile{loe}{\contentsline {lemma}{\ifthmt@listswap Lemma~7.25\else \numberline {7.25}Lemma\fi }{61}{lemma.7.25}\protected@file@percent }
\newlabel{lemma:MCE:ambig_corner_clique}{{7.25}{61}{}{lemma.7.25}{}}
\@writefile{lla}{\contentsline {section}{\numberline {\crtrefnumber{lemma:MCE:ambig_corner_clique}}lemma:MCE:ambig_corner_clique}{61}{lemma.7.25}\protected@file@percent }
\newlabel{lemma:MCE:ambig_corner_clique@cref}{{[lemma][25][7]7.25}{[1][61][]61}{}{}{}}
\@writefile{loe}{\contentsline {corollary}{\ifthmt@listswap Corollary~7.26\else \numberline {7.26}Corollary\fi }{62}{corollary.7.26}\protected@file@percent }
\newlabel{lemma:MCE:bdry_unambig}{{7.26}{62}{}{corollary.7.26}{}}
\@writefile{lla}{\contentsline {section}{\numberline {\crtrefnumber{lemma:MCE:bdry_unambig}}lemma:MCE:bdry_unambig}{62}{corollary.7.26}\protected@file@percent }
\newlabel{lemma:MCE:bdry_unambig@cref}{{[corollary][26][7]7.26}{[1][62][]62}{}{}{}}
\newlabel{ssec:PMNEs}{{7.4}{62}{\KawAngle condition}{subsection.7.4}{}}
\@writefile{lla}{\contentsline {section}{\numberline {\crtrefnumber{ssec:PMNEs}}ssec:PMNEs}{62}{subsection.7.4}\protected@file@percent }
\newlabel{ssec:PMNEs@cref}{{[subsection][4][7]7.4}{[1][62][]62}{}{}{}}
\@writefile{toc}{\contentsline {subsection}{\tocsubsection {}{7.4}{Kawasaki angle\xspace  condition}}{62}{subsection.7.4}\protected@file@percent }
\@writefile{loe}{\contentsline {definition}{\ifthmt@listswap Definition~7.27\else \numberline {7.27}Definition\fi }{62}{definition.7.27}\protected@file@percent }
\newlabel{eq:sumwT_sumbT_of_f_dfn}{{7.10}{62}{}{equation.7.10}{}}
\@writefile{lla}{\contentsline {section}{\numberline {\crtrefnumber{eq:sumwT_sumbT_of_f_dfn}}eq:sumwT_sumbT_of_f_dfn}{62}{equation.7.10}\protected@file@percent }
\newlabel{eq:sumwT_sumbT_of_f_dfn@cref}{{[equation][10][7]7.10}{[1][62][]62}{}{}{}}
\@writefile{loe}{\contentsline {definition}{\ifthmt@listswap Definition~7.28\else \numberline {7.28}Definition\fi \thmtformatoptarg {Kawasaki angle\xspace  condition}}{62}{definition.7.28}\protected@file@percent }
\newlabel{eq:MCE:sumwT_sumbT=pi}{{7.11}{62}{\Kawangle condition}{equation.7.11}{}}
\@writefile{lla}{\contentsline {section}{\numberline {\crtrefnumber{eq:MCE:sumwT_sumbT=pi}}eq:MCE:sumwT_sumbT=pi}{62}{equation.7.11}\protected@file@percent }
\newlabel{eq:MCE:sumwT_sumbT=pi@cref}{{[equation][11][7]7.11}{[1][62][]62}{}{}{}}
\@writefile{loe}{\contentsline {lemma}{\ifthmt@listswap Lemma~7.29\else \numberline {7.29}Lemma\fi }{62}{lemma.7.29}\protected@file@percent }
\newlabel{lemma:MCE:sumwT_sumbT_options}{{7.29}{62}{}{lemma.7.29}{}}
\@writefile{lla}{\contentsline {section}{\numberline {\crtrefnumber{lemma:MCE:sumwT_sumbT_options}}lemma:MCE:sumwT_sumbT_options}{62}{lemma.7.29}\protected@file@percent }
\newlabel{lemma:MCE:sumwT_sumbT_options@cref}{{[lemma][29][7]7.29}{[1][62][]62}{}{}{}}
\newlabel{eq:sumwT_sumbT_options}{{7.12}{62}{}{equation.7.12}{}}
\@writefile{lla}{\contentsline {section}{\numberline {\crtrefnumber{eq:sumwT_sumbT_options}}eq:sumwT_sumbT_options}{62}{equation.7.12}\protected@file@percent }
\newlabel{eq:sumwT_sumbT_options@cref}{{[equation][12][7]7.12}{[1][62][]62}{}{}{}}
\newlabel{eq:near:emb_vertex_angle_sum}{{7.13}{62}{\KawAngle condition}{equation.7.13}{}}
\@writefile{lla}{\contentsline {section}{\numberline {\crtrefnumber{eq:near:emb_vertex_angle_sum}}eq:near:emb_vertex_angle_sum}{62}{equation.7.13}\protected@file@percent }
\newlabel{eq:near:emb_vertex_angle_sum@cref}{{[equation][13][7]7.13}{[1][62][]62}{}{}{}}
\@writefile{loe}{\contentsline {definition}{\ifthmt@listswap Definition~7.30\else \numberline {7.30}Definition\fi }{62}{definition.7.30}\protected@file@percent }
\newlabel{dfn:improper}{{7.30}{62}{}{definition.7.30}{}}
\@writefile{lla}{\contentsline {section}{\numberline {\crtrefnumber{dfn:improper}}dfn:improper}{62}{definition.7.30}\protected@file@percent }
\newlabel{dfn:improper@cref}{{[definition][30][7]7.30}{[1][62][]62}{}{}{}}
\@writefile{loe}{\contentsline {lemma}{\ifthmt@listswap Lemma~7.31\else \numberline {7.31}Lemma\fi }{62}{lemma.7.31}\protected@file@percent }
\newlabel{lemma:MCE:improper_char}{{7.31}{62}{}{lemma.7.31}{}}
\@writefile{lla}{\contentsline {section}{\numberline {\crtrefnumber{lemma:MCE:improper_char}}lemma:MCE:improper_char}{62}{lemma.7.31}\protected@file@percent }
\newlabel{lemma:MCE:improper_char@cref}{{[lemma][31][7]7.31}{[1][62][]62}{}{}{}}
\@writefile{loe}{\contentsline {remark}{\ifthmt@listswap Remark~7.32\else \numberline {7.32}Remark\fi }{63}{remark.7.32}\protected@file@percent }
\newlabel{rmk:MCE:bdry_proper}{{7.32}{63}{}{remark.7.32}{}}
\@writefile{lla}{\contentsline {section}{\numberline {\crtrefnumber{rmk:MCE:bdry_proper}}rmk:MCE:bdry_proper}{63}{remark.7.32}\protected@file@percent }
\newlabel{rmk:MCE:bdry_proper@cref}{{[remark][32][7]7.32}{[1][63][]63}{}{}{}}
\newlabel{eq:MCE:sumwT_sumbT_bdry_0_pi}{{7.14}{63}{}{equation.7.14}{}}
\@writefile{lla}{\contentsline {section}{\numberline {\crtrefnumber{eq:MCE:sumwT_sumbT_bdry_0_pi}}eq:MCE:sumwT_sumbT_bdry_0_pi}{63}{equation.7.14}\protected@file@percent }
\newlabel{eq:MCE:sumwT_sumbT_bdry_0_pi@cref}{{[equation][14][7]7.14}{[1][63][]63}{}{}{}}
\@writefile{loe}{\contentsline {definition}{\ifthmt@listswap Definition~7.33\else \numberline {7.33}Definition\fi }{63}{definition.7.33}\protected@file@percent }
\newlabel{dfn:MCE:pMNE}{{7.33}{63}{}{definition.7.33}{}}
\@writefile{lla}{\contentsline {section}{\numberline {\crtrefnumber{dfn:MCE:pMNE}}dfn:MCE:pMNE}{63}{definition.7.33}\protected@file@percent }
\newlabel{dfn:MCE:pMNE@cref}{{[definition][33][7]7.33}{[1][63][]63}{}{}{}}
\@writefile{loe}{\contentsline {lemma}{\ifthmt@listswap Lemma~7.34\else \numberline {7.34}Lemma\fi }{63}{lemma.7.34}\protected@file@percent }
\newlabel{lemma:MCE:coloring_improper_verts}{{7.34}{63}{}{lemma.7.34}{}}
\@writefile{lla}{\contentsline {section}{\numberline {\crtrefnumber{lemma:MCE:coloring_improper_verts}}lemma:MCE:coloring_improper_verts}{63}{lemma.7.34}\protected@file@percent }
\newlabel{lemma:MCE:coloring_improper_verts@cref}{{[lemma][34][7]7.34}{[1][63][]63}{}{}{}}
\@writefile{loe}{\contentsline {definition}{\ifthmt@listswap Definition~7.35\else \numberline {7.35}Definition\fi }{63}{definition.7.35}\protected@file@percent }
\newlabel{eq:MCE:MCMalg_dfn}{{7.15}{63}{}{equation.7.15}{}}
\@writefile{lla}{\contentsline {section}{\numberline {\crtrefnumber{eq:MCE:MCMalg_dfn}}eq:MCE:MCMalg_dfn}{63}{equation.7.15}\protected@file@percent }
\newlabel{eq:MCE:MCMalg_dfn@cref}{{[equation][15][7]7.15}{[1][63][]63}{}{}{}}
\@writefile{loe}{\contentsline {proposition}{\ifthmt@listswap Proposition~7.36\else \numberline {7.36}Proposition\fi }{63}{proposition.7.36}\protected@file@percent }
\newlabel{lemma:MCE:Res}{{7.36}{63}{}{proposition.7.36}{}}
\@writefile{lla}{\contentsline {section}{\numberline {\crtrefnumber{lemma:MCE:Res}}lemma:MCE:Res}{63}{proposition.7.36}\protected@file@percent }
\newlabel{lemma:MCE:Res@cref}{{[proposition][36][7]7.36}{[1][63][]63}{}{}{}}
\newlabel{eq:MCE:Res_dfn}{{7.16}{63}{}{equation.7.16}{}}
\@writefile{lla}{\contentsline {section}{\numberline {\crtrefnumber{eq:MCE:Res_dfn}}eq:MCE:Res_dfn}{63}{equation.7.16}\protected@file@percent }
\newlabel{eq:MCE:Res_dfn@cref}{{[equation][16][7]7.16}{[1][63][]63}{}{}{}}
\newlabel{eq:induced_angle_sums}{{7.17}{63}{}{equation.7.17}{}}
\@writefile{lla}{\contentsline {section}{\numberline {\crtrefnumber{eq:induced_angle_sums}}eq:induced_angle_sums}{63}{equation.7.17}\protected@file@percent }
\newlabel{eq:induced_angle_sums@cref}{{[equation][17][7]7.17}{[1][63][]63}{}{}{}}
\@writefile{loe}{\contentsline {proposition}{\ifthmt@listswap Proposition~7.37\else \numberline {7.37}Proposition\fi }{64}{proposition.7.37}\protected@file@percent }
\newlabel{lemma:limit_of_pcMNE_is_pMNE}{{7.37}{64}{}{proposition.7.37}{}}
\@writefile{lla}{\contentsline {section}{\numberline {\crtrefnumber{lemma:limit_of_pcMNE_is_pMNE}}lemma:limit_of_pcMNE_is_pMNE}{64}{proposition.7.37}\protected@file@percent }
\newlabel{lemma:limit_of_pcMNE_is_pMNE@cref}{{[proposition][37][7]7.37}{[1][64][]64}{}{}{}}
\@writefile{toc}{\contentsline {section}{\tocsection {}{8}{Mandelstam-convex\xspace  embeddings\xspace  }}{64}{section.8}\protected@file@percent }
\newlabel{sec:MCE}{{8}{64}{\MCEsnoacrTITLE }{section.8}{}}
\@writefile{lla}{\contentsline {section}{\numberline {\crtrefnumber{sec:MCE}}sec:MCE}{64}{section.8}\protected@file@percent }
\newlabel{sec:MCE@cref}{{[section][8][]8}{[1][64][]64}{}{}{}}
\@writefile{toc}{\contentsline {subsection}{\tocsubsection {}{8.1}{Definition and basic properties}}{64}{thmt@dummyctr.dummy.229}\protected@file@percent }
\@writefile{loe}{\contentsline {definition}{\ifthmt@listswap Definition~8.1\else \numberline {8.1}Definition\fi }{64}{definition.8.1}\protected@file@percent }
\newlabel{dfn:pchord}{{8.1}{64}{}{definition.8.1}{}}
\@writefile{lla}{\contentsline {section}{\numberline {\crtrefnumber{dfn:pchord}}dfn:pchord}{64}{definition.8.1}\protected@file@percent }
\newlabel{dfn:pchord@cref}{{[definition][1][8]8.1}{[1][64][]64}{}{}{}}
\newlabel{pchord2}{{{{(ii)}}}{64}{}{Item.51}{}}
\@writefile{lla}{\contentsline {section}{\numberline {\crtrefnumber{pchord2}}pchord2}{64}{Item.51}\protected@file@percent }
\newlabel{pchord2@cref}{{[enumi][2][]{{(ii)}}}{[1][64][]64}{}{}{}}
\@writefile{loe}{\contentsline {definition}{\ifthmt@listswap Definition~8.2\else \numberline {8.2}Definition\fi }{64}{definition.8.2}\protected@file@percent }
\@writefile{loe}{\contentsline {remark}{\ifthmt@listswap Remark~8.3\else \numberline {8.3}Remark\fi }{64}{remark.8.3}\protected@file@percent }
\newlabel{rmk:MCE:pchord_outer_face}{{8.3}{64}{}{remark.8.3}{}}
\@writefile{lla}{\contentsline {section}{\numberline {\crtrefnumber{rmk:MCE:pchord_outer_face}}rmk:MCE:pchord_outer_face}{64}{remark.8.3}\protected@file@percent }
\newlabel{rmk:MCE:pchord_outer_face@cref}{{[remark][3][8]8.3}{[1][64][]64}{}{}{}}
\@writefile{loe}{\contentsline {definition}{\ifthmt@listswap Definition~8.4\else \numberline {8.4}Definition\fi \thmtformatoptarg {M-convex\xspace  weak embedding\xspace  }}{64}{definition.8.4}\protected@file@percent }
\newlabel{dfn:MCE:MCE}{{8.4}{64}{\MCEnoacr }{definition.8.4}{}}
\@writefile{lla}{\contentsline {section}{\numberline {\crtrefnumber{dfn:MCE:MCE}}dfn:MCE:MCE}{64}{definition.8.4}\protected@file@percent }
\newlabel{dfn:MCE:MCE@cref}{{[definition][4][8]8.4}{[1][64][]64}{}{}{}}
\newlabel{MCE4:properly_colored}{{{{(MCE4)}}}{64}{\MCEnoacr }{Item.52}{}}
\@writefile{lla}{\contentsline {section}{\numberline {\crtrefnumber{MCE4:properly_colored}}MCE4:properly_colored}{64}{Item.52}\protected@file@percent }
\newlabel{MCE4:properly_colored@cref}{{[enumi][4][]{{(MCE4)}}}{[1][64][]64}{}{}{}}
\newlabel{MCE5:Mpos_chords}{{{{(MCE5)}}}{64}{\MCEnoacr }{Item.53}{}}
\@writefile{lla}{\contentsline {section}{\numberline {\crtrefnumber{MCE5:Mpos_chords}}MCE5:Mpos_chords}{64}{Item.53}\protected@file@percent }
\newlabel{MCE5:Mpos_chords@cref}{{[enumi][5][]{{(MCE5)}}}{[1][64][]64}{}{}{}}
\@writefile{loe}{\contentsline {lemma}{\ifthmt@listswap Lemma~8.5\else \numberline {8.5}Lemma\fi }{64}{lemma.8.5}\protected@file@percent }
\newlabel{lemma:ambig=>triangular}{{8.5}{64}{}{lemma.8.5}{}}
\@writefile{lla}{\contentsline {section}{\numberline {\crtrefnumber{lemma:ambig=>triangular}}lemma:ambig=>triangular}{64}{lemma.8.5}\protected@file@percent }
\newlabel{lemma:ambig=>triangular@cref}{{[lemma][5][8]8.5}{[1][64][]64}{}{}{}}
\@writefile{loe}{\contentsline {lemma}{\ifthmt@listswap Lemma~8.6\else \numberline {8.6}Lemma\fi }{64}{lemma.8.6}\protected@file@percent }
\newlabel{lemma:MCE:add_chords}{{8.6}{64}{}{lemma.8.6}{}}
\@writefile{lla}{\contentsline {section}{\numberline {\crtrefnumber{lemma:MCE:add_chords}}lemma:MCE:add_chords}{64}{lemma.8.6}\protected@file@percent }
\newlabel{lemma:MCE:add_chords@cref}{{[lemma][6][8]8.6}{[1][64][]64}{}{}{}}
\@writefile{loe}{\contentsline {lemma}{\ifthmt@listswap Lemma~8.7\else \numberline {8.7}Lemma\fi }{65}{lemma.8.7}\protected@file@percent }
\newlabel{lemma:MCE:sticky}{{8.7}{65}{}{lemma.8.7}{}}
\@writefile{lla}{\contentsline {section}{\numberline {\crtrefnumber{lemma:MCE:sticky}}lemma:MCE:sticky}{65}{lemma.8.7}\protected@file@percent }
\newlabel{lemma:MCE:sticky@cref}{{[lemma][7][8]8.7}{[1][65][]65}{}{}{}}
\@writefile{toc}{\contentsline {subsection}{\tocsubsection {}{8.2}{Maximal cliques}}{65}{subsection.8.2}\protected@file@percent }
\@writefile{loe}{\contentsline {lemma}{\ifthmt@listswap Lemma~8.8\else \numberline {8.8}Lemma\fi }{65}{lemma.8.8}\protected@file@percent }
\newlabel{lemma:MCE:trivial_M-zero<=>clique}{{8.8}{65}{}{lemma.8.8}{}}
\@writefile{lla}{\contentsline {section}{\numberline {\crtrefnumber{lemma:MCE:trivial_M-zero<=>clique}}lemma:MCE:trivial_M-zero<=>clique}{65}{lemma.8.8}\protected@file@percent }
\newlabel{lemma:MCE:trivial_M-zero<=>clique@cref}{{[lemma][8][8]8.8}{[1][65][]65}{}{}{}}
\@writefile{loe}{\contentsline {lemma}{\ifthmt@listswap Lemma~8.9\else \numberline {8.9}Lemma\fi }{65}{lemma.8.9}\protected@file@percent }
\newlabel{lemma:MCE:Conv_vertices_injective}{{8.9}{65}{}{lemma.8.9}{}}
\@writefile{lla}{\contentsline {section}{\numberline {\crtrefnumber{lemma:MCE:Conv_vertices_injective}}lemma:MCE:Conv_vertices_injective}{65}{lemma.8.9}\protected@file@percent }
\newlabel{lemma:MCE:Conv_vertices_injective@cref}{{[lemma][9][8]8.9}{[1][65][]65}{}{}{}}
\@writefile{loe}{\contentsline {lemma}{\ifthmt@listswap Lemma~8.10\else \numberline {8.10}Lemma\fi }{65}{lemma.8.10}\protected@file@percent }
\newlabel{lemma:MCE:two_cliques_intersection}{{8.10}{65}{}{lemma.8.10}{}}
\@writefile{lla}{\contentsline {section}{\numberline {\crtrefnumber{lemma:MCE:two_cliques_intersection}}lemma:MCE:two_cliques_intersection}{65}{lemma.8.10}\protected@file@percent }
\newlabel{lemma:MCE:two_cliques_intersection@cref}{{[lemma][10][8]8.10}{[1][65][]65}{}{}{}}
\@writefile{lof}{\contentsline {figure}{\numberline {15}{\ignorespaces  External points\xspace  (left) and external chords\xspace  (right) are marked in red.}}{66}{figure.caption.23}\protected@file@percent }
\newlabel{fig:extcycle}{{15}{66}{\Extpts (left) and \extpchords (right) are marked in red}{figure.caption.23}{}}
\@writefile{lla}{\contentsline {section}{\numberline {\crtrefnumber{fig:extcycle}}fig:extcycle}{66}{figure.caption.23}\protected@file@percent }
\newlabel{fig:extcycle@cref}{{[figure][15][]15}{[1][66][]66}{}{}{}}
\@writefile{loe}{\contentsline {definition}{\ifthmt@listswap Definition~8.11\else \numberline {8.11}Definition\fi }{66}{definition.8.11}\protected@file@percent }
\newlabel{dfn:MCE:ext_on_edge}{{8.11}{66}{}{definition.8.11}{}}
\@writefile{lla}{\contentsline {section}{\numberline {\crtrefnumber{dfn:MCE:ext_on_edge}}dfn:MCE:ext_on_edge}{66}{definition.8.11}\protected@file@percent }
\newlabel{dfn:MCE:ext_on_edge@cref}{{[definition][11][8]8.11}{[1][66][]66}{}{}{}}
\@writefile{loe}{\contentsline {remark}{\ifthmt@listswap Remark~8.12\else \numberline {8.12}Remark\fi }{66}{remark.8.12}\protected@file@percent }
\newlabel{rmk:MCE:extpt_ordering}{{8.12}{66}{}{remark.8.12}{}}
\@writefile{lla}{\contentsline {section}{\numberline {\crtrefnumber{rmk:MCE:extpt_ordering}}rmk:MCE:extpt_ordering}{66}{remark.8.12}\protected@file@percent }
\newlabel{rmk:MCE:extpt_ordering@cref}{{[remark][12][8]8.12}{[1][66][]66}{}{}{}}
\@writefile{loe}{\contentsline {definition}{\ifthmt@listswap Definition~8.13\else \numberline {8.13}Definition\fi \thmtformatoptarg {External point\xspace  }}{66}{definition.8.13}\protected@file@percent }
\newlabel{dfn:MCE:extpt}{{8.13}{66}{\Extpt }{definition.8.13}{}}
\@writefile{lla}{\contentsline {section}{\numberline {\crtrefnumber{dfn:MCE:extpt}}dfn:MCE:extpt}{66}{definition.8.13}\protected@file@percent }
\newlabel{dfn:MCE:extpt@cref}{{[definition][13][8]8.13}{[1][66][]66}{}{}{}}
\@writefile{loe}{\contentsline {lemma}{\ifthmt@listswap Lemma~8.14\else \numberline {8.14}Lemma\fi }{66}{lemma.8.14}\protected@file@percent }
\newlabel{lemma:MCE:extpt_vs_vertex}{{8.14}{66}{}{lemma.8.14}{}}
\@writefile{lla}{\contentsline {section}{\numberline {\crtrefnumber{lemma:MCE:extpt_vs_vertex}}lemma:MCE:extpt_vs_vertex}{66}{lemma.8.14}\protected@file@percent }
\newlabel{lemma:MCE:extpt_vs_vertex@cref}{{[lemma][14][8]8.14}{[1][66][]66}{}{}{}}
\@writefile{loe}{\contentsline {remark}{\ifthmt@listswap Remark~8.15\else \numberline {8.15}Remark\fi }{67}{remark.8.15}\protected@file@percent }
\newlabel{rmk:MCE:clique_boundary_outward_bent}{{8.15}{67}{}{remark.8.15}{}}
\@writefile{lla}{\contentsline {section}{\numberline {\crtrefnumber{rmk:MCE:clique_boundary_outward_bent}}rmk:MCE:clique_boundary_outward_bent}{67}{remark.8.15}\protected@file@percent }
\newlabel{rmk:MCE:clique_boundary_outward_bent@cref}{{[remark][15][8]8.15}{[1][67][]67}{}{}{}}
\@writefile{loe}{\contentsline {lemma}{\ifthmt@listswap Lemma~8.16\else \numberline {8.16}Lemma\fi \thmtformatoptarg {External chord\xspace  }}{67}{lemma.8.16}\protected@file@percent }
\newlabel{lemma:MCE:extpchord}{{8.16}{67}{\Extpchord }{lemma.8.16}{}}
\@writefile{lla}{\contentsline {section}{\numberline {\crtrefnumber{lemma:MCE:extpchord}}lemma:MCE:extpchord}{67}{lemma.8.16}\protected@file@percent }
\newlabel{lemma:MCE:extpchord@cref}{{[lemma][16][8]8.16}{[1][67][]67}{}{}{}}
\@writefile{loe}{\contentsline {proposition}{\ifthmt@listswap Proposition~8.17\else \numberline {8.17}Proposition\fi \thmtformatoptarg {External cycle\xspace  }}{67}{proposition.8.17}\protected@file@percent }
\newlabel{lemma:MCE:outward_simple}{{8.17}{67}{\Extcycle }{proposition.8.17}{}}
\@writefile{lla}{\contentsline {section}{\numberline {\crtrefnumber{lemma:MCE:outward_simple}}lemma:MCE:outward_simple}{67}{proposition.8.17}\protected@file@percent }
\newlabel{lemma:MCE:outward_simple@cref}{{[proposition][17][8]8.17}{[1][67][]67}{}{}{}}
\@writefile{toc}{\contentsline {subsection}{\tocsubsection {}{8.3}{Flexible\xspace  faces}}{67}{subsection.8.3}\protected@file@percent }
\@writefile{loe}{\contentsline {definition}{\ifthmt@listswap Definition~8.18\else \numberline {8.18}Definition\fi }{67}{definition.8.18}\protected@file@percent }
\@writefile{loe}{\contentsline {corollary}{\ifthmt@listswap Corollary~8.19\else \numberline {8.19}Corollary\fi }{67}{corollary.8.19}\protected@file@percent }
\newlabel{lemma:MCE:inside_CycKmax=>rigid}{{8.19}{67}{}{corollary.8.19}{}}
\@writefile{lla}{\contentsline {section}{\numberline {\crtrefnumber{lemma:MCE:inside_CycKmax=>rigid}}lemma:MCE:inside_CycKmax=>rigid}{67}{corollary.8.19}\protected@file@percent }
\newlabel{lemma:MCE:inside_CycKmax=>rigid@cref}{{[corollary][19][8]8.19}{[1][67][]67}{}{}{}}
\@writefile{loe}{\contentsline {lemma}{\ifthmt@listswap Lemma~8.20\else \numberline {8.20}Lemma\fi }{67}{lemma.8.20}\protected@file@percent }
\newlabel{lemma:MCE:non_vertex_is_not_incident_to_active_face}{{8.20}{67}{}{lemma.8.20}{}}
\@writefile{lla}{\contentsline {section}{\numberline {\crtrefnumber{lemma:MCE:non_vertex_is_not_incident_to_active_face}}lemma:MCE:non_vertex_is_not_incident_to_active_face}{67}{lemma.8.20}\protected@file@percent }
\newlabel{lemma:MCE:non_vertex_is_not_incident_to_active_face@cref}{{[lemma][20][8]8.20}{[1][67][]67}{}{}{}}
\@writefile{loe}{\contentsline {corollary}{\ifthmt@listswap Corollary~8.21\else \numberline {8.21}Corollary\fi }{67}{corollary.8.21}\protected@file@percent }
\newlabel{cor:MCE:active_vertex_not_mid_edge}{{8.21}{67}{}{corollary.8.21}{}}
\@writefile{lla}{\contentsline {section}{\numberline {\crtrefnumber{cor:MCE:active_vertex_not_mid_edge}}cor:MCE:active_vertex_not_mid_edge}{67}{corollary.8.21}\protected@file@percent }
\newlabel{cor:MCE:active_vertex_not_mid_edge@cref}{{[corollary][21][8]8.21}{[1][67][]67}{}{}{}}
\@writefile{loe}{\contentsline {corollary}{\ifthmt@listswap Corollary~8.22\else \numberline {8.22}Corollary\fi }{67}{corollary.8.22}\protected@file@percent }
\newlabel{lemma:MCE:active_face_embedded}{{8.22}{67}{}{corollary.8.22}{}}
\@writefile{lla}{\contentsline {section}{\numberline {\crtrefnumber{lemma:MCE:active_face_embedded}}lemma:MCE:active_face_embedded}{67}{corollary.8.22}\protected@file@percent }
\newlabel{lemma:MCE:active_face_embedded@cref}{{[corollary][22][8]8.22}{[1][67][]67}{}{}{}}
\citation{RSS}
\citation{RSS}
\citation{RSS}
\citation{RSS}
\citation{RSS}
\citation{RSS}
\citation{RSS}
\@writefile{loe}{\contentsline {corollary}{\ifthmt@listswap Corollary~8.23\else \numberline {8.23}Corollary\fi }{68}{corollary.8.23}\protected@file@percent }
\newlabel{lemma:MCE:xTint_connected_open_avoids_cliques}{{8.23}{68}{}{corollary.8.23}{}}
\@writefile{lla}{\contentsline {section}{\numberline {\crtrefnumber{lemma:MCE:xTint_connected_open_avoids_cliques}}lemma:MCE:xTint_connected_open_avoids_cliques}{68}{corollary.8.23}\protected@file@percent }
\newlabel{lemma:MCE:xTint_connected_open_avoids_cliques@cref}{{[corollary][23][8]8.23}{[1][68][]68}{}{}{}}
\newlabel{eq:MCE:Rcc_dfn}{{8.1}{68}{\Flex faces}{equation.8.1}{}}
\@writefile{lla}{\contentsline {section}{\numberline {\crtrefnumber{eq:MCE:Rcc_dfn}}eq:MCE:Rcc_dfn}{68}{equation.8.1}\protected@file@percent }
\newlabel{eq:MCE:Rcc_dfn@cref}{{[equation][1][8]8.1}{[1][68][]68}{}{}{}}
\@writefile{loe}{\contentsline {corollary}{\ifthmt@listswap Corollary~8.24\else \numberline {8.24}Corollary\fi }{68}{corollary.8.24}\protected@file@percent }
\newlabel{lemma:MCE:collared_corner_active}{{8.24}{68}{}{corollary.8.24}{}}
\@writefile{lla}{\contentsline {section}{\numberline {\crtrefnumber{lemma:MCE:collared_corner_active}}lemma:MCE:collared_corner_active}{68}{corollary.8.24}\protected@file@percent }
\newlabel{lemma:MCE:collared_corner_active@cref}{{[corollary][24][8]8.24}{[1][68][]68}{}{}{}}
\@writefile{loe}{\contentsline {corollary}{\ifthmt@listswap Corollary~8.25\else \numberline {8.25}Corollary\fi }{68}{corollary.8.25}\protected@file@percent }
\newlabel{lemma:MCE:active_face=>active}{{8.25}{68}{}{corollary.8.25}{}}
\@writefile{lla}{\contentsline {section}{\numberline {\crtrefnumber{lemma:MCE:active_face=>active}}lemma:MCE:active_face=>active}{68}{corollary.8.25}\protected@file@percent }
\newlabel{lemma:MCE:active_face=>active@cref}{{[corollary][25][8]8.25}{[1][68][]68}{}{}{}}
\newlabel{ssec:pointed}{{8.4}{68}{Pointed \ptrons }{subsection.8.4}{}}
\@writefile{lla}{\contentsline {section}{\numberline {\crtrefnumber{ssec:pointed}}ssec:pointed}{68}{subsection.8.4}\protected@file@percent }
\newlabel{ssec:pointed@cref}{{[subsection][4][8]8.4}{[1][68][]68}{}{}{}}
\@writefile{toc}{\contentsline {subsection}{\tocsubsection {}{8.4}{Pointed pseudo-triangulations\xspace  }}{68}{subsection.8.4}\protected@file@percent }
\@writefile{loe}{\contentsline {definition}{\ifthmt@listswap Definition~8.26\else \numberline {8.26}Definition\fi }{68}{definition.8.26}\protected@file@percent }
\newlabel{dfn:MCE:ptrar}{{8.26}{68}{}{definition.8.26}{}}
\@writefile{lla}{\contentsline {section}{\numberline {\crtrefnumber{dfn:MCE:ptrar}}dfn:MCE:ptrar}{68}{definition.8.26}\protected@file@percent }
\newlabel{dfn:MCE:ptrar@cref}{{[definition][26][8]8.26}{[1][68][]68}{}{}{}}
\@writefile{loe}{\contentsline {remark}{\ifthmt@listswap Remark~8.27\else \numberline {8.27}Remark\fi }{68}{remark.8.27}\protected@file@percent }
\newlabel{rmk:MCE:angles_imply_ptrgle}{{8.27}{68}{}{remark.8.27}{}}
\@writefile{lla}{\contentsline {section}{\numberline {\crtrefnumber{rmk:MCE:angles_imply_ptrgle}}rmk:MCE:angles_imply_ptrgle}{68}{remark.8.27}\protected@file@percent }
\newlabel{rmk:MCE:angles_imply_ptrgle@cref}{{[remark][27][8]8.27}{[1][68][]68}{}{}{}}
\@writefile{loe}{\contentsline {lemma}{\ifthmt@listswap Lemma~8.28\else \numberline {8.28}Lemma\fi \thmtformatoptarg {\cite  {RSS}}}{68}{lemma.8.28}\protected@file@percent }
\newlabel{lemma:MCE:ptrar_no_chords}{{8.28}{68}{\cite {RSS}}{lemma.8.28}{}}
\@writefile{lla}{\contentsline {section}{\numberline {\crtrefnumber{lemma:MCE:ptrar_no_chords}}lemma:MCE:ptrar_no_chords}{68}{lemma.8.28}\protected@file@percent }
\newlabel{lemma:MCE:ptrar_no_chords@cref}{{[lemma][28][8]8.28}{[1][68][]68}{}{}{}}
\@writefile{loe}{\contentsline {proposition}{\ifthmt@listswap Proposition~8.29\else \numberline {8.29}Proposition\fi }{68}{proposition.8.29}\protected@file@percent }
\newlabel{lemma:MCE:ptrar_faces}{{8.29}{68}{}{proposition.8.29}{}}
\@writefile{lla}{\contentsline {section}{\numberline {\crtrefnumber{lemma:MCE:ptrar_faces}}lemma:MCE:ptrar_faces}{68}{proposition.8.29}\protected@file@percent }
\newlabel{lemma:MCE:ptrar_faces@cref}{{[proposition][29][8]8.29}{[1][68][]68}{}{}{}}
\citation{RSS}
\citation{applets}
\@writefile{lof}{\contentsline {figure}{\numberline {16}{\ignorespaces Geodesics inside a rigid non-pseudo-triangular\xspace  face $v$; see the proof of \cref  {lemma:MCE:ptrar_faces}. Here, $m$ is the number of corners $\nu $ of $v$ such that $\hat  {\alpha }(\nu )\in [0,\pi )$. }}{69}{figure.caption.24}\protected@file@percent }
\newlabel{fig:geodesics}{{16}{69}{Geodesics inside a rigid non-\ptrar face $\v $; see the proof of \cref {lemma:MCE:ptrar_faces}. Here, $m$ is the number of corners $\cor $ of $\v $ such that $\sumT (\cor )\in [0,\pi )$}{figure.caption.24}{}}
\@writefile{lla}{\contentsline {section}{\numberline {\crtrefnumber{fig:geodesics}}fig:geodesics}{69}{figure.caption.24}\protected@file@percent }
\newlabel{fig:geodesics@cref}{{[figure][16][]16}{[1][68][]69}{}{}{}}
\@writefile{loe}{\contentsline {corollary}{\ifthmt@listswap Corollary~8.30\else \numberline {8.30}Corollary\fi }{69}{corollary.8.30}\protected@file@percent }
\newlabel{lemma:MCE:face_classification}{{8.30}{69}{}{corollary.8.30}{}}
\@writefile{lla}{\contentsline {section}{\numberline {\crtrefnumber{lemma:MCE:face_classification}}lemma:MCE:face_classification}{69}{corollary.8.30}\protected@file@percent }
\newlabel{lemma:MCE:face_classification@cref}{{[corollary][30][8]8.30}{[1][69][]69}{}{}{}}
\@writefile{loe}{\contentsline {definition}{\ifthmt@listswap Definition~8.31\else \numberline {8.31}Definition\fi }{69}{definition.8.31}\protected@file@percent }
\newlabel{dfn:MCE:Vsact_Vbigons_Vtrs}{{8.31}{69}{}{definition.8.31}{}}
\@writefile{lla}{\contentsline {section}{\numberline {\crtrefnumber{dfn:MCE:Vsact_Vbigons_Vtrs}}dfn:MCE:Vsact_Vbigons_Vtrs}{69}{definition.8.31}\protected@file@percent }
\newlabel{dfn:MCE:Vsact_Vbigons_Vtrs@cref}{{[definition][31][8]8.31}{[1][69][]69}{}{}{}}
\@writefile{loe}{\contentsline {corollary}{\ifthmt@listswap Corollary~8.32\else \numberline {8.32}Corollary\fi }{69}{corollary.8.32}\protected@file@percent }
\newlabel{lemma:zero_corner=>rigid}{{8.32}{69}{}{corollary.8.32}{}}
\@writefile{lla}{\contentsline {section}{\numberline {\crtrefnumber{lemma:zero_corner=>rigid}}lemma:zero_corner=>rigid}{69}{corollary.8.32}\protected@file@percent }
\newlabel{lemma:zero_corner=>rigid@cref}{{[corollary][32][8]8.32}{[1][69][]69}{}{}{}}
\@writefile{toc}{\contentsline {section}{\tocsection {}{9}{Origami reconstruction algorithm\xspace  }}{69}{section.9}\protected@file@percent }
\newlabel{sec:ORA}{{9}{69}{\ORATITLE }{section.9}{}}
\@writefile{lla}{\contentsline {section}{\numberline {\crtrefnumber{sec:ORA}}sec:ORA}{69}{section.9}\protected@file@percent }
\newlabel{sec:ORA@cref}{{[section][9][]9}{[1][69][]69}{}{}{}}
\newlabel{sec:ORA_overview}{{9.1}{69}{Overview}{subsection.9.1}{}}
\@writefile{lla}{\contentsline {section}{\numberline {\crtrefnumber{sec:ORA_overview}}sec:ORA_overview}{69}{subsection.9.1}\protected@file@percent }
\newlabel{sec:ORA_overview@cref}{{[subsection][1][9]9.1}{[1][69][]69}{}{}{}}
\@writefile{toc}{\contentsline {subsection}{\tocsubsection {}{9.1}{Overview}}{69}{subsection.9.1}\protected@file@percent }
\@writefile{loe}{\contentsline {definition}{\ifthmt@listswap Definition~9.1\else \numberline {9.1}Definition\fi }{69}{definition.9.1}\protected@file@percent }
\newlabel{dfn:OR_move}{{9.1}{69}{}{definition.9.1}{}}
\@writefile{lla}{\contentsline {section}{\numberline {\crtrefnumber{dfn:OR_move}}dfn:OR_move}{69}{definition.9.1}\protected@file@percent }
\newlabel{dfn:OR_move@cref}{{[definition][1][9]9.1}{[1][69][]69}{}{}{}}
\newlabel{eq:Pivots_dfn}{{9.1}{70}{Overview}{equation.9.1}{}}
\@writefile{lla}{\contentsline {section}{\numberline {\crtrefnumber{eq:Pivots_dfn}}eq:Pivots_dfn}{70}{equation.9.1}\protected@file@percent }
\newlabel{eq:Pivots_dfn@cref}{{[equation][1][9]9.1}{[1][70][]70}{}{}{}}
\@writefile{loe}{\contentsline {definition}{\ifthmt@listswap Definition~9.2\else \numberline {9.2}Definition\fi \thmtformatoptarg {Folding ray}}{70}{definition.9.2}\protected@file@percent }
\newlabel{dfn:folding_ray}{{9.2}{70}{Folding ray}{definition.9.2}{}}
\@writefile{lla}{\contentsline {section}{\numberline {\crtrefnumber{dfn:folding_ray}}dfn:folding_ray}{70}{definition.9.2}\protected@file@percent }
\newlabel{dfn:folding_ray@cref}{{[definition][2][9]9.2}{[1][70][]70}{}{}{}}
\newlabel{eq:zero_type_corfpm}{{9.2}{70}{Overview}{equation.9.2}{}}
\@writefile{lla}{\contentsline {section}{\numberline {\crtrefnumber{eq:zero_type_corfpm}}eq:zero_type_corfpm}{70}{equation.9.2}\protected@file@percent }
\newlabel{eq:zero_type_corfpm@cref}{{[equation][2][9]9.2}{[1][70][]70}{}{}{}}
\newlabel{eq:rcrit_dfn}{{9.3}{70}{Overview}{equation.9.3}{}}
\@writefile{lla}{\contentsline {section}{\numberline {\crtrefnumber{eq:rcrit_dfn}}eq:rcrit_dfn}{70}{equation.9.3}\protected@file@percent }
\newlabel{eq:rcrit_dfn@cref}{{[equation][3][9]9.3}{[1][70][]70}{}{}{}}
\newlabel{sec:ORA_new_vert}{{9.2}{70}{Bounds on \texorpdfstring {$\rcrit $}{\~{$r$}}}{subsection.9.2}{}}
\@writefile{lla}{\contentsline {section}{\numberline {\crtrefnumber{sec:ORA_new_vert}}sec:ORA_new_vert}{70}{subsection.9.2}\protected@file@percent }
\newlabel{sec:ORA_new_vert@cref}{{[subsection][2][9]9.2}{[1][70][]70}{}{}{}}
\@writefile{toc}{\contentsline {subsection}{\tocsubsection {}{9.2}{Bounds on $\tilde  {r}$}}{70}{subsection.9.2}\protected@file@percent }
\@writefile{loe}{\contentsline {lemma}{\ifthmt@listswap Lemma~9.3\else \numberline {9.3}Lemma\fi }{70}{lemma.9.3}\protected@file@percent }
\newlabel{lemma:ORA:r_small}{{9.3}{70}{}{lemma.9.3}{}}
\@writefile{lla}{\contentsline {section}{\numberline {\crtrefnumber{lemma:ORA:r_small}}lemma:ORA:r_small}{70}{lemma.9.3}\protected@file@percent }
\newlabel{lemma:ORA:r_small@cref}{{[lemma][3][9]9.3}{[1][70][]70}{}{}{}}
\newlabel{eq:xTrout_geq_0}{{9.4}{70}{}{equation.9.4}{}}
\@writefile{lla}{\contentsline {section}{\numberline {\crtrefnumber{eq:xTrout_geq_0}}eq:xTrout_geq_0}{70}{equation.9.4}\protected@file@percent }
\newlabel{eq:xTrout_geq_0@cref}{{[equation][4][9]9.4}{[1][70][]70}{}{}{}}
\@writefile{lof}{\contentsline {figure}{\numberline {17}{\ignorespaces  Bending the edges of $\GDr $.}}{71}{figure.caption.25}\protected@file@percent }
\newlabel{fig:fout-bend}{{17}{71}{Bending the edges of $\protect \GDr $}{figure.caption.25}{}}
\@writefile{lla}{\contentsline {section}{\numberline {\crtrefnumber{fig:fout-bend}}fig:fout-bend}{71}{figure.caption.25}\protected@file@percent }
\newlabel{fig:fout-bend@cref}{{[figure][17][]17}{[1][71][]71}{}{}{}}
\@writefile{loe}{\contentsline {definition}{\ifthmt@listswap Definition~9.4\else \numberline {9.4}Definition\fi }{71}{definition.9.4}\protected@file@percent }
\newlabel{dfn:GDr}{{9.4}{71}{}{definition.9.4}{}}
\@writefile{lla}{\contentsline {section}{\numberline {\crtrefnumber{dfn:GDr}}dfn:GDr}{71}{definition.9.4}\protected@file@percent }
\newlabel{dfn:GDr@cref}{{[definition][4][9]9.4}{[1][71][]71}{}{}{}}
\@writefile{loe}{\contentsline {proposition}{\ifthmt@listswap Proposition~9.5\else \numberline {9.5}Proposition\fi }{71}{proposition.9.5}\protected@file@percent }
\newlabel{lemma:ORA:r_small_MCE}{{9.5}{71}{}{proposition.9.5}{}}
\@writefile{lla}{\contentsline {section}{\numberline {\crtrefnumber{lemma:ORA:r_small_MCE}}lemma:ORA:r_small_MCE}{71}{proposition.9.5}\protected@file@percent }
\newlabel{lemma:ORA:r_small_MCE@cref}{{[proposition][5][9]9.5}{[1][71][]71}{}{}{}}
\newlabel{eq:ORA:r_large}{{9.5}{72}{Bounds on \texorpdfstring {$\rcrit $}{\~{$r$}}}{equation.9.5}{}}
\@writefile{lla}{\contentsline {section}{\numberline {\crtrefnumber{eq:ORA:r_large}}eq:ORA:r_large}{72}{equation.9.5}\protected@file@percent }
\newlabel{eq:ORA:r_large@cref}{{[equation][5][9]9.5}{[1][72][]72}{}{}{}}
\@writefile{loe}{\contentsline {lemma}{\ifthmt@listswap Lemma~9.6\else \numberline {9.6}Lemma\fi }{72}{lemma.9.6}\protected@file@percent }
\newlabel{lemma:ORA:r_large_not_MCE}{{9.6}{72}{}{lemma.9.6}{}}
\@writefile{lla}{\contentsline {section}{\numberline {\crtrefnumber{lemma:ORA:r_large_not_MCE}}lemma:ORA:r_large_not_MCE}{72}{lemma.9.6}\protected@file@percent }
\newlabel{lemma:ORA:r_large_not_MCE@cref}{{[lemma][6][9]9.6}{[1][72][]72}{}{}{}}
\@writefile{loe}{\contentsline {corollary}{\ifthmt@listswap Corollary~9.7\else \numberline {9.7}Corollary\fi }{72}{corollary.9.7}\protected@file@percent }
\newlabel{lemma:ORA:correctness_vertex}{{9.7}{72}{}{corollary.9.7}{}}
\@writefile{lla}{\contentsline {section}{\numberline {\crtrefnumber{lemma:ORA:correctness_vertex}}lemma:ORA:correctness_vertex}{72}{corollary.9.7}\protected@file@percent }
\newlabel{lemma:ORA:correctness_vertex@cref}{{[corollary][7][9]9.7}{[1][72][]72}{}{}{}}
\@writefile{toc}{\contentsline {subsection}{\tocsubsection {}{9.3}{New vertex location (flexible\xspace  $\delta $)}}{72}{subsection.9.3}\protected@file@percent }
\@writefile{loe}{\contentsline {lemma}{\ifthmt@listswap Lemma~9.8\else \numberline {9.8}Lemma\fi }{72}{lemma.9.8}\protected@file@percent }
\newlabel{lemma:ORA:r_large}{{9.8}{72}{}{lemma.9.8}{}}
\@writefile{lla}{\contentsline {section}{\numberline {\crtrefnumber{lemma:ORA:r_large}}lemma:ORA:r_large}{72}{lemma.9.8}\protected@file@percent }
\newlabel{lemma:ORA:r_large@cref}{{[lemma][8][9]9.8}{[1][72][]72}{}{}{}}
\@writefile{loe}{\contentsline {corollary}{\ifthmt@listswap Corollary~9.9\else \numberline {9.9}Corollary\fi }{72}{corollary.9.9}\protected@file@percent }
\newlabel{lemma:ORA:ffout_in_xTint_corv}{{9.9}{72}{}{corollary.9.9}{}}
\@writefile{lla}{\contentsline {section}{\numberline {\crtrefnumber{lemma:ORA:ffout_in_xTint_corv}}lemma:ORA:ffout_in_xTint_corv}{72}{corollary.9.9}\protected@file@percent }
\newlabel{lemma:ORA:ffout_in_xTint_corv@cref}{{[corollary][9][9]9.9}{[1][72][]72}{}{}{}}
\@writefile{loe}{\contentsline {proposition}{\ifthmt@listswap Proposition~9.10\else \numberline {9.10}Proposition\fi }{72}{proposition.9.10}\protected@file@percent }
\newlabel{lemma:ORA:GDr_MCE1235}{{9.10}{72}{}{proposition.9.10}{}}
\@writefile{lla}{\contentsline {section}{\numberline {\crtrefnumber{lemma:ORA:GDr_MCE1235}}lemma:ORA:GDr_MCE1235}{72}{proposition.9.10}\protected@file@percent }
\newlabel{lemma:ORA:GDr_MCE1235@cref}{{[proposition][10][9]9.10}{[1][72][]72}{}{}{}}
\newlabel{eq:vertices_on_two_triangles}{{9.6}{72}{New vertex location (\flex \texorpdfstring {$\BCin $}{δ})}{equation.9.6}{}}
\@writefile{lla}{\contentsline {section}{\numberline {\crtrefnumber{eq:vertices_on_two_triangles}}eq:vertices_on_two_triangles}{72}{equation.9.6}\protected@file@percent }
\newlabel{eq:vertices_on_two_triangles@cref}{{[equation][6][9]9.6}{[1][72][]72}{}{}{}}
\newlabel{ssec:ORA:new_edges}{{9.4}{73}{Creating new edges (\flex \texorpdfstring {$\BCin $}{δ})}{subsection.9.4}{}}
\@writefile{lla}{\contentsline {section}{\numberline {\crtrefnumber{ssec:ORA:new_edges}}ssec:ORA:new_edges}{73}{subsection.9.4}\protected@file@percent }
\newlabel{ssec:ORA:new_edges@cref}{{[subsection][4][9]9.4}{[1][73][]73}{}{}{}}
\@writefile{toc}{\contentsline {subsection}{\tocsubsection {}{9.4}{Creating new edges (flexible\xspace  $\delta $)}}{73}{subsection.9.4}\protected@file@percent }
\@writefile{loe}{\contentsline {definition}{\ifthmt@listswap Definition~9.11\else \numberline {9.11}Definition\fi }{73}{definition.9.11}\protected@file@percent }
\newlabel{dfn:ORA:fmin_fmax}{{9.11}{73}{}{definition.9.11}{}}
\@writefile{lla}{\contentsline {section}{\numberline {\crtrefnumber{dfn:ORA:fmin_fmax}}dfn:ORA:fmin_fmax}{73}{definition.9.11}\protected@file@percent }
\newlabel{dfn:ORA:fmin_fmax@cref}{{[definition][11][9]9.11}{[1][73][]73}{}{}{}}
\@writefile{loe}{\contentsline {remark}{\ifthmt@listswap Remark~9.12\else \numberline {9.12}Remark\fi }{73}{remark.9.12}\protected@file@percent }
\newlabel{rmk:Ray_fall}{{9.12}{73}{}{remark.9.12}{}}
\@writefile{lla}{\contentsline {section}{\numberline {\crtrefnumber{rmk:Ray_fall}}rmk:Ray_fall}{73}{remark.9.12}\protected@file@percent }
\newlabel{rmk:Ray_fall@cref}{{[remark][12][9]9.12}{[1][73][]73}{}{}{}}
\@writefile{loe}{\contentsline {definition}{\ifthmt@listswap Definition~9.13\else \numberline {9.13}Definition\fi }{73}{definition.9.13}\protected@file@percent }
\newlabel{dfn:Kbigs}{{9.13}{73}{}{definition.9.13}{}}
\@writefile{lla}{\contentsline {section}{\numberline {\crtrefnumber{dfn:Kbigs}}dfn:Kbigs}{73}{definition.9.13}\protected@file@percent }
\newlabel{dfn:Kbigs@cref}{{[definition][13][9]9.13}{[1][73][]73}{}{}{}}
\@writefile{loe}{\contentsline {lemma}{\ifthmt@listswap Lemma~9.14\else \numberline {9.14}Lemma\fi }{73}{lemma.9.14}\protected@file@percent }
\newlabel{rmk:ffout_is_a_vertex_of_KTbig}{{9.14}{73}{}{lemma.9.14}{}}
\@writefile{lla}{\contentsline {section}{\numberline {\crtrefnumber{rmk:ffout_is_a_vertex_of_KTbig}}rmk:ffout_is_a_vertex_of_KTbig}{73}{lemma.9.14}\protected@file@percent }
\newlabel{rmk:ffout_is_a_vertex_of_KTbig@cref}{{[lemma][14][9]9.14}{[1][73][]73}{}{}{}}
\@writefile{loe}{\contentsline {lemma}{\ifthmt@listswap Lemma~9.15\else \numberline {9.15}Lemma\fi }{73}{lemma.9.15}\protected@file@percent }
\newlabel{lemma:ORA:Ksm_contained_in_clique}{{9.15}{73}{}{lemma.9.15}{}}
\@writefile{lla}{\contentsline {section}{\numberline {\crtrefnumber{lemma:ORA:Ksm_contained_in_clique}}lemma:ORA:Ksm_contained_in_clique}{73}{lemma.9.15}\protected@file@percent }
\newlabel{lemma:ORA:Ksm_contained_in_clique@cref}{{[lemma][15][9]9.15}{[1][73][]73}{}{}{}}
\@writefile{loe}{\contentsline {definition}{\ifthmt@listswap Definition~9.16\else \numberline {9.16}Definition\fi }{73}{definition.9.16}\protected@file@percent }
\@writefile{loe}{\contentsline {lemma}{\ifthmt@listswap Lemma~9.17\else \numberline {9.17}Lemma\fi }{73}{lemma.9.17}\protected@file@percent }
\newlabel{lemma:MCE:fmin_fmax_unique}{{9.17}{73}{}{lemma.9.17}{}}
\@writefile{lla}{\contentsline {section}{\numberline {\crtrefnumber{lemma:MCE:fmin_fmax_unique}}lemma:MCE:fmin_fmax_unique}{73}{lemma.9.17}\protected@file@percent }
\newlabel{lemma:MCE:fmin_fmax_unique@cref}{{[lemma][17][9]9.17}{[1][73][]73}{}{}{}}
\@writefile{lof}{\contentsline {figure}{\numberline {18}{\ignorespaces  New edges created during an origami reconstruction step\xspace  (\cref  {dfn:ORA:Chords}).}}{74}{figure.caption.26}\protected@file@percent }
\newlabel{fig:fout-cliques}{{18}{74}{New edges created during an \ORst (\cref {dfn:ORA:Chords})}{figure.caption.26}{}}
\@writefile{lla}{\contentsline {section}{\numberline {\crtrefnumber{fig:fout-cliques}}fig:fout-cliques}{74}{figure.caption.26}\protected@file@percent }
\newlabel{fig:fout-cliques@cref}{{[figure][18][]18}{[1][74][]74}{}{}{}}
\@writefile{loe}{\contentsline {definition}{\ifthmt@listswap Definition~9.18\else \numberline {9.18}Definition\fi }{74}{definition.9.18}\protected@file@percent }
\newlabel{dfn:ORA:pmspec}{{9.18}{74}{}{definition.9.18}{}}
\@writefile{lla}{\contentsline {section}{\numberline {\crtrefnumber{dfn:ORA:pmspec}}dfn:ORA:pmspec}{74}{definition.9.18}\protected@file@percent }
\newlabel{dfn:ORA:pmspec@cref}{{[definition][18][9]9.18}{[1][74][]74}{}{}{}}
\@writefile{loe}{\contentsline {definition}{\ifthmt@listswap Definition~9.19\else \numberline {9.19}Definition\fi }{74}{definition.9.19}\protected@file@percent }
\newlabel{dfn:ORA:Chords}{{9.19}{74}{}{definition.9.19}{}}
\@writefile{lla}{\contentsline {section}{\numberline {\crtrefnumber{dfn:ORA:Chords}}dfn:ORA:Chords}{74}{definition.9.19}\protected@file@percent }
\newlabel{dfn:ORA:Chords@cref}{{[definition][19][9]9.19}{[1][74][]74}{}{}{}}
\@writefile{loe}{\contentsline {lemma}{\ifthmt@listswap Lemma~9.20\else \numberline {9.20}Lemma\fi }{74}{lemma.9.20}\protected@file@percent }
\newlabel{lemma:ORA:spec}{{9.20}{74}{}{lemma.9.20}{}}
\@writefile{lla}{\contentsline {section}{\numberline {\crtrefnumber{lemma:ORA:spec}}lemma:ORA:spec}{74}{lemma.9.20}\protected@file@percent }
\newlabel{lemma:ORA:spec@cref}{{[lemma][20][9]9.20}{[1][74][]74}{}{}{}}
\newlabel{algo:spec2}{{{{(1)}}}{74}{}{Item.54}{}}
\@writefile{lla}{\contentsline {section}{\numberline {\crtrefnumber{algo:spec2}}algo:spec2}{74}{Item.54}\protected@file@percent }
\newlabel{algo:spec2@cref}{{[enumi][1][]{{(1)}}}{[1][74][]74}{}{}{}}
\newlabel{algo:spec3}{{{{(2)}}}{74}{}{Item.55}{}}
\@writefile{lla}{\contentsline {section}{\numberline {\crtrefnumber{algo:spec3}}algo:spec3}{74}{Item.55}\protected@file@percent }
\newlabel{algo:spec3@cref}{{[enumi][2][]{{(2)}}}{[1][74][]74}{}{}{}}
\newlabel{algo:spec1}{{{{(3)}}}{74}{}{Item.56}{}}
\@writefile{lla}{\contentsline {section}{\numberline {\crtrefnumber{algo:spec1}}algo:spec1}{74}{Item.56}\protected@file@percent }
\newlabel{algo:spec1@cref}{{[enumi][3][]{{(3)}}}{[1][74][]74}{}{}{}}
\newlabel{algo:spec4}{{{{(4)}}}{74}{}{Item.57}{}}
\@writefile{lla}{\contentsline {section}{\numberline {\crtrefnumber{algo:spec4}}algo:spec4}{74}{Item.57}\protected@file@percent }
\newlabel{algo:spec4@cref}{{[enumi][4][]{{(4)}}}{[1][74][]74}{}{}{}}
\newlabel{algo:spec5}{{{{(5)}}}{74}{}{Item.58}{}}
\@writefile{lla}{\contentsline {section}{\numberline {\crtrefnumber{algo:spec5}}algo:spec5}{74}{Item.58}\protected@file@percent }
\newlabel{algo:spec5@cref}{{[enumi][5][]{{(5)}}}{[1][74][]74}{}{}{}}
\@writefile{loe}{\contentsline {proposition}{\ifthmt@listswap Proposition~9.21\else \numberline {9.21}Proposition\fi }{75}{proposition.9.21}\protected@file@percent }
\newlabel{lemma:ORA:ORA_Cext_chords}{{9.21}{75}{}{proposition.9.21}{}}
\@writefile{lla}{\contentsline {section}{\numberline {\crtrefnumber{lemma:ORA:ORA_Cext_chords}}lemma:ORA:ORA_Cext_chords}{75}{proposition.9.21}\protected@file@percent }
\newlabel{lemma:ORA:ORA_Cext_chords@cref}{{[proposition][21][9]9.21}{[1][75][]75}{}{}{}}
\@writefile{loe}{\contentsline {definition}{\ifthmt@listswap Definition~9.22\else \numberline {9.22}Definition\fi }{75}{definition.9.22}\protected@file@percent }
\newlabel{dfn:GDout}{{9.22}{75}{}{definition.9.22}{}}
\@writefile{lla}{\contentsline {section}{\numberline {\crtrefnumber{dfn:GDout}}dfn:GDout}{75}{definition.9.22}\protected@file@percent }
\newlabel{dfn:GDout@cref}{{[definition][22][9]9.22}{[1][75][]75}{}{}{}}
\@writefile{loe}{\contentsline {corollary}{\ifthmt@listswap Corollary~9.23\else \numberline {9.23}Corollary\fi }{75}{corollary.9.23}\protected@file@percent }
\newlabel{lemma:ORA_output_is_MNE}{{9.23}{75}{}{corollary.9.23}{}}
\@writefile{lla}{\contentsline {section}{\numberline {\crtrefnumber{lemma:ORA_output_is_MNE}}lemma:ORA_output_is_MNE}{75}{corollary.9.23}\protected@file@percent }
\newlabel{lemma:ORA_output_is_MNE@cref}{{[corollary][23][9]9.23}{[1][75][]75}{}{}{}}
\@writefile{loe}{\contentsline {corollary}{\ifthmt@listswap Corollary~9.24\else \numberline {9.24}Corollary\fi }{75}{corollary.9.24}\protected@file@percent }
\newlabel{lemma:ORA:ORA_rigid_faces_descr}{{9.24}{75}{}{corollary.9.24}{}}
\@writefile{lla}{\contentsline {section}{\numberline {\crtrefnumber{lemma:ORA:ORA_rigid_faces_descr}}lemma:ORA:ORA_rigid_faces_descr}{75}{corollary.9.24}\protected@file@percent }
\newlabel{lemma:ORA:ORA_rigid_faces_descr@cref}{{[corollary][24][9]9.24}{[1][75][]75}{}{}{}}
\newlabel{algo_face1}{{{{(1)}}}{76}{}{Item.59}{}}
\@writefile{lla}{\contentsline {section}{\numberline {\crtrefnumber{algo_face1}}algo_face1}{76}{Item.59}\protected@file@percent }
\newlabel{algo_face1@cref}{{[enumi][1][]{{(1)}}}{[1][75][]76}{}{}{}}
\newlabel{algo_face2}{{{{(2)}}}{76}{}{Item.60}{}}
\@writefile{lla}{\contentsline {section}{\numberline {\crtrefnumber{algo_face2}}algo_face2}{76}{Item.60}\protected@file@percent }
\newlabel{algo_face2@cref}{{[enumi][2][]{{(2)}}}{[1][76][]76}{}{}{}}
\@writefile{loe}{\contentsline {definition}{\ifthmt@listswap Definition~9.25\else \numberline {9.25}Definition\fi }{76}{definition.9.25}\protected@file@percent }
\newlabel{dfn:ORA:coloring}{{9.25}{76}{}{definition.9.25}{}}
\@writefile{lla}{\contentsline {section}{\numberline {\crtrefnumber{dfn:ORA:coloring}}dfn:ORA:coloring}{76}{definition.9.25}\protected@file@percent }
\newlabel{dfn:ORA:coloring@cref}{{[definition][25][9]9.25}{[1][76][]76}{}{}{}}
\@writefile{loe}{\contentsline {proposition}{\ifthmt@listswap Proposition~9.26\else \numberline {9.26}Proposition\fi }{76}{proposition.9.26}\protected@file@percent }
\newlabel{thm:ORA_output_is_MCE}{{9.26}{76}{}{proposition.9.26}{}}
\@writefile{lla}{\contentsline {section}{\numberline {\crtrefnumber{thm:ORA_output_is_MCE}}thm:ORA_output_is_MCE}{76}{proposition.9.26}\protected@file@percent }
\newlabel{thm:ORA_output_is_MCE@cref}{{[proposition][26][9]9.26}{[1][76][]76}{}{}{}}
\@writefile{toc}{\contentsline {subsection}{\tocsubsection {}{9.5}{Comparing $\Gamma ^\ast $ and $\tilde  {\Gamma }^{\ast }$ (flexible\xspace  $\delta $)}}{76}{subsection.9.5}\protected@file@percent }
\@writefile{loe}{\contentsline {corollary}{\ifthmt@listswap Corollary~9.27\else \numberline {9.27}Corollary\fi }{76}{corollary.9.27}\protected@file@percent }
\newlabel{lemma:ORA:GDout_contains_GDr}{{9.27}{76}{}{corollary.9.27}{}}
\@writefile{lla}{\contentsline {section}{\numberline {\crtrefnumber{lemma:ORA:GDout_contains_GDr}}lemma:ORA:GDout_contains_GDr}{76}{corollary.9.27}\protected@file@percent }
\newlabel{lemma:ORA:GDout_contains_GDr@cref}{{[corollary][27][9]9.27}{[1][76][]76}{}{}{}}
\@writefile{loe}{\contentsline {lemma}{\ifthmt@listswap Lemma~9.28\else \numberline {9.28}Lemma\fi }{76}{lemma.9.28}\protected@file@percent }
\newlabel{lemma:ORA:vr_active}{{9.28}{76}{}{lemma.9.28}{}}
\@writefile{lla}{\contentsline {section}{\numberline {\crtrefnumber{lemma:ORA:vr_active}}lemma:ORA:vr_active}{76}{lemma.9.28}\protected@file@percent }
\newlabel{lemma:ORA:vr_active@cref}{{[lemma][28][9]9.28}{[1][76][]76}{}{}{}}
\@writefile{loe}{\contentsline {proposition}{\ifthmt@listswap Proposition~9.29\else \numberline {9.29}Proposition\fi }{77}{proposition.9.29}\protected@file@percent }
\newlabel{lemma:ORA:new_edge_at_least_one}{{9.29}{77}{}{proposition.9.29}{}}
\@writefile{lla}{\contentsline {section}{\numberline {\crtrefnumber{lemma:ORA:new_edge_at_least_one}}lemma:ORA:new_edge_at_least_one}{77}{proposition.9.29}\protected@file@percent }
\newlabel{lemma:ORA:new_edge_at_least_one@cref}{{[proposition][29][9]9.29}{[1][77][]77}{}{}{}}
\@writefile{loe}{\contentsline {remark}{\ifthmt@listswap Remark~9.30\else \numberline {9.30}Remark\fi }{77}{remark.9.30}\protected@file@percent }
\newlabel{rmk:one_edge}{{9.30}{77}{}{remark.9.30}{}}
\@writefile{lla}{\contentsline {section}{\numberline {\crtrefnumber{rmk:one_edge}}rmk:one_edge}{77}{remark.9.30}\protected@file@percent }
\newlabel{rmk:one_edge@cref}{{[remark][30][9]9.30}{[1][77][]77}{}{}{}}
\newlabel{ORA-single1}{{{{(1)}}}{77}{}{Item.61}{}}
\@writefile{lla}{\contentsline {section}{\numberline {\crtrefnumber{ORA-single1}}ORA-single1}{77}{Item.61}\protected@file@percent }
\newlabel{ORA-single1@cref}{{[enumi][1][]{{(1)}}}{[1][77][]77}{}{}{}}
\newlabel{ORA-single2}{{{{(2)}}}{77}{}{Item.62}{}}
\@writefile{lla}{\contentsline {section}{\numberline {\crtrefnumber{ORA-single2}}ORA-single2}{77}{Item.62}\protected@file@percent }
\newlabel{ORA-single2@cref}{{[enumi][2][]{{(2)}}}{[1][77][]77}{}{}{}}
\newlabel{ORA-single2.1p}{{{{(2.1)}}}{77}{}{Item.63}{}}
\@writefile{lla}{\contentsline {section}{\numberline {\crtrefnumber{ORA-single2.1p}}ORA-single2.1p}{77}{Item.63}\protected@file@percent }
\newlabel{ORA-single2.1p@cref}{{[enumii][1][2]{{(2.1)}}}{[1][77][]77}{}{}{}}
\newlabel{ORA-single2.1m}{{{{(2.1)}}}{77}{}{Item.63}{}}
\@writefile{lla}{\contentsline {section}{\numberline {\crtrefnumber{ORA-single2.1m}}ORA-single2.1m}{77}{Item.63}\protected@file@percent }
\newlabel{ORA-single2.1m@cref}{{[enumii][1][2]{{(2.1)}}}{[1][77][]77}{}{}{}}
\newlabel{ORA-single2.2p}{{{{(2.2)}}}{77}{}{Item.64}{}}
\@writefile{lla}{\contentsline {section}{\numberline {\crtrefnumber{ORA-single2.2p}}ORA-single2.2p}{77}{Item.64}\protected@file@percent }
\newlabel{ORA-single2.2p@cref}{{[enumii][2][2]{{(2.2)}}}{[1][77][]77}{}{}{}}
\newlabel{ORA-single2.2m}{{{{(2.2)}}}{77}{}{Item.64}{}}
\@writefile{lla}{\contentsline {section}{\numberline {\crtrefnumber{ORA-single2.2m}}ORA-single2.2m}{77}{Item.64}\protected@file@percent }
\newlabel{ORA-single2.2m@cref}{{[enumii][2][2]{{(2.2)}}}{[1][77][]77}{}{}{}}
\newlabel{ORA-single2.3p}{{{{(2.3)}}}{77}{}{Item.65}{}}
\@writefile{lla}{\contentsline {section}{\numberline {\crtrefnumber{ORA-single2.3p}}ORA-single2.3p}{77}{Item.65}\protected@file@percent }
\newlabel{ORA-single2.3p@cref}{{[enumii][3][2]{{(2.3)}}}{[1][77][]77}{}{}{}}
\newlabel{ORA-single2.3m}{{{{(2.3)}}}{77}{}{Item.65}{}}
\@writefile{lla}{\contentsline {section}{\numberline {\crtrefnumber{ORA-single2.3m}}ORA-single2.3m}{77}{Item.65}\protected@file@percent }
\newlabel{ORA-single2.3m@cref}{{[enumii][3][2]{{(2.3)}}}{[1][77][]77}{}{}{}}
\@writefile{lof}{\contentsline {figure}{\numberline {19}{\ignorespaces  Examples of (valid) rigid origami reconstruction steps\xspace  .}}{78}{figure.caption.27}\protected@file@percent }
\newlabel{fig:ORA-rigid}{{19}{78}{Examples of (valid) rigid \ORsts }{figure.caption.27}{}}
\@writefile{lla}{\contentsline {section}{\numberline {\crtrefnumber{fig:ORA-rigid}}fig:ORA-rigid}{78}{figure.caption.27}\protected@file@percent }
\newlabel{fig:ORA-rigid@cref}{{[figure][19][]19}{[1][78][]78}{}{}{}}
\newlabel{sec:ORA_TORA}{{9.6}{78}{Rigid \texorpdfstring {$\BCin $}{δ}}{subsection.9.6}{}}
\@writefile{lla}{\contentsline {section}{\numberline {\crtrefnumber{sec:ORA_TORA}}sec:ORA_TORA}{78}{subsection.9.6}\protected@file@percent }
\newlabel{sec:ORA_TORA@cref}{{[subsection][6][9]9.6}{[1][77][]78}{}{}{}}
\@writefile{toc}{\contentsline {subsection}{\tocsubsection {}{9.6}{Rigid $\delta $}}{78}{subsection.9.6}\protected@file@percent }
\@writefile{loe}{\contentsline {lemma}{\ifthmt@listswap Lemma~9.31\else \numberline {9.31}Lemma\fi }{78}{lemma.9.31}\protected@file@percent }
\newlabel{lemma:ORA:rigid_lines}{{9.31}{78}{}{lemma.9.31}{}}
\@writefile{lla}{\contentsline {section}{\numberline {\crtrefnumber{lemma:ORA:rigid_lines}}lemma:ORA:rigid_lines}{78}{lemma.9.31}\protected@file@percent }
\newlabel{lemma:ORA:rigid_lines@cref}{{[lemma][31][9]9.31}{[1][78][]78}{}{}{}}
\newlabel{eq:ORA:new_ptrgle}{{9.7}{78}{}{equation.9.7}{}}
\@writefile{lla}{\contentsline {section}{\numberline {\crtrefnumber{eq:ORA:new_ptrgle}}eq:ORA:new_ptrgle}{78}{equation.9.7}\protected@file@percent }
\newlabel{eq:ORA:new_ptrgle@cref}{{[equation][7][9]9.7}{[1][78][]78}{}{}{}}
\newlabel{ptrgle_char1}{{{{(1)}}}{78}{Rigid \texorpdfstring {$\BCin $}{δ}}{Item.66}{}}
\@writefile{lla}{\contentsline {section}{\numberline {\crtrefnumber{ptrgle_char1}}ptrgle_char1}{78}{Item.66}\protected@file@percent }
\newlabel{ptrgle_char1@cref}{{[enumi][1][]{{(1)}}}{[1][78][]78}{}{}{}}
\newlabel{ptrgle_char2}{{{{(2)}}}{78}{Rigid \texorpdfstring {$\BCin $}{δ}}{Item.67}{}}
\@writefile{lla}{\contentsline {section}{\numberline {\crtrefnumber{ptrgle_char2}}ptrgle_char2}{78}{Item.67}\protected@file@percent }
\newlabel{ptrgle_char2@cref}{{[enumi][2][]{{(2)}}}{[1][78][]78}{}{}{}}
\newlabel{eq:ptrgle_char2}{{9.8}{78}{Rigid \texorpdfstring {$\BCin $}{δ}}{equation.9.8}{}}
\@writefile{lla}{\contentsline {section}{\numberline {\crtrefnumber{eq:ptrgle_char2}}eq:ptrgle_char2}{78}{equation.9.8}\protected@file@percent }
\newlabel{eq:ptrgle_char2@cref}{{[equation][8][9]9.8}{[1][78][]78}{}{}{}}
\@writefile{loe}{\contentsline {definition}{\ifthmt@listswap Definition~9.32\else \numberline {9.32}Definition\fi }{78}{definition.9.32}\protected@file@percent }
\newlabel{dfn:ORA:col_of_v}{{9.32}{78}{}{definition.9.32}{}}
\@writefile{lla}{\contentsline {section}{\numberline {\crtrefnumber{dfn:ORA:col_of_v}}dfn:ORA:col_of_v}{78}{definition.9.32}\protected@file@percent }
\newlabel{dfn:ORA:col_of_v@cref}{{[definition][32][9]9.32}{[1][78][]78}{}{}{}}
\@writefile{loe}{\contentsline {definition}{\ifthmt@listswap Definition~9.33\else \numberline {9.33}Definition\fi }{78}{definition.9.33}\protected@file@percent }
\newlabel{dfn:ORA:rigid_ORst_descr}{{9.33}{78}{}{definition.9.33}{}}
\@writefile{lla}{\contentsline {section}{\numberline {\crtrefnumber{dfn:ORA:rigid_ORst_descr}}dfn:ORA:rigid_ORst_descr}{78}{definition.9.33}\protected@file@percent }
\newlabel{dfn:ORA:rigid_ORst_descr@cref}{{[definition][33][9]9.33}{[1][78][]78}{}{}{}}
\newlabel{eq:ORA:rigid_ORst_descr}{{9.9}{79}{}{equation.9.9}{}}
\@writefile{lla}{\contentsline {section}{\numberline {\crtrefnumber{eq:ORA:rigid_ORst_descr}}eq:ORA:rigid_ORst_descr}{79}{equation.9.9}\protected@file@percent }
\newlabel{eq:ORA:rigid_ORst_descr@cref}{{[equation][9][9]9.9}{[1][78][]79}{}{}{}}
\@writefile{loe}{\contentsline {lemma}{\ifthmt@listswap Lemma~9.34\else \numberline {9.34}Lemma\fi }{79}{lemma.9.34}\protected@file@percent }
\newlabel{lemma:ORA:rigid_Chords}{{9.34}{79}{}{lemma.9.34}{}}
\@writefile{lla}{\contentsline {section}{\numberline {\crtrefnumber{lemma:ORA:rigid_Chords}}lemma:ORA:rigid_Chords}{79}{lemma.9.34}\protected@file@percent }
\newlabel{lemma:ORA:rigid_Chords@cref}{{[lemma][34][9]9.34}{[1][79][]79}{}{}{}}
\@writefile{loe}{\contentsline {definition}{\ifthmt@listswap Definition~9.35\else \numberline {9.35}Definition\fi }{79}{definition.9.35}\protected@file@percent }
\newlabel{dfn:ORA:rigid_GDout_descr}{{9.35}{79}{}{definition.9.35}{}}
\@writefile{lla}{\contentsline {section}{\numberline {\crtrefnumber{dfn:ORA:rigid_GDout_descr}}dfn:ORA:rigid_GDout_descr}{79}{definition.9.35}\protected@file@percent }
\newlabel{dfn:ORA:rigid_GDout_descr@cref}{{[definition][35][9]9.35}{[1][79][]79}{}{}{}}
\@writefile{loe}{\contentsline {corollary}{\ifthmt@listswap Corollary~9.36\else \numberline {9.36}Corollary\fi }{79}{corollary.9.36}\protected@file@percent }
\newlabel{lemma:ORA:rigid_MCNE=>MCNE}{{9.36}{79}{}{corollary.9.36}{}}
\@writefile{lla}{\contentsline {section}{\numberline {\crtrefnumber{lemma:ORA:rigid_MCNE=>MCNE}}lemma:ORA:rigid_MCNE=>MCNE}{79}{corollary.9.36}\protected@file@percent }
\newlabel{lemma:ORA:rigid_MCNE=>MCNE@cref}{{[corollary][36][9]9.36}{[1][79][]79}{}{}{}}
\@writefile{loe}{\contentsline {lemma}{\ifthmt@listswap Lemma~9.37\else \numberline {9.37}Lemma\fi }{79}{lemma.9.37}\protected@file@percent }
\newlabel{lemma:ORA:rigid_rcrit_vs_GDr}{{9.37}{79}{}{lemma.9.37}{}}
\@writefile{lla}{\contentsline {section}{\numberline {\crtrefnumber{lemma:ORA:rigid_rcrit_vs_GDr}}lemma:ORA:rigid_rcrit_vs_GDr}{79}{lemma.9.37}\protected@file@percent }
\newlabel{lemma:ORA:rigid_rcrit_vs_GDr@cref}{{[lemma][37][9]9.37}{[1][79][]79}{}{}{}}
\@writefile{loe}{\contentsline {lemma}{\ifthmt@listswap Lemma~9.38\else \numberline {9.38}Lemma\fi }{80}{lemma.9.38}\protected@file@percent }
\newlabel{lemma:ORA:rigid_admits_valid_ORst}{{9.38}{80}{}{lemma.9.38}{}}
\@writefile{lla}{\contentsline {section}{\numberline {\crtrefnumber{lemma:ORA:rigid_admits_valid_ORst}}lemma:ORA:rigid_admits_valid_ORst}{80}{lemma.9.38}\protected@file@percent }
\newlabel{lemma:ORA:rigid_admits_valid_ORst@cref}{{[lemma][38][9]9.38}{[1][80][]80}{}{}{}}
\@writefile{loe}{\contentsline {definition}{\ifthmt@listswap Definition~9.39\else \numberline {9.39}Definition\fi }{80}{definition.9.39}\protected@file@percent }
\newlabel{dfn:convex_rigid_face}{{9.39}{80}{}{definition.9.39}{}}
\@writefile{lla}{\contentsline {section}{\numberline {\crtrefnumber{dfn:convex_rigid_face}}dfn:convex_rigid_face}{80}{definition.9.39}\protected@file@percent }
\newlabel{dfn:convex_rigid_face@cref}{{[definition][39][9]9.39}{[1][80][]80}{}{}{}}
\@writefile{loe}{\contentsline {lemma}{\ifthmt@listswap Lemma~9.40\else \numberline {9.40}Lemma\fi }{80}{lemma.9.40}\protected@file@percent }
\newlabel{lemma:ORA:iccar_valid}{{9.40}{80}{}{lemma.9.40}{}}
\@writefile{lla}{\contentsline {section}{\numberline {\crtrefnumber{lemma:ORA:iccar_valid}}lemma:ORA:iccar_valid}{80}{lemma.9.40}\protected@file@percent }
\newlabel{lemma:ORA:iccar_valid@cref}{{[lemma][40][9]9.40}{[1][80][]80}{}{}{}}
\newlabel{eq:ass_ptrar}{{9.10}{80}{}{equation.9.10}{}}
\@writefile{lla}{\contentsline {section}{\numberline {\crtrefnumber{eq:ass_ptrar}}eq:ass_ptrar}{80}{equation.9.10}\protected@file@percent }
\newlabel{eq:ass_ptrar@cref}{{[equation][10][9]9.10}{[1][80][]80}{}{}{}}
\newlabel{sec:ORA_terminates}{{9.7}{80}{Uniqueness and termination}{subsection.9.7}{}}
\@writefile{lla}{\contentsline {section}{\numberline {\crtrefnumber{sec:ORA_terminates}}sec:ORA_terminates}{80}{subsection.9.7}\protected@file@percent }
\newlabel{sec:ORA_terminates@cref}{{[subsection][7][9]9.7}{[1][80][]80}{}{}{}}
\@writefile{toc}{\contentsline {subsection}{\tocsubsection {}{9.7}{Uniqueness and termination}}{80}{subsection.9.7}\protected@file@percent }
\@writefile{loe}{\contentsline {proposition}{\ifthmt@listswap Proposition~9.41\else \numberline {9.41}Proposition\fi }{80}{proposition.9.41}\protected@file@percent }
\newlabel{lemma:ORA:uniqueness}{{9.41}{80}{}{proposition.9.41}{}}
\@writefile{lla}{\contentsline {section}{\numberline {\crtrefnumber{lemma:ORA:uniqueness}}lemma:ORA:uniqueness}{80}{proposition.9.41}\protected@file@percent }
\newlabel{lemma:ORA:uniqueness@cref}{{[proposition][41][9]9.41}{[1][80][]80}{}{}{}}
\citation{Pos_ICM}
\@writefile{loe}{\contentsline {theorem}{\ifthmt@listswap Theorem~9.42\else \numberline {9.42}Theorem\fi }{81}{theorem.9.42}\protected@file@percent }
\newlabel{lemma:ORA:ORA_termination}{{9.42}{81}{}{theorem.9.42}{}}
\@writefile{lla}{\contentsline {section}{\numberline {\crtrefnumber{lemma:ORA:ORA_termination}}lemma:ORA:ORA_termination}{81}{theorem.9.42}\protected@file@percent }
\newlabel{lemma:ORA:ORA_termination@cref}{{[theorem][42][9]9.42}{[1][81][]81}{}{}{}}
\@writefile{toc}{\contentsline {part}{\tocpart {Part}{3}{BCFW tilings}}{81}{part.3}\protected@file@percent }
\newlabel{part3}{{3}{81}{BCFW tilings}{part.3}{}}
\@writefile{lla}{\contentsline {section}{\numberline {\crtrefnumber{part3}}part3}{81}{part.3}\protected@file@percent }
\newlabel{part3@cref}{{[part][3][]3}{[1][81][]81}{}{}{}}
\@writefile{toc}{\contentsline {section}{\tocsection {}{10}{Mandelstam-convex\xspace  moduli spaces\xspace  }}{81}{section.10}\protected@file@percent }
\newlabel{sec:MCMS}{{10}{81}{\MCMSsTITLE }{section.10}{}}
\@writefile{lla}{\contentsline {section}{\numberline {\crtrefnumber{sec:MCMS}}sec:MCMS}{81}{section.10}\protected@file@percent }
\newlabel{sec:MCMS@cref}{{[section][10][]10}{[1][81][]81}{}{}{}}
\newlabel{ssec:MCMS:lggs}{{10.1}{81}{\LggsTITLE }{subsection.10.1}{}}
\@writefile{lla}{\contentsline {section}{\numberline {\crtrefnumber{ssec:MCMS:lggs}}ssec:MCMS:lggs}{81}{subsection.10.1}\protected@file@percent }
\newlabel{ssec:MCMS:lggs@cref}{{[subsection][1][10]10.1}{[1][81][]81}{}{}{}}
\@writefile{toc}{\contentsline {subsection}{\tocsubsection {}{10.1}{$L^\ast $-punctured\xspace  Grassmannian graphs\xspace  }}{81}{subsection.10.1}\protected@file@percent }
\@writefile{loe}{\contentsline {definition}{\ifthmt@listswap Definition~10.1\else \numberline {10.1}Definition\fi }{81}{definition.10.1}\protected@file@percent }
\citation{Hakimi}
\citation{Hakimi}
\citation{Hakimi}
\citation{Pos_ICM}
\citation{Pos_ICM}
\newlabel{eq:BCFW:helW+helB=deg}{{10.1}{82}{}{equation.10.1}{}}
\@writefile{lla}{\contentsline {section}{\numberline {\crtrefnumber{eq:BCFW:helW+helB=deg}}eq:BCFW:helW+helB=deg}{82}{equation.10.1}\protected@file@percent }
\newlabel{eq:BCFW:helW+helB=deg@cref}{{[equation][1][10]10.1}{[1][81][]82}{}{}{}}
\newlabel{eq:BCFW:sum_helW_helB=Egen}{{10.2}{82}{}{equation.10.2}{}}
\@writefile{lla}{\contentsline {section}{\numberline {\crtrefnumber{eq:BCFW:sum_helW_helB=Egen}}eq:BCFW:sum_helW_helB=Egen}{82}{equation.10.2}\protected@file@percent }
\newlabel{eq:BCFW:sum_helW_helB=Egen@cref}{{[equation][2][10]10.2}{[1][81][]82}{}{}{}}
\newlabel{eq:BCFW:helWgen=helBgen=0}{{10.3}{82}{\LggsTITLE }{equation.10.3}{}}
\@writefile{lla}{\contentsline {section}{\numberline {\crtrefnumber{eq:BCFW:helWgen=helBgen=0}}eq:BCFW:helWgen=helBgen=0}{82}{equation.10.3}\protected@file@percent }
\newlabel{eq:BCFW:helWgen=helBgen=0@cref}{{[equation][3][10]10.3}{[1][82][]82}{}{}{}}
\@writefile{loe}{\contentsline {lemma}{\ifthmt@listswap Lemma~10.2\else \numberline {10.2}Lemma\fi }{82}{lemma.10.2}\protected@file@percent }
\newlabel{lemma:BCFW:Rg_vs_Rg'_helW_vs_helB}{{10.2}{82}{}{lemma.10.2}{}}
\@writefile{lla}{\contentsline {section}{\numberline {\crtrefnumber{lemma:BCFW:Rg_vs_Rg'_helW_vs_helB}}lemma:BCFW:Rg_vs_Rg'_helW_vs_helB}{82}{lemma.10.2}\protected@file@percent }
\newlabel{lemma:BCFW:Rg_vs_Rg'_helW_vs_helB@cref}{{[lemma][2][10]10.2}{[1][82][]82}{}{}{}}
\newlabel{eq:BCFW:Rg_vs_Rg'_helW_vs_helB}{{10.4}{82}{}{equation.10.4}{}}
\@writefile{lla}{\contentsline {section}{\numberline {\crtrefnumber{eq:BCFW:Rg_vs_Rg'_helW_vs_helB}}eq:BCFW:Rg_vs_Rg'_helW_vs_helB}{82}{equation.10.4}\protected@file@percent }
\newlabel{eq:BCFW:Rg_vs_Rg'_helW_vs_helB@cref}{{[equation][4][10]10.4}{[1][82][]82}{}{}{}}
\@writefile{loe}{\contentsline {corollary}{\ifthmt@listswap Corollary~10.3\else \numberline {10.3}Corollary\fi }{82}{corollary.10.3}\protected@file@percent }
\newlabel{eq:BCFW:helWgen_Rc=helBgen_R}{{10.5}{82}{}{equation.10.5}{}}
\@writefile{lla}{\contentsline {section}{\numberline {\crtrefnumber{eq:BCFW:helWgen_Rc=helBgen_R}}eq:BCFW:helWgen_Rc=helBgen_R}{82}{equation.10.5}\protected@file@percent }
\newlabel{eq:BCFW:helWgen_Rc=helBgen_R@cref}{{[equation][5][10]10.5}{[1][82][]82}{}{}{}}
\newlabel{eq:BCFW:helWmin_dfn}{{10.6}{82}{\LggsTITLE }{equation.10.6}{}}
\@writefile{lla}{\contentsline {section}{\numberline {\crtrefnumber{eq:BCFW:helWmin_dfn}}eq:BCFW:helWmin_dfn}{82}{equation.10.6}\protected@file@percent }
\newlabel{eq:BCFW:helWmin_dfn@cref}{{[equation][6][10]10.6}{[1][82][]82}{}{}{}}
\@writefile{loe}{\contentsline {proposition}{\ifthmt@listswap Proposition~10.4\else \numberline {10.4}Proposition\fi \thmtformatoptarg {\cite  [Theorem~4]{Hakimi}}}{82}{proposition.10.4}\protected@file@percent }
\newlabel{lemma:OCP:Hakimi}{{10.4}{82}{\cite [Theorem~4]{Hakimi}}{proposition.10.4}{}}
\@writefile{lla}{\contentsline {section}{\numberline {\crtrefnumber{lemma:OCP:Hakimi}}lemma:OCP:Hakimi}{82}{proposition.10.4}\protected@file@percent }
\newlabel{lemma:OCP:Hakimi@cref}{{[proposition][4][10]10.4}{[1][82][]82}{}{}{}}
\@writefile{loe}{\contentsline {definition}{\ifthmt@listswap Definition~10.5\else \numberline {10.5}Definition\fi \thmtformatoptarg {\cite  [Definition~4.1]{Pos_ICM}}}{82}{definition.10.5}\protected@file@percent }
\newlabel{eq:BCFW:k(G)_dfn}{{10.7}{82}{\LggsTITLE }{equation.10.7}{}}
\@writefile{lla}{\contentsline {section}{\numberline {\crtrefnumber{eq:BCFW:k(G)_dfn}}eq:BCFW:k(G)_dfn}{82}{equation.10.7}\protected@file@percent }
\newlabel{eq:BCFW:k(G)_dfn@cref}{{[equation][7][10]10.7}{[1][82][]82}{}{}{}}
\@writefile{loe}{\contentsline {remark}{\ifthmt@listswap Remark~10.6\else \numberline {10.6}Remark\fi }{82}{remark.10.6}\protected@file@percent }
\newlabel{rmk:BCFW:gluing_bdv_into_bdvall}{{10.6}{82}{}{remark.10.6}{}}
\@writefile{lla}{\contentsline {section}{\numberline {\crtrefnumber{rmk:BCFW:gluing_bdv_into_bdvall}}rmk:BCFW:gluing_bdv_into_bdvall}{82}{remark.10.6}\protected@file@percent }
\newlabel{rmk:BCFW:gluing_bdv_into_bdvall@cref}{{[remark][6][10]10.6}{[1][82][]82}{}{}{}}
\citation{Pos}
\@writefile{loe}{\contentsline {corollary}{\ifthmt@listswap Corollary~10.7\else \numberline {10.7}Corollary\fi }{83}{corollary.10.7}\protected@file@percent }
\newlabel{lemma:OCP:Hakimi_cor}{{10.7}{83}{}{corollary.10.7}{}}
\@writefile{lla}{\contentsline {section}{\numberline {\crtrefnumber{lemma:OCP:Hakimi_cor}}lemma:OCP:Hakimi_cor}{83}{corollary.10.7}\protected@file@percent }
\newlabel{lemma:OCP:Hakimi_cor@cref}{{[corollary][7][10]10.7}{[1][83][]83}{}{}{}}
\@writefile{loe}{\contentsline {definition}{\ifthmt@listswap Definition~10.8\else \numberline {10.8}Definition\fi }{83}{definition.10.8}\protected@file@percent }
\newlabel{dfn:ORA:black_white_verts}{{10.8}{83}{}{definition.10.8}{}}
\@writefile{lla}{\contentsline {section}{\numberline {\crtrefnumber{dfn:ORA:black_white_verts}}dfn:ORA:black_white_verts}{83}{definition.10.8}\protected@file@percent }
\newlabel{dfn:ORA:black_white_verts@cref}{{[definition][8][10]10.8}{[1][83][]83}{}{}{}}
\@writefile{loe}{\contentsline {definition}{\ifthmt@listswap Definition~10.9\else \numberline {10.9}Definition\fi }{83}{definition.10.9}\protected@file@percent }
\newlabel{dfn:BCFW:terminal}{{10.9}{83}{}{definition.10.9}{}}
\@writefile{lla}{\contentsline {section}{\numberline {\crtrefnumber{dfn:BCFW:terminal}}dfn:BCFW:terminal}{83}{definition.10.9}\protected@file@percent }
\newlabel{dfn:BCFW:terminal@cref}{{[definition][9][10]10.9}{[1][83][]83}{}{}{}}
\@writefile{loe}{\contentsline {remark}{\ifthmt@listswap Remark~10.10\else \numberline {10.10}Remark\fi }{83}{remark.10.10}\protected@file@percent }
\newlabel{rmk:BCFW:terminal_vs_plabic_vs_plabip}{{10.10}{83}{}{remark.10.10}{}}
\@writefile{lla}{\contentsline {section}{\numberline {\crtrefnumber{rmk:BCFW:terminal_vs_plabic_vs_plabip}}rmk:BCFW:terminal_vs_plabic_vs_plabip}{83}{remark.10.10}\protected@file@percent }
\newlabel{rmk:BCFW:terminal_vs_plabic_vs_plabip@cref}{{[remark][10][10]10.10}{[1][83][]83}{}{}{}}
\@writefile{loe}{\contentsline {definition}{\ifthmt@listswap Definition~10.11\else \numberline {10.11}Definition\fi }{83}{definition.10.11}\protected@file@percent }
\newlabel{dfn:BCFW:lgg}{{10.11}{83}{}{definition.10.11}{}}
\@writefile{lla}{\contentsline {section}{\numberline {\crtrefnumber{dfn:BCFW:lgg}}dfn:BCFW:lgg}{83}{definition.10.11}\protected@file@percent }
\newlabel{dfn:BCFW:lgg@cref}{{[definition][11][10]10.11}{[1][83][]83}{}{}{}}
\newlabel{lgg1}{{{{(1)}}}{83}{}{Item.68}{}}
\@writefile{lla}{\contentsline {section}{\numberline {\crtrefnumber{lgg1}}lgg1}{83}{Item.68}\protected@file@percent }
\newlabel{lgg1@cref}{{[enumi][1][]{{(1)}}}{[1][83][]83}{}{}{}}
\newlabel{lgg2}{{{{(2)}}}{83}{}{Item.69}{}}
\@writefile{lla}{\contentsline {section}{\numberline {\crtrefnumber{lgg2}}lgg2}{83}{Item.69}\protected@file@percent }
\newlabel{lgg2@cref}{{[enumi][2][]{{(2)}}}{[1][83][]83}{}{}{}}
\newlabel{lgg3}{{{{(3)}}}{83}{}{Item.70}{}}
\@writefile{lla}{\contentsline {section}{\numberline {\crtrefnumber{lgg3}}lgg3}{83}{Item.70}\protected@file@percent }
\newlabel{lgg3@cref}{{[enumi][3][]{{(3)}}}{[1][83][]83}{}{}{}}
\@writefile{loe}{\contentsline {definition}{\ifthmt@listswap Definition~10.12\else \numberline {10.12}Definition\fi }{83}{definition.10.12}\protected@file@percent }
\newlabel{dfn:BCFW:lgg_dual}{{10.12}{83}{}{definition.10.12}{}}
\@writefile{lla}{\contentsline {section}{\numberline {\crtrefnumber{dfn:BCFW:lgg_dual}}dfn:BCFW:lgg_dual}{83}{definition.10.12}\protected@file@percent }
\newlabel{dfn:BCFW:lgg_dual@cref}{{[definition][12][10]10.12}{[1][83][]83}{}{}{}}
\@writefile{loe}{\contentsline {assumption}{\ifthmt@listswap Assumption~B\else \numberline {B}Assumption\fi }{83}{assumption.2}\protected@file@percent }
\newlabel{ass:lgg}{{B}{83}{}{assumption.2}{}}
\@writefile{lla}{\contentsline {section}{\numberline {\crtrefnumber{ass:lgg}}ass:lgg}{83}{assumption.2}\protected@file@percent }
\newlabel{ass:lgg@cref}{{[assumption][2][]B}{[1][83][]83}{}{}{}}
\newlabel{eq:ass_lgg}{{10.8}{83}{}{equation.10.8}{}}
\@writefile{lla}{\contentsline {section}{\numberline {\crtrefnumber{eq:ass_lgg}}eq:ass_lgg}{83}{equation.10.8}\protected@file@percent }
\newlabel{eq:ass_lgg@cref}{{[equation][8][10]10.8}{[1][83][]83}{}{}{}}
\@writefile{loe}{\contentsline {remark}{\ifthmt@listswap Remark~10.13\else \numberline {10.13}Remark\fi }{83}{remark.10.13}\protected@file@percent }
\newlabel{rmk:Vsact=Vfat}{{10.13}{83}{}{remark.10.13}{}}
\@writefile{lla}{\contentsline {section}{\numberline {\crtrefnumber{rmk:Vsact=Vfat}}rmk:Vsact=Vfat}{83}{remark.10.13}\protected@file@percent }
\newlabel{rmk:Vsact=Vfat@cref}{{[remark][13][10]10.13}{[1][83][]83}{}{}{}}
\@writefile{loe}{\contentsline {corollary}{\ifthmt@listswap Corollary~10.14\else \numberline {10.14}Corollary\fi }{83}{corollary.10.14}\protected@file@percent }
\newlabel{lemma:BCFW:ass_on_GD}{{10.14}{83}{}{corollary.10.14}{}}
\@writefile{lla}{\contentsline {section}{\numberline {\crtrefnumber{lemma:BCFW:ass_on_GD}}lemma:BCFW:ass_on_GD}{83}{corollary.10.14}\protected@file@percent }
\newlabel{lemma:BCFW:ass_on_GD@cref}{{[corollary][14][10]10.14}{[1][83][]83}{}{}{}}
\@writefile{loe}{\contentsline {remark}{\ifthmt@listswap Remark~10.15\else \numberline {10.15}Remark\fi }{84}{remark.10.15}\protected@file@percent }
\newlabel{rmk:BCFW:ass_propagates}{{10.15}{84}{}{remark.10.15}{}}
\@writefile{lla}{\contentsline {section}{\numberline {\crtrefnumber{rmk:BCFW:ass_propagates}}rmk:BCFW:ass_propagates}{84}{remark.10.15}\protected@file@percent }
\newlabel{rmk:BCFW:ass_propagates@cref}{{[remark][15][10]10.15}{[1][83][]84}{}{}{}}
\@writefile{loe}{\contentsline {remark}{\ifthmt@listswap Remark~10.16\else \numberline {10.16}Remark\fi }{84}{remark.10.16}\protected@file@percent }
\newlabel{rmk:BCFW:dual_loop_data_extraction}{{10.16}{84}{}{remark.10.16}{}}
\@writefile{lla}{\contentsline {section}{\numberline {\crtrefnumber{rmk:BCFW:dual_loop_data_extraction}}rmk:BCFW:dual_loop_data_extraction}{84}{remark.10.16}\protected@file@percent }
\newlabel{rmk:BCFW:dual_loop_data_extraction@cref}{{[remark][16][10]10.16}{[1][84][]84}{}{}{}}
\@writefile{toc}{\contentsline {subsection}{\tocsubsection {}{10.2}{M-convex\xspace  moduli spaces\xspace  }}{84}{subsection.10.2}\protected@file@percent }
\@writefile{loe}{\contentsline {definition}{\ifthmt@listswap Definition~10.17\else \numberline {10.17}Definition\fi \thmtformatoptarg {M-convex\xspace  moduli space\xspace  }}{84}{definition.10.17}\protected@file@percent }
\newlabel{dfn:BCFW:MCE_compatible}{{10.17}{84}{\MCMS }{definition.10.17}{}}
\@writefile{lla}{\contentsline {section}{\numberline {\crtrefnumber{dfn:BCFW:MCE_compatible}}dfn:BCFW:MCE_compatible}{84}{definition.10.17}\protected@file@percent }
\newlabel{dfn:BCFW:MCE_compatible@cref}{{[definition][17][10]10.17}{[1][84][]84}{}{}{}}
\newlabel{eq:MCMS_angles_vs_k}{{10.9}{84}{\MCMS }{equation.10.9}{}}
\@writefile{lla}{\contentsline {section}{\numberline {\crtrefnumber{eq:MCMS_angles_vs_k}}eq:MCMS_angles_vs_k}{84}{equation.10.9}\protected@file@percent }
\newlabel{eq:MCMS_angles_vs_k@cref}{{[equation][9][10]10.9}{[1][84][]84}{}{}{}}
\@writefile{loe}{\contentsline {lemma}{\ifthmt@listswap Lemma~10.18\else \numberline {10.18}Lemma\fi }{84}{lemma.10.18}\protected@file@percent }
\newlabel{lemma:BCFW:from_MCM_to_Glout}{{10.18}{84}{}{lemma.10.18}{}}
\@writefile{lla}{\contentsline {section}{\numberline {\crtrefnumber{lemma:BCFW:from_MCM_to_Glout}}lemma:BCFW:from_MCM_to_Glout}{84}{lemma.10.18}\protected@file@percent }
\newlabel{lemma:BCFW:from_MCM_to_Glout@cref}{{[lemma][18][10]10.18}{[1][84][]84}{}{}{}}
\@writefile{loe}{\contentsline {lemma}{\ifthmt@listswap Lemma~10.19\else \numberline {10.19}Lemma\fi }{84}{lemma.10.19}\protected@file@percent }
\newlabel{lemma:BCFW:ptrar_face_k=2}{{10.19}{84}{}{lemma.10.19}{}}
\@writefile{lla}{\contentsline {section}{\numberline {\crtrefnumber{lemma:BCFW:ptrar_face_k=2}}lemma:BCFW:ptrar_face_k=2}{84}{lemma.10.19}\protected@file@percent }
\newlabel{lemma:BCFW:ptrar_face_k=2@cref}{{[lemma][19][10]10.19}{[1][84][]84}{}{}{}}
\@writefile{loe}{\contentsline {remark}{\ifthmt@listswap Remark~10.20\else \numberline {10.20}Remark\fi }{84}{remark.10.20}\protected@file@percent }
\citation{origami1}
\@writefile{loe}{\contentsline {notation}{\ifthmt@listswap Notation~10.21\else \numberline {10.21}Notation\fi }{85}{notation.10.21}\protected@file@percent }
\newlabel{notn:RgFbd}{{10.21}{85}{}{notation.10.21}{}}
\@writefile{lla}{\contentsline {section}{\numberline {\crtrefnumber{notn:RgFbd}}notn:RgFbd}{85}{notation.10.21}\protected@file@percent }
\newlabel{notn:RgFbd@cref}{{[notation][21][10]10.21}{[1][85][]85}{}{}{}}
\@writefile{loe}{\contentsline {lemma}{\ifthmt@listswap Lemma~10.22\else \numberline {10.22}Lemma\fi }{85}{lemma.10.22}\protected@file@percent }
\newlabel{lemma:Rg_sum_bd_vs_chi}{{10.22}{85}{}{lemma.10.22}{}}
\@writefile{lla}{\contentsline {section}{\numberline {\crtrefnumber{lemma:Rg_sum_bd_vs_chi}}lemma:Rg_sum_bd_vs_chi}{85}{lemma.10.22}\protected@file@percent }
\newlabel{lemma:Rg_sum_bd_vs_chi@cref}{{[lemma][22][10]10.22}{[1][85][]85}{}{}{}}
\newlabel{eq:Rg_sum_bd_vs_chi}{{10.10}{85}{}{equation.10.10}{}}
\@writefile{lla}{\contentsline {section}{\numberline {\crtrefnumber{eq:Rg_sum_bd_vs_chi}}eq:Rg_sum_bd_vs_chi}{85}{equation.10.10}\protected@file@percent }
\newlabel{eq:Rg_sum_bd_vs_chi@cref}{{[equation][10][10]10.10}{[1][85][]85}{}{}{}}
\newlabel{eq:BCFW:sumbT_vs_chi}{{10.11}{85}{\MCMSs }{equation.10.11}{}}
\@writefile{lla}{\contentsline {section}{\numberline {\crtrefnumber{eq:BCFW:sumbT_vs_chi}}eq:BCFW:sumbT_vs_chi}{85}{equation.10.11}\protected@file@percent }
\newlabel{eq:BCFW:sumbT_vs_chi@cref}{{[equation][11][10]10.11}{[1][85][]85}{}{}{}}
\newlabel{eq:BCFW:sumbT_vs_RgFint}{{10.12}{85}{\MCMSs }{equation.10.12}{}}
\@writefile{lla}{\contentsline {section}{\numberline {\crtrefnumber{eq:BCFW:sumbT_vs_RgFint}}eq:BCFW:sumbT_vs_RgFint}{85}{equation.10.12}\protected@file@percent }
\newlabel{eq:BCFW:sumbT_vs_RgFint@cref}{{[equation][12][10]10.12}{[1][85][]85}{}{}{}}
\@writefile{loe}{\contentsline {corollary}{\ifthmt@listswap Corollary~10.23\else \numberline {10.23}Corollary\fi }{85}{corollary.10.23}\protected@file@percent }
\newlabel{lemma:BCFW:MCM_nonempty=>hel>=1}{{10.23}{85}{}{corollary.10.23}{}}
\@writefile{lla}{\contentsline {section}{\numberline {\crtrefnumber{lemma:BCFW:MCM_nonempty=>hel>=1}}lemma:BCFW:MCM_nonempty=>hel>=1}{85}{corollary.10.23}\protected@file@percent }
\newlabel{lemma:BCFW:MCM_nonempty=>hel>=1@cref}{{[corollary][23][10]10.23}{[1][85][]85}{}{}{}}
\newlabel{ssec:BCFW:MCM_vs_wtemb}{{10.3}{85}{Decorated \MCMSs and \wtembs }{subsection.10.3}{}}
\@writefile{lla}{\contentsline {section}{\numberline {\crtrefnumber{ssec:BCFW:MCM_vs_wtemb}}ssec:BCFW:MCM_vs_wtemb}{85}{subsection.10.3}\protected@file@percent }
\newlabel{ssec:BCFW:MCM_vs_wtemb@cref}{{[subsection][3][10]10.3}{[1][85][]85}{}{}{}}
\@writefile{toc}{\contentsline {subsection}{\tocsubsection {}{10.3}{Decorated M-convex\xspace  moduli spaces\xspace  and weak t-embeddings\xspace  }}{85}{subsection.10.3}\protected@file@percent }
\@writefile{loe}{\contentsline {definition}{\ifthmt@listswap Definition~10.24\else \numberline {10.24}Definition\fi }{85}{definition.10.24}\protected@file@percent }
\newlabel{dfn:MCMp_MCMpdec}{{10.24}{85}{}{definition.10.24}{}}
\@writefile{lla}{\contentsline {section}{\numberline {\crtrefnumber{dfn:MCMp_MCMpdec}}dfn:MCMp_MCMpdec}{85}{definition.10.24}\protected@file@percent }
\newlabel{dfn:MCMp_MCMpdec@cref}{{[definition][24][10]10.24}{[1][85][]85}{}{}{}}
\newlabel{eq:***}{{10.13}{85}{}{equation.10.13}{}}
\@writefile{lla}{\contentsline {section}{\numberline {\crtrefnumber{eq:***}}eq:***}{85}{equation.10.13}\protected@file@percent }
\newlabel{eq:***@cref}{{[equation][13][10]10.13}{[1][85][]85}{}{}{}}
\newlabel{eq:MdteoMP_dfn}{{10.14}{85}{}{equation.10.14}{}}
\@writefile{lla}{\contentsline {section}{\numberline {\crtrefnumber{eq:MdteoMP_dfn}}eq:MdteoMP_dfn}{85}{equation.10.14}\protected@file@percent }
\newlabel{eq:MdteoMP_dfn@cref}{{[equation][14][10]10.14}{[1][85][]85}{}{}{}}
\@writefile{loe}{\contentsline {notation}{\ifthmt@listswap Notation~10.25\else \numberline {10.25}Notation\fi }{85}{notation.10.25}\protected@file@percent }
\newlabel{notn:BCFW:moduli_of_Gfin_vs_Gbip}{{10.25}{85}{}{notation.10.25}{}}
\@writefile{lla}{\contentsline {section}{\numberline {\crtrefnumber{notn:BCFW:moduli_of_Gfin_vs_Gbip}}notn:BCFW:moduli_of_Gfin_vs_Gbip}{85}{notation.10.25}\protected@file@percent }
\newlabel{notn:BCFW:moduli_of_Gfin_vs_Gbip@cref}{{[notation][25][10]10.25}{[1][85][]85}{}{}{}}
\@writefile{loe}{\contentsline {remark}{\ifthmt@listswap Remark~10.26\else \numberline {10.26}Remark\fi }{85}{remark.10.26}\protected@file@percent }
\newlabel{rmk:MCMp->MCM_surj}{{10.26}{85}{}{remark.10.26}{}}
\@writefile{lla}{\contentsline {section}{\numberline {\crtrefnumber{rmk:MCMp->MCM_surj}}rmk:MCMp->MCM_surj}{85}{remark.10.26}\protected@file@percent }
\newlabel{rmk:MCMp->MCM_surj@cref}{{[remark][26][10]10.26}{[1][85][]85}{}{}{}}
\citation{origami1}
\@writefile{loe}{\contentsline {proposition}{\ifthmt@listswap Proposition~10.27\else \numberline {10.27}Proposition\fi }{86}{proposition.10.27}\protected@file@percent }
\newlabel{lemma:TE:TE_to_MCE_and_back}{{10.27}{86}{}{proposition.10.27}{}}
\@writefile{lla}{\contentsline {section}{\numberline {\crtrefnumber{lemma:TE:TE_to_MCE_and_back}}lemma:TE:TE_to_MCE_and_back}{86}{proposition.10.27}\protected@file@percent }
\newlabel{lemma:TE:TE_to_MCE_and_back@cref}{{[proposition][27][10]10.27}{[1][85][]86}{}{}{}}
\newlabel{lemma:TE:MCE_to_TE}{{10.27}{86}{}{proposition.10.27}{}}
\@writefile{lla}{\contentsline {section}{\numberline {\crtrefnumber{lemma:TE:MCE_to_TE}}lemma:TE:MCE_to_TE}{86}{proposition.10.27}\protected@file@percent }
\newlabel{lemma:TE:MCE_to_TE@cref}{{[proposition][27][10]10.27}{[1][85][]86}{}{}{}}
\newlabel{lemma:TE:TE_to_MCE}{{10.27}{86}{}{proposition.10.27}{}}
\@writefile{lla}{\contentsline {section}{\numberline {\crtrefnumber{lemma:TE:TE_to_MCE}}lemma:TE:TE_to_MCE}{86}{proposition.10.27}\protected@file@percent }
\newlabel{lemma:TE:TE_to_MCE@cref}{{[proposition][27][10]10.27}{[1][85][]86}{}{}{}}
\newlabel{lemma:ORA:terminal_vs_atr_no_dim}{{10.27}{86}{}{proposition.10.27}{}}
\@writefile{lla}{\contentsline {section}{\numberline {\crtrefnumber{lemma:ORA:terminal_vs_atr_no_dim}}lemma:ORA:terminal_vs_atr_no_dim}{86}{proposition.10.27}\protected@file@percent }
\newlabel{lemma:ORA:terminal_vs_atr_no_dim@cref}{{[proposition][27][10]10.27}{[1][85][]86}{}{}{}}
\newlabel{eq:ORA::mceTOwte_dfn_iso}{{10.15}{86}{}{equation.10.15}{}}
\@writefile{lla}{\contentsline {section}{\numberline {\crtrefnumber{eq:ORA::mceTOwte_dfn_iso}}eq:ORA::mceTOwte_dfn_iso}{86}{equation.10.15}\protected@file@percent }
\newlabel{eq:ORA::mceTOwte_dfn_iso@cref}{{[equation][15][10]10.15}{[1][85][]86}{}{}{}}
\@writefile{toc}{\contentsline {subsection}{\tocsubsection {}{10.4}{Dimension counting}}{86}{subsection.10.4}\protected@file@percent }
\@writefile{loe}{\contentsline {lemma}{\ifthmt@listswap Lemma~10.28\else \numberline {10.28}Lemma\fi }{86}{lemma.10.28}\protected@file@percent }
\newlabel{lemma:OCP:dim_atr}{{10.28}{86}{}{lemma.10.28}{}}
\@writefile{lla}{\contentsline {section}{\numberline {\crtrefnumber{lemma:OCP:dim_atr}}lemma:OCP:dim_atr}{86}{lemma.10.28}\protected@file@percent }
\newlabel{lemma:OCP:dim_atr@cref}{{[lemma][28][10]10.28}{[1][86][]86}{}{}{}}
\newlabel{eq:OCP:dim_atr}{{10.16}{86}{}{equation.10.16}{}}
\@writefile{lla}{\contentsline {section}{\numberline {\crtrefnumber{eq:OCP:dim_atr}}eq:OCP:dim_atr}{86}{equation.10.16}\protected@file@percent }
\newlabel{eq:OCP:dim_atr@cref}{{[equation][16][10]10.16}{[1][86][]86}{}{}{}}
\newlabel{eq:gdim_dfn}{{10.17}{86}{Dimension counting}{equation.10.17}{}}
\@writefile{lla}{\contentsline {section}{\numberline {\crtrefnumber{eq:gdim_dfn}}eq:gdim_dfn}{86}{equation.10.17}\protected@file@percent }
\newlabel{eq:gdim_dfn@cref}{{[equation][17][10]10.17}{[1][86][]86}{}{}{}}
\@writefile{loe}{\contentsline {lemma}{\ifthmt@listswap Lemma~10.29\else \numberline {10.29}Lemma\fi }{86}{lemma.10.29}\protected@file@percent }
\newlabel{lemma:ORA:terminal_vs_atr_dim_only}{{10.29}{86}{}{lemma.10.29}{}}
\@writefile{lla}{\contentsline {section}{\numberline {\crtrefnumber{lemma:ORA:terminal_vs_atr_dim_only}}lemma:ORA:terminal_vs_atr_dim_only}{86}{lemma.10.29}\protected@file@percent }
\newlabel{lemma:ORA:terminal_vs_atr_dim_only@cref}{{[lemma][29][10]10.29}{[1][86][]86}{}{}{}}
\newlabel{eq:ORA:terminal_vs_atr_dim_only}{{10.18}{86}{}{equation.10.18}{}}
\@writefile{lla}{\contentsline {section}{\numberline {\crtrefnumber{eq:ORA:terminal_vs_atr_dim_only}}eq:ORA:terminal_vs_atr_dim_only}{86}{equation.10.18}\protected@file@percent }
\newlabel{eq:ORA:terminal_vs_atr_dim_only@cref}{{[equation][18][10]10.18}{[1][86][]86}{}{}{}}
\@writefile{loe}{\contentsline {proposition}{\ifthmt@listswap Proposition~10.30\else \numberline {10.30}Proposition\fi }{87}{proposition.10.30}\protected@file@percent }
\newlabel{lemma:OCP:gdim_Mmce}{{10.30}{87}{}{proposition.10.30}{}}
\@writefile{lla}{\contentsline {section}{\numberline {\crtrefnumber{lemma:OCP:gdim_Mmce}}lemma:OCP:gdim_Mmce}{87}{proposition.10.30}\protected@file@percent }
\newlabel{lemma:OCP:gdim_Mmce@cref}{{[proposition][30][10]10.30}{[1][87][]87}{}{}{}}
\newlabel{eq:OCP:gdim_Mmce}{{10.19}{87}{}{equation.10.19}{}}
\@writefile{lla}{\contentsline {section}{\numberline {\crtrefnumber{eq:OCP:gdim_Mmce}}eq:OCP:gdim_Mmce}{87}{equation.10.19}\protected@file@percent }
\newlabel{eq:OCP:gdim_Mmce@cref}{{[equation][19][10]10.19}{[1][87][]87}{}{}{}}
\newlabel{eq:gdim_diff}{{10.20}{87}{Dimension counting}{equation.10.20}{}}
\@writefile{lla}{\contentsline {section}{\numberline {\crtrefnumber{eq:gdim_diff}}eq:gdim_diff}{87}{equation.10.20}\protected@file@percent }
\newlabel{eq:gdim_diff@cref}{{[equation][20][10]10.20}{[1][87][]87}{}{}{}}
\newlabel{ssec:combin_invar}{{10.5}{87}{Combinatorial invariance of \MCEsnoacr }{subsection.10.5}{}}
\@writefile{lla}{\contentsline {section}{\numberline {\crtrefnumber{ssec:combin_invar}}ssec:combin_invar}{87}{subsection.10.5}\protected@file@percent }
\newlabel{ssec:combin_invar@cref}{{[subsection][5][10]10.5}{[1][87][]87}{}{}{}}
\@writefile{toc}{\contentsline {subsection}{\tocsubsection {}{10.5}{Combinatorial invariance of M-convex\xspace  weak embeddings\xspace  }}{87}{subsection.10.5}\protected@file@percent }
\@writefile{loe}{\contentsline {proposition}{\ifthmt@listswap Proposition~10.31\else \numberline {10.31}Proposition\fi }{87}{proposition.10.31}\protected@file@percent }
\newlabel{lemma:BCFW:clique_vs_Rg}{{10.31}{87}{}{proposition.10.31}{}}
\@writefile{lla}{\contentsline {section}{\numberline {\crtrefnumber{lemma:BCFW:clique_vs_Rg}}lemma:BCFW:clique_vs_Rg}{87}{proposition.10.31}\protected@file@percent }
\newlabel{lemma:BCFW:clique_vs_Rg@cref}{{[proposition][31][10]10.31}{[1][87][]87}{}{}{}}
\newlabel{eq:BCFW:sumbTcond=0}{{10.21}{88}{Combinatorial invariance of \MCEsnoacr }{equation.10.21}{}}
\@writefile{lla}{\contentsline {section}{\numberline {\crtrefnumber{eq:BCFW:sumbTcond=0}}eq:BCFW:sumbTcond=0}{88}{equation.10.21}\protected@file@percent }
\newlabel{eq:BCFW:sumbTcond=0@cref}{{[equation][21][10]10.21}{[1][88][]88}{}{}{}}
\@writefile{loe}{\contentsline {corollary}{\ifthmt@listswap Corollary~10.32\else \numberline {10.32}Corollary\fi }{88}{corollary.10.32}\protected@file@percent }
\newlabel{lemma:BCFW:clique_vs_Rg_maximal}{{10.32}{88}{}{corollary.10.32}{}}
\@writefile{lla}{\contentsline {section}{\numberline {\crtrefnumber{lemma:BCFW:clique_vs_Rg_maximal}}lemma:BCFW:clique_vs_Rg_maximal}{88}{corollary.10.32}\protected@file@percent }
\newlabel{lemma:BCFW:clique_vs_Rg_maximal@cref}{{[corollary][32][10]10.32}{[1][88][]88}{}{}{}}
\@writefile{loe}{\contentsline {remark}{\ifthmt@listswap Remark~10.33\else \numberline {10.33}Remark\fi }{88}{remark.10.33}\protected@file@percent }
\newlabel{rmk:BCFW:clique_vs_Rg_1_vert}{{10.33}{88}{}{remark.10.33}{}}
\@writefile{lla}{\contentsline {section}{\numberline {\crtrefnumber{rmk:BCFW:clique_vs_Rg_1_vert}}rmk:BCFW:clique_vs_Rg_1_vert}{88}{remark.10.33}\protected@file@percent }
\newlabel{rmk:BCFW:clique_vs_Rg_1_vert@cref}{{[remark][33][10]10.33}{[1][88][]88}{}{}{}}
\@writefile{loe}{\contentsline {corollary}{\ifthmt@listswap Corollary~10.34\else \numberline {10.34}Corollary\fi }{88}{corollary.10.34}\protected@file@percent }
\newlabel{lemma:BCFW:NullE_vs_NullED}{{10.34}{88}{}{corollary.10.34}{}}
\@writefile{lla}{\contentsline {section}{\numberline {\crtrefnumber{lemma:BCFW:NullE_vs_NullED}}lemma:BCFW:NullE_vs_NullED}{88}{corollary.10.34}\protected@file@percent }
\newlabel{lemma:BCFW:NullE_vs_NullED@cref}{{[corollary][34][10]10.34}{[1][88][]88}{}{}{}}
\newlabel{eq:BCFW:NullE_vs_NullED}{{10.22}{88}{}{equation.10.22}{}}
\@writefile{lla}{\contentsline {section}{\numberline {\crtrefnumber{eq:BCFW:NullE_vs_NullED}}eq:BCFW:NullE_vs_NullED}{88}{equation.10.22}\protected@file@percent }
\newlabel{eq:BCFW:NullE_vs_NullED@cref}{{[equation][22][10]10.22}{[1][88][]88}{}{}{}}
\@writefile{loe}{\contentsline {definition}{\ifthmt@listswap Definition~10.35\else \numberline {10.35}Definition\fi }{88}{definition.10.35}\protected@file@percent }
\newlabel{dfn:twosep_lgg}{{10.35}{88}{}{definition.10.35}{}}
\@writefile{lla}{\contentsline {section}{\numberline {\crtrefnumber{dfn:twosep_lgg}}dfn:twosep_lgg}{88}{definition.10.35}\protected@file@percent }
\newlabel{dfn:twosep_lgg@cref}{{[definition][35][10]10.35}{[1][88][]88}{}{}{}}
\@writefile{loe}{\contentsline {corollary}{\ifthmt@listswap Corollary~10.36\else \numberline {10.36}Corollary\fi }{88}{corollary.10.36}\protected@file@percent }
\newlabel{lemma:fullysepMCE_vs_fullysep}{{10.36}{88}{}{corollary.10.36}{}}
\@writefile{lla}{\contentsline {section}{\numberline {\crtrefnumber{lemma:fullysepMCE_vs_fullysep}}lemma:fullysepMCE_vs_fullysep}{88}{corollary.10.36}\protected@file@percent }
\newlabel{lemma:fullysepMCE_vs_fullysep@cref}{{[corollary][36][10]10.36}{[1][88][]88}{}{}{}}
\@writefile{lof}{\contentsline {figure}{\numberline {20}{\ignorespaces  An example of $(\Gamma ^\ast ,\bm  {x}),(\Gamma ^\ast ,\bm  {x}')\in \mathcal  {M}_{\text  {\scalebox {0.85}{$\mathtt  {MCE}$}}}(\Gamma _{\!L^\ast })$ such that for each interior black corner $\nu $, we have $\hat  {\alpha }^\bullet _{\bm  {x}}(\nu ),\hat  {\alpha }^\bullet _{\bm  {x}'}(\nu )\in \{0,\pi \}$ with $\hat  {\alpha }^\bullet _{\bm  {x}}(\nu )\neq  \hat  {\alpha }^\bullet _{\bm  {x}'}(\nu )$; see \cref  {ex:BCFW:corner_comparison}. }}{89}{figure.caption.28}\protected@file@percent }
\newlabel{fig:corner-0-pi}{{20}{89}{An example of $(\GD ,\xd ),(\GD ,\yd )\in \MCM (\Gloop )$ such that for each interior black corner $\cor $, we have $\sumbTx (\cor ),\sumbTy (\cor )\in \{0,\pi \}$ with $\sumbTx (\cor )\neq \sumbTy (\cor )$; see \cref {ex:BCFW:corner_comparison}}{figure.caption.28}{}}
\@writefile{lla}{\contentsline {section}{\numberline {\crtrefnumber{fig:corner-0-pi}}fig:corner-0-pi}{89}{figure.caption.28}\protected@file@percent }
\newlabel{fig:corner-0-pi@cref}{{[figure][20][]20}{[1][89][]89}{}{}{}}
\@writefile{loe}{\contentsline {lemma}{\ifthmt@listswap Lemma~10.37\else \numberline {10.37}Lemma\fi }{89}{lemma.10.37}\protected@file@percent }
\newlabel{lemma:BCFW:corner_comparison}{{10.37}{89}{}{lemma.10.37}{}}
\@writefile{lla}{\contentsline {section}{\numberline {\crtrefnumber{lemma:BCFW:corner_comparison}}lemma:BCFW:corner_comparison}{89}{lemma.10.37}\protected@file@percent }
\newlabel{lemma:BCFW:corner_comparison@cref}{{[lemma][37][10]10.37}{[1][89][]89}{}{}{}}
\newlabel{corner_comparison1}{{{{(1)}}}{89}{}{Item.73}{}}
\@writefile{lla}{\contentsline {section}{\numberline {\crtrefnumber{corner_comparison1}}corner_comparison1}{89}{Item.73}\protected@file@percent }
\newlabel{corner_comparison1@cref}{{[enumi][1][]{{(1)}}}{[1][89][]89}{}{}{}}
\newlabel{corner_comparison2}{{{{(2)}}}{89}{}{Item.74}{}}
\@writefile{lla}{\contentsline {section}{\numberline {\crtrefnumber{corner_comparison2}}corner_comparison2}{89}{Item.74}\protected@file@percent }
\newlabel{corner_comparison2@cref}{{[enumi][2][]{{(2)}}}{[1][89][]89}{}{}{}}
\@writefile{loe}{\contentsline {example}{\ifthmt@listswap Example~10.38\else \numberline {10.38}Example\fi }{89}{example.10.38}\protected@file@percent }
\newlabel{ex:BCFW:corner_comparison}{{10.38}{89}{}{example.10.38}{}}
\@writefile{lla}{\contentsline {section}{\numberline {\crtrefnumber{ex:BCFW:corner_comparison}}ex:BCFW:corner_comparison}{89}{example.10.38}\protected@file@percent }
\newlabel{ex:BCFW:corner_comparison@cref}{{[example][38][10]10.38}{[1][89][]89}{}{}{}}
\@writefile{loe}{\contentsline {proposition}{\ifthmt@listswap Proposition~10.39\else \numberline {10.39}Proposition\fi }{89}{proposition.10.39}\protected@file@percent }
\newlabel{lemma:Res_of_MCE_is_MCE}{{10.39}{89}{}{proposition.10.39}{}}
\@writefile{lla}{\contentsline {section}{\numberline {\crtrefnumber{lemma:Res_of_MCE_is_MCE}}lemma:Res_of_MCE_is_MCE}{89}{proposition.10.39}\protected@file@percent }
\newlabel{lemma:Res_of_MCE_is_MCE@cref}{{[proposition][39][10]10.39}{[1][89][]89}{}{}{}}
\@writefile{loe}{\contentsline {lemma}{\ifthmt@listswap Lemma~10.40\else \numberline {10.40}Lemma\fi }{89}{lemma.10.40}\protected@file@percent }
\newlabel{lemma:Res_MCE}{{10.40}{89}{}{lemma.10.40}{}}
\@writefile{lla}{\contentsline {section}{\numberline {\crtrefnumber{lemma:Res_MCE}}lemma:Res_MCE}{89}{lemma.10.40}\protected@file@percent }
\newlabel{lemma:Res_MCE@cref}{{[lemma][40][10]10.40}{[1][89][]89}{}{}{}}
\newlabel{Res_MCE1}{{{{(1)}}}{89}{}{Item.75}{}}
\@writefile{lla}{\contentsline {section}{\numberline {\crtrefnumber{Res_MCE1}}Res_MCE1}{89}{Item.75}\protected@file@percent }
\newlabel{Res_MCE1@cref}{{[enumi][1][]{{(1)}}}{[1][89][]89}{}{}{}}
\newlabel{Res_MCE2}{{{{(2)}}}{90}{}{Item.76}{}}
\@writefile{lla}{\contentsline {section}{\numberline {\crtrefnumber{Res_MCE2}}Res_MCE2}{90}{Item.76}\protected@file@percent }
\newlabel{Res_MCE2@cref}{{[enumi][2][]{{(2)}}}{[1][89][]90}{}{}{}}
\newlabel{eq:Rg_Rgout_angle_relation}{{10.23}{90}{Combinatorial invariance of \MCEsnoacr }{equation.10.23}{}}
\@writefile{lla}{\contentsline {section}{\numberline {\crtrefnumber{eq:Rg_Rgout_angle_relation}}eq:Rg_Rgout_angle_relation}{90}{equation.10.23}\protected@file@percent }
\newlabel{eq:Rg_Rgout_angle_relation@cref}{{[equation][23][10]10.23}{[1][90][]90}{}{}{}}
\newlabel{eq:Rg_Rgout_bdry_angle_sum}{{10.24}{90}{Combinatorial invariance of \MCEsnoacr }{equation.10.24}{}}
\@writefile{lla}{\contentsline {section}{\numberline {\crtrefnumber{eq:Rg_Rgout_bdry_angle_sum}}eq:Rg_Rgout_bdry_angle_sum}{90}{equation.10.24}\protected@file@percent }
\newlabel{eq:Rg_Rgout_bdry_angle_sum@cref}{{[equation][24][10]10.24}{[1][90][]90}{}{}{}}
\citation{Floater}
\@writefile{loe}{\contentsline {lemma}{\ifthmt@listswap Lemma~10.41\else \numberline {10.41}Lemma\fi }{91}{lemma.10.41}\protected@file@percent }
\newlabel{lemma:injective_MCE_exists}{{10.41}{91}{}{lemma.10.41}{}}
\@writefile{lla}{\contentsline {section}{\numberline {\crtrefnumber{lemma:injective_MCE_exists}}lemma:injective_MCE_exists}{91}{lemma.10.41}\protected@file@percent }
\newlabel{lemma:injective_MCE_exists@cref}{{[lemma][41][10]10.41}{[1][91][]91}{}{}{}}
\citation{Kenyon_Sheffield}
\citation{CLR1}
\citation{AHBC_all_loop}
\citation{BCFW}
\citation{abcgpt}
\@writefile{toc}{\contentsline {section}{\tocsection {}{11}{BCFW tilings of Mandelstam-convex\xspace  moduli spaces\xspace  }}{92}{section.11}\protected@file@percent }
\newlabel{sec:BCFW}{{11}{92}{BCFW tilings of \MCMSsTITLE }{section.11}{}}
\@writefile{lla}{\contentsline {section}{\numberline {\crtrefnumber{sec:BCFW}}sec:BCFW}{92}{section.11}\protected@file@percent }
\newlabel{sec:BCFW@cref}{{[section][11][]11}{[1][92][]92}{}{}{}}
\newlabel{sec:BCFW_steps}{{11.1}{92}{BCFW steps}{subsection.11.1}{}}
\@writefile{lla}{\contentsline {section}{\numberline {\crtrefnumber{sec:BCFW_steps}}sec:BCFW_steps}{92}{subsection.11.1}\protected@file@percent }
\newlabel{sec:BCFW_steps@cref}{{[subsection][1][11]11.1}{[1][92][]92}{}{}{}}
\@writefile{toc}{\contentsline {subsection}{\tocsubsection {}{11.1}{BCFW steps}}{92}{subsection.11.1}\protected@file@percent }
\@writefile{loe}{\contentsline {definition}{\ifthmt@listswap Definition~11.1\else \numberline {11.1}Definition\fi \thmtformatoptarg {BCFW step}}{92}{definition.11.1}\protected@file@percent }
\newlabel{dfn:BCFW:step}{{11.1}{92}{BCFW step}{definition.11.1}{}}
\@writefile{lla}{\contentsline {section}{\numberline {\crtrefnumber{dfn:BCFW:step}}dfn:BCFW:step}{92}{definition.11.1}\protected@file@percent }
\newlabel{dfn:BCFW:step@cref}{{[definition][1][11]11.1}{[1][92][]92}{}{}{}}
\newlabel{BCFWstep1}{{{{(BCFW1)}}}{92}{BCFW step}{Item.77}{}}
\@writefile{lla}{\contentsline {section}{\numberline {\crtrefnumber{BCFWstep1}}BCFWstep1}{92}{Item.77}\protected@file@percent }
\newlabel{BCFWstep1@cref}{{[enumi][1][]{{(BCFW1)}}}{[1][92][]92}{}{}{}}
\newlabel{BCFWstep2}{{{{(BCFW2)}}}{92}{BCFW step}{Item.78}{}}
\@writefile{lla}{\contentsline {section}{\numberline {\crtrefnumber{BCFWstep2}}BCFWstep2}{92}{Item.78}\protected@file@percent }
\newlabel{BCFWstep2@cref}{{[enumi][2][]{{(BCFW2)}}}{[1][92][]92}{}{}{}}
\newlabel{BCFWstep3}{{{{(BCFW3)}}}{93}{BCFW step}{Item.79}{}}
\@writefile{lla}{\contentsline {section}{\numberline {\crtrefnumber{BCFWstep3}}BCFWstep3}{93}{Item.79}\protected@file@percent }
\newlabel{BCFWstep3@cref}{{[enumi][3][]{{(BCFW3)}}}{[1][92][]93}{}{}{}}
\newlabel{BCFWstep4}{{{{(BCFW4)}}}{93}{BCFW step}{Item.80}{}}
\@writefile{lla}{\contentsline {section}{\numberline {\crtrefnumber{BCFWstep4}}BCFWstep4}{93}{Item.80}\protected@file@percent }
\newlabel{BCFWstep4@cref}{{[enumi][4][]{{(BCFW4)}}}{[1][93][]93}{}{}{}}
\newlabel{eq:BCFW:step_split_hel}{{11.1}{93}{BCFW step}{equation.11.1}{}}
\@writefile{lla}{\contentsline {section}{\numberline {\crtrefnumber{eq:BCFW:step_split_hel}}eq:BCFW:step_split_hel}{93}{equation.11.1}\protected@file@percent }
\newlabel{eq:BCFW:step_split_hel@cref}{{[equation][1][11]11.1}{[1][93][]93}{}{}{}}
\@writefile{loe}{\contentsline {remark}{\ifthmt@listswap Remark~11.2\else \numberline {11.2}Remark\fi }{93}{remark.11.2}\protected@file@percent }
\@writefile{loe}{\contentsline {definition}{\ifthmt@listswap Definition~11.3\else \numberline {11.3}Definition\fi }{93}{definition.11.3}\protected@file@percent }
\newlabel{dfn:BCin-generic}{{11.3}{93}{}{definition.11.3}{}}
\@writefile{lla}{\contentsline {section}{\numberline {\crtrefnumber{dfn:BCin-generic}}dfn:BCin-generic}{93}{definition.11.3}\protected@file@percent }
\newlabel{dfn:BCin-generic@cref}{{[definition][3][11]11.3}{[1][93][]93}{}{}{}}
\@writefile{loe}{\contentsline {definition}{\ifthmt@listswap Definition~11.4\else \numberline {11.4}Definition\fi }{93}{definition.11.4}\protected@file@percent }
\newlabel{eq:MCMgen_Gl->Glout_dfn}{{11.2}{93}{}{equation.11.2}{}}
\@writefile{lla}{\contentsline {section}{\numberline {\crtrefnumber{eq:MCMgen_Gl->Glout_dfn}}eq:MCMgen_Gl->Glout_dfn}{93}{equation.11.2}\protected@file@percent }
\newlabel{eq:MCMgen_Gl->Glout_dfn@cref}{{[equation][2][11]11.2}{[1][93][]93}{}{}{}}
\@writefile{loe}{\contentsline {proposition}{\ifthmt@listswap Proposition~11.5\else \numberline {11.5}Proposition\fi }{93}{proposition.11.5}\protected@file@percent }
\newlabel{lemma:BCFW:BCFW_vs_OR_step_forward}{{11.5}{93}{}{proposition.11.5}{}}
\@writefile{lla}{\contentsline {section}{\numberline {\crtrefnumber{lemma:BCFW:BCFW_vs_OR_step_forward}}lemma:BCFW:BCFW_vs_OR_step_forward}{93}{proposition.11.5}\protected@file@percent }
\newlabel{lemma:BCFW:BCFW_vs_OR_step_forward@cref}{{[proposition][5][11]11.5}{[1][93][]93}{}{}{}}
\newlabel{eq:BCFW_vs_OR_step_forward}{{11.3}{93}{}{equation.11.3}{}}
\@writefile{lla}{\contentsline {section}{\numberline {\crtrefnumber{eq:BCFW_vs_OR_step_forward}}eq:BCFW_vs_OR_step_forward}{93}{equation.11.3}\protected@file@percent }
\newlabel{eq:BCFW_vs_OR_step_forward@cref}{{[equation][3][11]11.3}{[1][93][]93}{}{}{}}
\newlabel{sec:loop_BCFW_rec}{{11.2}{93}{Loop BCFW recursion and \oraTITLE }{subsection.11.2}{}}
\@writefile{lla}{\contentsline {section}{\numberline {\crtrefnumber{sec:loop_BCFW_rec}}sec:loop_BCFW_rec}{93}{subsection.11.2}\protected@file@percent }
\newlabel{sec:loop_BCFW_rec@cref}{{[subsection][2][11]11.2}{[1][93][]93}{}{}{}}
\@writefile{toc}{\contentsline {subsection}{\tocsubsection {}{11.2}{Loop BCFW recursion and origami reconstruction algorithm\xspace  }}{93}{subsection.11.2}\protected@file@percent }
\@writefile{loe}{\contentsline {algorithm}{\ifthmt@listswap Algorithm~11.6\else \numberline {11.6}Algorithm\fi \thmtformatoptarg {Loop BCFW recursion}}{93}{algorithm.11.6}\protected@file@percent }
\newlabel{dfn:BCFW:rec}{{11.6}{93}{Loop BCFW recursion}{algorithm.11.6}{}}
\@writefile{lla}{\contentsline {section}{\numberline {\crtrefnumber{dfn:BCFW:rec}}dfn:BCFW:rec}{93}{algorithm.11.6}\protected@file@percent }
\newlabel{dfn:BCFW:rec@cref}{{[algorithm][6][11]11.6}{[1][93][]93}{}{}{}}
\newlabel{dfn:BCFW1}{{{{(1)}}}{93}{Loop BCFW recursion}{Item.81}{}}
\@writefile{lla}{\contentsline {section}{\numberline {\crtrefnumber{dfn:BCFW1}}dfn:BCFW1}{93}{Item.81}\protected@file@percent }
\newlabel{dfn:BCFW1@cref}{{[enumi][1][]{{(1)}}}{[1][93][]93}{}{}{}}
\citation{abcgpt}
\citation{AHBC_all_loop}
\newlabel{dfn:BCFW2}{{{{(2)}}}{94}{Loop BCFW recursion}{Item.82}{}}
\@writefile{lla}{\contentsline {section}{\numberline {\crtrefnumber{dfn:BCFW2}}dfn:BCFW2}{94}{Item.82}\protected@file@percent }
\newlabel{dfn:BCFW2@cref}{{[enumi][2][]{{(2)}}}{[1][93][]94}{}{}{}}
\newlabel{dfn:BCFW3}{{{{(3)}}}{94}{Loop BCFW recursion}{Item.83}{}}
\@writefile{lla}{\contentsline {section}{\numberline {\crtrefnumber{dfn:BCFW3}}dfn:BCFW3}{94}{Item.83}\protected@file@percent }
\newlabel{dfn:BCFW3@cref}{{[enumi][3][]{{(3)}}}{[1][94][]94}{}{}{}}
\@writefile{loe}{\contentsline {remark}{\ifthmt@listswap Remark~11.7\else \numberline {11.7}Remark\fi }{94}{remark.11.7}\protected@file@percent }
\@writefile{loe}{\contentsline {definition}{\ifthmt@listswap Definition~11.8\else \numberline {11.8}Definition\fi \thmtformatoptarg {Branch of the origami reconstruction algorithm\xspace  }}{94}{definition.11.8}\protected@file@percent }
\newlabel{dfn:BCFW:exc}{{11.8}{94}{Branch of the \ORA }{definition.11.8}{}}
\@writefile{lla}{\contentsline {section}{\numberline {\crtrefnumber{dfn:BCFW:exc}}dfn:BCFW:exc}{94}{definition.11.8}\protected@file@percent }
\newlabel{dfn:BCFW:exc@cref}{{[definition][8][11]11.8}{[1][94][]94}{}{}{}}
\newlabel{eq:BCFW:BCFW_branch}{{11.4}{94}{Branch of the \ORA }{equation.11.4}{}}
\@writefile{lla}{\contentsline {section}{\numberline {\crtrefnumber{eq:BCFW:BCFW_branch}}eq:BCFW:BCFW_branch}{94}{equation.11.4}\protected@file@percent }
\newlabel{eq:BCFW:BCFW_branch@cref}{{[equation][4][11]11.4}{[1][94][]94}{}{}{}}
\newlabel{eq:MCMo_Zexc_dfn}{{11.5}{94}{Branch of the \ORA }{equation.11.5}{}}
\@writefile{lla}{\contentsline {section}{\numberline {\crtrefnumber{eq:MCMo_Zexc_dfn}}eq:MCMo_Zexc_dfn}{94}{equation.11.5}\protected@file@percent }
\newlabel{eq:MCMo_Zexc_dfn@cref}{{[equation][5][11]11.5}{[1][94][]94}{}{}{}}
\@writefile{loe}{\contentsline {definition}{\ifthmt@listswap Definition~11.9\else \numberline {11.9}Definition\fi }{94}{definition.11.9}\protected@file@percent }
\@writefile{loe}{\contentsline {proposition}{\ifthmt@listswap Proposition~11.10\else \numberline {11.10}Proposition\fi }{94}{proposition.11.10}\protected@file@percent }
\newlabel{lemma:MCMto=Res}{{11.10}{94}{}{proposition.11.10}{}}
\@writefile{lla}{\contentsline {section}{\numberline {\crtrefnumber{lemma:MCMto=Res}}lemma:MCMto=Res}{94}{proposition.11.10}\protected@file@percent }
\newlabel{lemma:MCMto=Res@cref}{{[proposition][10][11]11.10}{[1][94][]94}{}{}{}}
\newlabel{eq:MCMto=Res}{{11.6}{94}{}{equation.11.6}{}}
\@writefile{lla}{\contentsline {section}{\numberline {\crtrefnumber{eq:MCMto=Res}}eq:MCMto=Res}{94}{equation.11.6}\protected@file@percent }
\newlabel{eq:MCMto=Res@cref}{{[equation][6][11]11.6}{[1][94][]94}{}{}{}}
\@writefile{loe}{\contentsline {proposition}{\ifthmt@listswap Proposition~11.11\else \numberline {11.11}Proposition\fi }{94}{proposition.11.11}\protected@file@percent }
\newlabel{lemma:MCMto_open}{{11.11}{94}{}{proposition.11.11}{}}
\@writefile{lla}{\contentsline {section}{\numberline {\crtrefnumber{lemma:MCMto_open}}lemma:MCMto_open}{94}{proposition.11.11}\protected@file@percent }
\newlabel{lemma:MCMto_open@cref}{{[proposition][11][11]11.11}{[1][94][]94}{}{}{}}
\@writefile{toc}{\contentsline {subsection}{\tocsubsection {}{11.3}{Kinematic support\xspace  }}{95}{subsection.11.3}\protected@file@percent }
\@writefile{loe}{\contentsline {definition}{\ifthmt@listswap Definition~11.12\else \numberline {11.12}Definition\fi }{95}{definition.11.12}\protected@file@percent }
\newlabel{dfn:BCFW:kinsupp}{{11.12}{95}{}{definition.11.12}{}}
\@writefile{lla}{\contentsline {section}{\numberline {\crtrefnumber{dfn:BCFW:kinsupp}}dfn:BCFW:kinsupp}{95}{definition.11.12}\protected@file@percent }
\newlabel{dfn:BCFW:kinsupp@cref}{{[definition][12][11]11.12}{[1][95][]95}{}{}{}}
\@writefile{loe}{\contentsline {lemma}{\ifthmt@listswap Lemma~11.13\else \numberline {11.13}Lemma\fi }{95}{lemma.11.13}\protected@file@percent }
\newlabel{lemma:BCFW:dim_M0_irr}{{11.13}{95}{}{lemma.11.13}{}}
\@writefile{lla}{\contentsline {section}{\numberline {\crtrefnumber{lemma:BCFW:dim_M0_irr}}lemma:BCFW:dim_M0_irr}{95}{lemma.11.13}\protected@file@percent }
\newlabel{lemma:BCFW:dim_M0_irr@cref}{{[lemma][13][11]11.13}{[1][95][]95}{}{}{}}
\@writefile{loe}{\contentsline {corollary}{\ifthmt@listswap Corollary~11.14\else \numberline {11.14}Corollary\fi }{96}{corollary.11.14}\protected@file@percent }
\newlabel{lemma:MCE:fullysep<=kinsupp}{{11.14}{96}{}{corollary.11.14}{}}
\@writefile{lla}{\contentsline {section}{\numberline {\crtrefnumber{lemma:MCE:fullysep<=kinsupp}}lemma:MCE:fullysep<=kinsupp}{96}{corollary.11.14}\protected@file@percent }
\newlabel{lemma:MCE:fullysep<=kinsupp@cref}{{[corollary][14][11]11.14}{[1][96][]96}{}{}{}}
\@writefile{loe}{\contentsline {proposition}{\ifthmt@listswap Proposition~11.15\else \numberline {11.15}Proposition\fi }{96}{proposition.11.15}\protected@file@percent }
\newlabel{lemma:kinsupp=realizable}{{11.15}{96}{}{proposition.11.15}{}}
\@writefile{lla}{\contentsline {section}{\numberline {\crtrefnumber{lemma:kinsupp=realizable}}lemma:kinsupp=realizable}{96}{proposition.11.15}\protected@file@percent }
\newlabel{lemma:kinsupp=realizable@cref}{{[proposition][15][11]11.15}{[1][96][]96}{}{}{}}
\@writefile{loe}{\contentsline {example}{\ifthmt@listswap Example~11.16\else \numberline {11.16}Example\fi }{96}{example.11.16}\protected@file@percent }
\newlabel{ex:fullysep_BCFW_check}{{11.16}{96}{}{example.11.16}{}}
\@writefile{lla}{\contentsline {section}{\numberline {\crtrefnumber{ex:fullysep_BCFW_check}}ex:fullysep_BCFW_check}{96}{example.11.16}\protected@file@percent }
\newlabel{ex:fullysep_BCFW_check@cref}{{[example][16][11]11.16}{[1][96][]96}{}{}{}}
\newlabel{eq:dimZ_Zexc}{{11.7}{96}{\Kinsupp }{equation.11.7}{}}
\@writefile{lla}{\contentsline {section}{\numberline {\crtrefnumber{eq:dimZ_Zexc}}eq:dimZ_Zexc}{96}{equation.11.7}\protected@file@percent }
\newlabel{eq:dimZ_Zexc@cref}{{[equation][7][11]11.7}{[1][96][]96}{}{}{}}
\@writefile{lof}{\contentsline {figure}{\numberline {21}{\ignorespaces  A terminal MCE\xspace  $(\Gamma ^\ast ,\bm  {x})\in \mathcal  {M}_{\text  {\scalebox {0.85}{$\mathtt  {MCE}$}}}(\Gamma _{\!L^\ast })$ of $\Gamma _{\!L^\ast }\in \mathbf  {\Gamma }^{\text  {\scalebox {1}{$\text  {\scalebox {0.85}{$\mathtt  {BCFW}$}}$}}}_{k,n;L^\ast }$ (left) whose restriction $\operatorname  {Res}_{\Gamma ^\ast _1}(\Gamma ^\ast ,\bm  {x})\notin  \mathcal  {M}_{\text  {\scalebox {0.85}{$\mathtt  {MCE}$}}}(\Gamma _{1|L^\ast })$ is not an MCE\xspace  of $\Gamma _{1|L^\ast }$ (right). The red dashed line indicates the chord\xspace  violating~\begingroup \let \perh@ps \textup  {MCE5:Mpos_chords}\endgroup  for $\operatorname  {Res}_{\Gamma ^\ast _1}(\Gamma ^\ast ,\bm  {x})$. See \cref  {ex:counter}. }}{97}{figure.caption.29}\protected@file@percent }
\newlabel{fig:counter-kinsupp}{{21}{97}{A terminal \MCE $(\GDfin ,\xdfin )\in \MCM (\Gfin )$ of $\Gfin \in \BCGs $ (left) whose restriction $\ResGx _1(\GDfin ,\xdfin )\notin \MCM (\Gloopsub _1)$ is not an \MCE of $\Gloopsub _1$ (right). The red dashed line indicates the \pchord violating~\itemref {MCE5:Mpos_chords} for $\ResGx _1(\GDfin ,\xdfin )$. See \cref {ex:counter}}{figure.caption.29}{}}
\@writefile{lla}{\contentsline {section}{\numberline {\crtrefnumber{fig:counter-kinsupp}}fig:counter-kinsupp}{97}{figure.caption.29}\protected@file@percent }
\newlabel{fig:counter-kinsupp@cref}{{[figure][21][]21}{[1][97][]97}{}{}{}}
\@writefile{loe}{\contentsline {example}{\ifthmt@listswap Example~11.17\else \numberline {11.17}Example\fi \thmtformatoptarg {Full $2$-separation\xspace  is not sufficient for kinematic support\xspace  }}{97}{example.11.17}\protected@file@percent }
\newlabel{ex:counter}{{11.17}{97}{\Fullysepon is not sufficient for \kinsupp }{example.11.17}{}}
\@writefile{lla}{\contentsline {section}{\numberline {\crtrefnumber{ex:counter}}ex:counter}{97}{example.11.17}\protected@file@percent }
\newlabel{ex:counter@cref}{{[example][17][11]11.17}{[1][97][]97}{}{}{}}
\@writefile{loe}{\contentsline {conjecture}{\ifthmt@listswap Conjecture~11.18\else \numberline {11.18}Conjecture\fi \thmtformatoptarg {Combinatorial criterion for kinematic support\xspace  }}{97}{conjecture.11.18}\protected@file@percent }
\newlabel{conj:kinsupp}{{11.18}{97}{Combinatorial criterion for \kinsupp }{conjecture.11.18}{}}
\@writefile{lla}{\contentsline {section}{\numberline {\crtrefnumber{conj:kinsupp}}conj:kinsupp}{97}{conjecture.11.18}\protected@file@percent }
\newlabel{conj:kinsupp@cref}{{[conjecture][18][11]11.18}{[1][97][]97}{}{}{}}
\@writefile{toc}{\contentsline {subsection}{\tocsubsection {}{11.4}{BCFW tilings of M-convex\xspace  moduli spaces\xspace  }}{97}{subsection.11.4}\protected@file@percent }
\@writefile{loe}{\contentsline {theorem}{\ifthmt@listswap Theorem~11.19\else \numberline {11.19}Theorem\fi \thmtformatoptarg {BCFW tilings of M-convex\xspace  moduli spaces\xspace  }}{97}{theorem.11.19}\protected@file@percent }
\newlabel{thm:BCFW:triang_MCE}{{11.19}{97}{BCFW tilings of \MCMSs }{theorem.11.19}{}}
\@writefile{lla}{\contentsline {section}{\numberline {\crtrefnumber{thm:BCFW:triang_MCE}}thm:BCFW:triang_MCE}{97}{theorem.11.19}\protected@file@percent }
\newlabel{thm:BCFW:triang_MCE@cref}{{[theorem][19][11]11.19}{[1][97][]97}{}{}{}}
\@writefile{toc}{\contentsline {section}{\tocsection {}{12}{Finishing the proof}}{98}{section.12}\protected@file@percent }
\newlabel{sec:finish}{{12}{98}{Finishing the proof}{section.12}{}}
\@writefile{lla}{\contentsline {section}{\numberline {\crtrefnumber{sec:finish}}sec:finish}{98}{section.12}\protected@file@percent }
\newlabel{sec:finish@cref}{{[section][12][]12}{[1][98][]98}{}{}{}}
\newlabel{ssec:BCFW_triang_final1}{{12.1}{98}{BCFW tilings of ambient loop momentum amplituhedra}{subsection.12.1}{}}
\@writefile{lla}{\contentsline {section}{\numberline {\crtrefnumber{ssec:BCFW_triang_final1}}ssec:BCFW_triang_final1}{98}{subsection.12.1}\protected@file@percent }
\newlabel{ssec:BCFW_triang_final1@cref}{{[subsection][1][12]12.1}{[1][98][]98}{}{}{}}
\@writefile{toc}{\contentsline {subsection}{\tocsubsection {}{12.1}{BCFW tilings of ambient loop momentum amplituhedra}}{98}{thmt@dummyctr.dummy.364}\protected@file@percent }
\@writefile{loe}{\contentsline {theorem}{\ifthmt@listswap Theorem~12.1\else \numberline {12.1}Theorem\fi \thmtformatoptarg {BCFW tilings of ambient loop momentum amplituhedra}}{98}{theorem.12.1}\protected@file@percent }
\newlabel{lemma:BCLOOP:MPknL_tiling}{{12.1}{98}{BCFW tilings of ambient loop momentum amplituhedra}{theorem.12.1}{}}
\@writefile{lla}{\contentsline {section}{\numberline {\crtrefnumber{lemma:BCLOOP:MPknL_tiling}}lemma:BCLOOP:MPknL_tiling}{98}{theorem.12.1}\protected@file@percent }
\newlabel{lemma:BCLOOP:MPknL_tiling@cref}{{[theorem][1][12]12.1}{[1][98][]98}{}{}{}}
\newlabel{eq:Gfin_cd}{{12.1}{98}{BCFW tilings of ambient loop momentum amplituhedra}{equation.12.1}{}}
\@writefile{lla}{\contentsline {section}{\numberline {\crtrefnumber{eq:Gfin_cd}}eq:Gfin_cd}{98}{equation.12.1}\protected@file@percent }
\newlabel{eq:Gfin_cd@cref}{{[equation][1][12]12.1}{[1][98][]98}{}{}{}}
\newlabel{eq:Gfin_cd_sqcup}{{12.2}{98}{BCFW tilings of ambient loop momentum amplituhedra}{equation.12.2}{}}
\@writefile{lla}{\contentsline {section}{\numberline {\crtrefnumber{eq:Gfin_cd_sqcup}}eq:Gfin_cd_sqcup}{98}{equation.12.2}\protected@file@percent }
\newlabel{eq:Gfin_cd_sqcup@cref}{{[equation][2][12]12.2}{[1][98][]98}{}{}{}}
\newlabel{eq:kinsupp_einj_automatic}{{12.3}{99}{BCFW tilings of ambient loop momentum amplituhedra}{equation.12.3}{}}
\@writefile{lla}{\contentsline {section}{\numberline {\crtrefnumber{eq:kinsupp_einj_automatic}}eq:kinsupp_einj_automatic}{99}{equation.12.3}\protected@file@percent }
\newlabel{eq:kinsupp_einj_automatic@cref}{{[equation][3][12]12.3}{[1][99][]99}{}{}{}}
\@writefile{loe}{\contentsline {remark}{\ifthmt@listswap Remark~12.2\else \numberline {12.2}Remark\fi }{99}{remark.12.2}\protected@file@percent }
\newlabel{rmk:Gfin_reduced}{{12.2}{99}{}{remark.12.2}{}}
\@writefile{lla}{\contentsline {section}{\numberline {\crtrefnumber{rmk:Gfin_reduced}}rmk:Gfin_reduced}{99}{remark.12.2}\protected@file@percent }
\newlabel{rmk:Gfin_reduced@cref}{{[remark][2][12]12.2}{[1][99][]99}{}{}{}}
\newlabel{ssec:collapsed_MCE}{{12.2}{99}{Collapsed \MCEsnoacr }{subsection.12.2}{}}
\@writefile{lla}{\contentsline {section}{\numberline {\crtrefnumber{ssec:collapsed_MCE}}ssec:collapsed_MCE}{99}{subsection.12.2}\protected@file@percent }
\newlabel{ssec:collapsed_MCE@cref}{{[subsection][2][12]12.2}{[1][99][]99}{}{}{}}
\@writefile{toc}{\contentsline {subsection}{\tocsubsection {}{12.2}{Collapsed M-convex\xspace  weak embeddings\xspace  }}{99}{subsection.12.2}\protected@file@percent }
\@writefile{loe}{\contentsline {lemma}{\ifthmt@listswap Lemma~12.3\else \numberline {12.3}Lemma\fi }{99}{lemma.12.3}\protected@file@percent }
\newlabel{lemma:BCFW:counting_stars}{{12.3}{99}{}{lemma.12.3}{}}
\@writefile{lla}{\contentsline {section}{\numberline {\crtrefnumber{lemma:BCFW:counting_stars}}lemma:BCFW:counting_stars}{99}{lemma.12.3}\protected@file@percent }
\newlabel{lemma:BCFW:counting_stars@cref}{{[lemma][3][12]12.3}{[1][99][]99}{}{}{}}
\newlabel{eq:counting_stars}{{12.4}{99}{}{equation.12.4}{}}
\@writefile{lla}{\contentsline {section}{\numberline {\crtrefnumber{eq:counting_stars}}eq:counting_stars}{99}{equation.12.4}\protected@file@percent }
\newlabel{eq:counting_stars@cref}{{[equation][4][12]12.4}{[1][99][]99}{}{}{}}
\newlabel{eq:CollW=FflWsink}{{12.5}{99}{Collapsed \MCEsnoacr }{equation.12.5}{}}
\@writefile{lla}{\contentsline {section}{\numberline {\crtrefnumber{eq:CollW=FflWsink}}eq:CollW=FflWsink}{99}{equation.12.5}\protected@file@percent }
\newlabel{eq:CollW=FflWsink@cref}{{[equation][5][12]12.5}{[1][99][]99}{}{}{}}
\@writefile{lof}{\contentsline {figure}{\numberline {22}{\ignorespaces  Computing $\Sloc _\rho $ and $\Tloc _\rho $ in the proof of \cref  {lemma:BCFW:counting_stars}.}}{100}{figure.caption.30}\protected@file@percent }
\newlabel{fig:S-rho}{{22}{100}{Computing $\protect \Sloc _\rho $ and $\protect \Tloc _\rho $ in the proof of \cref {lemma:BCFW:counting_stars}}{figure.caption.30}{}}
\@writefile{lla}{\contentsline {section}{\numberline {\crtrefnumber{fig:S-rho}}fig:S-rho}{100}{figure.caption.30}\protected@file@percent }
\newlabel{fig:S-rho@cref}{{[figure][22][]22}{[1][100][]100}{}{}{}}
\newlabel{eq:dbloc>=|FflWmid|}{{12.6}{100}{Collapsed \MCEsnoacr }{equation.12.6}{}}
\@writefile{lla}{\contentsline {section}{\numberline {\crtrefnumber{eq:dbloc>=|FflWmid|}}eq:dbloc>=|FflWmid|}{100}{equation.12.6}\protected@file@percent }
\newlabel{eq:dbloc>=|FflWmid|@cref}{{[equation][6][12]12.6}{[1][100][]100}{}{}{}}
\newlabel{ssec:BCFW_triang_final2}{{12.3}{101}{BCFW tilings of ambient loop \mtas }{subsection.12.3}{}}
\@writefile{lla}{\contentsline {section}{\numberline {\crtrefnumber{ssec:BCFW_triang_final2}}ssec:BCFW_triang_final2}{101}{subsection.12.3}\protected@file@percent }
\newlabel{ssec:BCFW_triang_final2@cref}{{[subsection][3][12]12.3}{[1][101][]101}{}{}{}}
\@writefile{toc}{\contentsline {subsection}{\tocsubsection {}{12.3}{BCFW tilings of ambient loop momentum-twistor\xspace  amplituhedra\xspace  }}{101}{subsection.12.3}\protected@file@percent }
\@writefile{loe}{\contentsline {theorem}{\ifthmt@listswap Theorem~12.4\else \numberline {12.4}Theorem\fi \thmtformatoptarg {BCFW tilings of ambient loop momentum-twistor\xspace  amplituhedra\xspace  }}{101}{theorem.12.4}\protected@file@percent }
\newlabel{lemma:BCLOOP:AAknL_tiling}{{12.4}{101}{BCFW tilings of ambient loop \mtas }{theorem.12.4}{}}
\@writefile{lla}{\contentsline {section}{\numberline {\crtrefnumber{lemma:BCLOOP:AAknL_tiling}}lemma:BCLOOP:AAknL_tiling}{101}{theorem.12.4}\protected@file@percent }
\newlabel{lemma:BCLOOP:AAknL_tiling@cref}{{[theorem][4][12]12.4}{[1][101][]101}{}{}{}}
\citation{FGLS}
\citation{FGLS}
\citation{FGLS}
\citation{FGLS}
\citation{FL}
\citation{FGLS}
\citation{FGLS}
\citation{FL}
\citation{AHT}
\citation{KW}
\newlabel{eq:Coll_square}{{12.7}{102}{BCFW tilings of ambient loop \mtas }{equation.12.7}{}}
\@writefile{lla}{\contentsline {section}{\numberline {\crtrefnumber{eq:Coll_square}}eq:Coll_square}{102}{equation.12.7}\protected@file@percent }
\newlabel{eq:Coll_square@cref}{{[equation][7][12]12.7}{[1][102][]102}{}{}{}}
\@writefile{loe}{\contentsline {corollary}{\ifthmt@listswap Corollary~12.5\else \numberline {12.5}Corollary\fi }{102}{corollary.12.5}\protected@file@percent }
\newlabel{cor:from_tMtiing_to_Mtiling}{{12.5}{102}{}{corollary.12.5}{}}
\@writefile{lla}{\contentsline {section}{\numberline {\crtrefnumber{cor:from_tMtiing_to_Mtiling}}cor:from_tMtiing_to_Mtiling}{102}{corollary.12.5}\protected@file@percent }
\newlabel{cor:from_tMtiing_to_Mtiling@cref}{{[corollary][5][12]12.5}{[1][102][]102}{}{}{}}
\newlabel{Mtil1}{{{{(1)}}}{102}{}{Item.84}{}}
\@writefile{lla}{\contentsline {section}{\numberline {\crtrefnumber{Mtil1}}Mtil1}{102}{Item.84}\protected@file@percent }
\newlabel{Mtil1@cref}{{[enumi][1][]{{(1)}}}{[1][102][]102}{}{}{}}
\newlabel{Mtil2}{{{{(2)}}}{102}{}{Item.85}{}}
\@writefile{lla}{\contentsline {section}{\numberline {\crtrefnumber{Mtil2}}Mtil2}{102}{Item.85}\protected@file@percent }
\newlabel{Mtil2@cref}{{[enumi][2][]{{(2)}}}{[1][102][]102}{}{}{}}
\newlabel{ssec:flip_proj}{{12.4}{102}{Sign flip and linear projection loop amplituhedra}{subsection.12.4}{}}
\@writefile{lla}{\contentsline {section}{\numberline {\crtrefnumber{ssec:flip_proj}}ssec:flip_proj}{102}{subsection.12.4}\protected@file@percent }
\newlabel{ssec:flip_proj@cref}{{[subsection][4][12]12.4}{[1][102][]102}{}{}{}}
\@writefile{toc}{\contentsline {subsection}{\tocsubsection {}{12.4}{Sign flip and linear projection loop amplituhedra}}{102}{subsection.12.4}\protected@file@percent }
\@writefile{loe}{\contentsline {definition}{\ifthmt@listswap Definition~12.6\else \numberline {12.6}Definition\fi }{102}{definition.12.6}\protected@file@percent }
\@writefile{loe}{\contentsline {remark}{\ifthmt@listswap Remark~12.7\else \numberline {12.7}Remark\fi }{102}{remark.12.7}\protected@file@percent }
\newlabel{rmk:FL_FGLS_compare}{{12.7}{102}{}{remark.12.7}{}}
\@writefile{lla}{\contentsline {section}{\numberline {\crtrefnumber{rmk:FL_FGLS_compare}}rmk:FL_FGLS_compare}{102}{remark.12.7}\protected@file@percent }
\newlabel{rmk:FL_FGLS_compare@cref}{{[remark][7][12]12.7}{[1][102][]102}{}{}{}}
\citation{KW}
\citation{KW}
\citation{AHTT}
\citation{PSBW}
\@writefile{loe}{\contentsline {lemma}{\ifthmt@listswap Lemma~12.8\else \numberline {12.8}Lemma\fi \thmtformatoptarg {\cite  [Definition~3.8]{KW}}}{103}{lemma.12.8}\protected@file@percent }
\newlabel{lemma:KW_intersect_Z_dim}{{12.8}{103}{\cite [Definition~3.8]{KW}}{lemma.12.8}{}}
\@writefile{lla}{\contentsline {section}{\numberline {\crtrefnumber{lemma:KW_intersect_Z_dim}}lemma:KW_intersect_Z_dim}{103}{lemma.12.8}\protected@file@percent }
\newlabel{lemma:KW_intersect_Z_dim@cref}{{[lemma][8][12]12.8}{[1][103][]103}{}{}{}}
\@writefile{loe}{\contentsline {definition}{\ifthmt@listswap Definition~12.9\else \numberline {12.9}Definition\fi }{103}{definition.12.9}\protected@file@percent }
\@writefile{loe}{\contentsline {lemma}{\ifthmt@listswap Lemma~12.10\else \numberline {12.10}Lemma\fi }{103}{lemma.12.10}\protected@file@percent }
\newlabel{lemma:LOOP:proj_subset_amb}{{12.10}{103}{}{lemma.12.10}{}}
\@writefile{lla}{\contentsline {section}{\numberline {\crtrefnumber{lemma:LOOP:proj_subset_amb}}lemma:LOOP:proj_subset_amb}{103}{lemma.12.10}\protected@file@percent }
\newlabel{lemma:LOOP:proj_subset_amb@cref}{{[lemma][10][12]12.10}{[1][103][]103}{}{}{}}
\newlabel{eq:TREE:proj_subset_cl_amb}{{12.8}{103}{}{equation.12.8}{}}
\@writefile{lla}{\contentsline {section}{\numberline {\crtrefnumber{eq:TREE:proj_subset_cl_amb}}eq:TREE:proj_subset_cl_amb}{103}{equation.12.8}\protected@file@percent }
\newlabel{eq:TREE:proj_subset_cl_amb@cref}{{[equation][8][12]12.8}{[1][103][]103}{}{}{}}
\newlabel{eq:KW_minors}{{12.9}{103}{Sign flip and linear projection loop amplituhedra}{equation.12.9}{}}
\@writefile{lla}{\contentsline {section}{\numberline {\crtrefnumber{eq:KW_minors}}eq:KW_minors}{103}{equation.12.9}\protected@file@percent }
\newlabel{eq:KW_minors@cref}{{[equation][9][12]12.9}{[1][103][]103}{}{}{}}
\@writefile{loe}{\contentsline {theorem}{\ifthmt@listswap Theorem~12.11\else \numberline {12.11}Theorem\fi \thmtformatoptarg {BCFW tilings of loop amplituhedra}}{103}{theorem.12.11}\protected@file@percent }
\newlabel{lemma:proj_tiling}{{12.11}{103}{BCFW tilings of loop amplituhedra}{theorem.12.11}{}}
\@writefile{lla}{\contentsline {section}{\numberline {\crtrefnumber{lemma:proj_tiling}}lemma:proj_tiling}{103}{theorem.12.11}\protected@file@percent }
\newlabel{lemma:proj_tiling@cref}{{[theorem][11][12]12.11}{[1][103][]103}{}{}{}}
\newlabel{proj_tiling1}{{{{(1)}}}{103}{BCFW tilings of loop amplituhedra}{Item.86}{}}
\@writefile{lla}{\contentsline {section}{\numberline {\crtrefnumber{proj_tiling1}}proj_tiling1}{103}{Item.86}\protected@file@percent }
\newlabel{proj_tiling1@cref}{{[enumi][1][]{{(1)}}}{[1][103][]103}{}{}{}}
\newlabel{proj_tiling2}{{{{(2)}}}{103}{BCFW tilings of loop amplituhedra}{Item.87}{}}
\@writefile{lla}{\contentsline {section}{\numberline {\crtrefnumber{proj_tiling2}}proj_tiling2}{103}{Item.87}\protected@file@percent }
\newlabel{proj_tiling2@cref}{{[enumi][2][]{{(2)}}}{[1][103][]103}{}{}{}}
\citation{PSW}
\newlabel{proj_tiling3}{{{{(3)}}}{104}{BCFW tilings of loop amplituhedra}{Item.88}{}}
\@writefile{lla}{\contentsline {section}{\numberline {\crtrefnumber{proj_tiling3}}proj_tiling3}{104}{Item.88}\protected@file@percent }
\newlabel{proj_tiling3@cref}{{[enumi][3][]{{(3)}}}{[1][103][]104}{}{}{}}
\newlabel{eq:LOOP:proj=amb}{{12.10}{104}{BCFW tilings of loop amplituhedra}{equation.12.10}{}}
\@writefile{lla}{\contentsline {section}{\numberline {\crtrefnumber{eq:LOOP:proj=amb}}eq:LOOP:proj=amb}{104}{equation.12.10}\protected@file@percent }
\newlabel{eq:LOOP:proj=amb@cref}{{[equation][10][12]12.10}{[1][103][]104}{}{}{}}
\@writefile{toc}{\contentsline {section}{\tocsection {Appendix}{A}{Loop BCFW recursion in momentum-twistor space}}{105}{appendix.A}\protected@file@percent }
\newlabel{ssec:APP:RP3}{{A}{105}{Loop BCFW recursion in momentum-twistor space}{appendix.A}{}}
\@writefile{lla}{\contentsline {section}{\numberline {\crtrefnumber{ssec:APP:RP3}}ssec:APP:RP3}{105}{appendix.A}\protected@file@percent }
\newlabel{ssec:APP:RP3@cref}{{[section][1][]A}{[1][104][]105}{}{}{}}
\@writefile{loe}{\contentsline {definition}{\ifthmt@listswap Definition~A.1\else \numberline {A.1}Definition\fi }{105}{definition.A.1}\protected@file@percent }
\newlabel{dfn:APP:mtconf}{{A.1}{105}{}{definition.A.1}{}}
\@writefile{lla}{\contentsline {section}{\numberline {\crtrefnumber{dfn:APP:mtconf}}dfn:APP:mtconf}{105}{definition.A.1}\protected@file@percent }
\newlabel{dfn:APP:mtconf@cref}{{[definition][1][1]A.1}{[1][105][]105}{}{}{}}
\newlabel{mtconf1}{{{{(1)}}}{105}{}{Item.89}{}}
\@writefile{lla}{\contentsline {section}{\numberline {\crtrefnumber{mtconf1}}mtconf1}{105}{Item.89}\protected@file@percent }
\newlabel{mtconf1@cref}{{[enumi][1][]{{(1)}}}{[1][105][]105}{}{}{}}
\newlabel{mtconf2}{{{{(2)}}}{105}{}{Item.90}{}}
\@writefile{lla}{\contentsline {section}{\numberline {\crtrefnumber{mtconf2}}mtconf2}{105}{Item.90}\protected@file@percent }
\newlabel{mtconf2@cref}{{[enumi][2][]{{(2)}}}{[1][105][]105}{}{}{}}
\newlabel{mtconf3}{{{{(3)}}}{105}{}{Item.91}{}}
\@writefile{lla}{\contentsline {section}{\numberline {\crtrefnumber{mtconf3}}mtconf3}{105}{Item.91}\protected@file@percent }
\newlabel{mtconf3@cref}{{[enumi][3][]{{(3)}}}{[1][105][]105}{}{}{}}
\newlabel{eq:mtwphi_dfn}{{A.1}{105}{Loop BCFW recursion in momentum-twistor space}{equation.A.1}{}}
\@writefile{lla}{\contentsline {section}{\numberline {\crtrefnumber{eq:mtwphi_dfn}}eq:mtwphi_dfn}{105}{equation.A.1}\protected@file@percent }
\newlabel{eq:mtwphi_dfn@cref}{{[equation][1][1]A.1}{[1][105][]105}{}{}{}}
\newlabel{eq:APP:mtmapT_dfn}{{A.2}{105}{Loop BCFW recursion in momentum-twistor space}{equation.A.2}{}}
\@writefile{lla}{\contentsline {section}{\numberline {\crtrefnumber{eq:APP:mtmapT_dfn}}eq:APP:mtmapT_dfn}{105}{equation.A.2}\protected@file@percent }
\newlabel{eq:APP:mtmapT_dfn@cref}{{[equation][2][1]A.2}{[1][105][]105}{}{}{}}
\@writefile{loe}{\contentsline {remark}{\ifthmt@listswap Remark~A.2\else \numberline {A.2}Remark\fi }{105}{remark.A.2}\protected@file@percent }
\newlabel{rmk:APP:cliques_vs_lines}{{A.2}{105}{}{remark.A.2}{}}
\@writefile{lla}{\contentsline {section}{\numberline {\crtrefnumber{rmk:APP:cliques_vs_lines}}rmk:APP:cliques_vs_lines}{105}{remark.A.2}\protected@file@percent }
\newlabel{rmk:APP:cliques_vs_lines@cref}{{[remark][2][1]A.2}{[1][105][]105}{}{}{}}
\bibstyle{alpha}
\bibdata{loop_ampl}
\bibcite{Affolter}{Aff23}
\bibcite{AGPR}{AGPR24}
\bibcite{AHBC_all_loop}{AHBC{$^{+}$}11}
\bibcite{abcgpt}{AHBC{$^{+}$}16}
\bibcite{AHCC}{AHCC10}
\bibcite{AHT}{AHT14}
\bibcite{AHTT}{AHTT18}
\bibcite{BCFW}{BCFW05}
\bibcite{BaiHe}{BH15}
\bibcite{BHL}{BHL16}
\bibcite{BaWe}{BW20}
\bibcite{CLR1}{CLR23}
\bibcite{CLSBW}{CLSBW23}
\bibcite{DFLP}{DFLP19}
\bibcite{ELPTSBW}{EZLP{$^{+}$}23}
\bibcite{ELT}{EZLT25}
\bibcite{FoGo}{FG06}
\bibcite{FGLS}{FGLS24}
\bibcite{FL}{FL23}
\bibcite{Floater}{Flo03}
\bibcite{applets}{Gal}
\bibcite{Zono}{Gal18}
\bibcite{crit}{Gal23}
\bibcite{origami1}{Gal24}
\bibcite{HSP}{GPW22}
\bibcite{Hakimi}{Hak65}
\bibcite{HZ_notes}{HZ18}
\bibcite{Kasteleyn}{Kas61}
\@writefile{toc}{\contentsline {section}{\tocsection {Appendix}{}{References}}{106}{section*.31}\protected@file@percent }
\bibcite{Kawasaki}{Kaw89}
\bibcite{Kenyon_conf}{Ken00}
\bibcite{Kenyon_height}{Ken08}
\bibcite{Kenyon_lectures}{Ken09}
\bibcite{Kenyon_conf_loops}{Ken14}
\bibcite{KLRR}{KLRR22}
\bibcite{KLS}{KLS13}
\bibcite{Kenyon_Sheffield}{KS04}
\bibcite{KW}{KW19}
\bibcite{Lam_dimers}{Lam15}
\bibcite{LamCDM}{Lam16}
\bibcite{Lovasz_1987}{Lov87}
\bibcite{Lovasz_Plummer}{LP86}
\bibcite{LPW}{LPW23}
\bibcite{Lus2}{Lus94}
\bibcite{MuSp}{MS17}
\bibcite{Pos}{Pos06}
\bibcite{Pos_ICM}{Pos18}
\bibcite{PSBW}{PSBW23}
\bibcite{PSW}{PSW09}
\bibcite{RhSk}{RS05}
\bibcite{RSS_expansive}{RSS03}
\bibcite{RSS}{RSS06}
\bibcite{Smirnov_cluster}{Smi10}
\bibcite{SpeyerVariations}{Spe16}
\bibcite{Streinu}{Str00}
\bibcite{Streinu_ptr}{Str05}
\bibcite{Tessler_notes}{Tes25}
\newlabel{tocindent-1}{0pt}
\newlabel{tocindent0}{63.44928pt}
\newlabel{tocindent1}{71.66179pt}
\newlabel{tocindent2}{0pt}
\newlabel{tocindent3}{0pt}
\gdef \@abspage@last{107}

